Exploiting Opportunistic Physical Design in Large-scale Data Analytics

Large-scale systems, such as MapReduce and Hadoop, perform aggressive materialization of intermediate job results in order to support fault tolerance. When jobs correspond to exploratory queries submitted by data analysts, these materializations yield a large set of materialized views that typically capture common computation among successive queries from the same analyst, or even across queries of different analysts who test similar hypotheses. We propose to treat these views as an opportunistic physical design and use them for the purpose of query optimization. We develop a novel query-rewrite algorithm that addresses the two main challenges in this context: how to search the large space of rewrites, and how to reason about views that contain UDFs (a common feature in large-scale data analytics). The algorithm, which provably finds the minimum-cost rewrite, is inspired by nearest-neighbor searches in non-metric spaces. We present an extensive experimental study on real-world datasets with a prototype data-analytics system based on Hive. The results demonstrate that our approach can result in dramatic performance improvements on complex data-analysis queries, reducing total execution time by an average of 61% and up to two orders of magnitude.

==> Makefile <==
SHELL := /bin/bash
TEXFORMATS := ".:styles/:" 
TEXINPUTS  := ".:pics/:styles/:"
BSTINPUTS  := ".:pics/:styles/:"
SRC = Odyssey
#SRC = bfr-proof

compile:
	export TEXFORMATS=${TEXFORMATS};  \
	export TEXINPUTS=${TEXINPUTS};  \
	export BSTINPUTS=${BSTINPUTS};  \
	bibtex ${SRC};  \
	pdflatex ${SRC}; 


==> newtext.tex <==
\subsection{Determining O\fakesc{pt}C\fakesc{ost}}\label{sec-ocost}

The final utility of the UDF model we developed in 
in the section that it can provide a lower-bound on the cost of 
rewrite produced by a view $v$ for a query $q$, without having
to first find a valid rewrite.
The utility of  a lower bound enables
the enumeration of the candidate views based their potential 
to provide a low cost rewrite, which forms the basis of the $\VF{}$
algorithm that we develop in the reminder of the paper.

Suppose that $v$ is guessed to be complete with respect to $q$, 
the set difference between the attributes, filters and group-bys representation 
of $q$ and $v$ is referred to as the {\em fix}.
Fix denotes a hypothetical UDF that applies up to three local function that can
transform $v$'s representation into $q$'s.
The three local functions correspond to those that add or drop attributes in $v$
to make it equivalent to $q$, apply selection predicate, and group-bys needed to make
$v$ and $q$ identical.
Note that a UDF containing such a local function may not really exist, but finding
it is a computationally hard problem.

\onefig{fig-example-fix}{Example of the fix between a view $v$ and a query $q$}{2in}

\begin{example}
Suppose that $v$ is given by attribues $\{a,b,c\}$, no applied filters, and no group-bys. 
Now, suppose that $q$ is given by $\{b,c,d\}$, filter $d < 10$, and group-by $c$, such that
to produce $d$ requires $a$ and $b$, which is present in $v$.
It is clear that $v$ is guessed to be complete with respect to $q$.
The fix of $v$ with respect to $q$ is given by three local functions:
a) A local function that produces $d$ from $a$ and $b$,
b) Applies the selection predicate $d < 10$ on the inputs,
and c) Applies a group-by on $c$.
This is captured by the Figure~\ref{fig-example-fix}.
\end{example}

Note that the application of fix does not guarantee that $v$ will result in a valid rewrite 
for the same reason that  guessed to be complete can result in a false positive.
We have to invoke a rewrite algorithm which produces a rewrite
containing compensations from $L_R$.
The composition of the local functions in the compensation
transforms $v$'s representation to $q$.
Both assume that the required
compensation operations can be applied independently of each other to $v$.

The fix can be used as a lower-bound for the actual bound by appealing to 
the following intuition.
The fix denotes a hypothetical UDF that may not exist in reality since 


==> old/Bestfirst_workflow_rewrite-rewrite1.tex <==
\section{Best-First Rewrite}\label{sec-best-first-workflow-rewrite}

Given a plan $W$ with $n$ targets,
the $\WF{}$ algorithm produces an {\em optimal} rewrite $r^*$ of $W$ in
a  {\em work efficient} manner.
The rewrite $r^*$ is {\em optimal}  in the sense that there cannot be a cheaper
rewrite for $W$ than $r^*$, where $r^*$ can be composed of rewrites found at multiple targets in $W$.
The proposed algorithm is also {\em work efficient} in the sense
that it will never explore more of the solution space than the minimum
necessary to find $r^*$.

The bottom-up approach exhaustively looks at every target in $W$ for a valid rewrite
but considers each target in isolation.
In contrast, our algorithm spawns $n$ concurrent (i.e., non-isolated)
search problems at each of the targets in $W$.
We take advantage of the concurrent searches in that whenever
we find a rewrite at a target we can use this to aid in pruning the
search space of other targets in $W$.
Moreover even when an incremental search at a target
does not yield a rewrite, this can still aid in pruning the space at other targets.

\begin{comment}
The high-level structure of the $\WF{}$ algorithm is as follows.
\begin{enumerate}
  \item \textsc{initialize} the \VF{} for each target
  \begin{itemize}%
  \renewcommand{\labelitemi}{$\cdot$}
    \item Set $W_i$ as the best rewrite found so far for target \node{i}
  \end{itemize}
  \item \textsc{loop} until obtaining $r^*$
  \begin{itemize}%
    \renewcommand{\labelitemi}{$\cdot$}
    \item Identify the next minimum target $W_i$ to incrementally search
    \item \Refine{} $W_i$ using \VF{}
  \end{itemize}
\end{enumerate}
\end{comment}


\begin{algorithm}[!h]
\caption{Optimal rewrite of $W$ using $\VF$\label{alg-main-setup}}
{\small
\begin{algorithmic}[1]
\Function{$\WF$}{$W$, $V$}
\ForAll{$W_i \in W$}\Comment{Init Step}\label{line-wf-init}
  \State $\VF$.{\sc Init}($W_i$, $V$)
  \State $W_i$.$\minPlumb$ \qlet $W_i$ \Comment{original plan to produce $W_i$}
  \State $W_i$.$\minCost$ \qlet $\cost(W_i)$\Comment{plan cost}
\EndFor \label{line-wf-init-end}
% \State $W_i \qlet W_n$
% \While{$W_i$ $\not= -1$}\label{line-rewrite-wf-start-while-loop}
%   \State $W_i, d_i \qlet \FindNextMinTarget(W_n)$\label{line-wf-find-next-min}
%   \State $\RefineTarget(W_i)$ {\bf if} $W_i \not= -1$
% \EndWhile\label{line-rewrite-wf-end-while-loop}
\Repeat\label{line-rewrite-wf-start-while-loop}
  \State $W_i, d_i \qlet \FindNextMinTarget(W_n)$\label{line-wf-find-next-min}
  \State $\RefineTarget(W_i)$ {\bf if} $W_i \not= -1$
\Until{$W_i$ $= -1$}\label{line-rewrite-wf-end-while-loop}
\State Rewrite $W$ using $W_n.\minPlumb$
\EndFunction
\end{algorithmic}}
\end{algorithm}


Algorithm~\ref{alg-main-setup} presents the main \WF{} function.
The initialization for each target $W_i \in W$ is shown in 
lines~\ref{line-wf-init}--\ref{line-wf-init-end}.
$\minPlumb$ records the best rewrite of $W_i$ found so far,
and its cost is recorded in $\minCost$.
After initialization it begins the best-first rewrite search process by starting
at the final node of the plan (i.e., $W_n$) and then continues to ask for the
next minimum target in $W$ to begin/resume the search.
This is given by line~\ref{line-wf-find-next-min} inside the primary repeat loop,
which identifies the next target $W_i$ to resume the incremental search by
invoking Algorithm~\ref{alg-find-next-min}.
The return value $W_i$ corresponds to the next target to resume searching, while return value
$d_i$ represents the minimum \ocost{} of a rewrite for $W$ that has not been examined so far.
In other words, at this stage of execution \WF{} has examined all possible rewrites whose cost is less than $d_i$.
Next \WF{} invokes Algorithm~\ref{alg-refine-dag} which calls the \Refine{} function of the \VF{} at target $W_i$.
This asks the \VF{} to examine only the next candidate view for that target, as determined by its \ocost{},
and this forms the basis of the incremental nature of \WF{}.
While the \VF{} performs an incremental search at each target, the \WF{} performs an incremental search
in the space of all possible rewrites for $W$.
%In a sense, $d_i$ never decreases and \WF{} stops when $d_i$ equals $\cost(r^*)$ as we show later.
In a sense, ordering the candidate views by increasing \ocost{} at each target, along with the lower-bound nature
of \ocost{} ensures that $d_i$ never decreases and \WF{} stops when $d_i$ equals $\cost(r^*)$ as we show later.

\begin{algorithm}[!h]
\caption{Find next min target to refine\label{alg-find-next-min}}
{\small
\begin{algorithmic}[1]
\Function{$\FindNextMinTarget$}{$W_i$}
\State $W' \qlet \mbox{empty}$;  $sum \qlet 0$; $d' \qlet \infty$
\State $d_i \qlet \VF.\mbox{\sc Peek}()$
\ForAll{incoming vertex $\node{j}$ of $\node{i}$}\label{line-refine-target-vertex}
  \State $W_k, d_k$ \qlet $\FindNextMinTarget(W_j)$
  \State $sum \qlet sum + d_k$
  \If{$d' > d_k$ and $W_k \not= -1$}
    \State $W' \qlet W_k$
    \State $d' \qlet d_k$
  \EndIf
\EndFor
\State $sum$ \qlet $sum + \cost(\node{i})$
\If{$\min(sum,d_i) \geq W_i.\minCost$}
  \State \Return $-1, W_i.\minCost$
\ElsIf{$sum < d_i$}
  \State \Return $W'$, $sum$
\Else
  \State \Return $W_i$, $d_i$
\EndIf
\EndFunction
\end{algorithmic}}
\end{algorithm}


The recursive algorithm given in Algorithm~\ref{alg-find-next-min} identifies the target to be refined next
in $W$ as well as the minimum cost (\ocost) of a possible rewrite for $W_i$.
Let $r$ denote a rewrite of $W_i$ using a candidate view at the instance of the \VF{} at $W_i$.
Let $r'$ denote a rewrite obtained by combining rewrites found at the ancestors of $W_i$.
The value $d_i$ (\VF.\Peek) captures the minimum possible cost of $r$, while $sum$ (sum of \VF.\Peek{} at ancestors) captures the minimum possible cost of  $r'$.
If both $sum$ and $d_i$ are greater than or equal to $W_i.\minCost$ this means that $W_i$ and all of its
ancestors cannot provide a lower cost rewrite than the best rewrite already found for $W_i$
and there is no need to further refine $W_i$ or any of its ancestors
for the remainder of the algorithm.
If $sum$ is less than $d_i$, let $W'$ represent the ancestor target with the minimum cost candidate view in $r'$,
 and hence must be the next target to refine.
If $d_i$ is less than or equal to $sum$, then $W_i$ must be the next target to refine.



\begin{algorithm}[!t]
\caption{Queries \VF{} in best-first manner\label{alg-refine-dag}}
{\small
\begin{algorithmic}[1]
\Function{$\RefineTarget$}{$W_i$}
\State $r$ \qlet \VF.{\sc Refine}($W_i$)
 \If{$r$ is not empty}
   \If{$\cost(r) < W_i.\minCost$}
     \State $W_i.\minPlumb$ \qlet $r$
     \State $W_i.\minCost$ \qlet $\cost(r)$
      \ForAll{outgoing vertex $\node{k}$ of $\node{i}$}% \Comment{towards $W_n$}
       \State $\PropagateBestRewrites$($\node{k}$)\label{line-view-finder-propagate-best-plans}
     \EndFor
   \EndIf
 \EndIf
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{$\PropagateBestRewrites$}{$\node{i}$}
\State $r$ \qlet $\node{i}$
\ForAll{incoming $\node{j}$ of $\node{i}$}
  \State $r \qlet r \cup W_j.\minPlumb$
\EndFor
\If{$\cost(r)$ < $W_i.\minCost$}
   \State $W_i.\minCost$ \qlet $\cost(r)$
   \State $W_i.\minPlumb$ \qlet $r$
   \ForAll{outgoing $\node{k}$ of $\node{i}$}
     \State $\PropagateBestRewrites$($\node{k}$)
   \EndFor
\EndIf
\EndFunction
\end{algorithmic}
}
\end{algorithm}



Algorithm~\ref{alg-refine-dag} describes the process for refining a target $W_i$ which was
previously identified by Algorithm~\ref{alg-find-next-min}.
Refinement is a two-step process.
First it obtains a rewrite $r$ of $W_i$ from \VF{} if one exists.
The cost of the rewrite $r$ obtained by $\RefineTarget$ is compared against the best
rewrite found so far at $W_i$ and then if found to be lesser suitably updates $W_i.\minPlumb{}$ and $W_i.\minCost{}$.
In the second step it tries to use $r$ as part of a rewrite of $W$ using
the recursive function given by $\PropagateBestRewrites$ in Algorithm~\ref{alg-refine-dag}.
The recursion pushes the rewrite $r$ downward toward $W_n$, and if it succeeds $r$ becomes part
of the best rewrite of $W$ found so far.  
Example~\ref{ex-algo-description} shows how \WF{} attempts to rewrite a sample plan.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Example %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\onefig{fig-optcost-algo-illustration}
{Three targets $n_1, n_2$ and $n_3$ with  
candidate views ordered by their $\ocost{}$ $a$--$f$.}
{2.75in}

\begin{example}\label{ex-algo-description}
Figure~\ref{fig-optcost-algo-illustration} shows a plan containing
three nodes $n_1, n_2$ and $n_3$, where $n_3$ represents $W_n$.
The 5 candiate views $a$--$f$ are arranged by their
$\ocost{}$ from the target nodes.
For example, $b$ is placed at $\ocost{}$ of 6 from $n_3$.
The cost of nodes $n_1,n_2,n_3$ is 6,5,2 respectively, 
hence $n_3.\minPlumb{}$ (i.e.,$W_n.\minPlumb{}$) begins with \cost{}=13.

In the first step of the algorithm,
the cheapest potential rewrite for $n_3$ is determined to be
$(a=1)$+$(c=2)$+$(n_3=2)$ having a total \ocost{} of 5, 
whereas the next cheapest possible rewrite of $n_3$ using $b$ has an \ocost{} of 6.
$\FindNextMinTarget$ chooses $a$ as the first candidate view to $\Refine{}$ 
within $a+c+n_3$ because the $\ocost{}$ of $a$ (=1) is less than $c$ (=2).
After refining $a$, the actual $\cost{}$ of $a$ is found to be 4, which is shown 
by the dashed line from $a$ in Figure~\ref{fig-optcost-algo-illustration}.
Therefore $n_1.\minCost{}$ is set to 4.
Now since the best known rewrite for 
$n_3$ is $(a=4)$+$(n_2=5)$+$(n_3=2)$ is 11, 
the value $n_3.\minCost{}$ is updated from 13 to 11 by $\PropagateBestRewrites{}$. 

Next it attempts the rewrite for $n_3$ using $b$ with an $\ocost{}$ of 6, 
which is less than the next best choice of $(d=3)$+$(c=2)$+$(n_3=2)$
with a total $\ocost{}$ of 7.
The \cost{} of the rewrite of $n_3$ using $b$ was found to be 12 as indicated 
in Figure~\ref{fig-optcost-algo-illustration}.
Since $n_3.\minCost{}$ is already 11, it is not updated.

The next best choice for $n_3$ is the rewrite with the $\ocost{}$ of 7.
Within that rewrite, $\FindNextMinTarget{}$ chooses to refine $c$,
yielding a rewrite for $n_2$ whose actual cost is 4,
so $n_2.\minCost{}$ is set to 4.
Then $n_3.\minPlumb{}$ and $n_3.\minCost${} are set to be
$(a=4)$+$(c=4)$+$(n_3=2)$ with a total cost of 10.
Figure~\ref{fig-optcost-algo-illustration} captures
this present state of the algorithm after the first three rewrite attempts.

The algorithm would proceed to the next best possible rewrite of
$(d=3)$+$(c=4)$+$(n_3=2)$ with \ocost{} of 9 which is still better 
than the best known rewrite of $n_3$ with cost of 10.
The algorithm terminates when there are no possible rewrites remaining for 
$W_n$ with a \ocost{} less than $W_n.\minCost${}.
%hence the algorithm cannot stop until it is examined.
%Finally, $e$ can be pruned as it exceeds the current $\minCost{}$ at $n_3$.
Any view with an \ocost{} greater than their target node's $\minCost${} can be pruned away, 
e.g., $e$ at $n_3$ (since $11>10$) and $f$ at $n_1$ (since $5>4$).
\end{example}


It it noteworthy in Example~\ref{ex-algo-description} that the algorithm did not
start at $n_3$ first, and had it examined all the candidate
views of $n_3$ first as a bottom-up approach would have done, it would have
examined a larger search space than necessary.



\begin{theorem}
The $\WF{}$ finds the optimal rewrite $r^*$ of $W$ and is work efficient.
\end{theorem}

\begin{proof}
% Should search far enough
Finding the optimal rewrite requires that the algorithm
must not terminate before finding $r^*$.
Ensuring work efficiency requires that the algorithm
should not examine any candidate views
that cannot be possibly included in $r^*$.
First we prove these properties for a $W$ containing a single target, 
then extend to an arbitrary plan containing $n$ targets.
For the single target case, the algorithm must examine
every candidate view with $\ocost{}$ less than or equal to $\cost(r^*)$,
but must not examine any candidate view with $\ocost{}$ greater than $\cost(r^*)$.

Proof by contradiction is as follows.
Suppose that the algorithm found a candidate view $v$, 
which resulted in a rewrite $r$.
Suppose that the candidate view $v^*$ which produces the optimal rewrite $r^*$
is not considered by the algorithm before terminating
thus incorrectly reporting
$r$ as the optimal rewrite 
even though $\cost(r^*) < \cost(r)$.
As the candidate view $v$ was examined before $v^*$ from the $\PQ$, it must have
been the case that $\ocost(v) < \ocost(v^*)$.
Once $v$ was found $W_n.\minCost{}$ is set to $\cost(r)$, which means the algorithm
will not terminate until all candidate views whose $\ocost{}$ is less than or equal
to $W_n.\minCost{}$ (i.e., $\cost(r)$) have been found.
Combining the above inequalities with the lower bound property of $\ocost{}$ with
respect to $\cost{}$, we have:

$\ocost(v) < \ocost(v^*) \leq \cost(r^*) < \cost(r) = W_n.\minCost$.

This means that the algorithm must have examined $v^*$ (and consequently $r^*$) before terminating.
Hence the contradiction that $r$ was reported as the best rewrite.

For a general case of $W$ containing $n$ targets,
we show that our  algorithm with $n$ priority queues
can be reduced to an equivalent problem of a
single global priority queue.
The queue contains all possible rewrites that include all candidate
views from every target, and each rewrite is ordered
by its \ocost{}.  
We omit this reduction due to lack of space.
Given we have already shown these properties for the
single queue case, this reduction proves the optimality and work efficiency
of the general case.\qed
\end{proof}

\begin{comment}
\begin{proof}
% SHORTENED DUE TO LACK OF SPACE
% Should search far enough
To ensure that the algorithm finds the optimal rewrite $r^*$ of $W$,
it suffices to show that it will not terminate before finding $r^*$.
This implies that the algorithm will examine
every candidate view with $\ocost{}$ less than or equal to $r^*$.
In other words, the algorithm must examine
all candidate views that could possibly be included in $r^*$.

% Should not search too many
Next, work efficiency of the algorithm requires that the algorithm
does not examine any candidate views with $\ocost{}$ greater than $r^*$.
In other words, the algorithm should not examine any candidate views
that cannot be possibly included in $r^*$.

We first show these results for $W$ containing a single target, then
extend them to an arbitrary plan containing $n$ targets.

To show that the algorithm will find the optimal rewrite of $W$,
suppose that the algorithm found a candidate view $v$, which resulted in a rewrite $r$.
Suppose that the candidate view $v^*$ which results in an optimal rewrite $r^*$
is not examined by the algorithm before terminating.
In other words, the algorithm incorrectly reported
$r$ as the best rewrite when $\cost(r^*) < \cost(r)$.

As the candidate view $v$ was examined before $v^*$ from the $\PQ$, it must have
been the case that $\ocost(v) < \ocost(v^*)$.

Once $v$ was found $W_n.\minCost{}$ is set to $\cost(r)$, which means the algorithm
will not terminate until all candidate views whose $\ocost{}$ is less than or equal
to $W_n.\minCost{}$ (i.e., $\cost(r)$) have been found.

By combining the above inequalities with the lower bound property of $\ocost{}$ with
respect to $\cost{}$, we have that:

$\ocost(v) < \ocost(v^*) \leq \cost(r^*) < \cost(r) = W_n.\minCost$.

This means that the algorithm must have examined $v^*$ (and consequently $r^*$) before terminating,
which results in a contradiction that $r$ was reported as the best rewrite.

% SJ: Good text but repeating
% From the above result, we can see that the algorithm will examine all candidate views with
% $\ocost{}$ less than or equal to $\cost(r^*)$ but terminate before examining
% a candidate view with $\ocost{}$ greater than $\cost(r^*)$, taken together shows that
% the algorithm finds the optimal rewrite $r^*$ and is work efficient for a single target.

For a general case of $W$ containing $n$ targets,
we only need to show that our  algorithm with $n$ priority queues
can be reduced to an equivalent problem containing 
a single global priority queue of all 
possible rewrites where each rewrite is ordered
by its \ocost{}.  
We omit this reduction due to lack of space.
Given we have already shown the algorithm works for
a single queue case, this reduction proves the optimality
of the general case.\qed


% RETAIN THE REMAINDER OF THIS PROOF HERE.
For a general case of a workflow $W$ containing $n$ targets, we first observe that
our $\WF$ algorithm by identifying the minimum candidate view at
each iteration
reduces the $n$ priority queues (one at each target) of candidate views into a single
``virtual'' priority queue containing ``composite'' candidate views formed
by those drawn from different targets.
In contrast to the incremental explosion of the space of candidate views by our algorithm,
the reduction from multiple priority queues to a single priority queue $\PQ'$ here
follows a pre-explosion of the space of candidate views into composite views
before the start of the algorithm in order to decouple the composite view
creation process from the rewrite search process.
We will later show that the $\ocost{}$ function on the composite views is still a lower
bound on the $\cost{}$ function on the rewrites yielded by these composite views.
% TODO: Can be expanded quite a bit to show how we avoid the explosion by caching the
% best known cost for each target
The reduction happens as follows:
First, generate all possible candidate views at all targets in $W$.
Next, add all the candidate views at $W_n$ to $\PQ'$ such that
each candidate view $v$ is now recorded as a composite view
denoted by the pair $(v, W_n)$.
For all parents target of $W_n$, form all possible composite views
by taking one candidate view from each parent target of $W_n$.
The composite view records its candidate views as well as the targets from
which they are drawn.
We keep doing this recursively by exploding one or multiple
targets at a time till we have completely exhausted all the
combinations of targets in the workflow.

The $\ocost{}$ of a composite view is the sum of the $\ocost{}$ of each
candidate view in the composite to its corresponding target (say, $a$),
plus the sum of the $\cost{}$ of the targets in the workflow that lie
in the remaining path from the targets in the composite view to $W_n$
(say, $b$).
The $\cost{}$ of a rewrite yielded by a composite view is the sum of the
rewrites yielded by the each
candidate view in the composite to its corresponding target (say $c$),
plus the sum of the $\cost{}$ of the targets in the workflow that lie
in the remaining path from the targets in the composite view to $W_n$
(i.e., $b$).

To show that $\ocost{}$ still lower bounds $\cost{}$, we observe that
for each of the candidate views in the composite its $\ocost{}$ contribution
lower bounds the $\cost{}$ of the rewrite it yields (i.e., $a \leq c$),
while the sum of the $\cost{}$ of the remaining targets in the workflow
(i.e., $b$) is common to both $\ocost{}$ and $\cost{}$ of the composite views.

Given that we have reduced the $n$ target $\PQ$ to a single equivalent one
$\PQ'$ and shown that $\ocost{}$ is still a lower bound of $\cost{}$,
our algorithm finds the optimal rewrite $r^*$ and is work efficient. \qed
\end{proof}
\end{comment}



==> old/Bestfirst_workflow_rewrite-rewrite2.tex <==
\section{Best-First Rewrite}\label{sec-best-first-workflow-rewrite}

The $\WF{}$ algorithm produces a rewrite 
$r^∗$ of $W$ that can be composed of rewrites found at multiple targets in $W$. 
The computed rewrite $r^*$ has provably the \emph{minimum cost} among all possible rewrites in the same class. 
Moreover, the algorithm is \emph{work-efficient}: even though $\cost(r^*)$ is not known a-priori, it will never examine any candidate view with $\ocost{}$
higher than the optimal cost $\cost(r^*)$. 
Intuitively, the algorithm explores only the part of the search space that 
is needed to provably find the optimal rewrite.
We prove that $\WF{}$ finds $r^*$ while being work-efficient in Section~\ref{sec-wf-proof}.

\begin{comment}
The $\WF{}$ algorithm produces an {\em optimal} rewrite $r^*$ of 
a plan $W$ in a  {\em work efficient} manner.
The rewrite $r^*$ is {\em optimal} as there cannot be a cheaper
rewrite for $W$ than $r^*$, where $r^*$ can be composed of rewrites found at multiple targets in $W$.
% The proposed algorithm is also {\em work efficient} in the sense
% that it will never explore more of the solution space than the minimum
% necessary to find $r^*$.
We formally define the work efficiency property as follows:
$\WF{}$ will not examine any candidate view with $\ocost{}$ greater than $\cost(r^*)$.
We prove both these properties of our algorithm in Section~\ref{sec-wf-proof}.
\end{comment}

The algorithm begins with $W$ itself being the best rewrite for the plan. 
It then spawns $n$ concurrent search problems at each of the targets in 
$W$ and works in iterations to find a better rewrite. 
In each iteration, the algorithm chooses one target $W_i$
and examines a candidate view at $W_i$.
The algorithm makes use of the result of this step to aid in pruning the
search space of other targets in $W$. 
To be work efficient,
the algorithm must choose wisely the next candidate view to examine.
As we will show below, the $\ocost$ functionality plays an essential role
in choosing the next target to refine.

%The key feature of our method is the $\ocost$ functionality that allows the $\WF{}$
%to incrementally search the space of rewrites of $W$, such that $\WF$
%finds the optimal rewrite of $W$ in a work efficient manner.


The $\WF$ uses an instance of the $\VF$ at each target to search
the space of rewrites. 
We will describe the details of $\VF$ in Section~\ref{sec-viewfinder}. 
In this section, $\VF$ is used as a black box that provides the following 
functions:
%
%The $\WF$ treats $\VF$ as a black-box until Section~\ref{sec-viewfinder} 
% and exploits its $\ocost$ functionality
%to incrementally search the space of rewrites for $W$.
%We assume that the $\VF{}$ at each target implements three functions: 
(1) {\sc Init} creates the search space of candidate views ordered by their $\ocost{}$, 
(2) {\sc Peek} provides the $\ocost{}$ of the \textit{next} candidate view, and
(3) {\sc Refine} searches for a rewrite of the target using the next candidate view,
which involves trying to apply the fix.
An important property of {\sc Refine} is the following: 
there are no remaining rewrites to be found for the corresponding
target that have a cost less than the value of {\sc Peek}.

\begin{comment} 
After every step of the incremental search at some target $W_i$ the following two properties are true.

\begin{enumerate}
\item The $\VF$ at target $W_i$ performs an incremental expansion to some
 cost value $d$ as requested by the $\WF{}$, and there are no remaining
 rewrites to be found for $W_i$ that has a cost less than $d$.

\item After the $\WF$ performs an incremental expansion of the $\VF$ at $W_i$ to cost $d$,
there are no remaining rewrites to be found for $W$ 
with cost less than $d'$, where $d' \leq d$.

\end{enumerate}
\end{comment}

\begin{comment}
The bottom-up approach exhaustively looks at every target in $W$ for a valid rewrite
but considers each target in isolation.
In contrast, our algorithm spawns $n$ concurrent (i.e., non-isolated)
search problems at each of the targets in $W$.
We take advantage of the concurrent searches in that whenever
we find a rewrite at a target we can use this to aid in pruning the
search space of other targets in $W$.
Moreover even when an incremental search at a target
does not yield a rewrite, this can still aid in pruning the space at other targets.
\end{comment}


\begin{comment}
The high-level structure of the $\WF{}$ algorithm is as follows.
\begin{enumerate}
  \item \textsc{initialize} the \VF{} for each target
  \begin{itemize}%
  \renewcommand{\labelitemi}{$\cdot$}
    \item Set $W_i$ as the best rewrite found so far for target \node{i}
  \end{itemize}
  \item \textsc{loop} until obtaining $r^*$
  \begin{itemize}%
    \renewcommand{\labelitemi}{$\cdot$}
    \item Identify the next minimum target $W_i$ to incrementally search
    \item \Refine{} $W_i$ using \VF{}
  \end{itemize}
\end{enumerate}
\end{comment}

\subsection{Algorithm}

In this section, we present the details of our $\WF{}$ algorithm and in 
the following section we provide an example that illustrates how the 
algorithm works on a small instance of the problem.

\begin{algorithm}[!h]
\caption{Optimal rewrite of $W$ using $\VF$\label{alg-main-setup}}
{\small
\begin{algorithmic}[1]
\Function{$\WF$}{$W$, $V$}
\ForAll{$W_i \in W$}\Comment{Init Step per target}\label{line-wf-init}
  \State $\VF$.{\sc Init}($W_i$, $V$)
  \State $\minPlumb_i$ \qlet $W_i$ \Comment{original plan to produce $W_i$}
  \State $\minCost_i$ \qlet $\cost(W_i)$\Comment{plan cost}
\EndFor \label{line-wf-init-end} \vspace{.2in}
% \State $W_i \qlet W_n$
% \While{$W_i$ $\not= -1$}\label{line-rewrite-wf-start-while-loop}
%   \State $W_i, d_i \qlet \FindNextMinTarget(W_n)$\label{line-wf-find-next-min}
%   \State $\RefineTarget(W_i)$ {\bf if} $W_i \not= -1$
% \EndWhile\label{line-rewrite-wf-end-while-loop}
\Repeat\label{line-rewrite-wf-start-while-loop}
  \State $(W_i, d) \qlet \FindNextMinTarget(W_n)$\label{line-wf-find-next-min}
  \State $\RefineTarget(W_i)$ {\bf if} $W_i \not= \mbox{NULL}$
\Until{$W_i$ $= \mbox{NULL}$}\label{line-rewrite-wf-end-while-loop}
\State Rewrite $W$ using $\minPlumb_n$
\EndFunction
\end{algorithmic}}
\end{algorithm}

Algorithm~\ref{alg-main-setup} presents the main \WF{} function, which
primarily repeats the following procedure:
Choose the best target $W_i$ (by $\FindNextMinTarget$) and
refine it by asking \VF{} to examine the
next candidate view (using $\RefineTarget$).

For each target $W_i \in W$,
the algorithm maintains 
the best rewrite 
$\minPlumb_i$ 
of $W_i$ found so far
and its cost $\minCost_i$ (which are initialized in
%The initialization for each target $W_i \in W$ is shown in 
lines~\ref{line-wf-init}--\ref{line-wf-init-end}).
%$\minPlumb_i$ records the best rewrite of $W_i$ found so far,
%and its cost is recorded in $\minCost_i$.
%After initialization it begins the best-first rewrite search process by starting
%at the final node of the plan (i.e., $W_n$) and then continues to ask for the
%next minimum target in $W$ to begin/resume the search.
The main loop iterates the search procedure % and updates $\minPlumb_i$
until there is no target that can possibly
improve $\minPlumb_n$, at which point $r^*$ has been identified.
%
% inside the primary repeat loop,
%which identifies the next target $W_i$ to resume the incremental search by
%invoking Algorithm~\ref{alg-find-next-min}.

In line~\ref{line-wf-find-next-min},
the return value $W_i$ of $\FindNextMinTarget$
corresponds to the next target to continue searching, while 
$d$ represents the minimum \ocost{} of a rewrite for $W_n$ 
involving a candidate view at $W_i$
that has not been examined so far.
As we will see shortly, $\FindNextMinTarget()$ examines views in increasing $\ocost{}$
order at each target and so can guarantee that the return value $d$ can never decrease. 
This property ensures that $\WF{}$ has examined all possible rewrites for $W$ with actual cost less than $d$.
This allows for early termination --- there is no need to continue searching 
if the best rewrite found so far is less than or equal to $d$. 

%
% In other words, at this stage of execution \WF{} has 
% examined all possible rewrites whose actual cost is less than $d$.

%Next \WF{} invokes Algorithm~\ref{alg-refine-dag} which calls the \Refine{} function of the \VF{} at target $W_i$.
%This asks the \VF{} to examine only the next candidate view for that target, as determined by its \ocost{},
%and this forms the basis of the incremental nature of \WF{}.
%While the \VF{} performs an incremental search at each target, the \WF{} performs an incremental search
%in the space of all possible rewrites for $W$.
%In a sense, $d_i$ never decreases and \WF{} stops when $d_i$ equals $\cost(r^*)$ as we show later.

\begin{algorithm}[!h]
\caption{Find next min target to refine\label{alg-find-next-min}}
{\small
\begin{algorithmic}[1]
\Function{$\FindNextMinTarget$}{$W_i$}
\State  $d' \qlet 0$; $W_{MIN} \qlet \mbox{NULL}$; $d_{MIN} \qlet \infty$
\ForAll{incoming vertex $\node{j}$ of $\node{i}$}\label{line-refine-ancestor-start}
  \State $(W_k, d)$ \qlet $\FindNextMinTarget(W_j)$
  \State $d' \qlet d' + d$
  \If{$d_{MIN} > d$ and $W_k \not= \mbox{NULL}$}\label{line-start-w-min}
    \State $W_{MIN} \qlet W_k$
    \State $d_{MIN} \qlet d$
  \EndIf\label{line-end-w-min}
\EndFor
\State $d'$ \qlet $d' + \cost(\node{i})$\label{line-refine-ancestor-end}
\State $d_i \qlet \VF.\mbox{\sc Peek}()$\label{line-refine-here}
\If{$\min(d',d_i) \geq \minCost_i$} \label{line-nothing-better}
  \State \Return $(\mbox{NULL}, \minCost_i)$
\ElsIf{$d' < d_i$}\label{line-d-i-loses}
  \State \Return $(W_{MIN}, d')$
\Else
  \State \Return $(W_i, d_i)$ \label{line-d-i-wins}
\EndIf
\EndFunction
\end{algorithmic}}
\end{algorithm}

$\FindNextMinTarget{}$,
given in Algorithm~\ref{alg-find-next-min}, 
identifies the next target to be refined 
in $W$, as well as the minimum cost (\ocost) of a possible rewrite for $W_i$.
There can be three outcomes of a search at a target $W_i$.
Case 1: $W_i$ and all its ancestors cannot provide a better rewrite.
Case 2: An ancestor target of $W_i$ can provide a better rewrite.
Case 3: $W_i$ can provide a better rewrite.
By recursively making the above determination at each target in $W$,
the algorithm identifies the best target to refine next.

% (1) There is no rewrite better than $\minPlumb_i$,
% (2) A rewrite $r'$ obtained by combining rewrites found at the 
% ancestors of $W_i$ has the best \ocost{} $d'$,
% and (3) A rewrite $r_i$ of $W_i$ using a candidate view 
% at $W_i$ has the best \ocost{} $d_i$.
%
%
%Let $r$ denote a rewrite of $W_i$ using a candidate view at the instance of the \VF{} at $W_i$.
%Let $r'$ denote a rewrite obtained by combining rewrites found at the ancestors of $W_i$.
The algorithm finds the best 
rewrite obtained by combining rewrites found at the 
ancestors of $W_i$.
This rewrite has an \ocost{} of $d'$, which is acquired by summing 
the \VF.\Peek{} values at the ancestors of $W_i$
using the recursive procedure and the cost of $\node{i}$
(lines~\ref{line-refine-ancestor-start}--\ref{line-refine-ancestor-end}).
Note that we also record the
target $W_{MIN}$ representing the ancestor target with the minimum \ocost{} candidate view 
(lines~\ref{line-start-w-min}--\ref{line-end-w-min}).
Next, we assign $d_i$ to the next candidate view at $W_i$
using \VF.\Peek{} (line~\ref{line-refine-here}).

Now the algorithm deals with the three cases outlined above.
If both $d'$ and $d_i$ are greater than or equal to $\minCost_i$ (case 1), 
there is no need to search any further at $W_i$ (line~\ref{line-nothing-better}).
% If both $d'$ and $d_i$ are greater than or equal to $\minCost_i$ this means that $W_i$ and all of its
% ancestors cannot provide a lower cost rewrite than the best rewrite already found for $W_i$
% and there is no need to further refine $W_i$ or any of its ancestors
% for the remainder of the algorithm (i.e., case (1)).
If $d'$ is less than $d_i$ (line~\ref{line-d-i-loses}), then
$W_{MIN}$ is the next target to refine (case 2).
Else (line~\ref{line-d-i-wins}), $W_i$ is the next target to refine (case 3).

%If $d'$ is less than $d_i$, let $W_{MIN}$ represent the ancestor target with the minimum cost candidate view in $r'$,
% and hence must be the next target to refine.
%If $d_i$ is less than or equal to $d'$, then $W_i$ must be the next target to refine.

\begin{algorithm}[!t]
\caption{Queries \VF{} in best-first manner\label{alg-refine-dag}}
{\small
\begin{algorithmic}[1]
\Function{$\RefineTarget$}{$W_i$}
\State $r_i$ \qlet \VF.{\sc Refine}($W_i$)\label{line-obtain-rewrite}
 \If{$r_i \not= \mbox{NULL}$ and $\cost(r_i) < \minCost_i$}\label{line-compare-rewrite}
     \State $\minPlumb_i$ \qlet $r_i$
     \State $\minCost_i$ \qlet $\cost(r_i)$
      \ForAll{edge ($\node{i}$, $\node{k}$)}% \Comment{towards $W_n$}
       \State $\PropagateBestRewrites$($\node{k}$)\label{line-view-finder-propagate-best-plans}
     \EndFor
 \EndIf\label{line-compare-rewrite-end}
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{$\PropagateBestRewrites$}{$\node{i}$}
\State $r_i$ \qlet plan initialized to $\node{i}$\label{line-rewrite-r-i-start}
\ForAll{edge ($\node{j}$, $\node{i}$)}
  \State Add $\minPlumb_j$ to $r_i$
\EndFor\label{line-rewrite-r-i-end}
\If{$\cost(r_i)$ < $\minCost_i$}\label{line-rewrite-r-i-wins}
   \State $\minCost_i$ \qlet $\cost(r_i)$
   \State $\minPlumb_i$ \qlet $r_i$
   \ForAll{edge ($\node{i}$, $\node{k}$)}
     \State $\PropagateBestRewrites$($\node{k}$)
   \EndFor
\EndIf\label{line-rewrite-r-i-wins-end}
\EndFunction
\end{algorithmic}
}
\end{algorithm}

Algorithm~\ref{alg-refine-dag} describes the process of refining a target $W_i$.
Refinement is a two-step process.
First it obtains a rewrite $r_i$ of $W_i$ from \VF{} if one exists (line~\ref{line-obtain-rewrite}).
The cost of the rewrite $r_i$ obtained by $\RefineTarget$ is compared against the best
rewrite found so far at $W_i$.
If $r_i$ is found to be cheaper, the algorithm suitably updates $\minPlumb_i$ and $\minCost_i$ 
(lines~\ref{line-compare-rewrite}--\ref{line-compare-rewrite-end}).
In the second step (line~\ref{line-view-finder-propagate-best-plans}),
it tries to use $r_i$ as part of a rewrite of $W$ using
the recursive function given by $\PropagateBestRewrites$ in Algorithm~\ref{alg-refine-dag}.
After this two-step refinement
process, $\minPlumb_n$ contains the best rewrite of $W$ found so far.  

The recursion procedure given by $\PropagateBestRewrites$
pushes downward the new $\minPlumb_i$ 
along the outgoing nodes and towards $\node{n}$. 
At each step it composes a rewrite $r_i$ using the immediate ancestor nodes of $\node{i}$
(lines~\ref{line-rewrite-r-i-start}--\ref{line-rewrite-r-i-end}).
It compares $r_i$ with $\minPlumb_i$ and updates $\minPlumb_i$ if $r_i$ is found
to be cheaper (lines~\ref{line-rewrite-r-i-wins}--\ref{line-rewrite-r-i-wins-end}).
%
%The recursion pushes the rewrite $r$ downward toward $W_n$, and if it succeeds $r$ becomes part
%of the best rewrite of $W$ found so far.  

\subsection{Algorithm Example}
Example~\ref{ex-algo-description} shows how \WF{} attempts to rewrite a sample plan.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Example %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\onefig{fig-optcost-algo-illustration}
{Three targets $n_1, n_2$ and $n_3$ with  
candidate views ordered by their $\ocost{}$ $a$--$f$.}
{2.25in}

\begin{example}\label{ex-algo-description}
Figure~\ref{fig-optcost-algo-illustration} shows a plan containing
three nodes $n_1, n_2$ and $n_3$, where $n_3$ represents $W_n$.
The five candidate views $a$--$f$ are arranged by their
$\ocost{}$ from the target nodes.
For example, $b$ is placed at $\ocost{}$ of 6 for node $n_3$.
The cost of nodes $n_1,n_2,n_3$ is 6, 5, 2 respectively, 
hence $\minPlumb{}_3$ (i.e.,$\minPlumb{}_n$) begins with \cost{}=13.

In the first step of the algorithm,
the cheapest potential rewrite for $n_3$ is determined to be
$(a=1)$+$(c=2)$+$(n_3=2)$ having a total \ocost{} of 5, 
whereas the next cheapest possible rewrite of $n_3$ using $b$ has an \ocost{} of 6.
$\FindNextMinTarget$ chooses $a$ as the first candidate view to $\Refine{}$ 
within $a+c+n_3$ because the $\ocost{}$ of $a$ (=1) is less than $c$ (=2).
After refining $a$, the actual $\cost{}$ of $a$ is found to be 4, which is shown 
as a label inside the triangle.
Note this cost is not known ahead of time, which is why the view is originally 
at cost of 1.
Therefore $\minCost{}_1$ is set to 4.
Now since the best known rewrite for 
$n_3$ is $(a=4)$+$(n_2=5)$+$(n_3=2)$ is 11, 
the value $\minCost{}_3$ is updated from 13 to 11 by $\PropagateBestRewrites{}$. 

Next it attempts the rewrite for $n_3$ using $b$ with an $\ocost{}$ of 6, 
which is less than the next best choice of $(d=3)$+$(c=2)$+$(n_3=2)$
with a total $\ocost{}$ of 7.
The \cost{} of the rewrite of $n_3$ using $b$ was found to be 12 as indicated 
in Figure~\ref{fig-optcost-algo-illustration}.
Since $\minCost{}_3$ is already 11, it is not updated.

The next best choice for $n_3$ is the rewrite with the $\ocost{}$ of 7.
Within that rewrite, $\FindNextMinTarget{}$ chooses to refine $c$,
yielding a rewrite for $n_2$ whose actual cost is 4,
so $\minCost{}_2$ is set to 4.
Then $\minPlumb{}_3$ and $\minCost_3$ are set to be
$(a=4)$+$(c=4)$+$(n_3=2)$ with a total cost of 10.
Figure~\ref{fig-optcost-algo-illustration} captures
this present state of the algorithm after the first three rewrite attempts.

The algorithm would proceed to the next best possible rewrite of
$(d=3)$+$(c=4)$+$(n_3=2)$ with \ocost{} of 9 which is still better 
than the best known rewrite of $n_3$ with cost of 10.
The algorithm terminates when there are no possible rewrites remaining for 
$W_n$ with a \ocost{} less than $\minCost_n$.
%hence the algorithm cannot stop until it is examined.
%Finally, $e$ can be pruned as it exceeds the current $\minCost{}$ at $n_3$.
Any view with an \ocost{} greater than their target node's $\minCost${} can be pruned away, 
e.g., $e$ at $n_3$ (since $11>10$) and $f$ at $n_1$ (since $5>4$).
\end{example}

It is noteworthy in Example~\ref{ex-algo-description} that had the algorithm
started at $n_3$ first, it would have examined all the candidate
views of $n_3$, resulting in a larger search space than necessary.

\subsection{Proof of Correctness}\label{sec-wf-proof}

The following theorem provides the proof of correctness and 
the work efficiency property of our $\WF{}$ algorithm.
Due to lack of space, the proof of Theorem~\ref{thm-work-efficient}
 is provided in the extended version~\cite{Lefe2013}.

\begin{theorem}\label{thm-work-efficient}
The $\WF{}$ finds the optimal rewrite $r^*$ of $W$ and is work efficient.
\end{theorem}

\begin{proof}
% Should search far enough
Finding the optimal rewrite requires that the algorithm
must not terminate before finding $r^*$.
Ensuring work efficiency requires that the algorithm
should not examine any candidate views
that cannot be possibly included in $r^*$.
First we show these properties for a $W$ containing a single target, 
then provide an outline of how to extend these results
to an arbitrary plan containing $n$ targets.
For the single target case, the algorithm must examine
every candidate view with $\ocost{}$ less than or equal to $\cost(r^*)$,
but must not examine any candidate view with $\ocost{}$ greater than $\cost(r^*)$.
A proof by contradiction is not given here due to lack of space.
The remainder of the proof is provided in the extended version~\cite{Lefe2013}.
\end{proof}

\begin{comment}  % LACK OF SPACE FOR ICDE version
Proof by contradiction is as follows.
Suppose that the algorithm found a candidate view $v$, 
which resulted in a rewrite $r$.
Suppose that the candidate view $v^*$ which produces the optimal rewrite $r^*$
is not considered by the algorithm before terminating
thus incorrectly reporting
$r$ as the optimal rewrite 
even though $\cost(r^*) < \cost(r)$.
As the candidate view $v$ was examined before $v^*$ from the $\PQ$, it must have
been the case that $\ocost(v) < \ocost(v^*)$.
Once $v$ was found $\minCost{}_n$ is set to $\cost(r)$, which means the algorithm
will not terminate until all candidate views whose $\ocost{}$ is less than or equal
to $\minCost{}_n$ (i.e., $\cost(r)$) have been found.
Combining the above inequalities with the lower bound property of $\ocost{}$ with
respect to $\cost{}$, we have:

$\ocost(v) < \ocost(v^*) \leq \cost(r^*) < \cost(r) = \minCost_n$.

This means that the algorithm must have examined $v^*$ (and consequently $r^*$) before terminating.
Hence the contradiction that $r$ was reported as the best rewrite.

Consider the general case of $W$ containing $n$ targets.
It suffices to show that the algorithm, using $\FindNextMinTarget{}$,
reduces the $n$ priority queues
to an equivalent problem of a single global priority queue.
The queue contains all possible rewrites that include all candidate
views from every target, and each rewrite is ordered by its \ocost{}.  
This reduction is straightforward and omitted due to lack of space.
% Given we have already shown these properties for the
% single queue case, this reduction proves the optimality and work efficiency
% of the general case.\qed
\end{proof}
%\end{comment}



\begin{comment}
\begin{proof}
% SHORTENED DUE TO LACK OF SPACE
% Should search far enough
To ensure that the algorithm finds the optimal rewrite $r^*$ of $W$,
it suffices to show that it will not terminate before finding $r^*$.
This implies that the algorithm will examine
every candidate view with $\ocost{}$ less than or equal to $r^*$.
In other words, the algorithm must examine
all candidate views that could possibly be included in $r^*$.

% Should not search too many
Next, work efficiency of the algorithm requires that the algorithm
does not examine any candidate views with $\ocost{}$ greater than $r^*$.
In other words, the algorithm should not examine any candidate views
that cannot be possibly included in $r^*$.

We first show these results for $W$ containing a single target, then
extend them to an arbitrary plan containing $n$ targets.

To show that the algorithm will find the optimal rewrite of $W$,
suppose that the algorithm found a candidate view $v$, which resulted in a rewrite $r$.
Suppose that the candidate view $v^*$ which results in an optimal rewrite $r^*$
is not examined by the algorithm before terminating.
In other words, the algorithm incorrectly reported
$r$ as the best rewrite when $\cost(r^*) < \cost(r)$.

As the candidate view $v$ was examined before $v^*$ from the $\PQ$, it must have
been the case that $\ocost(v) < \ocost(v^*)$.

Once $v$ was found $\minCost{}_n$ is set to $\cost(r)$, which means the algorithm
will not terminate until all candidate views whose $\ocost{}$ is less than or equal
to $\minCost{}_n$ (i.e., $\cost(r)$) have been found.

By combining the above inequalities with the lower bound property of $\ocost{}$ with
respect to $\cost{}$, we have that:

$\ocost(v) < \ocost(v^*) \leq \cost(r^*) < \cost(r) = \minCost_n$.

This means that the algorithm must have examined $v^*$ (and consequently $r^*$) before terminating,
which results in a contradiction that $r$ was reported as the best rewrite.

% SJ: Good text but repeating
% From the above result, we can see that the algorithm will examine all candidate views with
% $\ocost{}$ less than or equal to $\cost(r^*)$ but terminate before examining
% a candidate view with $\ocost{}$ greater than $\cost(r^*)$, taken together shows that
% the algorithm finds the optimal rewrite $r^*$ and is work efficient for a single target.

For a general case of $W$ containing $n$ targets,
we only need to show that our  algorithm with $n$ priority queues
can be reduced to an equivalent problem containing 
a single global priority queue of all 
possible rewrites where each rewrite is ordered
by its \ocost{}.  
We omit this reduction due to lack of space.
Given we have already shown the algorithm works for
a single queue case, this reduction proves the optimality
of the general case.\qed


% RETAIN THE REMAINDER OF THIS PROOF HERE.
For a general case of a workflow $W$ containing $n$ targets, we first observe that
our $\WF$ algorithm by identifying the minimum candidate view at
each iteration
reduces the $n$ priority queues (one at each target) of candidate views into a single
``virtual'' priority queue containing ``composite'' candidate views formed
by those drawn from different targets.
In contrast to the incremental explosion of the space of candidate views by our algorithm,
the reduction from multiple priority queues to a single priority queue $\PQ'$ here
follows a pre-explosion of the space of candidate views into composite views
before the start of the algorithm in order to decouple the composite view
creation process from the rewrite search process.
We will later show that the $\ocost{}$ function on the composite views is still a lower
bound on the $\cost{}$ function on the rewrites yielded by these composite views.
% TODO: Can be expanded quite a bit to show how we avoid the explosion by caching the
% best known cost for each target
The reduction happens as follows:
First, generate all possible candidate views at all targets in $W$.
Next, add all the candidate views at $W_n$ to $\PQ'$ such that
each candidate view $v$ is now recorded as a composite view
denoted by the pair $(v, W_n)$.
For all parents target of $W_n$, form all possible composite views
by taking one candidate view from each parent target of $W_n$.
The composite view records its candidate views as well as the targets from
which they are drawn.
We keep doing this recursively by exploding one or multiple
targets at a time till we have completely exhausted all the
combinations of targets in the workflow.

The $\ocost{}$ of a composite view is the sum of the $\ocost{}$ of each
candidate view in the composite to its corresponding target (say, $a$),
plus the sum of the $\cost{}$ of the targets in the workflow that lie
in the remaining path from the targets in the composite view to $W_n$
(say, $b$).
The $\cost{}$ of a rewrite yielded by a composite view is the sum of the
rewrites yielded by the each
candidate view in the composite to its corresponding target (say $c$),
plus the sum of the $\cost{}$ of the targets in the workflow that lie
in the remaining path from the targets in the composite view to $W_n$
(i.e., $b$).

To show that $\ocost{}$ still lower bounds $\cost{}$, we observe that
for each of the candidate views in the composite its $\ocost{}$ contribution
lower bounds the $\cost{}$ of the rewrite it yields (i.e., $a \leq c$),
while the sum of the $\cost{}$ of the remaining targets in the workflow
(i.e., $b$) is common to both $\ocost{}$ and $\cost{}$ of the composite views.

Given that we have reduced the $n$ target $\PQ$ to a single equivalent one
$\PQ'$ and shown that $\ocost{}$ is still a lower bound of $\cost{}$,
our algorithm finds the optimal rewrite $r^*$ and is work efficient. \qed
\end{proof}
\end{comment}



==> old/Bestfirst_workflow_rewrite.tex <==
\section{Best-First Workflow Rewrite}\label{sec-best-first-workflow-rewrite}

Given a workflow $W$ with $n$ targets,
the $\WF{}$ algorithm produces an {\em optimal} rewrite $r^*$ of $W$ in
a  {\em work efficient} manner.
The rewrite $r^*$ is {\em optimal}  in the sense that there cannot be a cheaper
rewrite for $W$ than $r^*$, where $r^*$ can be composed of rewrites found at multiple targets in $W$.
The proposed algorithm is also {\em work efficient} in the sense
that it will never explore more of the solution space than the minimum
necessary to find $r^*$.

The bottom-up approach exhaustively looks at every target in $W$ for a valid rewrite
but considers each target in isolation.
In contrast, our algorithm spawns $n$ concurrent (i.e., non-isolated)
search problems at each of the targets in $W$.
We take advantage of the concurrent searches in that whenever
we find a rewrite at a target we can use this to aid in pruning the
search space of other targets in the workflow.
Moreover even when an incremental search at a target
does not yield a rewrite, this can still aid in pruning the space at other targets.

\begin{comment}
The high-level structure of the $\WF{}$ algorithm is as follows.
\begin{enumerate}
  \item \textsc{initialize} the \VF{} for each target
  \begin{itemize}%
  \renewcommand{\labelitemi}{$\cdot$}
    \item Set $W_i$ as the best rewrite found so far for target \node{i}
  \end{itemize}
  \item \textsc{loop} until obtaining $r^*$
  \begin{itemize}%
    \renewcommand{\labelitemi}{$\cdot$}
    \item Identify the next minimum target $W_i$ to incrementally search
    \item \Refine{} $W_i$ using \VF{}
  \end{itemize}
\end{enumerate}
\end{comment}


\begin{algorithm}[!h]
\caption{Optimal rewrite of $W$ using $\VF$\label{alg-main-setup}}
{\small
\begin{algorithmic}[1]
\Function{$\WF$}{$W$, $V$}
\ForAll{$W_i \in W$}\Comment{Init Step}\label{line-wf-init}
  \State $\VF$.{\sc Init}($W_i$, $V$)
  \State $W_i$.$\minPlumb$ \qlet $W_i$ \Comment{original workflow at $W_i$}
  \State $W_i$.$\minCost$ \qlet $\cost(W_i)$\Comment{workflow cost}
\EndFor \label{line-wf-init-end}
% \State $W_i \qlet W_n$
% \While{$W_i$ $\not= -1$}\label{line-rewrite-wf-start-while-loop}
%   \State $W_i, d_i \qlet \FindNextMinTarget(W_n)$\label{line-wf-find-next-min}
%   \State $\RefineTarget(W_i)$ {\bf if} $W_i \not= -1$
% \EndWhile\label{line-rewrite-wf-end-while-loop}
\Repeat\label{line-rewrite-wf-start-while-loop}
  \State $W_i, d_i \qlet \FindNextMinTarget(W_n)$\label{line-wf-find-next-min}
  \State $\RefineTarget(W_i)$ {\bf if} $W_i \not= -1$
\Until{$W_i$ $= -1$}\label{line-rewrite-wf-end-while-loop}
\State Rewrite $W$ using $W_n.\minPlumb$
\EndFunction
\end{algorithmic}}
\end{algorithm}


Algorithm~\ref{alg-main-setup} presents the main \WF{} function.
The initialization for each target $W_i \in W$ is shown in 
lines~\ref{line-wf-init}--\ref{line-wf-init-end}.
$\minPlumb$ records the best rewrite of $W_i$ found so far,
and its cost is recorded in $\minCost$.
After initialization it begins the best-first rewrite search process by starting
at the final node of the workflow ($W_n$) and then continues to ask for the
next minimum target in $W$ to begin/resume the search.
This is given by line~\ref{line-wf-find-next-min} inside the primary repeat loop,
which identifies the next target $W_i$ to resume the incremental search by
invoking Algorithm~\ref{alg-find-next-min}.
The return value $W_i$ corresponds to the next target to resume searching, while return value
$d_i$ represents the minimum \ocost{} of a rewrite for $W$ that has not been examined so far.
In other words, at this stage of execution \WF{} has examined all possible rewrites whose cost is less than $d_i$.
Next \WF{} invokes Algorithm~\ref{alg-refine-dag} which calls the \Refine{} function of the \VF{} at target $W_i$.
This asks the \VF{} to examine only the next candidate view for that target, as determined by its \ocost{},
and this forms the basis of the incremental nature of \WF{}.
While the \VF{} performs an incremental search at each target, the \WF{} performs an incremental search
in the space of all possible rewrites for $W$.
%In a sense, $d_i$ never decreases and \WF{} stops when $d_i$ equals $\cost(r^*)$ as we show later.
In a sense, ordering the candidate views by increasing \ocost{} at each target, along with the lower-bound nature
of \ocost{} ensures that $d_i$ never decreases and \WF{} stops when $d_i$ equals $\cost(r^*)$ as we show later.

\begin{algorithm}[!h]
\caption{Find next min target to refine\label{alg-find-next-min}}
{\small
\begin{algorithmic}[1]
\Function{$\FindNextMinTarget$}{$W_i$}
\State $W' \qlet \mbox{empty}$;  $sum \qlet 0$; $d' \qlet \infty$
\State $d_i \qlet \VF.\mbox{\sc Peek}()$
\ForAll{incoming vertex $\node{j}$ of $\node{i}$}\label{line-refine-target-vertex}
  \State $W_k, d_k$ \qlet $\FindNextMinTarget(W_j)$
  \State $sum \qlet sum + d_k$
  \If{$d' > d_k$ and $W_k \not= -1$}
    \State $W' \qlet W_k$
    \State $d' \qlet d_k$
  \EndIf
\EndFor
\State $sum$ \qlet $sum + \cost(\node{i})$
\If{$\min(sum,d_i) \geq W_i.\minCost$}
  \State \Return $-1, W_i.\minCost$
\ElsIf{$sum < d_i$}
  \State \Return $W'$, $sum$
\Else
  \State \Return $W_i$, $d_i$
\EndIf
\EndFunction
\end{algorithmic}}
\end{algorithm}


The recursive algorithm given in Algorithm~\ref{alg-find-next-min} identifies the target to be refined next
in the workflow $W$ as well as the minimum cost (\ocost) of a possible rewrite for $W_i$.
Let $r$ denote a rewrite of $W_i$ using a candidate view at the instance of the \VF{} at $W_i$.
Let $r'$ denote a rewrite obtained by combining rewrites found at the ancestors of $W_i$.
The value $d_i$ (\VF.\Peek) captures the minimum possible cost of $r$, while $sum$ (sum of \VF.\Peek{} at ancestors) captures the minimum possible cost of  $r'$.
If both $sum$ and $d_i$ are greater than or equal to $W_i.\minCost$ this means that $W_i$ and all of its
ancestors cannot provide a lower cost rewrite than the best rewrite already found for $W_i$
and there is no need to further refine $W_i$ or any of its ancestors
for the remainder of the algorithm.
If $sum$ is less than $d_i$, let $W'$ represent the ancestor target with the minimum cost candidate view in $r'$,
 and hence must be the next target to refine.
If $d_i$ is less than or equal to $sum$, then $W_i$ must be the next target to refine.



\begin{algorithm}[!t]
\caption{Queries \VF{} in best-first manner\label{alg-refine-dag}}
{\small
\begin{algorithmic}[1]
\Function{$\RefineTarget$}{$W_i$}
\State $r$ \qlet \VF.{\sc Refine}($W_i$)
 \If{$r$ is not empty}
   \If{$\cost(r) < W_i.\minCost$}
     \State $W_i.\minPlumb$ \qlet $r$
     \State $W_i.\minCost$ \qlet $\cost(r)$
      \ForAll{outgoing vertex $\node{k}$ of $\node{i}$}% \Comment{towards $W_n$}
       \State $\PropagateBestRewrites$($\node{k}$)\label{line-view-finder-propagate-best-plans}
     \EndFor
   \EndIf
 \EndIf
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{$\PropagateBestRewrites$}{$\node{i}$}
\State $r$ \qlet $\node{i}$
\ForAll{incoming $\node{j}$ of $\node{i}$}
  \State $r \qlet r \cup W_j.\minPlumb$
\EndFor
\If{$\cost(r)$ < $W_i.\minCost$}
   \State $W_i.\minCost$ \qlet $\cost(r)$
   \State $W_i.\minPlumb$ \qlet $r$
   \ForAll{outgoing $\node{k}$ of $\node{i}$}
     \State $\PropagateBestRewrites$($\node{k}$)
   \EndFor
\EndIf
\EndFunction
\end{algorithmic}
}
\end{algorithm}



Algorithm~\ref{alg-refine-dag} describes the process for refining a target $W_i$ which was
previously identified by Algorithm~\ref{alg-find-next-min}.
Refinement is a two-step process.
First it obtains a rewrite $r$ of $W_i$ from \VF{} if one exists.
The cost of the rewrite $r$ obtained by $\RefineTarget$ is compared against the best
rewrite found so far at $W_i$ and then if found to be lesser suitably updates $W_i.\minPlumb{}$ and $W_i.\minCost{}$.
In the second step it tries to use $r$ as part of a rewrite of $W$ using
the recursive function given by $\PropagateBestRewrites$ in Algorithm~\ref{alg-refine-dag}.
The recursion pushes the rewrite $r$ downward toward $W_n$, and if it succeeds $r$ becomes part
of the best rewrite of $W$ found so far.  
Example~\ref{ex-algo-description} shows how \WF{} attempts to rewrite a sample workflow.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Example %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\onefig{fig-optcost-algo-illustration}
{Three workflow nodes $n_1, n_2$ and $n_3$ with  
candidate views ordered by their $\ocost{}$ $a$--$f$.}
{2.75in}

\begin{example}\label{ex-algo-description}
Figure~\ref{fig-optcost-algo-illustration} shows a workflow containing
three nodes $n_1, n_2$ and $n_3$, where $n_3$ represents $W_n$.
The 5 candiate views $a$--$f$ are arranged by their
$\ocost{}$ from the target nodes.
For example, $b$ is placed at $\ocost{}$ of 6 from $n_3$.
The cost of nodes $n_1,n_2,n_3$ is 6,5,2 respectively, 
hence $n_3.\minPlumb{}$ (i.e.,$W_n.\minPlumb{}$) begins with \cost{}=13.

In the first step of the algorithm,
the cheapest potential rewrite for $n_3$ is determined to be
$(a=1)$+$(c=2)$+$(n_3=2)$ having a total \ocost{} of 5, 
whereas the next cheapest possible rewrite of $n_3$ using $b$ has an \ocost{} of 6.
$\FindNextMinTarget$ chooses $a$ as the first candidate view to $\Refine{}$ 
within $a+c+n_3$ because the $\ocost{}$ of $a$ (=1) is less than $c$ (=2).
After refining $a$, the actual $\cost{}$ of $a$ is found to be 4, which is shown 
by the dashed line from $a$ in Figure~\ref{fig-optcost-algo-illustration}.
Therefore $n_1.\minCost{}$ is set to 4.
Now since the best known rewrite for 
$n_3$ is $(a=4)$+$(n_2=5)$+$(n_3=2)$ is 11, 
the value $n_3.\minCost{}$ is updated from 13 to 11 by $\PropagateBestRewrites{}$. 

Next it attempts the rewrite for $n_3$ using $b$ with an $\ocost{}$ of 6, 
which is less than the next best choice of $(d=3)$+$(c=2)$+$(n_3=2)$
with a total $\ocost{}$ of 7.
The \cost{} of the rewrite of $n_3$ using $b$ was found to be 12 as indicated 
in Figure~\ref{fig-optcost-algo-illustration}.
Since $n_3.\minCost{}$ is already 11, it is not updated.

The next best choice for $n_3$ is the rewrite with the $\ocost{}$ of 7.
Within that rewrite, $\FindNextMinTarget{}$ chooses to refine $c$,
yielding a rewrite for $n_2$ whose actual cost is 4,
so $n_2.\minCost{}$ is set to 4.
Then $n_3.\minPlumb{}$ and $n_3.\minCost${} are set to be
$(a=4)$+$(c=4)$+$(n_3=2)$ with a total cost of 10.
Figure~\ref{fig-optcost-algo-illustration} captures
this present state of the algorithm after the first three rewrite attempts.

The algorithm would proceed to the next best possible rewrite of
$(d=3)$+$(c=4)$+$(n_3=2)$ with \ocost{} of 9 which is still better 
than the best known rewrite of $n_3$ with cost of 10.
The algorithm terminates when there are no possible rewrites remaining for 
$W_n$ with a \ocost{} less than $W_n.\minCost${}.
%hence the algorithm cannot stop until it is examined.
%Finally, $e$ can be pruned as it exceeds the current $\minCost{}$ at $n_3$.
Any view with an \ocost{} greater than their target node's $\minCost${} can be pruned away, 
e.g., $e$ at $n_3$ (since $11>10$) and $f$ at $n_1$ (since $5>4$).
\end{example}


It it noteworthy in Example~\ref{ex-algo-description} that the algorithm did not
start at $n_3$ first, and had it examined all the candidate
views of $n_3$ first as a bottom-up approach would have done, it would have
examined a larger search space than necessary.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UGLINESS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\input{scenario}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}
The $\WF{}$ finds the optimal rewrite $r^*$ of workflow $W$ and is work efficient.
\end{theorem}

\begin{proof}
% Should search far enough
Finding the optimal rewrite requires that the algorithm
must not terminate before finding $r^*$.
Ensuring work efficiency requires that the algorithm
should not examine any candidate views
that cannot be possibly included in $r^*$.
First we prove these properties for a workflow $W$ containing a single target, 
then extend to an arbitrary workflow containing $n$ targets.
For the single target case, the algorithm must examine
every candidate view with $\ocost{}$ less than or equal to $\cost(r^*)$,
but must not examine any candidate view with $\ocost{}$ greater than $\cost(r^*)$.

Proof by contradiction is as follows.
Suppose that the algorithm found a candidate view $v$, 
which resulted in a rewrite $r$.
Suppose that the candidate view $v^*$ which produces the optimal rewrite $r^*$
is not considered by the algorithm before terminating
thus incorrectly reporting
$r$ as the optimal rewrite 
even though $\cost(r^*) < \cost(r)$.
As the candidate view $v$ was examined before $v^*$ from the $\PQ$, it must have
been the case that $\ocost(v) < \ocost(v^*)$.
Once $v$ was found $W_n.\minCost{}$ is set to $\cost(r)$, which means the algorithm
will not terminate until all candidate views whose $\ocost{}$ is less than or equal
to $W_n.\minCost{}$ (i.e., $\cost(r)$) have been found.
Combining the above inequalities with the lower bound property of $\ocost{}$ with
respect to $\cost{}$, we have:

$\ocost(v) < \ocost(v^*) \leq \cost(r^*) < \cost(r) = W_n.\minCost$.

This means that the algorithm must have examined $v^*$ (and consequently $r^*$) before terminating.
Hence the contradiction that $r$ was reported as the best rewrite.

For a general case of a workflow $W$ containing $n$ targets,
we show that our  algorithm with $n$ priority queues
can be reduced to an equivalent problem of a
single global priority queue.
The queue contains all possible rewrites that include all candidate
views from every target, and each rewrite is ordered
by its \ocost{}.  
We omit this reduction due to lack of space.
Given we have already shown these properties for the
single queue case, this reduction proves the optimality and work efficiency
of the general case.\qed
\end{proof}

\begin{comment}
\begin{proof}
% SHORTENED DUE TO LACK OF SPACE
% Should search far enough
To ensure that the algorithm finds the optimal rewrite $r^*$ of $W$,
it suffices to show that it will not terminate before finding $r^*$.
This implies that the algorithm will examine
every candidate view with $\ocost{}$ less than or equal to $r^*$.
In other words, the algorithm must examine
all candidate views that could possibly be included in $r^*$.

% Should not search too many
Next, work efficiency of the algorithm requires that the algorithm
does not examine any candidate views with $\ocost{}$ greater than $r^*$.
In other words, the algorithm should not examine any candidate views
that cannot be possibly included in $r^*$.

We first show these results for a workflow $W$ containing a single target, then
extend them to an arbitrary workflow containing $n$ targets.

To show that the algorithm will find the optimal rewrite of $W$,
suppose that the algorithm found a candidate view $v$, which resulted in a rewrite $r$.
Suppose that the candidate view $v^*$ which results in an optimal rewrite $r^*$
is not examined by the algorithm before terminating.
In other words, the algorithm incorrectly reported
$r$ as the best rewrite when $\cost(r^*) < \cost(r)$.

As the candidate view $v$ was examined before $v^*$ from the $\PQ$, it must have
been the case that $\ocost(v) < \ocost(v^*)$.

Once $v$ was found $W_n.\minCost{}$ is set to $\cost(r)$, which means the algorithm
will not terminate until all candidate views whose $\ocost{}$ is less than or equal
to $W_n.\minCost{}$ (i.e., $\cost(r)$) have been found.

By combining the above inequalities with the lower bound property of $\ocost{}$ with
respect to $\cost{}$, we have that:

$\ocost(v) < \ocost(v^*) \leq \cost(r^*) < \cost(r) = W_n.\minCost$.

This means that the algorithm must have examined $v^*$ (and consequently $r^*$) before terminating,
which results in a contradiction that $r$ was reported as the best rewrite.

% SJ: Good text but repeating
% From the above result, we can see that the algorithm will examine all candidate views with
% $\ocost{}$ less than or equal to $\cost(r^*)$ but terminate before examining
% a candidate view with $\ocost{}$ greater than $\cost(r^*)$, taken together shows that
% the algorithm finds the optimal rewrite $r^*$ and is work efficient for a single target.

For a general case of a workflow $W$ containing $n$ targets,
we only need to show that our  algorithm with $n$ priority queues
can be reduced to an equivalent problem containing 
a single global priority queue of all 
possible rewrites where each rewrite is ordered
by its \ocost{}.  
We omit this reduction due to lack of space.
Given we have already shown the algorithm works for
a single queue case, this reduction proves the optimality
of the general case.\qed


% RETAIN THE REMAINDER OF THIS PROOF HERE.
For a general case of a workflow $W$ containing $n$ targets, we first observe that
our $\WF$ algorithm by identifying the minimum candidate view at
each iteration
reduces the $n$ priority queues (one at each target) of candidate views into a single
``virtual'' priority queue containing ``composite'' candidate views formed
by those drawn from different targets.
In contrast to the incremental explosion of the space of candidate views by our algorithm,
the reduction from multiple priority queues to a single priority queue $\PQ'$ here
follows a pre-explosion of the space of candidate views into composite views
before the start of the algorithm in order to decouple the composite view
creation process from the rewrite search process.
We will later show that the $\ocost{}$ function on the composite views is still a lower
bound on the $\cost{}$ function on the rewrites yielded by these composite views.
% TODO: Can be expanded quite a bit to show how we avoid the explosion by caching the
% best known cost for each target
The reduction happens as follows:
First, generate all possible candidate views at all targets in $W$.
Next, add all the candidate views at $W_n$ to $\PQ'$ such that
each candidate view $v$ is now recorded as a composite view
denoted by the pair $(v, W_n)$.
For all parents target of $W_n$, form all possible composite views
by taking one candidate view from each parent target of $W_n$.
The composite view records its candidate views as well as the targets from
which they are drawn.
We keep doing this recursively by exploding one or multiple
targets at a time till we have completely exhausted all the
combinations of targets in the workflow.

The $\ocost{}$ of a composite view is the sum of the $\ocost{}$ of each
candidate view in the composite to its corresponding target (say, $a$),
plus the sum of the $\cost{}$ of the targets in the workflow that lie
in the remaining path from the targets in the composite view to $W_n$
(say, $b$).
The $\cost{}$ of a rewrite yielded by a composite view is the sum of the
rewrites yielded by the each
candidate view in the composite to its corresponding target (say $c$),
plus the sum of the $\cost{}$ of the targets in the workflow that lie
in the remaining path from the targets in the composite view to $W_n$
(i.e., $b$).

To show that $\ocost{}$ still lower bounds $\cost{}$, we observe that
for each of the candidate views in the composite its $\ocost{}$ contribution
lower bounds the $\cost{}$ of the rewrite it yields (i.e., $a \leq c$),
while the sum of the $\cost{}$ of the remaining targets in the workflow
(i.e., $b$) is common to both $\ocost{}$ and $\cost{}$ of the composite views.

Given that we have reduced the $n$ target $\PQ$ to a single equivalent one
$\PQ'$ and shown that $\ocost{}$ is still a lower bound of $\cost{}$,
our algorithm finds the optimal rewrite $r^*$ and is work efficient. \qed
\end{proof}
\end{comment}



==> old/Bestfirstplumbing.old.tex <==
\section{Problem Overview}

Given as input an evolutionary query workflow $W$, and a set of existing
materialized views $V$, we want to find a rewrite of $W$ that
minimizes the total execution cost of $W$.
\begin{comment}
We decompose this problem into two sub-problems.
First, we introduce a $\ViewFinder{}$ which 
given a query, a set of candidate artifacts, 
and a set of transformational rules finds the cheapest rewrite workflow of the target, 
if such a plan exists.
Next, utilizing the $\ViewFinder{}$ at each target, 
we introduce a workflow rewrite algorithm $\WorkflowRewrite{}$ that obtains the
lowest cost workflow rewrite plan of $W$, while performing minimum amount of work.
\end{comment}
The problem of finding a rewrite of a query using materialized views
is known to be NP-complete even considering a language 
for both queries and views belonging to the simple class
of conjunctive queries~\cite{Levy1995}.
In this work, we consider a much richer workflow language that
includes UDFs
thus making our problem at least as hard as the case for conjunctive query rewrites.
% Furthermore, existing candidates may only be {\em partial} solutions with 
% respect to the target, thus we have to consider creating new candidates by {\em merging}
% existing candidates, which explodes the space further.
Finding an optimal rewrite of $q$ requires considering all 
combinations of materialized views and transformation rules, which
makes the solution search space exponential in the
number of materialized views and the number of transformation rules.
In essence, finding the rewrite workflow for a single target
in a workflow is expensive.

\begin{comment}
\begin{algorithm}[htp]\label{algn-main-setup}
\begin{algorithmic}[1]
\State {\sf sub} $\WorkflowRewrite$($W$)\\
\Comment{Produces an optimal rewrite of $W$ using $\ViewFinder$}
\State $p^* \qlet W_n$\Comment{Original workflow}
\If{{\bf {\em simple/traditional} variant}} 
   \State $p$ \qlet $\ViewFinder(t_n)$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
\ElsIf{{\bf {\em bottom-up greedy} variant}}
   \ForAll{$t_i$ in $\{t_n \cdots t_1\}$}
    \State $p \qlet \ViewFinder(t_i) \cup \{q_{i+1} \cdots q_n\}$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
   \EndFor
\EndIf
\State Rewrite $W$ using $p^*$
\end{algorithmic}
\end{algorithm}

Given the $\ViewFinder{}$ only finds a rewrite of a single target, 
a workflow rewrite algorithm is required in order to 
to find an optimal rewrite plan for the entire workflow
in the most efficient manner with the aid of the $\ViewFinder{}$. 
To show that finding an optimal rewrite plan for the workflow is 
not straightforward, consider two simple approaches, 
namely {\em simple} and {\em greedy}, as shown in 
the procedure $\WorkflowRewrite$.
The simple variant queries the $\ViewFinder{}$ for a rewrite plan for
$t_n$, using it as the workflow rewrite plan of $W$.
The intuition here that
the {\em optimal} rewrite plan of $t_n$ produced by the 
$\ViewFinder{}$ is also the optimal rewrite plan for $W$.
So, the most likely outcome of applying the simple variant is
that we may not find any rewrite plans for $t_n$.
\end{comment}

Given a workflow $W$ as input, the 
$\ViewFinder{}$ searches for a rewrite workflow for $W_n$
using the existing materialized views $V$ in the system.
Note that the $\ViewFinder{}$ may not be able to find a rewrite for $W_n$
in some cases as $L_R \subseteq L_W$.
For instance, if $W_n$ contains a UDF that is not part of the rewrite
transformation language, the $\ViewFinder{}$
may not be able to produce a rewrite for $W_n$ in spite of allowing
it sufficient time.
Another side-effect of $L_R \subseteq L_W$ is that the $\ViewFinder{}$
has to look for rewrites at other targets in $W$ even if found a rewrite at $W_n$.
One strategy is to search for plans at the other targets $W_i$ in $W$ 
in a bottom-up manner starting with $W_{n-1}$.
If a rewrite $r$ is found at $W_i$, $r$ can be expressed as a rewrite 
for $W_n$ by combing $r$ with the remaining part of the workflow 
indicated by $q_{i+1} \cdots q_n$.
One major drawback of this algorithm is that 
it may search a long time for rewrites at 
a target $W_i$, while it could have quickly obtained
a rewrite another target had it looked there first 
as shown in Example~\ref{example-greedy-plumbing}.

% when we can try to find {\em shorter} plans at other targets of $W$.
% As we will see later that it is more time consuming for the
% $\ViewFinder$ to find longer plans (as there are many of them) 
% as compared to finding shorter plans, which are quick to find.
% The following example shows why the {\em greedy} variant
% may not do the best possible job of finding efficiently a rewrite plan for $W$.
\begin{minipage}{0.75\columnwidth}
\vspace{0.1in}
\begin{example}\label{example-greedy-plumbing}
% Figure~\ref{fig-greedy-plumbing-fails} shows an example of
The figure alongside shows an example of 
finding a rewrite workflow for $W$ using a bottom up approach. 
Suppose that the $\ViewFinder{}$ could not find a rewrite for 
targets $W_n$ and $W_{n-2}$ due to the lack of expressivity 
of the rewrite language with respect to the language of the workflow,
yet was able to find an expensive rewrite for $W_{n-1}$.
The bottom-up algorithm would have performed much better had
it looked for cheap rewrites at $W_{n-3}$ instead of
trying to find a rewrite for $W_{n-2} \cdots W_{n}$.
\end{example}
\end{minipage}%
\begin{minipage}{0.25\columnwidth}
\centering
\includegraphics[width=0.75in]{fig-greedy-plumbing-fails}
\end{minipage}
\vspace{0.2in}

The bottom-up variant of the $\ViewFinder{}$
is not {\em work efficient} in the sense that
it did not make use a rewrite found in $W_i$
to bound the search space at another target $W_j$ in the workflow.
For example, had the bottom-up strategy first found the cheap
rewrite at $W_{n-3}$ it may not have needed the exhaustively
search the space at $W_n$ and $W_{n-2}$, and perhaps
may have stopped sooner at $W_{n-1}$.
Note that searching for all possible rewrites at $W_n$ and $W_{n-2}$
is extremely time consuming especially if there are many
materialized views in the system.
The inefficiency of the bottom-up approach is in-part due to 
not considering the rich interactions that are possible between the 
$n$ search problems at each of the targets in $W$.

% Note that being able to take advantage of the interactions
% between the $n$ rewrite search problems at each of the targets
% requires the design of the $\ViewFinder{}$ 
% to be {\em incremental} in that it can find
% cheaper plans first and expensive plans later as well as
% has the ability to stop early if a cheaper plan is found
% at some other target that obviates the need to search 
% further at a particular target.

In this paper, we propose a work efficient algorithm
by breaking the problem into two components, 
$\ViewFinder{}$ finds the best possible rewrite
for a single workflow input and $\WorkflowRewrite{}$
that tries to combine the rewrites found for all the $n$ targets
into a globally optimal rewrite for $W_n$.
The $\WorkflowRewrite{}$, on the other hand, concurrently looks for rewrites for each of the $n$
targets, while maintaining the cheapest ({\em best}) 
rewrite for $W$ found thus far.
Additionally, by communicating the success or failure in finding
a rewrite at a target $W_i$ with other the targets in the workflow,
the approach obviates the need to look in sub-spaces
where it is not possible to find a cheaper rewrite for $W$.
This forms the best-first nature of our proposed algorithm.
In the following section, we will provide a design of an algorithm
which will find the {\em optimal rewrite} for a given workflow, while
also being {\em work efficient}

Our design of an $\ViewFinder{}$ is inspired by nearest neighbor finding problems
in metric spaces (e.g., road networks) where computing the distances between 
objects can be computationally expensive.
For instance, in the case of road networks the distance between two vertices
requires the invocation of a shortest path algorithm
to find the shortest path between two vertices.
Next, the network distance between
the two vertices can be determined by summing up the edge weights along the shortest path.
In such metric spaces, a common strategy to avoid expensive
network distance computations between vertices is by making
use of an alternate distance function (e.g., Euclidean or the geodesic distance function)
that is easy to compute (i.e., not requiring a search process) 
with the desirable property it is always less than or equal to 
the network distance function.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the network distance between vertices.

Our current problem domain has a similar properties to 
nearest neighbor searches in metric spaces, such as the one described above. 
We are given a materialized view $v$ and a query $q$
such that the cost function $\cost()$ 
corresponds to the amount of time or effort required 
in transforming $v$ so that it produces an output that is
identical to that produced by $q$.
As will be discussed later, this problem is known to be NP-hard, 
which means that finding a rewrite 
workflow for $q$ using $v$ requires examining all possible
rewrites involving $v$ and testing their {\em equivalence} with $q$.
This is expensive as the number of possible rewrites of $q$ involving
$v$ is exponential in the number of transformation rules in the system.
In other words, computing the rewrite plan for $q$ using $v$
first requires finding a rewrite plan for $q$, which is a search
process similar to the shortest computation in road networks.
The intuition here is that we want to make use of another distance
function, which is easy to compute and has some desirable with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$ 
that takes as input $v$ and $q$ and always provides a 
lower-bound on $\cost()$ without enumerating 
all possible rewrites of $q$ involving $v$.
In other words, if $r$ is the cheapest rewrite plan
of $q$ involving $r$, we have that $\cost(r) \leq \ocost(v,q)$.

While the details of the $\ViewFinder{}$ algorithm and the cost
functions will will be provided in a later section, 
for the sake of developing the $\WorkflowRewrite{}$ algorithm,
it is sufficient to model $\ViewFinder{}$ as a black-box 
$\ViewFinder(W_i, d, d',\cost(), \ocost())$, $d < d'$, that takes
as input a workflow $W_i$, two thresholds $d, d'$, 
a cost function $\cost()$, an optimistic cost function $\ocost{}$
and outputs a single rewrite $r$ of $W_i$ with the following properties:

\begin{enumerate}

\item $r$ is a rewrite workflow for $W_i$ using $V$ and the transformation rules

\item The invocation of the $\ViewFinder(W_i,d,d')$ such that $d < d'$ 
examines all rewrites of $W_i$ whose optimistic cost is less than or equal to $d'$.
Moreover, any subsequent invocation of 
$\ViewFinder(t_i, d', d", \cost(), \ocost())$, such that $d' < d"$,
will not produce a rewrite whose optimistic cost is less than or equal to $d'$.

\item $d < \ocost(r) \leq d'$ such that $r$ has the lowest
cost among all the plans found by $\ViewFinder{}$ in this invocation.

% \item The time taken (or cost) to answer $\ViewFinder(t_i,d,d")$ is 
% just a little more than the time taken to answer 
% $\ViewFinder(t_1, d, d')$ and $\ViewFinder(t_1, d', d")$. 
\end{enumerate}

\section{Best-First Workflow Rewrite}

\begin{comment}
\begin{algorithm}[htp]\label{algn-main-setup}
\begin{algorithmic}[1]
\State {\sf sub} $\WorkflowRewrite$($W$)\\
\Comment{Produces an optimal rewrite of $W$ using $\ViewFinder$}
\ForAll{$t_i \in W$}\Comment{Init Step}
  \State $t_i$.$\seenSoFar$ \qlet 0 \Comment{nothing explored}
  \State $t_i$.$\minPlumb$ \qlet $W_i$ \Comment{original workflow}
  \State $t_i$.$\minCost$ \qlet $\cost(W_i)$\Comment{workflow cost} 
\EndFor
\State $d_0$ (=$t_n.\seenSoFar$) $< d_1$ $< \cdots$ $< d_l$ (= $q_m.\minCost)$ is a number sequence
\State $i \qlet 1$
    \While{$t_n.\seenSoFar \leq t_n.\minCost$}
      \If{{\bf {\em simple} variant}} 
        \State $p$ \qlet $\ViewFinder(t_n, d_{i-1}, d_{i})$
        \If{$\cost(p)$ < $t_n.\minPlumb$}
           \State $t_n.\minPlumb \qlet p$
           \State $t_n.\minCost \qlet \cost(p)$
        \EndIf
      \ElsIf{{\bf {\em greedy} variant}}\\
        \Comment{Perform {\em simple} variant for all targets $t_i \in \{t_n \cdots t_i\}$} 
      \ElsIf{{\bf {\em best-first} variant}} 
         \State $\RefineTarget(t_n, d_i)$
      \EndIf
      \State $t_n.\seenSoFar \qlet{} d_i$
      \State $i$ \qlet{} $i + 1$
    \EndWhile
\State Rewrite $W$ using $t_n.\minPlumb$
\end{algorithmic}
\end{algorithm}
\end{comment}

Given a workflow $W$ with $n$ targets as input, the
$\WorkflowRewrite{}$ algorithm produces an {\em optimal} rewrite workflow of $W$ that is 
also {\em work efficient}.
As we will show later, 
our algorithm is {\em optimal} in the sense that there cannot be a cheaper
rewrite workflow $r^*$ for $W$ than the one found by the algorithm.
In particular, we will show that the algorithm will not
terminate early before finding $r^*$, even if $r^*$ is composed 
of rewrite plans found at multiple targets in $W$.
In other words, the rewrite of $W$ found by the $\WorkflowRewrite{}$
is always the cheapest for a given implementation of the $\ViewFinder{}$.
The proposed algorithm is also {\em work efficient} in the sense
that the total amount of work that the algorithm asks of the $\ViewFinder{}$ 
to find the optimal rewrite of $W$ is bounded a term that 
is a little more than $\cost(r^*)$.
In essence, the proposed algorithm will always find the optimal
rewrite of $W$ with very little redundant work.

% Initially, for all $t_i \in W$, the algorithm records the cheapest
% known plan to be $W_i$ and its costs.
In contrast to the bottom-up approach which looks for the cheapest
rewrite at each of the targets in $W$,
our proposed algorithm spawns $n$ concurrent
search problems at each of the targets in $W$.
At each target the extent of the search space is initially
bounded by $\cost(W_i)$, which represents the user-written
workflow up to the target.
The goal here is to find a cheaper rewrite workflow for $W_n$ 
using the materialized views $V$ in the system.
The algorithm searches each of the target $W_i$
for rewrites within a certain optimistic cost interval $[0, \cost(W_i)]$
with the aid of the $\ViewFinder{}$.
If a rewrite $r$ is found for a target $W_i$, the algorithm
will try to use it to come up with a cheaper rewrite for $W_n$.
Moreover, the cost of $r$ can be used to prune the search
space of other targets in the workflow.
Furthermore, even the failure to find a rewrite plan is useful
in this context, and can be used to prune the search space of 
{\em sibling} targets, which we will define later.

Algorithm~\ref{algn-main-setup} provides an implementation of the
$\WorkflowRewrite{}$ algorithm that takes as inputs a workflow $W$,
a cost function $\cost(.)$ and an optimistic cost function $\ocost(.)$
and produces the optimal rewrite of $W_n$.
At the start of the algorithm, for all targets $W_i \in W$, 
the target $W_i$ and the two cost functions $\cost$ and $\ocost$
are registered with the $\ViewFinder{}$.
Next, $W_i.\minPlumb$ and $W_i.\minCost$ record the cheapest
rewrite and the cheapest rewrite cost, which are
initially assigned to the user-written
workflow $W_i$ and its cost $\cost(W_i)$, respectively.
Finally, the value of $W_i.\seenSoFar{}$ is set to 0 indicating
the extents of the search space that has already been explored.
The algorithm divides the search space extents
$[0, W_n.\minCost]$ into $l+1$ values, given by $d_0 \cdots d_{l}$.
At each iteration the algorithm will use the  
$\ViewFinder{}$ via the $\RefineTarget{}$ 
to examines all rewrites of $W_n$ up to an optimistic cost of $d_i$.
The algorithm terminates if $W_n.\seenSoFar$ 
is greater than $W_n.\minPlumb{}$ indicating that we have
completely exhausted the search space for $W_n$.
The rewrite at $W_n.\minPlumb{}$ at the end of the algorithm
is applied to $W$ and represents the optimal rewrite workflow for $W$.
Note that while the algorithm invokes $\RefineTarget{}$ on $W_n$,
the search will propagate to all the other targets in $W$ in a bottom-up fashion.

\begin{algorithm}[htp]
\caption{Optimal rewrite of $W$ using $\ViewFinder$\label{algn-main-setup}}
\begin{algorithmic}[1]
\State {\sf sub} $\WorkflowRewrite$($W$, $\cost(.)$, $\ocost(.)$)
\ForAll{$W_i \in W$}\Comment{Init Step}
  \State $\ViewFinder$.{\sc Register}($W_i$, $\cost(.)$, $\ocost(.)$)
  \State $W_i$.$\seenSoFar$ \qlet 0 \Comment{nothing explored}
  \State $W_i$.$\minPlumb$ \qlet $W_i$ \Comment{original workflow}
  \State $W_i$.$\minCost$ \qlet $\cost(W_i)$\Comment{workflow cost} 
\EndFor
\State $d_0$ (=$W_n.\seenSoFar$) $< d_1$ $< \cdots$ $< d_l$ (= $W_n.\minCost)$ is a number sequence
\State $i \qlet 1$
    \While{$W_n.\seenSoFar < W_n.\minCost$}\label{line-rewrite-wf-start-while-loop}
      \State $\RefineTarget(W_n, d_i)$
      \State $i$ \qlet{} $i + 1$
    \EndWhile\label{line-rewrite-wf-end-while-loop}
\State Rewrite $W$ using $W_n.\minPlumb$
\end{algorithmic}
\end{algorithm}


% SJ: Alkis had this but I repurposed it above..
% To show this, suppose that the condition of the while loop is not satisfied. 
% Then, any plan that has not been examined clearly satisfies the following property: 
% $\cost(p) + d_{i-1} \geq d_i \geq \cost(t_i.\minPlumb)$, 
% which implies that $\cost(p) + d_{i-1} \geq \cost(t_i.\minPlumb)$ 
% since $d_i \leq \cost(p)$.


% \onefig{fig-greedy-plumbing-fails}
% {Setup shows a workflow where bottom-up greedy method of
%   looking for plans performs poorly}{0.75in}

\begin{algorithm}[!htp]
\caption{Queries \ViewFinder{} in best-first manner\label{algn-refine-dag}}
\begin{algorithmic}[1]
\State {\sf sub} $\RefineTarget$($W_i$, $d$)
%\Return {\bf if} $d \leq t_i$.$\seenSoFar$ 
\If{$W_i.\seenSoFar < W_i.\minCost$}\label{line-view-compare-seen-mincost}
 \State $r$ \qlet \ViewFinder($W_i$, $W_i.\seenSoFar$, $\min(d, W_i.\minCost))$
 \State $W_i.\seenSoFar \qlet d$
 \If{$r$ is not empty} 
   \If{$\cost(r) < W_i.\minCost$}
     \State $W_i.\minPlumb$ \qlet $r$
     \State $W_i.\minCost$ \qlet $\cost(r)$
      \ForAll{outgoing vertex $q_j$ of $q_i$} \Comment{towards $W_n$, (a)}
       \State $\PropagateBestRewrites$($q_j$)\label{line-view-finder-propagate-best-plans}
     \EndFor
     \State $\PropagateStats(q_i, \cost(r), \up, \_)$\Comment{to ancestors,(b)}\label{line-refine-target-prop-stats-up}
     \State $d \qlet{} \min(d, \cost(r))$ 
   \EndIf
 \EndIf
 \ForAll{outgoing vertex $q_j$ of $q_i$} \Comment{to siblings, (c)}
  \State $\PropagateStats(q_j, \_, \down, q_i)$\label{line-refine-target-prop-stats-down}
 \EndFor
\EndIf
\ForAll{incoming vertex $q_j$ of $q_i$}\label{line-refine-target-vertex}
  \State $\RefineTarget$($W_j$, $d$ - $\cost(q_i)$)
\EndFor\label{line-refine-target-vertex-end}
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{algn-refine-dag} provides an implementation of 
$\RefineTarget{}$, which is invoked on a target $W_i$ with a cost value $d$. 
It queries the $\ViewFinder{}$ for rewrites for a target $W_i$ 
up to an optimistic cost of $d$.
Note that if $W_i.\seenSoFar > W_i.\minCost$, we have completely exhausted
the search space and as there is no need to look for additional rewrites for $W_i$
beyond $W_i.\minCost$ (line~\ref{line-view-compare-seen-mincost}).
Any rewrite $r$ found by the $\ViewFinder{}$ corresponds to the 
cheapest plan among all those whose optimistic cost is less than equal to $d$.
If $r$ is cheaper than $W_i.\minCost$,
we first update $W_i.\minPlumb{}$ to $r$ and set $W_i.\minCost{}$ to $\cost(r)$.
% Else, we query the $\ViewFinder{}$ to obtain a rewrite $r$ (or none) for $W_i$
% exhausting the search space up to $d$ from $W_i$ and 
% advancing $W_i.\seenSoFar$ to $d$.
Next, $\RefineTarget{}$  is applied to 
all targets $W_j$, such that $q_j$ is an incoming vertex 
of $q_i$, but with a reduced search extent $d - \cost(q_i)$
(lines~\ref{line-refine-target-vertex}--\ref{line-refine-target-vertex-end}).
The reduction in the search extents of $W_j$
accounts for the overhead cost of $\cost(q_i)$ that a rewrite $r'$ of
$W_j$ would have to bear compared to a rewrite $r$ of $W_i$, when
both $r$ and $r'$ are expressed as rewrites of $W_n$.
The $\RefineTarget{}$ algorithm returns back to $\WorkflowRewrite{}$
algorithm when search space of all targets in $W$ have been expanded.

\onefig{fig-propagate-stats}
{If a rewrite $r$ is found for $W_i$, a) $r$ is pushed towards $W_n$,
 and the search spaces of the c) ancestor vertices and d) sibling vertices of $W_i$
 are potentially pruned}{2.75in}

Note that the structure of the $\RefineTarget{}$ algorithm
first searches for cheap rewrites at all targets,
propagating the best plans that are found to other targets,
before searching very deeply at any target.
There are three opportunities for search problem at
$W_i$ to prune the search space at other targets in $W$.
The three cases are captured in Figure~\ref{fig-propagate-stats}
and are described below.

\begin{enumerate}

\item[Case (a)] A rewrite $r$ is found at $W_i$ means that  
we can try to see if we can obtain a cheaper rewrite for
$W_n$ that makes use of $r$. 

\item[Case (b)] If a rewrite $r$ is found in $W_i$, 
then there is no need to search for a rewrite plan at
a target $W_j$ associated with an ancestor vertex $q_j$ of $q_i$
that is more expensive than $\cost(r)$.

\item[Case (c)] Regardless of whether a rewrite is found or not at $W_i$, 
the set of {\em sibling} targets of $W_i$ that rely on the
an {\em optimistic estimate} of finding the cheapest rewrite plan for $W_i$.
We will convey to those targets that the
cheapest plan for $W_i$ cannot be cheaper
than $\min(d, \cost(r))$, where $\cost(r)$ is $\infty$ if
$r$ was not found.

\end{enumerate}

We now explain each of the three cases in more details
by referring to Figure~\ref{fig-propagate-stats}a--c
as well as the implementations provided in 
Algorithms~\ref{algn-refine-dag}--\ref{algn-propagate-maxdist}.

\paragraph*{Case (a)} 
If the $\ViewFinder{}$ found a rewrite $r$ at $t_i$ 
that was cheaper than $W_i$.$\minPlumb$ as shown
in Figure~\ref{fig-propagate-stats}a, we want to
try to see if $r$ could be used to obtain a cheaper plan for $W_n$.
This is captured by line~\ref{line-view-finder-propagate-best-plans}
of the $\RefineTarget{}$ procedure. 
We try to recursively push $r$ towards $W_n$ staring with
all the outgoing vertices of $q_i$.
For an outgoing vertex $q_m$ of $q_i$ as shown in Figure~\ref{fig-propagate-stats}a, 
we compute plan $r'$ formed by including $r$, and the $\minPlumb$ of the other incoming
vertices of $q_m$ other than $q_i$.
If $r'$ is cheaper than $W_m.\minPlumb$, 
we update $W_m.\minPlumb$ to $r'$ and recursively apply 
the same process to all the outgoing vertices of $q_m$, 
possibly reaching $q_n$.
This process is captured by the $\PropagateBestRewrites{}$ procedure
in Algorithm~\ref{algn-propagate-maxdist}, which 
is invoked whenever a cheaper rewrite is found at any target.

\paragraph*{Case (b)}
When a rewrite $r$ at target $W_i$ is found, it means that 
it is sufficient for all the ancestor vertices of $q_i$ 
to look for rewrites cheaper than $r$.
Suppose that $q_j$ is the only incoming vertex of $q_i$.
It is sufficient to look for rewrites at $W_j$ 
that are less than $\cost(r) - \cost(q_i)$.
In other words, $W_j.\minCost{}$ can be set to $\cost(r) - \cost(q_i)$
if it is not already less than that value. 

Now, consider the more general case of $q_i$
containing multiple incoming vertices in addition to $q_j$
as shown in Figure~\ref{fig-propagate-stats}b.
A rewrite at $q_j$ is only feasible if it is cheaper than
$\cost(r) - \cost(q_i)$ minus the most {\em optimistic 
estimate} on the other incoming vertices $q_k \ne q_j$ of $q_i$.
The optimistic estimate of a target $W_k$ is a lower
bound estimate on finding a rewrite at $W_k$, or at its ancestor targets. 
The procedure $\ComputeMinCostEstimate{}$ 
in Algorithm~\ref{algn-propagate-maxdist} recursively
computes the optimistic possible rewrite cost at $q_k$
as the minimum of $W_k.\seenSoFar$, or the $\cost(q_k)$ plus
the sum of the optimistic cost of the incoming vertices of $t_k$, and so on.
For example, in Figure~\ref{fig-propagate-stats}c where
$q_i$ contains two incoming vertices, $q_j$ and $q_k$,
the optimistic estimate of $W_k$ is $W_k.\seenSoFar{}$.
So, any rewrite at $W_j$ that is more expensive than 
$\cost(r) - \cost(q_i) - W_k.\seenSoFar{}$ is not feasible,
which means that $W_j.\minCost$ can be reduced to that value
if it is not already lesser than that value.
The procedure $\PropagateStats{}$ in 
Algorithm~\ref{algn-propagate-maxdist} with $\dir{}$ flag set to 
$\up{}$ restricts the $\minCost{}$ values of ancestors of $W_i$
when $r$ is found at $W_i$.

\paragraph*{Case (c)}
Regardless of whether a rewrite $r$ at $W_i$ is
found or not, the value of $W_i.\seenSoFar{}$ increased, 
which means that the optimistic estimate of finding
a rewrite at $W_i$ has also increased.
This means that we would have to update the 
$\minCost{}$ values of those
vertices in $W$ that used the optimistic
estimate of $W_i$
as part of the $\ComputeMinCostEstimate{}$ computation.
We loosely refer to these set of vertices as {\em sibling}
vertices of $q_i$, such that their $\minCost{}$ values
depend on the optimistic estimate of $W_i$.
In Figure~\ref{fig-propagate-stats}c, shows the identity
of two sibling vertices $q_c$ and $q_e$ which are 
sibling vertices of $q_i$.
The procedure $\PropagateStats{}$ in
Algorithm~\ref{algn-propagate-maxdist} with $\dir{}$ flag set to 
$\down{}$ recomputes the $\minCost{}$ values of the sibling
vertices of $q_i$.

\begin{minipage}{0.65\columnwidth}
\vspace{0.1in}
\begin{example}
The figure alongside shows a setup containing three
vertex $q_i, q_j$ and $q_k$ as well as their corresponding 
$\cost{}$, $\seenSoFar{}$, and $\minCost{}$ values.
Suppose the $\ViewFinder{}$ found a rewrite $r$ for $W_i$ at a cost of 7. 
First, $W_i.\minPlumb{}$ is set to $r$ and $W_i.\minCost{}$ to 7.
The $\PropagateBestRewrites{}$ procedure would update
$W_k.\minPlumb{}$ to $r \cup q_k$ and $W_k.\minCost{}$ to 8
as $W_k.\minCost{} = 10  > \cost(r) + \cost(q_i) = 8$. 
Finally, $W_j.\minCost{}$ is set to 6 because any rewrite to be
cheaper than $r$ at $W_j$ should be less than $\cost(r) - \cost(q_i)$.
\end{example}
\end{minipage}%
\hspace{0.02in}%
\begin{minipage}{0.3\columnwidth}%
\centering
\includegraphics[width=1in]{fig-refine-target-example}
\end{minipage}
\vspace{0.2in}


\begin{algorithm}[!h]
\caption{Propagating stats between search problems\label{algn-propagate-maxdist}}
\begin{algorithmic}[1]
\State {\sf sub} $\PropagateStats$($q_i$, $e$, $\dir$, $q_k$)
\If{$\dir$ = $\up$}
  \If{$W_i.\minCost > e$}\Comment{Improves known best plan?}
    \State $W_i.\minCost$ \qlet $e$
    \ForAll{incoming $q_j$ of $q_i$} 
      \State $e_j \qlet \ComputeMinCostEstimate(q_j)$
      \State $s$ \qlet{} $s + e_j$
    \EndFor
    \ForAll{incoming $q_j$ of $q_i$} 
      \State $\PropagateStats$($q_j$, $e$ - ($\cost(q_i)$ + $s$ - $e_j$), $\up$, \_)
    \EndFor
  \EndIf
\ElsIf{$\dir$ = $\down$}
    \ForAll{incoming $q_j$ of $q_i$} 
      \State $e_j \qlet \ComputeMinCostEstimate(q_j)$
      \State $s$ \qlet{} $s + e_j$
    \EndFor
    \ForAll{incoming $q_j \ne q_k$ of $q_i$} 
      \State $\PropagateStats$($q_j$, $W_i.\minCost$ - ($\cost(q_i)$ + $s$ - $e_j$), $\up$, \_)
    \EndFor
    \ForAll{outgoing $q_j$ of $q_i$} 
      \State $\PropagateStats$($q_j$, \_ , $\down$, $q_i$)
    \EndFor
\EndIf
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\State {\sf sub} $\ComputeMinCostEstimate$($q_i$)
\State $s' \qlet \cost(q_i)$
\ForAll{incoming $q_j$ of $q_i$} 
  \State $s'$ \qlet{} $s'$ + $\ComputeMinCostEstimate(q_j)$
\EndFor
\State \Return $\min(W_i.\seenSoFar, s')$
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\State {\sf sub} $\PropagateBestRewrites$($q_i$)\\
\Comment{Propagate a downward rewrite}
\State $r$ = $q_i \cup W_k.\minPlumb, \forall$ incoming $q_k$ of $q_i$
\If{$\cost(r)$ < $W_i.\minCost$}
   \State $W_i.\minCost$ \qlet $\cost(r)$
   \State $W_i.\minPlumb$ \qlet $r$
   \ForAll{outgoing $q_j$ of $q_i$} 
     \State $\PropagateBestRewrites$($q_j$)
   \EndFor
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{lemma}
The $\WorkflowRewrite$ will find
the optimal rewrite of $W$ and is also work efficient.
\end{lemma}

\begin{proof}
Let us first consider the simple case of a workflow with
a single target $W_n$.
Assume that the $\WorkflowRewrite$ algorithm did not return the optimal
rewrite $r^*$ of $W$.
In other words, $\cost(r^*) < W_n.\minCost$ by the time the 
while loop (lines~\ref{line-rewrite-wf-start-while-loop}--%
\ref{line-rewrite-wf-end-while-loop}) of the algorithm ended.
As $r^*$ was not found by the algorithm,
we have: $\ocost(r^*) > d_i = W_n.\seenSoFar \geq  W_n.\minCost > \cost(r^*)$, 
which is a contradiction as $\ocost(r^*) > \cost(r^*)$ violates
the property of the $\ocost{}$ function.

We can extend the above result to a workflow containing multiple targets.
Let us suppose that the optimal rewrite $r^*$ is made up of
rewrites found at multiple targets, one such being $r$ at $W_k$.
The last invocation of $\RefineTarget(W_n, d_i)$ before
the while loop terminated would have resulted
in a subsequent invocation of $\RefineTarget{}$ on $W_k$, given by
$\RefineTarget(W_k, d' = d_i - \cost(q_{k+1} \cdots q_n))$.
This can be verified by following the recursion invocation
in lines~\ref{line-refine-target-vertex}--\ref{line-refine-target-vertex-end}
of procedure $\RefineTarget{}$.
Note that $\{q_{k+1} \cdots q_n\}$ corresponds to the part of the workflow 
that transforms the output of $W_k$ into the output of $W_n$.
Note that the case of the search problem 
at $W_k$ terminating well before $r$ could be found at $W_k$
is not feasible, as it implies that $W_k.\minCost < \cost(r)$.
This means that there is a cheaper rewrite than $r^*$ that
obviated the need for $W_i$ to search beyond $W_k.\minCost$.
If we did not find $r$ at $W_k$, 
we have that $d' < \ocost(p)$, or $d_i < \ocost(p) + \cost(q_{k+1} \cdots q_n))$.
As $r$ is a part of (or equal to ) $r^*$, we have that
$\cost(r) + \cost(q_{i+1} \cdots q_n) \leq 
\cost(r^*) < W_n.\minCost < d_i = W_n.\seenSoFar{} < \ocost(r) + \cost(q_{i+1} \cdots q_n)$,
we have a contradiction in $\cost(r) < \ocost(r)$.

We now analyze the work efficiency of the algorithm.
Suppose that $r^*$ is the final optimal
rewrite of $W$ that is produced at the end of the algorithm.
Suppose that just before the start of the last invocation
of $\RefineTarget(W_n, d_i)$, $W_n.\minPlumb = r^*$.
In other words, $W_n$ already found $r^*$ before the last
invocation of the while loop.
The $\RefineTarget{}$, the algorithm invokes
with $\ViewFinder{}$ with $\min(d_i, t_n.\minCost)$, which means
that in this case the algorithm is work optimal in the sense
that the algorithm does not perform any additional work
beyond $\cost(r^*)$.
However, the algorithm ends up performing additional work
for the case that $\cost(r^*) < \cost(W_n.\minPlumb)$
at the beginning of the final $\RefineTarget{}$ invocation.
The plan corresponding to $r^*$ is found during the course of the
recursion process at some other target in $W$, such that
$d_i$ becomes less than $t_n.\minCost$ as the recursion finishes.
The extra work that the algorithm performs in this case is bounded
by $d_i - \cost(r^*)$ at one target and $n \cdot (d_i - \cost(r^*))$
for the entire workflow.
Had we sampled the range $[0, \cost(W_n)]$ into equal intervals,
the additional work performed by the algorithm is 
bounded by $n.\frac{\cost(W_n)}{l}$.
In other words, if we sample the interval more often, we can reduce the 
extra work done by the algorithm but it will also increase
the number of invocation of the $\ViewFinder{}$ algorithm. \qed
\end{proof}


==> old/Conclusion.tex <==
\section{Conclusion}

We presented a method to take advantage of
opportunistically created materialized views that can significantly 
speedup queries in a large-scale data analytics system.
With the aid of a UDF model and a lower-bound $\ocost{}$
function we developed in this paper,
the \WF{} algorithm produces the optimal rewrite
while being work-efficient.
We presented 8 evolutionary queries for realistic scenarios and demonstrated 
dramatic performance improvements 
with an average of 61\% and up to two orders of magnitude.

Because storage is not infinite, future work will address the problem of 
identifying the most beneficial views to retain. 
%which are the beneficial views to retain in the system given that 
% There is a tension between what is good for the system (throughput)
% \textit{vs} what is good for the individual user (latency).
We will look at view retention strategies from the point of
overall system benefit considering these decisions are affected by 
view maintenance costs, which is an aspect we did not address in this paper.

\begin{comment}
We presented and evaluated system that is beneficial for evolutionary 
analytical workflows and a rewrite algorithm 
that is work-efficient and finds the optimal workflow rewrite given the available views.
We prove \WF{} has a work-efficient property which allows it to examine only those views
necessary to find the optimal rewrite, and no additional views.
This property is due to the lower-bound provided by our \ocost{} function.
We also presented 8 evolutionary workflows for realistic scenarios along with a 
microbenchmark that will be made available with the paper.

There is a tension between what is good for the system (throughput)
vs. what is good for the individual user (latency).
%This tension manifests itself in a few places.
To address latency we could consider predicate pushdown into some views.
However this results in more specific views benefiting 
certain queries at the expense of more general views that may
potentially benefit many queries.
This tension also exists when considering extensions to $L_R$ with
more UDFs that benefit some users, but creates 
a larger space of rewrites for all users.
%the provider could make a UDF part of $L_R$
%which would make rewriting slower for all users 
%but may benefit a specific user.
%The person who adds a new log does not get any benefit.

Pruning has been shown to be an effective strategy to control the space of candidate views
to improve scalability of a rewrite algorithm.
%Our approach does not preclude these methods.
\WF{} does not preclude pruning, and will find the best rewrite among the candidate views available.
% Similarly \RE{} need not examine all permutations of the transformation rules but could use heuristic methods to
% avoid considering some of the permutations.
%The view selection problem addresses how to choose views that provide a good
%benefit for a representative workload which is measured by the reduction in 
%workload cost plus the cost to maintain the views.
%In this work we are concerned with the view rewriting problem which determines how
%to use any of the existing views to benefit a query.
%View maintenance considerations impact the view selection problem rather than
%the view rewriting problem that we address in this work.
%Although in our system there are no updates-in-place, views
%may need to be maintained as new log data arrives.
View maintenance affects cost-benefit decisions required by a view selection algorithm,
which we do not address in this work.

% We view our system as  a proving ground for understanding the value of data
% as well as establishing the process of extracting that value.
% Once the value and  precise  process are identified
% then efficiency becomes paramount and formal ETL methods and data warehousing solutions
% may be considered.

\end{comment}


==> old/Costing-udfs.tex <==
\section{Using the Model to Perform Rewrites}\label{sec-costing-udfs}

In this section we describe how to use the model to check for
equivalence and containment.  
Then we describe perform cost estimates using the model.


\subsection{Equivalence Testing}\label{sec-udfs-equi}

Our goal is to  leverage any previously computed results that can 
be reused toward answering a new query. 
Thus, we need to check when two results are equivalent.
Given a query $q$, and a view $v$, we can test for semantic equivalence
in terms of our model by ensuring that the properties $A$, $F$, and $G$
of $q$ and $v$ are identical. 
This makes the equivalence check  quick and easy to perform.
The purpose of the equivalence check is to determine if we have found
a valid rewrite of $q$.  


\subsection{Determining Partial or Complete Solutions}\label{sec-guess-rewrite}

When $v$ is not equivalent to $q$, we can rewrite $q$ using $v$
if $v$ \textit{contains} $q$ using the model.
Checking containment is a known hard problem even for conjunctive 
queries under bag or set semantics~\cite{Jayr2006}.
Because it is hard, we make a guess that only serves 
as a quick conservative approximation of containment.
This conservative guess allows us to focus 
computational efforts toward checking containment on the most promising previous 
results and avoid computational effort for likely hopeless cases.

We provide a function $\complete(q,v)$ that 
takes an optimistic approach,
representing a \emph{guess} that a complete rewrite of $q$ exists using only $v$.
This guess requires the following necessary conditions
as described in~\cite{Hale2001} (SPJ) and~\cite{Gold2001} (SPJG)
that a view must satisfy to participate in a complete rewrite of $q$.
% although these conditions are not sufficient to
% confirm the existence of an equivalent rewrite using $v$.

\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item $v$ contains all the attributes required by $q$; or contains all the 
    necessary attributes to produce those attributes in $q$ that are not in $v$
\item $v$ contains weaker selection predicates than $q$
\item $v$ is less aggregated than $q$
\end{enumerate}

The function $\complete(q,v)$ performs these checks and returns true if $v$
satisfies the properties i--iii with respect to $q$.
Note these conditions under-specify the requirements for
determining that a valid rewrite exists, thus a guess may
result in a false positive, but will never result in a false negative.
% The purpose of $\complete(q,v)$ is to provide a quick way to distinguish 
% between views that can possibly produce a rewrite and views than cannot.
% Since rewriting is an expensive process, this will help avoid examining views 
% that cannot produce valid rewrites. 

\subsection{Costing a UDF}
A UDF is compposed of a series of local functions, where each local 
function is map or reduce task.
Local functions are grouped into MR jobs, hence a UDF can span multiple jobs.
A job in the MR framework represents a materialization point.
To cost each MR job, we use the simple cost model in~\cite{Nyki2010}, 
which provides a cost function for a query $q$ composed of 
$n$ jobs $\{J_1, \cdots, J_n\}$. 
The cost of each job is expressed as a linear combination of 
the cost to read the data ($C_{m}$) and apply a map task,
the cost of sorting and copying ($C_{s}$),
the cost to transfer data ($C_{t}$),
the cost to aggregate data ($C_{r}$) and apply a reduce task,
and finally the cost to materialize the output of the job ($C_{w}$).

{{\small
\begin{equation} \label{eq-cost}
\cost(q,D) = \sum_{i=1}^{n} C_{m}(J_i,D_i) +  C_{s}(J_i,D_i) +  C_{t}(J_i,D_i) + C_{r}(J_i,D_i) +  C_{w}(J_i,D_i)
\end{equation} }}
where $D_1 = D$ which corresponds to the input data to which $q$ is applied.
Data $D_{i}$ forms the input of job $J_i$.


In this formulation, local functions correspond to a map task and/or the reduce task.
Even though there only 3 allowed operations (from Section~\ref{}) in a local function,
a local function can perform an arbitrary number of these operations on an 
input, complicating their costing.

For this reason, we desire a conservative way to estimate the cost of a local function.
Suppose that a local function performs a set $S$ of operations, then
we define the following weak property of our cost optimizer.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be any set of operations represented by the UDF model.
Let $\cost(S,D)$ be defined as the total cost of performing all operations 
in $S$ on a database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
%Taking the minimum cost of an operation in $S$ provides a lower bound on the
%cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
%Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
%of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must rely on the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter 
with high selectivity and a group-by operation with higher cost than 
applying the filter,
when considering the operations independently on database $D$.
Let $S'$ contain only group-by.
Suppose that applying the filter before group-by results in few or no tuples streamed to 
group-by.
Then applying group-by can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.


       
By this model, we only have to develop cost models for the three operations
that make up local functions.
This may not be suitable for many UDFs where these operations may be extremely
computationally expensive, resulting in a poor cost estimation.
For these cases, we provide a way to scale the cost of a local function
with regard to the cost estimate.
This can be done by specifying a scalar on the $C_m$ and $C_r$ components
of the cost model, which can be provided by the UDF developer or can be 
obtained by running a micro job on a subset of the input data.  
Given that UDFs can perform arbitrarily complex functions in MR, 
a typical approach is to run a small sample job (micro job) to obtain
more realistic cost estimates.


\subsection{Lower-bound on Cost}

Now that we have a quick way to determine if a view $v$ can potentially 
produce a rewrite for query $q$,  and a method for costing UDFs, 
we would like to compute a quick lower bound on the cost of any
\textit{potential} rewrite -- without having to actually find a valid rewrite, 
which is computationally hard.
To do this, we will utilize our UDF model and the non-subsumable cost property 
when computing the lower-bound.  



Suppose that $v$ is guessed to be complete with respect to $q$, and $r$ 
denotes a valid rewrite of $q$ using $v$.
Given $v$ as input, the transformations performed by $r$ must produce 
an output that is equivalent to $q$.
Notice that using the UDF model, the representation of $q$ in terms of $A,F,G$
can be compared with that of $v$ in terms of $A,F,G$.
Then the transformation produced by $r$ is given by the set difference between the attributes, filters and group-bys representation 
of $q$ and $v$ and is referred to as the {\em fix}.


\onefig{fig-example-fix}{Example of the fix between a view $v$ and a query $q$}{3in}


As an example, we show a view $v$ and a query $q$ in Figure~\ref{fig-example-fix}
annotated using the model.
Suppose that $v$ is given by attributes $\{a,b,c\}$, no applied filters, and no group-bys. 
Now, suppose that $q$ is given by $\{b,c,d\}$, filter $d < 10$, and group-by $c$, such that
to produce $d$ requires $a$ and $b$, which is present in $v$.
It is clear that $v$ is guessed to be complete with respect to $q$ because
$v$ has the required attributes to produce $q$ and it has weaker selection and 
group-by predicates than $q$.
Since it passes the $\complete(q,v)$ test, 
the fix of $v$ with respect to $q$ is given by the following operations 
as shown in Figure~\ref{fig-example-fix}:
Produce $d$ from $a$ and $b$; Apply filter $d < 10$; and apply group-by on $c$.



The notion of the fix means that to be a valid rewrite, $r$ needs to 
find a sequence of UDFs (or equivalently, local functions), 
that when applied to $v$ will produce $q$.
Finding  this sequence of local functions is the same problem as finding a valid rewite, 
which is a hard problem.
If the fix is non-empty, then at least one local function must be applied to produce a 
valid rewrite.
This local function must apply all operations in the fix.
We can obtain the cost of this local function using our UDF cost model.
By the non-subsumable cost property, the cost of this local function 
would be the cost of the cheapest operation in the fix.
This cost value corresponds to the lower-bound of any valid rewrite $r$.

We define an optimistic cost function $\ocost(q,v)$ that provides the lower-bound on any 
rewrite $r$ of query $q$ using view $v$. 
The properties of $\ocost(q,v)$ are that it is very quick to compute
(i.e., does not require acutally finding a rewrite and then obtaining its cost), 
and $$\ocost(q,v) \leq \cost(r)$$
When searching for the optimal rewrite $r*$ of $W$,  
$\ocost{}$  enables the enumeration of the candidate 
views based their potential to provide a low cost rewrite, 
as we describe in the next section.



==> old/Costing-udfs2.tex <==
\section{Using the Model to Perform Rewrites}\label{sec-costing-udfs}

Our goal is to  leverage any previously computed results that can 
be reused toward answering a new query and the model aids us in achieving
this goal in three ways.  
First, it provides a way to check for equivalence.
Second, it can aid in the costing of UDFs.
Third, it can be used to provide a lower-bound on the cost of
potential rewrite.

\subsection{Equivalence Testing}\label{sec-equivalence}

If we consider the annotated edges of a plan $W$ as views, then we can look 
for rewrites using existing views and test for semantic equivalence
in terms of our model using the properties $A$, $F$, and $G$.
If two views are not identical, our system considers transformations (compensations)
to existing views to make them equivalent.

We need to test when a view $v$ can produce a rewrite for an edge in the annotated plan $W$.
For simplicity, we refer to this edge as a query $q$.  
Query $q$ can be rewritten using view $v$
if $v$ \textit{contains} $q$.
Checking containment is a known hard problem~\cite{Jayr2006} even for conjunctive 
queries, hence we make a guess that only serves 
as a quick conservative approximation of containment.
This conservative guess allows us to focus 
computational efforts toward checking containment on the most promising previous 
results and avoid wasting computational effort.


We provide a function $\complete(q,v)$ that performs this heuristic check, 
which we describe next.
$\complete(q,v)$ takes an optimistic approach,
representing a \emph{guess} that a complete rewrite of $q$ exists using only $v$.
This guess requires the following necessary conditions
as described in~\cite{Hale2001} (SPJ) and~\cite{Gold2001} (SPJGA)
that a view must satisfy to participate in a complete rewrite of $q$, 
although these conditions are not sufficient to
confirm the existence of an equivalent rewrite using $v$.

\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item $v$ contains all the attributes required by $q$; or contains all the 
    necessary attributes to produce those attributes in $q$ that are not in $v$
\item $v$ contains weaker selection predicates than $q$
\item $v$ is less aggregated than $q$
\end{enumerate}

The function $\complete(q,v)$ performs these checks and returns true if $v$
satisfies the properties i--iii with respect to $q$.
Note these conditions under-specify the requirements for
determining that a valid rewrite exists, thus a guess may
result in a false positive, but will never result in a false negative.
The purpose of $\complete(q,v)$ is to provide a quick way to distinguish 
between views that can possibly produce a rewrite and views than cannot.
Since rewriting is an expensive process, this will help avoid examining views 
that cannot produce valid rewrites. 

\subsection{Costing a UDF}


We extend the simple cost model in~\cite{Nyki2010}, 
which provides a cost function for MR jobs that we use to cost UDFs.
Their cost function only considers data ``data'' costs, but we extend it to 
account for the computation cost of local functions.  
Since  a UDF can be composed of $n$ jobs, 
the cost of each job is expressed as a linear combination of 
the cost to read the data and apply a map task ($C_{m}$),
the cost of sorting and copying ($C_{s}$),
the cost to transfer data ($C_{t}$),
the cost to aggregate data and apply a reduce task ($C_{r}$),
and finally the cost to materialize the output of the job ($C_{w}$).
A job in the MR framework represents a materialization point.
In this cost model, we can account for the cost of the map and reduce
processing by making use of our UDF model as we describe below.


In this formulation, a local function corresponds to a map or reduce task.
Note that local functions can only perform the three operations 
(in the previous section), although they can perform an arbitrary number of these 
operations on their input.
This complicates the costing of local functions since it is not clear how the different operations performed within a single local function actually interact with each other.
Without a white-box approach or a sampling-based approach (micro job) it is 
difficult to estimate the cost of local functions constituting a UDF.
For this reason we desire a conservative way to estimate the cost of a local function,
which we do by appealing to the following property of any cost model for a function that 
performs a set $S$ of operations.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $\cost(S,D)$ be defined as the total cost of performing all operations 
in $S$ on a database instance $D$.
% Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
% cannot be applied on $D$.
The cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S) $$ 
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
%Taking the minimum cost of an operation in $S$ provides a lower bound on the
%cost of $S$ given $D$.
%Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
%Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
%of the least expensive operation in $S$.
The gray-box model of the UDFs only captures enough information about the local functions
to be able to use it to provide a cost corresponding to the least expensive operation performed on the input.
% A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
% i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason cannot use the most expensive operation 
in $S$ (i.e., $\max(\cost(x,D), \forall x \in S)$), 
since it requires $\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter 
with high selectivity and a group-by operation with higher cost than 
applying the filter,
when considering the operations independently on database $D$.
Let $S'$ contain only group-by.
Suppose that applying the filter before group-by results in few or no tuples streamed to 
group-by.
Then applying group-by can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.  $\qquad \blacksquare$ 
       
By making use of this property, we can cost the map and reduce functions as the
 cost to read the input data and apply the cheapest operation on the input.
This greatly simplifies the design of our cost model as we now only have to 
consider 3 operation types.
A consequence of modelling map and reduce costs by operation types as opposed to 
the actual computation is that it may underestimate the cost of very expensive 
local functions. 
To remedy this, the UDF developer may specify a scalar value
to magnify the cost of computationally intensive local functions e.g., NLP tagger.
As a standard way for initially calibrating the cost model to the three operation types,
we run a small sample job (micro-job) to obtain realistic cost estimates.
       


\subsection{Lower-bound on Cost}

Now that we have a quick way to determine if a view $v$ can potentially 
produce a rewrite for query $q$,  and a method for costing UDFs, 
we would like to compute a quick lower bound on the cost of any
\textit{potential} rewrite -- without having to actually find a valid rewrite, 
which is computationally hard.
To do this, we will utilize our UDF model and the non-subsumable cost property 
when computing the lower-bound.  



Suppose that $v$ is guessed to be complete with respect to $q$, and $r$ 
denotes a valid rewrite of $q$ using $v$.
Given $v$ as input, the transformations performed by $r$ must produce 
an output that is equivalent to $q$.
Notice that using the UDF model, the representation of $q$ in terms of $A,F,G$
can be compared with that of $v$ in terms of $A,F,G$.
Then the transformation produced by $r$ is given by the set difference between the attributes, filters and group-bys representation 
of $q$ and $v$ and is referred to as the {\em fix}.


\onefig{fig-example-fix}{Example of the fix between a view $v$ and a query $q$}{3in}


As an example, we show a view $v$ and a query $q$ in Figure~\ref{fig-example-fix}
annotated using the model.
Suppose that $v$ is given by attributes $\{a,b,c\}$, no applied filters, and no group-bys. 
Now, suppose that $q$ is given by $\{b,c,d\}$, filter $d < 10$, and group-by $c$, such that
to produce $d$ requires $a$ and $b$, which is present in $v$.
It is clear that $v$ is guessed to be complete with respect to $q$ because
$v$ has the required attributes to produce $q$ and it has weaker selection and 
group-by predicates than $q$.
Since it passes the $\complete(q,v)$ test, 
the fix of $v$ with respect to $q$ is given by the following operations 
as shown in Figure~\ref{fig-example-fix}:
Produce $d$ from $a$ and $b$; Apply filter $d < 10$; and apply group-by on $c$.

The notion of the fix means that to be a valid rewrite, $r$ needs to 
find a sequence of UDFs (or equivalently, local functions), 
that when applied to $v$ will produce $q$.
Finding  this sequence of local functions is the same problem as finding a valid rewite, 
which is a hard problem.
If the fix is non-empty, then at least one local function must be applied to produce a 
valid rewrite.
This local function must apply all operations in the fix.
We can obtain the cost of this local function using our UDF cost model.
By the non-subsumable cost property, the cost of this local function 
would be the cost of the cheapest operation in the fix.
This cost value corresponds to the lower-bound of any valid rewrite $r$.

We define an optimistic cost function $\ocost(q,v)$ that provides the lower-bound on any 
rewrite $r$ of query $q$ using view $v$. 
The properties of $\ocost(q,v)$ are that it is very quick to compute
(i.e., does not require acutally finding a rewrite and then obtaining its cost), 
and $$\ocost(q,v) \leq \cost(r)$$
When searching for the optimal rewrite $r*$ of $W$,  
$\ocost{}$  enables the enumeration of the candidate 
views based their potential to provide a low cost rewrite, 
as we describe in the next section.



==> old/Discussion.tex <==
\section{Discussion and Future Work}




Some notes 
\begin{itemize}
  \item Storage space is not infinite.  Clearly there is a tradeoff between
  retaining all previous answers and retaining only those that are most beneficial.
  However, commodity disk storage is very inexpensive, about \$0.04/GB.
  As we have shown it is very beneficial to retain views materialized 
  during query processing.  
  \item While in our current scenario log files are append only and do not 
  allow update-in-place, these extracted views do incur a maintenance overhead
  as log data grows.
  
  \item Addressing the problem of maintenance cost vs. benefit is an area of future
  work, which can leverage much prior work in this area.  
  Furthermore here we do not incur view creation cost as our views are created
  as part of query execution.  
  Thus the decision for view selection in our scenario becomes a decision only 
  to keep the view rather than to create the view.
  
  \item There is a small overhead to storing each output as a materialized view.
  As the data is typically written to disk somewhere in the DFS, usually temp 
  space by default, and the extra overhead lies primarily in the cost to 
  create the metadata for the views.
  The extra cost to replicate the temp outputs is contained in the DFS write
  cost as the inputs to one job are DFS files, thus the previous outputs were
  written with the standard DFS replication.  
  Even if they were only written to tmp directories using no additional replication
  the additional cost to write DFS replicas is nearly equivalent to the cost to
  writing a single replica as by nature replicas can be created in parallel
  at distinct nodes.

 \item Another consideration we believe is effective in our scenario
 is to not maximize benefit for a single current query, 
 but rather try to maximize benefit for many future queries 
 due to the high cost of log extraction and evolutionary nature of the workflows. 
 One approach toward this goal is to not apply predicate pushdown into 
 views that are guessed to be complete, or the composite views of 
 merged views.
 Adding specific predicates to a view can render it very useful for the 
 current query but possibly useless for later follow-on queries or
 queries posed later by other users in the system.
 Because our workflow rewriting algorithm provides an optimal rewrite of the
 workflow using \ocost{}, the choice of predicate pushdown lies with
 \ocost{}.
 In our scenario it appears intuitive to extract and retain more general views
 before making them too specific. 
 Loss of generality makes the views less useful for rewriting, and since
 or method serves the functions of both query rewriting and view selection 
 we prefer to avoid predicate pushdown that is too aggressive.
 Furthermore from a platform provider perspective it makes sense to 
 do as much useful work for the entire system as possible rather than
 maximizing benefit for a single query alone.
 While this eschews common approaches to answering queries using views,
 Even though a user may experience a slightly higher query execution time,
 that user may likely be posing a very similar query in the near future 
 and at that time he will observe the benefits himself, 
 as well as other users may get the benefits of a more general view.
 
 \item Pruning.
  Pruning is orthogonal to our approach.
  We can also benefit from pruning methods.
  Our method will still find the cheapest rewrite in an incremental
  way (optimal work) given the space of views to be considered.
  Our algorithm produces the optimal rewrite given the views under consideration.
  i.e. the cheapest rewrite in the pruned space. 
 
 The \WF{} algorithm finds the optimal rewrite using views given those
 views available.  Pruning could also be applied, and we do some pruning in
 that we eliminate from consideration those views which can never be 
 part of a valid rewrite for a given query e.g. they have additional filters
 that cannot be removed.
 Further dominance-based pruning could be applied as much as desired given
 the tolerance for potentially sub-optimal rewrite.
 In practice, dominance-based pruning is often used to restricte the 
 exponential growth of the space of candidate views to be considered for rewrite 
 (and for view selection).  
 We note that \WF{} and \ocost{} do not exclude pruning techniques applied
 to the views to be considered by the algorithm.
 Views may be pruned before applying \WF{} and \ocost{},
 which will incrementally search the space of rewrite solutions given
 any set of views, and output the optimal rewrite solution.
 However, any pruning by the \WF{} or \ocost{} may result in a sub-optimal
 rewrite solution.
 
   
 
 
 
 

\end{itemize}


==> old/Experimental_evaluation-rewrite1.tex <==
\section{Experimental Evaluation}\label{sec-experimental-evaluation}

In the following experiments we show the performance
of our system using real social media data and evolutionary queries.
Due to the log nature of the data, the need for data exploration
and the types of analytical functions which can include complex
UDFs, an analyst has significant freedom in revising versions 
of the same query.
First, we formally capture the revision \emph{expressions} in our evaluation using 
a microbenchmark that we present here.
Second, we present a microbenchmark that is intended to highlight common types
of revisions that a real analyst would perform.
Third, we evaluate three scenarios:
a) {\em query evolution} where 
a user may get benefit from previous version of his query,
b) {\em user evolution} where
a new user in the system may get benefit from other users' query.
c) {\em system evolution} where a new analyst may get increasing
benefit as the system matures.
We show results for these cases using query execution time, 
data moved (bytes),
and percent improvement in execution time of the rewritten query compared to
the original query. 
Fourth, we show that good rewrites are found even 
when identical materialized views are excluded from
consideration thus showing the advantages of our method compared to
those which only use cached results.
Fifth, we compare our rewrite with those of a state of the art
commercial database system.
Lastly, since storage is not infinite we evaluate the robustness of our rewrite 
algorithm given a view storage reclamation policy.

\subsection{Setup}
% UDF is written in Hive, perl, python, MR but the transformation applied
% by the UDF is expressed in terms of a grammar that describes how an input
% attributes, filter and groupby properties are modified by the UDF.

Our evaluation setup consists of 20 machines running
Hadoop, Hive/Pig, and Oozie.
Our UDFs are implemented in several languages 
such as SQL, Java, Perl and Python.
Some UDFs implemented in our system beyond
basic SQL operators are
text sentiment, sentence tokenizer, lat/lng extractor, 
word count, restaurant menu similarity, and geographical 
tiling, among others.
The queries are checked against the grammar of the UDFs.
Next, we check data dependencies after which
we parallelize the given query based on its 
dependency graph structure.
We then convert this to a Oozie workflow 
which serves as an execution coordinator.
The Oozie workflow nodes are executed on Hive~\cite{Thus2009}
or Hive-CLI for those UDFs that are not expressible by 
HiveQL (e.g., Perl UDFs).

We evaluate our system using three logs totaling over 1TB.
A Twitter log containing 800GB of tweets, 
a Foursquare log containing 250GB of user check-ins, 
and Landmark log containing 7GB of 5 million landmarks including their locations.
The identity of a social network user (\texttt{user\_id}) is common across
the Twitter and Foursquare logs, while
the identity of a landmark (\texttt{location\_id}) 
is common across the Foursquare and Landmarks logs.

Hive currently lacks a mature query optimizer
and a {\em what-if} optimizer functionality to obtain cost
estimates for hypothetical configurations.
Additionally, it cannot consider 
UDFs and their costs properly.
For these reasons, we employ the cost model 
developed for M/R frameworks in~\cite{Nyki2010}
that considers basic data statistics, number of map/reduce 
tasks, and number of jobs.

\subsection{Evolutionary Query Scenarios}

The evaluation consists of 8 analysts that write queries 
related to marketing scenarios involving restaurants,
which are described in Table~\ref{tab-experiment-scenarios}.
Each analyst's exploration
consists of 4 evolutionary versions.
Each version captures the analyst's iterative attempt in bringing the
query closer to his intended goal.
In the following set of experiments, $A_iv_j$
corresponds to the Analyst $i$ running version $j$ 
of his evolutionary query.
We give a high-level description of these queries in 
Table~\ref{tab-experiment-scenarios} left column, and 
describe one query ($A_2v_2$) in Example~\ref{ex-query-a2v2}.
% we will provide all 
%queries as a first step towards a benchmark for evolutionary queries.
We use these 32 queries in our evaluation, and will provide
them in a subsequent publication.

\begin{example}\label{ex-query-a2v2}
$A_2v_2$:
Find users with affluent friends that tweet 
positively about food, and visit a lot of pubs.

$G_1$: EXTRACT from Foursquare log.
EXTRACT restaurant name from text.
FILTER by check-ins to wine places.
GROUPBY user, compute count.
Find MAX user check-in.
Compute check-in score for each user.

$G_2$: EXTRACT user from Twitter log.
Compute FOOD-SENTIMENT score for each user.

$G_3$: CLASSIFY user's tweets from Twitter log as affluent or not.
GROUPBY affluent users, compute affluent tweet count.
Find MAX count among all users.
COMPUTE an affluent score for each user.

$G_4$: Create social network from Twitter log
using tweet source and dest.
GROUPBY user pair in social network, count tweets. 
Find MAX tweets between a user pair.
Assign friendship strength score to each user pair.

JOIN subgoals $G_1$, $G_2$, and $G_3$ based on user\_id .
JOIN with $G_4$ based on friend\_id .
Threshold based on checkin score, food-sentiment score, 
friendship score, and affluent score.
\end{example}

NO-BFR represents the original execution time
without rewrite, while BFR represents the execution time
after rewrite using $\WF$ and
DPR represents the bottom-up approach that does not make use of \ocost{}.
DPR finds the best rewrite
for each target and then identifies a subset of these to obtain $r^*$ 
using a dynamic programming algorithm.
Furthermore we limit both algorithms from considering more than
$n$-way joins, where we limit $n=4$ simply for practical reasons.

\subsection{Results}

\onefig{fig-slug-illustration}
{Dimensions of change between query versions}{2.2in}

\subsubsection{Microbenchmark}

Given the evolutionary nature of our scenarios, we 
capture the changes across the versions by defining and presenting
a {\em micro-benchmark} for the set of evolutionary 
queries evaluated here.

 (P) Parameters: While keeping the structure of the query unchanged, 
the parameters of the operations are modified to allow for 
more or less tuples in the results (Figure~\ref{fig-slug-illustration}P).
For example, the analyst may alter a select predicate or a top-k value to allow more
or less data in the output.
Here we evaluate the effect of changing the parameters of the query while
keeping the same structure.

 (L) Logs: An analyst may augment a query with 
a new log to obtain richer results (Figure~\ref{fig-slug-illustration}L).
Here we evaluate the effect of adding a new log to a query.

 (U) UDFs: An analyst may replace a set of operations in the 
query with a specialized UDF (Figure~\ref{fig-slug-illustration}U).
The analyst can also add a new UDF to the system which contributes
to the divergence of $L_W$ from $L_R$.
Here we evaluate the effect of replacing possibly multiple
operations with a UDF.

 (G) Sub-Goal Queries: An analyst writes several sub-queries
that each achieves a single goal and then joins these to obtain 
the final output (Figure~\ref{fig-slug-illustration}G).
This query structure has the benefit that parameters of each sub-goal
can be evolved as in Figure~\ref{fig-slug-illustration}P.
Here we evaluate the effect of adding or removing subgoals from the query.

These four dimensions \{P,L,U,G\} inform the 
changes between one version and the next. 

\twofigrow{fig-we-novf-vs-vf-running-time}
{fig-we-novf-vs-vf-time-improvement}
{Query evolution comparisons for (a) query execution time (log-scale)
and (b) execution time improvement}{3in}

\begin{comment}
% SJ: Removed it for SIGMOD submission

\onefig{fig-mb-execution-time-comparison}
{Microbenchmark results showing execution time}{2.35in}


Our microbenchmark starts with a set of simple initial workflows
$P_0, L_0, U_0, G_0$, each representing one of the PLUG dimensions.
Within each dimension, 2-3 evolved 
versions of the initial workflow are evaluated.
Each evolution captures one case of a rewrite-friendly 
change and another case that is not.
The rewrites are restricted to using only the original workflow
(e.g., $P_0$).
The different dimensions and their 
evolutions are meant to show the variations across 
the dimensions as well as variations within a dimension.
Figure~\ref{fig-mb-execution-time-comparison} 
presents the results of the microbenchmark 
experiments, where the y-axis shows the workflow
execution time in seconds and x-axis shows the workflows and their
evolutions.

$P_0$ performs extract, a simple groupby and then a select operation.
$P_1$ modifies $P_0$ by altering the select predicate,
while $P_2$ alters the groupby.
Both changes result in more tuples being output compared to $P_0$.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
$P_1$ is more conducive to rewrite because the rewrite 
is able to use the output from the groupby in $P_0$, while
$P_2$ had to recompute the groupby thus could not benefit
much from $P_0$.
$P$ represents a dimension where
the structure of the workflow remains the same 
while the parameters are varied.
Depending on the nature of the change to $P$,
one can expect opportunities for rewrite using MVs from $P_0$.

$G_0$ contains a single sub-goal.
$G_1$ adds a sub-goal with some commonality with the sub-goal in $G_0$,
while $G_2$ adds a sub-goal that has nothing
in common with $G_0$.
Both changes resulted in a richer answer compared to $G_0$.
$G$ represents a dimension where there is an opportunity
of reusing the entire original subgoal.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
depending on the similarities between the
newly added subgoal $G_1$ and the original $G_0$,
there can be ample opportunities for rewrite 
of the new subgoal using MVs from $G_0$.

$U_0$ contains extract, select, group and project.
$U_1$ replaces the select in $U_0$ with a UDF that is in $L_R$, 
$U_2$ replaces the select in $U_0$ with a UDF that is not in $L_R$, 
$U_3$ replaces the select in $U_0$ with the same UDF that is not in $L_R$.
$U_1$ and $U_3$ place the UDF before
the groupby in $U_0$ while $U_2$ places the UDF after the groupby.
Since the UDF in $U_1$ is in $L_R$, there are opportunities
for rewrite of both the UDF and the groupby from $U_0$.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
 when the UDF is not in $L_R$,
the rewrite becomes sensitive to its position in the workflow.
Thus, due to $U_2$'s position it could reuse 
the groupby in $U_0$, while $U_3$ could not.
$U$ represents a dimension
where UDFs offer opportunities for rewrite if they are in $L_R$,
otherwise the rewrite is sensitive to their position in the workflow.

$L_0$ contains extract, select, project, groupby on a 
single log $l_a$.
$L_1$ replaces $l_a$ with a $2\times$ larger log $l_b$, while
$L_2$ uses both the logs by applying
extract, select, project, groupby on $l_b$
and then joins the result with an extract of $l_a$.
Both changes resulted in a richer answer compared to $L_0$.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
$L$ represents a dimension where there 
may not be opportunities for rewrite 
using the original workflow, unless one log subsumes the other.

Even though the microbenchmark examines the effect
of changing one dimension at a time, in a normal 
use-case the analyst may vary many of the dimensions at 
the same time.  
\end{comment}

In a typical use-case the analyst may vary 
multiple dimensions at the same time.  
Table~\ref{tab-experiment-scenarios} right column 
captures the PLUG changes
made from the original query $Q$ to each of the subsequent
revisions.
For instance, using the PLUG microbenchmark Analyst2's query 
evolution is be described as:
\begin{center}
$Q \rightarrow \{L,G,P\} \rightarrow \{G,P\} \rightarrow \{U,G,P\}$
\end{center}

The analyst begins with initial query $Q$ (i.e., $A_2v_1$)
then adds a log $L$, modifies sub-goals $G$ and structure parameters $P$ 
to obtain version 2 (i.e., $A_2v_2$), and so on.
The ordering $\{L,G,P\}$ indicates the $L$ dimension 
likely affects the rewrites more than $\{G,P\}$.

\subsubsection{Query Evolution}

\threefig{fig-ue-novf-vs-vf-running-time}
{fig-ue-novf-vs-vf-data-moved}
{fig-ue-novf-vs-vf-time-improvement}
{User Evolution Comparisons for (a) query execution time (log-scale)(b) data moved
(c) execution time improvement}{2.15in}

% \threefig{fig-we-novf-vs-vf-running-time}
% {fig-we-novf-vs-vf-data-moved}
% {fig-we-novf-vs-vf-time-improvement}
% {Query Evolution Comparisons showing (a) execution time (b) data moved
% (c) percentage improvement}{2.2in}
 
Here we present results for the query evolution scenario, 
where an analyst $A_i$ executes
the first version of his query (e.g., $A_iv_1$) and
follows by posing the subsequent versions (e.g., $A_iv_2$).
Each subsequent version is rewritten given the existence of all 
materialized views created from executing the previous versions.

Figure~\ref{fig-we-novf-vs-vf-running-time}(a) shows the performance of
the rewritten query versus the original query and 
Figure~\ref{fig-we-novf-vs-vf-running-time}(b) shows the percentage
improvement in query execution time.
These figures show that the execution time is always lower for the rewritten
query.
Figure~\ref{fig-we-novf-vs-vf-running-time}(b) shows
an execution time improvement of at least 10\%, and up to 90\%.
The amount of data moved (i.e., read/write/shuffle) closely followed the trend
in Figure~\ref{fig-we-novf-vs-vf-running-time}(a).
The data moved results are not reported here
but we present the result for the user evolution case in Section~\ref{sec-experiments-ue}.
The significant savings in execution time can be attributed to moving much less data,
not having to re-ETL the raw logs whenever possible, 
and the ability of BFR{} to reuse and repurpose prior computation from all previous query versions.
These results show the benefit of rewriting queries as well as 
our algorithm's ability  to take advantage of MVs from previous versions 
in the query evolution scenario.

While both BFR and DPR produce the optimal rewrite $r^*$,
our BFR algorithm searches a considerably
smaller amount of space and attempts far fewer rewrites 
compared to the DPR algorithm.
We do not present these results here, but show this comparison
next for the user evolution experiments where the search space is 
larger due to the presence of many more materialized views.


\begin{comment}
Next we compare the space searched by both algorithms.
While both BFR and DPR produce the optimal workflow rewrite $r^*$,
it can be seen from Figure~\ref{fig-bfs-vs-dp-merge-attempts}
 that BFR algorithm searches a considerably
smaller amount of space and attempts far fewer rewrites 
compared to the DPR algorithm.
Recall the search for $r^*$ requires examining an exponential space of candidate views
in the worse case.
This search includes all of the existing candidate views and all of the 
views created as part of the rewrite search process (i.e., merged views).
The number of rewrite attempts corresponds to the views guessed to be
complete that we encounter during our search process, which are given to $\RE{}$
to attempt to find a rewrite.
As noted previously this process is computationally expensive.
Notice in most cases our algorithm attempts far fewer rewrites, thus
avoiding that expense.
This is due to our algorithms use of $\ocost{}$ that examines the promising
candidate views earlier.
Our results show for most cases it is possible to 
find $r^*$ by considering far fewer candidates
views in Figure~\ref{fig-bfs-vs-dp-merge-attempts}(a) and
orders of magnitude fewer
rewrites in Figure~\ref{fig-bfs-vs-dp-merge-attempts}(b).

Notice in the worst case our algorithm degenerates into 
the DPR approach when a rewrite does not exist or $r^*$ 
is really expensive, requiring both algorithms to 
examine a large part of the space.
This can be seen in $A_4v_2$, $A_5v_2$, and $A_7v_2$.
It is worthwhile to note that these three cases involved UDFs
that were not part of $L_R$.
From microbenchmark $U_2$ and $U_3$ we saw that UDF rewrites are sensitive
to the position of the UDF in the workflow, especially
those that are not in $L_R$.
Interestingly this only happens in version 2 where the materialized
views that exist are only those from version 1.
But it can be seen that our algorithm does much better for all subsequent iterations
(versions 3 and 4) where there are more materialized views in the system.
Later we will show this effect in the user evolution scenario ---
where any materialized view in the system created by any user may be used for
rewrite --- our algorithm beats DPR by several orders of magnitude
for all cases.
This highlights the utility of \ocost{}.
Even for these degenerative cases we can never search more space than DPR.

\twofig{fig-bfs-vs-dp-merge-attempts}
{fig-bfs-vs-dp-refine-attempts}
{Number of (a) candidate views considered and (b) rewrite
attempts during workflow evolution}
{1.75in}

% 
%\onefig{fig-bfs-vs-dp-merge-attempts}{Number of candidate views 
%examined for each algorithm during workflow evolution}{2.75in}
%\onefig{fig-bfs-vs-dp-refine-attempts}{Number of rewrite
%attempts performed by
%each algorithm during workflow evolution}{2.75in}
%
%Figure~\ref{fig-bfs-vs-dp-merge-attempts}(b) reports the number
%of rewrites attempted by each algorithm.
%Recall from Section~\ref{sec-rewrite-enumeration} that
%finding an equivalent rewrite involves enumerating
%all possible rewrites of a view using $L_R$.  
%Given the known computational complexity of attempting a rewrite,
%the work efficiency of an algorithm can also be evaluated
%by the number of rewrites it attempts.  
%From the figure it can be seen that our algorithm always attempts
%far fewer rewrites than the bottom-up approach, and 
%in many instances at least an order of magnitude fewer.
\end{comment}

\begin{comment}
Note that $r^*$ can be composed of rewrites found
at multiple targets.  
Some of the additional rewrites that our algorithm attempted 
include those where it failed to find an equivalent rewrite and 
those which produced a equivalent rewrite but were not part of $r^*$.
Rewrite attempts in the second case are those that
had a lower \ocost{} than $\ocost(r^*)$
but their \cost{} was actually more than $\cost(r^*)$
thus exposing the limitation of our weak lower bound
of the \ocost{} function.
Yet clearly this result shows even our basic \ocost{} 
function can provide significant savings.
cases.
1. fails to find a rewrite
2. finds a rewrite but is not part of r* as its actual cost is higher
3. it is part of r*
\end{comment}

\subsubsection{User Evolution}\label{sec-experiments-ue}
\threefig{fig-ue-bfs-vs-dp-candidates-explored}
{fig-ue-bfs-vs-dp-refine-attempts}
{fig-ue-bfs-vs-dp-time-comparison}
{User Evolution Comparisons for 
(a) Candidate views considered, (b) Refine attempts, and (c) Runtime (log-scale)}
{2.15in}

Next we evaluate the case of a new analyst entering the system
and executing the first version of his query given that
all the other analysts having executed their queries.
The system rewrites $A_iv_1$ using the existing
materialized views from all other analyst queries.
Figure~\ref{fig-ue-novf-vs-vf-running-time} shows the performance of
the rewritten versus the original query.
Figure~\ref{fig-ue-novf-vs-vf-running-time}(a) shows the query execution
time while Figure~\ref{fig-ue-novf-vs-vf-running-time}(b) shows the 
data moved (read/write/shuffle).
It can be seen from these figures that the execution time is always lower for the rewritten
query, with a similar trend in the amount of data moved.
The percentage improvement in execution time is given in 
Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) where it can be
seen that our system results in an improvement of about 50\%, 
and up to 90\%.
These results show the benefit of rewriting queries using
MVs from previous versions in the user evolution scenario.

% Given enough materialized views in the system, 
% intuitively a new analyst can expect some benefit from them
% if there is overlap with at least one other analyst.
% Overlap in this domain is quite common given there is
% a small set of operations that most queries build upon,
% such as identifying people's friends (social network), 
% their likes (sentiment), 
% and locations they visit (check-in).

Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}
compares the performance of the BFR and DPR algorithms 
by measuring how much of
the rewrite search space each algorithm explores.
The candidate views considered corresponds to 
all the existing candidate views and all the 
views created as part of the rewrite search process (i.e., merged views).
The number of rewrite attempts corresponds to the views guessed to be
complete that we encounter during our search process, 
each of which are given to $\RE{}$ to attempt to find a rewrite.
As noted previously this process is computationally expensive.
These result show for most cases it is possible to 
find $r^*$ by considering far fewer candidates
views as in Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(a),
orders of magnitude fewer
rewrites in Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(b),
resulting in significant savings in runtime as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(c)
due to our algorithm's use of $\ocost{}$ that enables
considering the promising candidate views earlier.
% This shows our algorithm results in a significant reduction
% in the rewrite search space.

\subsubsection{System Improvement Over Time}\label{sec-experiments-system-improves}

In our scenario materialized views are artifacts left 
behind from previously executed queries.
To show that system performance improves over time we present two 
evaluations.
First we execute $A_5v_3$ with no analyst's queries 
in the system, then we repeatedly add another analyst and re-execute 
$A_5v_3$ to show improvements as more analysts are present in the system.
We chose $A_5v_3$ as it uses all three logs as it has
more opportunities to find commonality with other queries.
Table~\ref{fig-se-novf-vs-vf-time-improvement} reports the 
execution time improvement of $A_5v_3$ using our 
 rewrite algorithm as the number of other analysts increase.
We use the query execution time when no
other analysts are present in the system as the baseline, 
and report percentage improvement relative to this baseline.
Table~\ref{fig-se-novf-vs-vf-time-improvement} 
clearly shows an increasing benefit for an
incoming analyst as more users are present in the system.
The benefit is obviously dependent on the amount of similarity to other
analysts' queries, and in this example there is quite a bit of benefit
even when one other analyst is present.

% \onefig{fig-se-novf-vs-vf-time-improvement}{Improvement in execution time of $A_5v_3$ as more
% analysts are present in the system}{2.5in}

\begin{table}
\vspace{-0.10in}
\caption{\label{fig-se-novf-vs-vf-time-improvement}
Improvement in execution time of $A_5v_3$ as more
analysts become present in the system}
\centering
\begin{tabular}{| p{2.5cm} | p{1cm}| p{1cm} | p{1cm}| p{1cm} | p{1cm}|}
\hline
Analyst in System & 1 & 2--3 & 4 & 5--7 \\ \hline
Improvement    & 0\% & 73\% & 75\% & 88\% \\ \hline
\end{tabular}
\vspace{-0.13in}
\end{table}

\begin{comment}
% SJ: Earlier version of the experiments that talked about rewrites etc. We will now
%     deal with RUNNING TIME OF THE algorithms
Secondly after the system has been in use for a few 
months, we show that the existing materialized views in 
the system can aid in rewriting workflows.
We evaluate the rewrites produced by our algorithm with 
increasing numbers of materialized views present in the system.
We retained about 4,800 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 scenarios and our microbenchmark.
This setup is intended to represent a mature system with many views 
left behind from previous execution runs.
Then we try to rewrite one analyst's workflow ($A_3v_1$) given
a random sampling of the existing views.
From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms (``BFR'' and ``DPR'') 
pruned from consideration views that cannot be used in a rewrite 
for a given target for the following reasons. 
A materialized view was pruned if it belonged to a different log, 
if it had a predicate condition that could not be removed,
or if it was a view previously created for any of Analyst3's workflows.
After pruning, the number of materialized views available for each target was
slightly more than 250.  
This experiment was performed ten times for each 
algorithm, and a scatter plot of the results are given in
Figure~\ref{fig-mv-vary-num-candidates}.


\twofig{fig-mv-vary-num-candidates}{fig-mv-vary-rewrites}
{Number of candidates considered (a) and the number of rewrites produced (b) (log-scale)}
{1.75in}

Figure~\ref{fig-mv-vary-num-candidates}(a) shows for each 
experiment performed, BFR creates several times fewer
candidate views.
Because BFR uses \ocost{}, 
it can avoid considering candidate views whose \ocost{}
is more expensive than $\cost(r^*)$.
Clearly the space of newly merged views is exponential in the worst case
as noted in~\cite{Agra2000}.  
These results show that BFR cannot escape this exponential space,
but typically results in creating and searching a smaller space than DPR approach.
Due to the known computational complexity of the problem, any solution that
avoids searching the entire space must resort to pruning which can result in sub-optimal rewrite.
Additional pruning could be applied to reduce the search space, 
but our algorithm will still find the best rewrite in the space it considers.

However, the larger benefit of BFR can be seen in 
Figure~\ref{fig-mv-vary-num-candidates}(b) 
which shows BFR is able to find $r^*$ by obtaining
far fewer rewrites than DPR in each case, and orders of magnitude fewer
for most cases.
The saving from (a) is primarily driven by how \emph{far} $r^*$ is into the space
in relation to the entire space, while the savings from (b)
is driven by \ocost{}'s ability to examine
more promising candidate views before less promising views.

%Furthermore, the more the views that exist, the more likely at least
%some of these will be useful for rewrites. 
%the faster \VF{} can find them, apply them, and terminate early
%by obtaining $r^*$ due to its incremental search behavior.
%we can examine candidates by the potential order of usefulness 
%(i.e. increasing optcost)
\end{comment}

\subsubsection{Runtime Comparison with DPR}

% SJ: Earlier version of the experiments that talked about rewrites etc. We will now
%     deal with RUNNING TIME OF THE algorithms
After the system has been in use for a few 
months, there is a large pool of existing materialized
views in the system that can aid in rewriting queries.
We evaluate the runtime performance of our algorithm (i.e., BFR) and DPR with 
increasing number of materialized views present in the system.
We retained about 9,600 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 scenarios and our microbenchmark.
This setup is intended to represent a mature system with many views 
left behind from previous execution runs.
Then we try to rewrite one analyst's query ($A_3v_1$) given
a random sampling of the existing views.
% From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms (``BFR'' and ``DPR'') 
pruned from consideration views that cannot be used in a rewrite 
for a given target for the following reasons. 
A materialized view was pruned if it belonged to a different log, 
if it had a predicate condition that could not be removed,
or if it was a view that is identical to target in Analyst3's plan.
After pruning, the number of materialized views available for each target was
slightly more than 1000.  
This experiment was performed several times for each 
algorithm, and a scatter plot of the results are given in
Figure~\ref{fig-mv-vary-run-time}.

\onefig{fig-mv-vary-run-time}
{Runtime of BFR and DPR for varying number of MVs in the system}{2.75in}

Figure~\ref{fig-mv-vary-run-time} shows the algorithm runtime
for increasing number of materialized views given to the system.
The results show that DPR becomes prohibitively expensive even when 250 MVs
are present in the system.
BFR on the other hand scales much better than DPR and the runtime is
under 1000 seconds even when the system has 1000 relevent views to the given query. 
We note that the runtime of DPR may also be too expensive for systems where the execution time
of most queries is not more than a few tens of seconds.
For such cases, one can resort to
additional pruning to reduce the search space, 
but BFR algorithm will still find the best rewrite in the space it considers.

\subsubsection{Comparison with Caching-based methods}\label{sec-experiments-restore}


\onefig{fig-restore-comparison-execution-improvement}
{Execution time improvement for query evolution using BFR
  and ReStore}{2in}

Here we compare our approach against caching-based methods such as ReStore~\cite{Elgh2012} that only
consider reusing identical answers.
Figure~\ref{fig-restore-comparison-execution-improvement} shows the query execution time
improvements for query evolution of Analyst 1.
The results shows that both BFR and ReStore are identical for $A_1v_2$, while
ReStore is a worse than BFR for $A_1v_2$ and significantly worse for $A_1v_3$.
Reusing cached results is clearly effective although their performance
can be quite unpredictable as good performance is contigent on identical answers being
present in the system.

\begin{table}[h!]
\vspace{-0.2in}
\caption{\label{fig-re-novf-vs-vf-time-improvement}
Improvement in execution time of user evolution using BFR with 
and without identical views}
{\small
\centering
\begin{tabular}{| p{1.5cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}|p{0.40cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}|}
\hline
Analyst & $A_1$ & $A_2$ & $A_3$ & $A_4$ & $A_5$ & $A_6$ & $A_7$ & $A_8$ \\ \hline
BFR(with) & 57\% & 64\% & 86\% & 85\% & 78\% & 98\% & 88\% & 84\% \\ \hline
BFR(without) & 57\% & 64\% & 83\% & 85\% & 51\% & 96\% & 88\% & 84\% \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}

However, to illustrate the robustness of our rewrite algorithm way beyond simple caching
methods, we present an experiment where we prune away all identical views from the solution space.
This setup represents the worst-case for caching-based methods,
as caching methods will not be able to find any rewrites, thus will 
result in no improvement.
%caching-based methods are not nearly as effective as our approach.
Table~\ref{fig-re-novf-vs-vf-time-improvement}
reports the percentage improvement using our algorithm when identical views are present (with), 
and after pruning them all away (without).
Our algorithm results in good improvement
with and without identical views, showing only a slight
performance drop without identical views 
for all analysts except $A_5$.
This is because $A_5$ had previously benefited from an identical view corresponding
to restaurant similarity which it now had to recompute.
Note that identical views constituted only 7\% of 
the view storage space here.
Given that analysts pose different but related queries in an evolutionary scenario,
any method that relies solely on exact matching will have limited benefit.



\subsubsection{Comparison with DB-X}
To verify that our system produces good rewrites, we compared the rewrites 
produced by our algorithm with a widely-used commercial database system (DB-X) 
and data from the TPC-H \cite{tpcds} benchmark.
DB-X was tuned to its highest optimization level as well as 
set to consider all views for query rewriting.
To represent artifacts from prior executions in our system
we created MVs using  the {\tt LINEITEM} table.
One MV is a groupby-count on {\tt L\_ORDERKEY, L\_SUPPKEY} 
and the other is a groupby-count on {\tt L\_ORDERKEY, L\_PARTKEY}.
We used both systems to produce rewrites for three queries and then compared
their estimated cost using the DB-X query optimizer.
The first query tests if DB-X will produce a rewrite 
that involves a join of the two syntactically relevant MVs.
The second query tests groupby unrolling while reusing the count 
aggregate, while the third query tests a more complicated case of reusing 
count aggregate as well as a max aggregate on one of the keys. 
In the first query, DB-X did not use the MVs for the rewrite 
which made it 3X worse than the rewrite produced by
our system. 
In the second query, both DB-X  and our system produced
identical rewrites, resulting in the same cost. 
In the third query, DB-X did not make use of an MV, 
whereas our rewrite did resulting in a 5X savings. 
This experiment shows 
that our rewrite algorithm produces  rewrites comparable to a
state of the art commercial system. 
%Given that we also allow UDFs in our rewrite 
%language, we will use our rewrite algorithm in the bottom-up (DPR) approach.

\subsubsection{View Storage Maintenance}\label{sec-experiments-gc}

\begin{table}
\caption{\label{fig-ga-improvement-vs-storage-reclaimed}
Execution Time Improvement after reclaiming 10\% to 90\% of the 
view storage space}
{\small
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Reclaimed Storage & $10\%$ & $20\%$ & $30\%$ & $50\%$ & $70\%$ &$90\%$\\ \hline
Improvement & 89\% & 88\% & 86\% & 82\% & 58\% & 30\% \\ \hline
\end{tabular}
}
\vspace{-0.14in}
\end{table}

Since storage is not infinite a reclamation policy is necessary.
Although many policies are possible, we demonstrate the robustness of our approach 
using two unsophisticated policies since this is not focus of our work.
The first randomly drops views to reclaim 10\%--90\% 
of the view (configuration) storage space and then we run the $A_5v_3$ query 
as used in Section~\ref{sec-experiments-system-improves}. 
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
reports the average query execution time improvement when applying our rewrite algorithm after reclaiming 
various amounts of storage space randomly.
Each test is repeated twice (different randomizations) and we report the average improvement.
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
shows that our system produces rewrites that give good improvement even as the view storage 
space decreases.

The second policy considered is one that drops all of the \textit{best} views for a 
query, representing an adversarial storage reclamation policy.
The best views are those with the ability produce a low cost rewrite, 
thus such a policy would drop any view that is identical to a target in the plan.
Table~\ref{fig-re-novf-vs-vf-time-improvement}
indirectly captures the performance
of our rewrite algorithm given an adversarial policy showing the robustness of our system even 
when there are no identical views for the targets in the plan of a query.
% Best refers to those views that have maximum benefit 
% with lowest cost, 
%, although in the current work we do not consider maintenance cost.
%
% which is exactly the effect measured by the previous experiment
% where our approach shows only slight performance loss after
% dropping the identical views.
% Taken together, the previous two experiments show the
% robustness of our system and rewrite algorithm.

The hardness of designing a good policy is equivalent to a view selection problem with a storage constraint.
Certainly better methods~\cite{Mami2012} could be applied but we leave this for future work.


\begin{comment}
\subsubsection{Garbage Collection}

Next how garbage collection does not result in significant loss
of performance. 

Next we briefly consider the effects garbage collection on 
our algorithm performance and workflow execution time.
Garbage collection can be applied to recover storage space
or to reduce the runtime of the rewriting algorithm.
Figure~\ref{fig-mv-vary-num-candidates}(a) shows the space of
candidate views is exponential, thus arguing to keep the
number of views lower.  
Figure~\ref{fig-mv-vary-num-candidates}(b) shows that even 
for higher numbers of available views randomly 'retained' 
among all available views, our algorithm 
only needs to find very few rewrites to obtain $r^*$.

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%% End of File

\begin{comment}
\begin{enumerate}

\item Analyst1 wants to find influential users who are
interested in food with the goal that
these users could be target of a future advertisement campaign.
The evolution of this scenario will propose increasingly
sophisticated interpretations of what it means to be ``influential''.

\item Analyst2 wants to identity 100 wine lovers so that he can 
send them a coupon for a new wine being introduced in the market. 
The evolution of this scenario will investigate 
increasingly sophisticated ways of finding out if a user is a ``wine lover''.

\item Analyst3 wants to start a birthday gift recommendation service where friends
can send a gift certificate to a user $u$ who's birthday is around the corner.
We want to generate 5 restaurant choices based on $u$'s preferences and alert
$u$'s friends to $u$'s upcoming birthday and offer them a choice
of discount certificates to the 5 restaurants.
The evolution in this scenario will investigate how to determine
if a user likes a restaurant enough to visit it on his birthday,
how to suggest a diverse set of recommendations as well as
how to suggest restaurants that would cater to $u$'s close set of friends.

\item Analyst4 wants to provide restaurants with a breakdown of their
customer population. 
In particular, the analyst wants to provide breakdowns in terms of who goes to a
particular restaurant.
The analyst may also want to perform analysis in terms for geographical area.
For instance, for any area which are the popular restaurants by categories etc.
The goal of this scenario is to perform increasingly complicated analytical 
operations on the log.

\item Analyst5 wants give restaurant owners a poaching tool in the 
the following sense.
For each restaurant $r$, we identify customers who go to a ``similar'' 
restaurant in the area but do not visit $r$.
Using the list, the owner of $r$ may send these customers a coupon.
The evolutionary nature of the problem is to find out how to determine
``similar'' restaurants.

\item Analyst6 tries to find out if restaurants are losing their
loyal customers.
In other words, we want to identify those customers 
who used to visit frequently but now slowly
stopped visiting the restaurant, but are still visiting other restaurants in the area.
The restaurant owner can send them a coupon to win them back.
The evolutionary nature of this scenario will focus on 
how to identify prior active users.

\item Analyst7 wants to go by the maxim in business that problems should be caught
as soon as possible. 
For each restaurant in the system, try to identify common problems that
users have reported about the restaurant.
For example, have customers complained about food, service, issues with premises etc.
Moreover, if there is a successful restaurant of the same category, 
what makes it successful.
The evolutionary nature of this scenario will focus on compiling
issues under different categories.

\item Analyst8 wants to identity what category (i.e., american, indian,
chinese, steak) of restaurants is missing from a
certain region. For example, one of the outcome can be that 
Cupertino could really use a Moroccan restaurant. 
The evolutionary nature of this scenario will focus on how to 
find out if there is a need for a good restaurant in a certain
category and if so what is the nature of their clientele etc.

The use-case for our system that it is being used internally
by analysts who work for restaurant marketing company that gets commission
from sending users to restaurants or providing restaurant 
owners analytics support to aid them in their business decisions.
Each analyst starts out with a single log file and expanding
to all the three log files during the course of their
evolutionary workflow.
{\it The idea here is not to get too carried away by the quality
of the answers we get but write workflow structures that capture
the spirit of these scenarios.}


\end{itemize}


The desirable property of the $\cost{}$ is that it must be cheap to compute.
Since a full query optimizer may be too expensive, we use a model of a query optimizer.
We treat this model as a black box, in this way $\RE{}$ and $\ocost{}$ can
utilize any functionality provided by the model or improvements to the model.
%For an RDBMS, a cost model such as in~\cite{x,y} could be used.  
%Because we evaluate our framework in a MapReduce execution system, 

Our cost model is based on the one in~\cite{Nyki2010}, 
which reduces a query $q$ to a set of $m$ jobs $\{J_1, \cdots, J_m\}$. 
The cost of each job is expressed as a linear combination of 
the cost to read the data ($C_{r}$)
the cost of sorting and copying ($C_{s}$),
the cost to transfer data ($C_{t}$).
and the cost to write the output of the job ($C_{w}$).

\begin{equation} \label{eq-cost}
\cost(q,v) = \sum_{i=1}^{m} C_{r}(J_i,v_i) +  C_{s}(J_i,v_i) +  C_{t}(J_i,v_i) +  C_{w}(J_i,v_i)
\end{equation}
where $v_1 = v$, and $v_{i}$ forms the input of $J_i$.

               
To keep the $\cost{}$ function inexpensive, our model does not consider re-ordering 
of joins, predicate push down, or other types of optimizations involved in 
group bys and udfs, but does merge sequential operations (e.g. a sequence of filters)
into the same job whenever possible.


This is a reasonable approach given that we have already committed to creating $v$,
and the $\RE{}$ explores all possible rewrites, such a cost function serves
our purposes here.  

An extension to this basic cost model could consider push downs when computing the cost
to create $v$.  The requirements to including push-downs into the optimization
process would be to employ a cost model $\cost{}$ that is able to 
apply all possible join orderings to creating $v$ along with applying filters 
to all orders.  

Appendix~\ref{appendix-pushdown} provides a proof for using $\RE{}$ and $\ocost$ with an extended 
$\cost{}$ function that considers join ordering and predicate pushdowns,
while still producing a correct lower bound for $\RE{(v,q)}$.

There are 2 reasons we do not consider predicate push downs here.
First $\cost{}$ becomes much more expensive to invoke due to considering all 
of the ordering options. 
Second, we may not wish to push down a filter into $v$ since this could render $v$ 
less useful for answering future queries.  
A more sophisticated algorithm could weigh the cost and benefits of different 
versions of $v$ (with and without filters) given their benefit to other queries 
and their added cost due to avoiding filter push downs.

\subsubsection{Comparison with DB2 and ReStore:}

Show that our $\VF{}$ performs better rewrites compared to 
the DB2 design advisor.
We also need to emphasize that there is a significant ETL time with DB2
which we will not consider for this experiment.

{\em Run the workflow A4-v1 and store the MVs of all targets
  produced by this workflow in DB2. Next, we
give DB2 queries corresponding to $W_n \cdots W_1$ of the A4-v2.
We obtain DB2 cost estimates for the rewrites provided by DB2. 
Next we obtain the rewrite $r^*$that our algorithm provides and 
get it costed using the DB2 cost model.
Hopefully, we can show using the DB2 cost model 
that $r^*$ is cheaper than its own rewrite.

Graph: DB2 optimizer estimated time units (y-axis) against 
DB2 rewrite and $r^*$ for A4-v2 (x-axis).
We may try to do it for all workflows,  A1 thru A8

{
\color{red}
\sout{
Graph2: It would also make sense to take care of ReStore early
on so that we do not have to keep comparing with it through
the rest of the section.} (as per Alkis's comments)
}
}

\item Weakness of $\ocost{}$ on the work efficiency of the
$\VF{}$.
Measure the total rewrites possible (P),
number of rewrites we explored (T),
number of rewrites explored that we should not have explored (E)
(y-axis) vs. three variants of $\ocost{}$ in x-axis.

P here denotes the complexity of a non-incremental algorithm,
T is the total work done by us, E is wasted work among T.

\item Graph on time taken to find $r^*$ (y-axis) vs.
{\em features} of the workflow. Features of the workflow include
$n$, number of joins, udfs etc.

Graph on time taken to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 
  
\item Graph on number of rewrites explored to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 

\item Compare our algorithm with diminished
versions of the algorithm.
Graph on estimated cost of $r^*$ (y-axis) vs. 
remove modules of the $\VF{}$ one by one.
For example, we could reduce the expressivity of $L_R$, joins etc.
This set of experiment will show the benefit of added complexity.\\

{\color{red}

Alkis says: ``I think that this should go first, so that the other experiments utilize the full-featured algorithm''

Response: OK
}

{\color{red}
\sout{We could handle ReStore here as one way of performing equivalent
rewrites}.
}
\end{enumerate}


{\em 
{\color{red}

Alkis: ``Do we know the theoretical complexity of our view-rewrite algorithm?''

Response: Our rough calculation is as follows.

The complexity of the $\WF{}$ is $O(n.l)$, where
$l$ is the number of samplings of the cost range $[0, \cost(W_n)]$.
$l$ can be chosen to be $n$ 
so that the $\WF{}$ algorithm is 
bounded by $O(n^2)$.

The $\VF{}$ is bounded by $O(|V|^{k_1} 2^{k_2})$ where 
$k_1$ represents the maximum number of candidates that
may be explored (generated + existing) by the $\VF{}$, 
while $k_2$ is a small constant 
representing the number of transformation rules in the system.
$k_1$ is bounded by $n$ as in the worse case $W_n$ may
contain $n-1$ joins.
Assuming all joins are of the same cost, the most expensive rewrite
for $W_n$ may contain up to $O(n)$ joins.
Hence, the complexity of the $\VF{}$ for a single target
is bounded by $O(|V|^n 2^{k_2})$.

The complexity of the entire algorithm is bounded by:
$O(n^2 + n \cdot |V|^n 2^{k_2})$, where $k_2 << |V|$.

}

\end{comment}


==> old/Experimental_evaluation-rewrite2.tex <==
\section{Experimental Evaluation}\label{sec-experimental-evaluation}

\twofigrow{fig-we-novf-vs-vf-running-time}
{fig-we-novf-vs-vf-time-improvement}
{Query evolution comparisons for (a) query execution time (log-scale)
and (b) execution time improvement}{3in}

In this section, we present an experimental study we conducted in order to 
validate the effectiveness of $\WF{}$ in finding low-cost rewrites of complex queries. 
We first evaluate our methods in two scenarios.
The {\em query evolution} scenario (Section~\ref{sec-query-evolution}) represents a user 
iteratively refining queries within a single session.
This scenario evaluates the benefit that each new query version receives from the opportunistic
views created by previous versions of the query.
The {\em user evolution} scenario (Section~\ref{sec-experiments-ue}) represents a new user
  entering the system presenting a new query.
This scenario evaluates the benefit a new query receives from the opportunistic
views created by queries of other users.
We compare the performance of our algorithm for the user evolution scenario (Section~\ref{sec-scalability})
with a baseline dynamic programming approach
that searches at all targets without using $\ocost{}$.
Next, we evaluate the scalability  (Section~\ref{sec-scalability}) of our rewrite algorithm in comparison
to the dynamic programming approach.
We then compare our method to cache-based methods (Section~\ref{sec-experiments-restore}) 
 that can only reuse identical previous results.
We show the performance of our method (Section~\ref{sec-experiments-storage-reclamation}) under a storage reclamation policy that drops opportunistic views.
Lastly, as a sanity check (Section~\ref{sec-experiments-dbx}) we compare the quality of rewrites produced by our algorithm with a state-of-the-art  DBMS.


\subsection{Methodology}\label{sec-evaluation-setup}
% UDF is written in Hive, perl, python, MR but the transformation applied
% by the UDF is expressed in terms of a grammar that describes how an input
% attributes, filter and groupby properties are modified by the UDF.

Our experimental system consists of 20 machines running Hadoop.
We use HiveQL as the declarative query language, and Oozie as a
job coordinator.
UDFs are implemented in Java, Perl, and Python and executed
using the HiveCLI.
Some UDFs implemented in our system are log parser/extractor,
text sentiment classifier, sentence tokenizer, lat/lon extractor, 
word count, restaurant menu similarity, and geographical 
tiling, among others.


Hive currently lacks a  {\em what-if} optimizer functionality, which is needed 
to obtain cost estimates for hypothetical plans.
%Additionally, it cannot consider UDFs and their costs properly.
For these reasons, we created a  what-if optimizer that uses the cost model 
developed for MR frameworks in~\cite{Nyki2010} that considers basic data statistics, 
number of map and reduce tasks, and number of jobs.

Our experiments use the following three real-world datasets totaling over 1TB:
a Twitter log containing 800GB of tweets, 
a Foursquare log containing 250GB of user check-ins, 
and a Landmark log containing 7GB of 5 million landmarks including their locations.
The identity of a social network user (\texttt{user\_id}) is common across
the Twitter and Foursquare logs, while the identity of a landmark
 (\texttt{location\_id}) is common across the Foursquare and Landmarks logs.


The metrics we report during evaluation of query performance are execution time in seconds
and the amount of data manipulated (read/write/shuffle) in GB. %, and the runtime of the rewrite algorithm in seconds.
% For these experiments, \textsc{bfr} denotes  the use of our \WF{} algorithm and opportunistic views, 
% while \textsc{no-bfr} represents execution time of the original query plan.
% For the algorithm evaluations, \textsc{dpr} represents a dynamic programming approach
% that does not use \ocost{} and searches for all rewrites at every target.
When comparing $\WF{}$ to the Dynamic Programming algorithm, we use the following metrics: running time to 
find the rewrite, the number of candidate views examined during the search for rewrites,
and the number of valid rewrites produced.
%\textsc{dpr}  finds the best rewrite for each target and then identifies a subset 
 %of these to obtain $r^*$ using a dynamic programming algorithm.
We limit both algorithms from considering more than
$4$-way joins simply for practical reasons.


\subsubsection{Evolutionary Query Workload}\label{sec-evauation-query-scenarios}

Our test workload simulates 8 analysts who write complex queries containing 
UDFs, representing realistic marketing scenarios for restaurants.
%We derived these representative queries from extensive conversations with 
%business users on their typical analytics use cases.
 %, which are described in 
 %Table~\ref{tab-experiment-scenarios}.
Each analyst in our scenario creates 4 versions of a query, representing the query's evolutions
during data exploration and hypothesis testing.
We use these 32 queries for all of our evaluations.
%Each query version captures the analyst's iterative 
%...attempt  at bringing the query closer to her intended goal.
%refinements to the query during data exploration and hypothesis testing.
On average, the original plan of a query creates 17 opportunistic materialized views.

We give a high-level description of these queries in 
Table~\ref{tab-experiment-scenarios}.
We modeled our analyst queries after observing query evolutions
%We modeled our analyst queries after query evolutions we observed 
in three domains -- Yahoo! Pipes
%~\cite{Yahoo2012} 
queries using public web data,
Taverna~\cite{Taverna2012} scientific workflows using biological science data,
and TPC-DS~\cite{tpcds} interactive queries using warehouse data.
Common changes between versions that we identified include
a parameter change %to a selection predicate or a top-k value
to allow for more or less data in the results,
adding a new subgoal to the query,
adding a new UDF or replacing operations with a specialized UDF, and 
incorporating additional data sources to obtain richer results.
Each of our query versions are revised in this manner, and each
revision includes at least two types of changes.
%Based on the common types of revisions we identified in these domains, 




\begin{comment}
\onefig{fig-slug-illustration}
{Dimensions of change between query versions}{2.2in}

We modeled our analyst queries by observing query evolutions
%We modeled our analyst queries after query evolutions we observed 
in three domains -- Yahoo! Pipes~\cite{Yahoo2012} queries using public web data,
 Taverna~\cite{Taverna2012} scientific workflows using biological science data,
and TPC-DS~\cite{Tpc2012} interactive queries using warehouse data.
Based on the common types of revisions we identified in these domains, 
we define the following 
dimensions of change that the describe changes between each query version
in Table~\ref{tab-experiment-scenarios}.

(P) Parameters: Most of the query remains unchanged except for modifications
to parameters that allow greater or fewer answers in the query results.  
(Figure~\ref{fig-slug-illustration}P).
For example, the analyst may alter a select predicate or a top-\textsc{k} value
 to allow for more or less data in the results.
 
 (L) Logs: An analyst may augment a query with a new log to obtain richer 
results (Figure~\ref{fig-slug-illustration}L).

(U) UDFs: An analyst may replace operations in the query with a 
specialized UDF (Figure~\ref{fig-slug-illustration}U) to the system,
which contributes to the divergence of $L_W$ from $L_R$.

(G) Sub-Goals: An analyst includes (or removes) sub-goals that join to
obtain the final output (Figure~\ref{fig-slug-illustration}G).

These four dimensions \{P,L,U,G\} informally describe the changes from one 
query version to the next. 
For instance, the right-side column of Table~\ref{tab-experiment-scenarios},
describes the changes in Analyst2's four query versions as follows.
\begin{center}
$Q \rightarrow \{P,L,G\} \rightarrow \{P,G\} \rightarrow \{P,U,G\}$
\end{center}

The analyst begins with initial query $Q$ (i.e., $A_2v_1$) then adds a log $L$,
 modifies a sub-goal $G$ and parameters $P$ to obtain version 2 
 (i.e., $A_2v_2$) from $Q$, and so on.
 %The ordering $\{L,G,P\}$ indicates the $L$ dimension 
%likely affects the rewrite cost more than $\{G,P\}$.
\end{comment}



In the following set of experiments, $A_iv_j$ corresponds to the Analyst $i$ 
running version $j$ of her query.
We describe one Analyst's query in more depth using Example~\ref{ex-query-a2v2}.

\begin{example}\label{ex-query-a2v2}
$A_2v_2$:
Find users with affluent friends that tweet 
positively about food, and visit a lot of pubs.


(a): EXTRACT from Foursquare log.
EXTRACT restaurant name from text.
FILTER by check-ins to wine places.
GROUPBY user, compute count.
Find MAX user check-in.
Compute check-in score for each user.

(b): EXTRACT user from Twitter log.
Compute FOOD-SENTIMENT score for each user.

(c): CLASSIFY user's tweets from Twitter log as affluent or not.
GROUPBY affluent users, compute affluent tweet count.
Find MAX count among all users.
COMPUTE an affluent score for each user.

(d): Create social network from Twitter log
using tweet source and dest.
GROUPBY user pair in social network, count tweets. 
Find MAX tweets between a user pair.
Assign friendship strength score to each user pair.

JOIN (a), (b), and (c) on user\_id.
Then JOIN with (d) based on friend\_id .
Threshold based on checkin score, food-sentiment score, 
friendship score, and affluent score.
\end{example}


\subsection{Experimental Results}


\threefig{fig-ue-novf-vs-vf-running-time}
{fig-ue-novf-vs-vf-data-moved}
{fig-ue-novf-vs-vf-time-improvement}
{User Evolution Comparisons for (a) query execution time (log-scale)(b) data moved
(c) execution time improvement}{2in}


\subsubsection{Query Evolution}\label{sec-query-evolution}

 
This section presents results for the query evolution scenario, where a user's 
new query can benefit from opportunistic views created during execution 
of previous versions of the query.
In this experiment, an analyst (e.g., $A_i$) executes the first version of his query (e.g., $A_iv_1$) 
followed by issuing each subsequent version 
(e.g., $A_iv_2$, $A_iv_3$, $A_iv_4$).
Subsequent versions of a query are rewritten 
given the benefit of all opportunistic materialized views from previous versions of the query.

Figure~\ref{fig-we-novf-vs-vf-running-time}(a) shows the performance of
the original query plan (\textsc{no-bfr} in graph) and 
the optimized query plan after rewriting with \WF{} (\textsc{bfr} in graph).
%This figure shows the execution time for each subsequent version of the query 
%is consistently lower when using  our method (\textsc{bfr}).
Figure~\ref{fig-we-novf-vs-vf-running-time}(b) shows the corresponding 
percent improvement in execution time for $\WF{}$ over the baseline 
original plan resulting from 10\% up to 90\% improvement, representing
an average improvement of 61\% and up to two orders of magnitude.
As a concrete data point, $A_5v_4$ requires 54 minutes to execute in the baseline system,
but only  55 seconds after $\WF{}$ finds a suitable rewrite.
The amount of data manipulated (i.e., read/write/shuffle bytes) closely followed the
same trend in Figure~\ref{fig-we-novf-vs-vf-running-time}(a).
% Data moved results are not reported here because later we present the results 
% showing similar data movement trends for the user evolution experiments in 
% Section~\ref{sec-experiments-ue}, 
%Figure~\ref{fig-ue-novf-vs-vf-running-time}(b).
The significant savings in execution time for $\WF{}$ 
can be attributed to moving much less data, 
and avoiding the costly re-extraction of data from raw logs whenever possible, 
due to our algorithm's ability to reuse prior computation from 
all previous query versions, i.e., opportunistic materialized views.
%These results show the benefit of our methods for the query evolution scenario,
%where a user benefits from opportunistic views created during execution
%of 

\subsubsection{User Evolution}\label{sec-experiments-ue}

This section presents results showing the benefit of our methods for the 
user evolution scenario, where a user benefits from opportunistic views 
created during execution of other user's queries.
In this scenario, a new analyst 
arrives and executes the first version of his query given that
all of the other analysts have previously executed their queries in the system.
Our \WF{} algorithm rewrites $A_iv_1$ using the opportunistic materialized 
views from all other analyst queries.

Figure~\ref{fig-ue-novf-vs-vf-running-time}(a) shows the query execution
time while Figure~\ref{fig-ue-novf-vs-vf-running-time}(b) shows the 
data manipulated (read/write/shuffle) for $\WF{}$ and the original plan.
The results demonstrate that query execution time is always lower 
with $\WF{}$, with a similar trend in the amount of data moved.
The percentage improvement in execution time is given in 
Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) where it can be
seen that our system results in an improvement of about 50\%--90\%.


\begin{table}[!h]
\caption{\label{fig-se-novf-vs-vf-time-improvement}
Improvement in execution time of $A_5v_3$ as more
analysts become present in the system}
\centering
\begin{tabular}{| p{2.45cm} | p{0.35cm}| p{0.45cm} | p{0.45cm}| p{0.45cm} | p{0.45cm}|  p{0.45cm} | p{0.45cm}|}
\hline
Analysts  in System & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\ \hline
Improvement    & 0\% & 73\% & 73\% & 75\% & 89\% & 89\% & 89\% \\ \hline
\end{tabular}
\end{table}

As an additional experiment, we show the increasing benefit a user may receive
each time a new analyst arrives and executes their queries.
To show this, first we execute $A_5v_3$ with no opportunistic views in the system,
to create a baseline execution time.
We ``add'' another analyst by executing all four versions of that
analyst's query, creating new opportunistic views. 
Then we re-execute $A_5v_3$ and report the performance 
improvement for  $A_5v_3$ over the baseline as new analysts are added.
We chose $A_5v_3$ as it is a complex query using all three logs. 
Table~\ref{fig-se-novf-vs-vf-time-improvement} reports the 
execution time improvement as analysts are added, 
showing an increasing benefit as more users are present in the system.
The benefit is obviously dependent on similarity to other
analysts' queries.


\subsubsection{Runtime Comparison of $\WF{}$ and DPR}\label{sec-scalability}

\threefig{fig-ue-bfs-vs-dp-candidates-explored}
{fig-ue-bfs-vs-dp-refine-attempts}
{fig-ue-bfs-vs-dp-time-comparison}
{Algorithm Comparisons for
(a) Candidate views considered, (b) Refine attempts, and (c) Runtime (log-scale)}
{2.15in}

To evaluate the effectiveness of $\WF{}$ to prune the search space of rewrites, 
we compare it against the baseline {\sc dpr} algorithm that exhaustively 
searches the space in order to find the same minimum-cost rewrite. 
First we evaluate the algorithms during the user evolution experiments, 
where the only views in the system are those created by the other users.
This resulted in approximately 100 views for each user evolution experiment.
Next we evaluate the algorithm runtime as we vary the number of views in the system
from 1--1000 to show how the algorithms scale with an increasing number of views.

Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}
compares the performance of the $\WF{}$ and the dynamic programming algorithm ({\sc dpr} in graph)
% by measuring how much of
% the rewrite search space each algorithm explores 
during the user evolution experiment.
While both algorithms find the minimum-cost rewrite $r^*$, these
figures show that $\WF{}$ searches much less of the space to find the 
minimum cost rewrite than does {\sc dpr}.
Candidate views considered in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(a)
corresponds to all the existing views ($V$)  and those views created during 
the rewrite search process (i.e., merged views).
The number of rewrite attempts corresponds to the candidate views examined by
 $\RE{}$ when searching for a valid rewrite with low cost.
%As noted previously this process is computationally expensive.
These results show for many cases it is possible for $\WF{}$ 
to find $r^*$ by considering far fewer candidate views as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(a), 
and orders of magnitude fewer rewrites attempted as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(b),
resulting in significant savings in algorithm  runtime as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(c).
This savings is due to \WF{}'s use of $\ocost{}$ that enables
considering the promising candidate views earlier in the search,
and exploding the space of candidate views incrementally as needed.
% This shows our algorithm results in a significant reduction
% in the rewrite search space.

The next experiment evaluates the runtime performance of $\WF{}$ and 
\textsc{dpr} with an increasing number of materialized views in the system.
We retained about 9,600 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 Analyst scenarios.
% This setup is intended to represent a mature system with many opportunistic 
% views created by previous queries.
We use the $\WF{}$ and \textsc{dpr} algorithms to find rewrites for one 
analyst's query ($A_3v_1$) given a uniform random sampling of subsets of 
the existing 9,600 views to show how the algorithms scale with the number 
of materialized views in the system.
% From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms pruned views at a given target as follows:
a view was pruned if it did not reference the same log as the target,
if it had a predicate condition preventing it from being used in a rewrite for 
the target, or if it was a view that is identical to the target.
Identical views were removed because those do not help to test the scalability
of the algorithms.
After pruning, the number of materialized views available for each target was
slightly more than 1000.  
This experiment was performed many times for each algorithm at a given sample
size.


\onefig{fig-mv-vary-run-time}
{Runtime of $\WF{}$ and DPR for varying number of MVs in the system}{2.5in}

Figure~\ref{fig-mv-vary-run-time} shows the algorithm runtime
for increasing number of materialized views in the system.
\textsc{dpr} becomes prohibitively expensive even when 250 MVs
are present in the system.
$\WF{}$ on the other hand scales much better than \textsc{dpr} and has
a runtime under 1000 seconds even when the system has 1000  views relevant
to the given query. 
% The runtime of \textsc{bfr} may also be too expensive for systems 
% where the execution time of most queries is not more than a few tens of 
% seconds.
While this runtime is not trivial, we note that these are complex queries
involving UDFs that run for thousands of seconds.
%Note that these are complex queries involving UDFs that run for thousands
%of seconds.
The amount of time spent to rewrite the query plus the execution
time of the optimized query is far less than the execution time of unoptimized queries.
For instance, Figure~\ref{fig-ue-novf-vs-vf-running-time}(a) 
reports a query execution time of 451 seconds for $A_5$ optimized versus 
2134 seconds for unoptimized. 
Even if the rewrite time were 1000 seconds (in this case it is actually 3.1 seconds
as seen in Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(c)), 
the end-to-end execution time would be lower by 11 minutes or 32\%. 

However, additional pruning techniques~\cite{Agra2000} can 
be used to reduce the number of views, thereby reducing 
the algorithm search space.
We note that \WF{} will find the minimum cost rewrite in the space it considers.

\subsubsection{Comparison with Caching-based methods}\label{sec-experiments-restore}

Here we compare our approach against caching-based methods 
such as ReStore~\cite{Elgh2012} that only reuse identical answers (i.e.,
existing views that require no compensation).
%i.e., answers generated by identical plans.
Figure~\ref{fig-restore-comparison-execution-improvement} shows the 
query execution time improvements for query evolution of Analyst 1.
The results show that both $\WF{}$ and ReStore are identical for $A_1v_2$, while
ReStore is worse than $\WF{}$ for $A_1v_2$ and significantly worse for $A_1v_3$.
Reusing cached results can  clearly be effective.
However, performance is highly dependent upon the presence of identical 
answers previously generated in the system as cache methods lack
a robust capability to reuse previous results.

\onefig{fig-restore-comparison-execution-improvement}
{Execution time improvement for query evolution using $\WF{}$ 
  and ReStore}{2in}

\begin{table}[h!]
\caption{\label{fig-re-novf-vs-vf-time-improvement}
Improvement in execution time of user evolution using $\WF{}$ without identical views}
{\small
\centering
\begin{tabular}{| p{1.5cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}|p{0.40cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}|}
\hline
Analyst & $A_1$ & $A_2$ & $A_3$ & $A_4$ & $A_5$ & $A_6$ & $A_7$ & $A_8$ \\ \hline
%BFR(with) & 57\% & 64\% & 86\% & 85\% & 78\% & 98\% & 88\% & 84\% \\ \hline
$\WF{}$ & 57\% & 64\% & 83\% & 85\% & 51\% & 96\% & 88\% & 84\% \\ \hline
\end{tabular}
}
\end{table}

To illustrate the robustness of our rewrite algorithm beyond caching-based
methods, we present an experiment where we prune away all identical views from 
the solution space.
Removing all identical views represents the worst-case scenario for 
caching-based methods.
Such methods will not be able to find \textit{any} rewrites, resulting in 0\% improvement. 
%caching-based methods are not nearly as effective as our approach.
Table~\ref{fig-re-novf-vs-vf-time-improvement}
reports the percentage improvement using \WF{} when identical views 
have been pruned from consideration.
Our algorithm results in very good performance improvement, and these results 
are comparable to the results in Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) 
that represents the same experiment without pruning identical views.
Table~\ref{fig-re-novf-vs-vf-time-improvement} shows a performance 
drop for $A_5$ compared to the results reported in 
Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) for $A_5$. 
This is because $A_5$ had previously benefited from an identical view corresponding
to restaurant similarity which it has to recompute.
Note that identical views constituted only 7\% of  the view storage space in 
this experiment.
Given that analysts pose different but related queries in an evolutionary scenario,
any method that relies solely on identical matching can have limited benefit.



\subsubsection{Storage Reclamation}\label{sec-experiments-storage-reclamation}

\begin{table}
\caption{\label{fig-ga-improvement-vs-storage-reclaimed}
Execution Time Improvement after reclaiming 10\% to 90\% of the 
view storage space}
{\small
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Reclaimed Storage & $10\%$ & $20\%$ & $30\%$ & $50\%$ & $70\%$ &$90\%$\\ \hline
Improvement & 89\% & 88\% & 86\% & 82\% & 58\% & 30\% \\ \hline
\end{tabular}
}
\end{table}

Since storage is not infinite a reclamation policy is necessary.
We demonstrate the robustness of our approach using unsophisticated 
policies, since reclamation is not the focus of this work.
The first simple policy randomly drops views to reclaim 10\%--90\% 
of the view storage space.
%As a baseline, we execute the before dropping any views.
After each reclamation, we run the $A_5v_3$ query 
(used in Section~\ref{sec-experiments-ue})
after applying our rewrite algorithm, and 
compare it to a baseline without our rewrite algorithm.
%and report the percentage improvement in execution time over the baseline
%of \textsc{no-bfr}.
Each test is repeated twice (different randomizations).
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
reports the average execution time improvement for $A_5v_3$ after reclaiming
 various amounts of storage space. % randomly.
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
shows that our system is able to find good rewrites for $A_5v_3$ using the 
remaining views available,
%even when much of the storage space is reclaimed.
until most of the storage space is reclaimed.

Second, Table~\ref{fig-re-novf-vs-vf-time-improvement} provides another perspective 
on how storage reclamation can affect the effectiveness of $\WF{}$. 
Specifically, we observe that $\WF{}$ is able to find good rewrites 
even if the optimal views for each query are removed. 
These results suggest that our approach is robust to ``bad'' 
choices made by the reclamation policy, provided some good views remain in the system.\looseness=-1 
% The best views are those with the ability produce a low cost rewrite, 
% thus such a policy would drop any view that is identical to a target in the plan.
% Table~\ref{fig-re-novf-vs-vf-time-improvement} directly captures the 
% performance of our algorithm given an adversarial policy, showing our 
% algorithm maintains good performance.
% This shows the robustness of our system even with a bad storage reclamation 
% policy that drops all of the best views.
% Best refers to those views that have maximum benefit 
% with lowest cost, 
%, although in the current work we do not consider maintenance cost.
%
% which is exactly the effect measured by the previous experiment
% where our approach shows only slight performance loss after
% dropping the identical views.
% Taken together, the previous two experiments show the
% robustness of our system and rewrite algorithm.

The hardness of designing a good policy is equivalent to the view selection 
problem with a storage constraint.
Certainly better methods~\cite{Mami2012} could be applied but we 
leave this for future work.


\subsubsection{Comparison with DB-X}\label{sec-experiments-dbx}

To verify that our system produces good rewrites, we compared our rewrites
to those of a widely-used commercial database system (DB-X)
using data from the TPC-H~\cite{tpcds} benchmark.
DB-X was tuned to its highest optimization level as well as
set to consider all views for query rewriting.
We created two materialized views on the {\tt LINEITEM} table:
group-by--count on {\tt L\_ORDERKEY, L\_SUPPKEY},
and group-by--count on {\tt L\_ORDERKEY, L\_PARTKEY}.
% Our goal was to verify  the rewrites produced by $\WF{}$
% were not significantly worse than those produced by DB-X.
To test the rewrites produced by both systems,
 we use three queries on the {\tt LINEITEM} table:
a) groupby on {\tt L\_ORDERKEY, L\_SUPPKEY, L\_PARTKEY}
b) group-by on {\tt L\_ORDERKEY} with count aggregate, and
c) group-by on {\tt L\_ORDERKEY} with count and max aggregate
on {\tt L\_SUPPKEY}.
The resulting rewrites were given to the DB-X query optimizer,
which provided a cost estimate for each rewrite.

$\WF{}$ made use of both materialized views for the first query while
DB-X did not make use of them which resulted in a rewrite
that was 3$\times$ worse than the rewrite produced by $\WF$.
For the second query both $\WF{}$ and DB-X resulted in identical
rewrites.
For the third query, DB-X did not make use of a materialized view,
whereas $\WF{}$ did resulting in a 5$\times$ improvement over DB-X.
% Our sanity check experiment shows that our rewrite algorithm 
% produces rewrites that are competitive to a state of the art commercial system.
$\WF{}$ produces rewrites competitive to a state-of-the-art commercial DBMS on queries that 
are much simpler than our setup. Using the DBMS to rewrite the complex 
queries in our workload would most likely result in very little improvement. 


\begin{comment}
\subsubsection{Garbage Collection}

Next how garbage collection does not result in significant loss
of performance. 

Next we briefly consider the effects garbage collection on 
our algorithm performance and workflow execution time.
Garbage collection can be applied to recover storage space
or to reduce the runtime of the rewriting algorithm.
Figure~\ref{fig-mv-vary-num-candidates}(a) shows the space of
candidate views is exponential, thus arguing to keep the
number of views lower.  
Figure~\ref{fig-mv-vary-num-candidates}(b) shows that even 
for higher numbers of available views randomly 'retained' 
among all available views, our algorithm 
only needs to find very few rewrites to obtain $r^*$.

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%% End of File

\begin{comment}
\begin{enumerate}

\item Analyst1 wants to find influential users who are
interested in food with the goal that
these users could be target of a future advertisement campaign.
The evolution of this scenario will propose increasingly
sophisticated interpretations of what it means to be ``influential''.

\item Analyst2 wants to identity 100 wine lovers so that he can 
send them a coupon for a new wine being introduced in the market. 
The evolution of this scenario will investigate 
increasingly sophisticated ways of finding out if a user is a ``wine lover''.

\item Analyst3 wants to start a birthday gift recommendation service where friends
can send a gift certificate to a user $u$ who's birthday is around the corner.
We want to generate 5 restaurant choices based on $u$'s preferences and alert
$u$'s friends to $u$'s upcoming birthday and offer them a choice
of discount certificates to the 5 restaurants.
The evolution in this scenario will investigate how to determine
if a user likes a restaurant enough to visit it on his birthday,
how to suggest a diverse set of recommendations as well as
how to suggest restaurants that would cater to $u$'s close set of friends.

\item Analyst4 wants to provide restaurants with a breakdown of their
customer population. 
In particular, the analyst wants to provide breakdowns in terms of who goes to a
particular restaurant.
The analyst may also want to perform analysis in terms for geographical area.
For instance, for any area which are the popular restaurants by categories etc.
The goal of this scenario is to perform increasingly complicated analytical 
operations on the log.

\item Analyst5 wants give restaurant owners a poaching tool in the 
the following sense.
For each restaurant $r$, we identify customers who go to a ``similar'' 
restaurant in the area but do not visit $r$.
Using the list, the owner of $r$ may send these customers a coupon.
The evolutionary nature of the problem is to find out how to determine
``similar'' restaurants.

\item Analyst6 tries to find out if restaurants are losing their
loyal customers.
In other words, we want to identify those customers 
who used to visit frequently but now slowly
stopped visiting the restaurant, but are still visiting other restaurants in the area.
The restaurant owner can send them a coupon to win them back.
The evolutionary nature of this scenario will focus on 
how to identify prior active users.

\item Analyst7 wants to go by the maxim in business that problems should be caught
as soon as possible. 
For each restaurant in the system, try to identify common problems that
users have reported about the restaurant.
For example, have customers complained about food, service, issues with premises etc.
Moreover, if there is a successful restaurant of the same category, 
what makes it successful.
The evolutionary nature of this scenario will focus on compiling
issues under different categories.

\item Analyst8 wants to identity what category (i.e., american, indian,
chinese, steak) of restaurants is missing from a
certain region. For example, one of the outcome can be that 
Cupertino could really use a Moroccan restaurant. 
The evolutionary nature of this scenario will focus on how to 
find out if there is a need for a good restaurant in a certain
category and if so what is the nature of their clientele etc.

The use-case for our system that it is being used internally
by analysts who work for restaurant marketing company that gets commission
from sending users to restaurants or providing restaurant 
owners analytics support to aid them in their business decisions.
Each analyst starts out with a single log file and expanding
to all the three log files during the course of their
evolutionary workflow.
{\it The idea here is not to get too carried away by the quality
of the answers we get but write workflow structures that capture
the spirit of these scenarios.}


\end{itemize}


The desirable property of the $\cost{}$ is that it must be cheap to compute.
Since a full query optimizer may be too expensive, we use a model of a query optimizer.
We treat this model as a black box, in this way $\RE{}$ and $\ocost{}$ can
utilize any functionality provided by the model or improvements to the model.
%For an RDBMS, a cost model such as in~\cite{x,y} could be used.  
%Because we evaluate our framework in a MapReduce execution system, 

Our cost model is based on the one in~\cite{Nyki2010}, 
which reduces a query $q$ to a set of $m$ jobs $\{J_1, \cdots, J_m\}$. 
The cost of each job is expressed as a linear combination of 
the cost to read the data ($C_{r}$)
the cost of sorting and copying ($C_{s}$),
the cost to transfer data ($C_{t}$).
and the cost to write the output of the job ($C_{w}$).

\begin{equation} \label{eq-cost}
\cost(q,v) = \sum_{i=1}^{m} C_{r}(J_i,v_i) +  C_{s}(J_i,v_i) +  C_{t}(J_i,v_i) +  C_{w}(J_i,v_i)
\end{equation}
where $v_1 = v$, and $v_{i}$ forms the input of $J_i$.

               
To keep the $\cost{}$ function inexpensive, our model does not consider re-ordering 
of joins, predicate push down, or other types of optimizations involved in 
group bys and udfs, but does merge sequential operations (e.g. a sequence of filters)
into the same job whenever possible.


This is a reasonable approach given that we have already committed to creating $v$,
and the $\RE{}$ explores all possible rewrites, such a cost function serves
our purposes here.  

An extension to this basic cost model could consider push downs when computing the cost
to create $v$.  The requirements to including push-downs into the optimization
process would be to employ a cost model $\cost{}$ that is able to 
apply all possible join orderings to creating $v$ along with applying filters 
to all orders.  

Appendix~\ref{appendix-pushdown} provides a proof for using $\RE{}$ and $\ocost$ with an extended 
$\cost{}$ function that considers join ordering and predicate pushdowns,
while still producing a correct lower bound for $\RE{(v,q)}$.

There are 2 reasons we do not consider predicate push downs here.
First $\cost{}$ becomes much more expensive to invoke due to considering all 
of the ordering options. 
Second, we may not wish to push down a filter into $v$ since this could render $v$ 
less useful for answering future queries.  
A more sophisticated algorithm could weigh the cost and benefits of different 
versions of $v$ (with and without filters) given their benefit to other queries 
and their added cost due to avoiding filter push downs.

\subsubsection{Comparison with DB2 and ReStore:}

Show that our $\VF{}$ performs better rewrites compared to 
the DB2 design advisor.
We also need to emphasize that there is a significant ETL time with DB2
which we will not consider for this experiment.

{\em Run the workflow A4-v1 and store the MVs of all targets
  produced by this workflow in DB2. Next, we
give DB2 queries corresponding to $W_n \cdots W_1$ of the A4-v2.
We obtain DB2 cost estimates for the rewrites provided by DB2. 
Next we obtain the rewrite $r^*$that our algorithm provides and 
get it costed using the DB2 cost model.
Hopefully, we can show using the DB2 cost model 
that $r^*$ is cheaper than its own rewrite.

Graph: DB2 optimizer estimated time units (y-axis) against 
DB2 rewrite and $r^*$ for A4-v2 (x-axis).
We may try to do it for all workflows,  A1 thru A8

{
\color{red}
\sout{
Graph2: It would also make sense to take care of ReStore early
on so that we do not have to keep comparing with it through
the rest of the section.} (as per Alkis's comments)
}
}

\item Weakness of $\ocost{}$ on the work efficiency of the
$\VF{}$.
Measure the total rewrites possible (P),
number of rewrites we explored (T),
number of rewrites explored that we should not have explored (E)
(y-axis) vs. three variants of $\ocost{}$ in x-axis.

P here denotes the complexity of a non-incremental algorithm,
T is the total work done by us, E is wasted work among T.

\item Graph on time taken to find $r^*$ (y-axis) vs.
{\em features} of the workflow. Features of the workflow include
$n$, number of joins, udfs etc.

Graph on time taken to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 
  
\item Graph on number of rewrites explored to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 

\item Compare our algorithm with diminished
versions of the algorithm.
Graph on estimated cost of $r^*$ (y-axis) vs. 
remove modules of the $\VF{}$ one by one.
For example, we could reduce the expressivity of $L_R$, joins etc.
This set of experiment will show the benefit of added complexity.\\

{\color{red}

Alkis says: ``I think that this should go first, so that the other experiments utilize the full-featured algorithm''

Response: OK
}

{\color{red}
\sout{We could handle ReStore here as one way of performing equivalent
rewrites}.
}
\end{enumerate}


{\em 
{\color{red}

Alkis: ``Do we know the theoretical complexity of our view-rewrite algorithm?''

Response: Our rough calculation is as follows.

The complexity of the $\WF{}$ is $O(n.l)$, where
$l$ is the number of samplings of the cost range $[0, \cost(W_n)]$.
$l$ can be chosen to be $n$ 
so that the $\WF{}$ algorithm is 
bounded by $O(n^2)$.

The $\VF{}$ is bounded by $O(|V|^{k_1} 2^{k_2})$ where 
$k_1$ represents the maximum number of candidates that
may be explored (generated + existing) by the $\VF{}$, 
while $k_2$ is a small constant 
representing the number of transformation rules in the system.
$k_1$ is bounded by $n$ as in the worse case $W_n$ may
contain $n-1$ joins.
Assuming all joins are of the same cost, the most expensive rewrite
for $W_n$ may contain up to $O(n)$ joins.
Hence, the complexity of the $\VF{}$ for a single target
is bounded by $O(|V|^n 2^{k_2})$.

The complexity of the entire algorithm is bounded by:
$O(n^2 + n \cdot |V|^n 2^{k_2})$, where $k_2 << |V|$.

}

\end{comment}

\begin{comment}
% SJ: Earlier version of the experiments that talked about rewrites etc. We will now
%     deal with RUNNING TIME OF THE algorithms
Secondly after the system has been in use for a few 
months, we show that the existing materialized views in 
the system can aid in rewriting workflows.
We evaluate the rewrites produced by our algorithm with 
increasing numbers of materialized views present in the system.
We retained about 4,800 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 scenarios and our microbenchmark.
This setup is intended to represent a mature system with many views 
left behind from previous execution runs.
Then we try to rewrite one analyst's workflow ($A_3v_1$) given
a random sampling of the existing views.
From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms (``BFR'' and ``DPR'') 
pruned from consideration views that cannot be used in a rewrite 
for a given target for the following reasons. 
A materialized view was pruned if it belonged to a different log, 
if it had a predicate condition that could not be removed,
or if it was a view previously created for any of Analyst3's workflows.
After pruning, the number of materialized views available for each target was
slightly more than 250.  
This experiment was performed ten times for each 
algorithm, and a scatter plot of the results are given in
Figure~\ref{fig-mv-vary-num-candidates}.


\twofig{fig-mv-vary-num-candidates}{fig-mv-vary-rewrites}
{Number of candidates considered (a) and the number of rewrites produced (b) (log-scale)}
{1.75in}

Figure~\ref{fig-mv-vary-num-candidates}(a) shows for each 
experiment performed, BFR creates several times fewer
candidate views.
Because BFR uses \ocost{}, 
it can avoid considering candidate views whose \ocost{}
is more expensive than $\cost(r^*)$.
Clearly the space of newly merged views is exponential in the worst case
as noted in~\cite{Agra2000}.  
These results show that BFR cannot escape this exponential space,
but typically results in creating and searching a smaller space than DPR approach.
Due to the known computational complexity of the problem, any solution that
avoids searching the entire space must resort to pruning which can result in sub-optimal rewrite.
Additional pruning could be applied to reduce the search space, 
but our algorithm will still find the best rewrite in the space it considers.

However, the larger benefit of BFR can be seen in 
Figure~\ref{fig-mv-vary-num-candidates}(b) 
which shows BFR is able to find $r^*$ by obtaining
far fewer rewrites than DPR in each case, and orders of magnitude fewer
for most cases.
The saving from (a) is primarily driven by how \emph{far} $r^*$ is into the space
in relation to the entire space, while the savings from (b)
is driven by \ocost{}'s ability to examine
more promising candidate views before less promising views.

%Furthermore, the more the views that exist, the more likely at least
%some of these will be useful for rewrites. 
%the faster \VF{} can find them, apply them, and terminate early
%by obtaining $r^*$ due to its incremental search behavior.
%we can examine candidates by the potential order of usefulness 
%(i.e. increasing optcost)
\end{comment}



==> old/Experimental_evaluation-rewrite3.tex <==
\section{Experimental Evaluation}\label{sec-experimental-evaluation}

\twofigrow{fig-we-novf-vs-vf-running-time}
{fig-we-novf-vs-vf-time-improvement}
{Query evolution comparisons for (a) query execution time (log-scale)
and (b) execution time improvement}{3in}

In this section, we present an experimental study we conducted in order to 
validate the effectiveness of $\WF{}$ in finding low-cost rewrites of complex queries. 
We first evaluate our methods in two scenarios.
The {\em query evolution} scenario (Section~\ref{sec-query-evolution}) represents a user 
iteratively refining queries within a single session.
This scenario evaluates the benefit that each new query version receives from the opportunistic
views created by previous versions of the query.
The {\em user evolution} scenario (Section~\ref{sec-experiments-ue}) represents a new user
  entering the system presenting a new query.
This scenario evaluates the benefit a new query receives from the opportunistic
views created by queries of other users.
We compare the performance of our algorithm for the user evolution scenario (Section~\ref{sec-scalability})
with a baseline dynamic programming approach
that searches at all targets without using $\ocost{}$.
Next, we evaluate the scalability  (Section~\ref{sec-scalability}) of our rewrite algorithm in comparison
to the dynamic programming approach.
We then compare our method to cache-based methods (Section~\ref{sec-experiments-restore}) 
 that can only reuse identical previous results.
Lastly, we show the performance of our method (Section~\ref{sec-experiments-storage-reclamation}) under a storage reclamation policy that drops opportunistic views.
% Lastly, as a sanity check (Section~\ref{sec-experiments-dbx}) we compare the quality of rewrites produced by our algorithm with a state-of-the-art  DBMS.


\subsection{Methodology}\label{sec-evaluation-setup}
% UDF is written in Hive, perl, python, MR but the transformation applied
% by the UDF is expressed in terms of a grammar that describes how an input
% attributes, filter and groupby properties are modified by the UDF.

Our experimental system consists of 20 machines running Hadoop.
We use HiveQL as the declarative query language, and Oozie as a
job coordinator.
UDFs are implemented in Java, Perl, and Python and executed
using the HiveCLI.
Some UDFs implemented in our system are log parser/extractor,
text sentiment classifier, sentence tokenizer, lat/lon extractor, 
word count, restaurant menu similarity, and geographical 
tiling, among others.



Our experiments use the following three real-world datasets totalling over 1TB:
a Twitter log containing 800GB of tweets, 
a Foursquare log containing 250GB of user check-ins, 
and a Landmark log containing 7GB of 5 million landmarks including their locations.
The identity of a social network user (\texttt{user\_id}) is common across
the Twitter and Foursquare logs, while the identity of a landmark
 (\texttt{location\_id}) is common across the Foursquare and Landmarks logs.


The metrics we report during evaluation of query performance are execution time in seconds
and the amount of data manipulated (read/write/shuffle) in GB. %, and the runtime of the rewrite algorithm in seconds.
For these experiments, \textsc{bfr} denotes  the use of our \WF{} algorithm and opportunistic views, 
while \textsc{no-bfr} represents execution time of the original query plan.
For the algorithm evaluations, \textsc{dpr} represents a dynamic programming approach
that does not use \ocost{} and searches for all rewrites at every target.
When comparing $\WF{}$ to the Dynamic Programming algorithm, we use the following metrics: running time to 
find the rewrite, the number of candidate views examined during the search for rewrites,
and the number of valid rewrites produced.
\textsc{dpr}  finds the best rewrite for each target and then identifies a subset 
 of these to obtain $r^*$ using a dynamic programming algorithm.
%We limit both algorithms from considering more than 
% $4$-way joins simply for practical reasons.


\subsection{Evolutionary Query Workload}\label{sec-evauation-query-scenarios}

Our test workload simulates 8 analysts who write complex queries containing 
UDFs, representing realistic marketing scenarios for restaurants.
%We derived these representative queries from extensive conversations with 
%business users on their typical analytics use cases.
 %, which are described in 
 %Table~\ref{tab-experiment-scenarios}.
Each analyst in our scenario creates 4 versions of a query, representing the query's evolutions
during data exploration and hypothesis testing.
We use these 32 queries for all of our evaluations.
%Each query version captures the analyst's iterative 
%...attempt  at bringing the query closer to her intended goal.
%refinements to the query during data exploration and hypothesis testing.
On average, the original plan of a query creates 17 opportunistic materialized views.

In the following set of experiments, $A_iv_j$ corresponds to the Analyst $i$ 
running version $j$ of her query.
We describe one Analyst's query in more depth using Example~\ref{ex-query-a2v2}, while
a detailed description of all 32 queries is in~\cite{lefe2013c}.

\begin{example}\label{ex-query-a2v2}
$A_2v_2$:
Find users with affluent friends that tweet 
positively about food, and visit a lot of pubs.


(a): EXTRACT from Foursquare log.
EXTRACT restaurant name from text.
FILTER by check-ins to wine places.
GROUPBY user, compute count.
Find MAX user check-in.
Compute check-in score for each user.

(b): EXTRACT user from Twitter log.
Compute FOOD-SENTIMENT score for each user.

(c): CLASSIFY user's tweets from Twitter log as affluent or not.
GROUPBY affluent users, compute affluent tweet count.
Find MAX count among all users.
COMPUTE an affluent score for each user.

(d): Create social network from Twitter log
using tweet source and dest.
GROUPBY user pair in social network, count tweets. 
Find MAX tweets between a user pair.
Assign friendship strength score to each user pair.

JOIN (a), (b), and (c) on user\_id.
Then JOIN with (d) based on friend\_id .
Threshold based on checkin score, food-sentiment score, 
friendship score, and affluent score.
\end{example}


\subsection{Experimental Results}


\threefig{fig-ue-novf-vs-vf-running-time}
{fig-ue-novf-vs-vf-data-moved}
{fig-ue-novf-vs-vf-time-improvement}
{User Evolution Comparisons for (a) query execution time (log-scale)(b) data moved
(c) execution time improvement}{2in}


\subsubsection{Query Evolution}\label{sec-query-evolution}

 
This section presents results for the query evolution scenario, where a user's 
new query can benefit from opportunistic views created during execution 
of previous versions of the query.
In this experiment, an analyst (e.g., $A_i$) executes the first version of his query (e.g., $A_iv_1$) 
followed by issuing each subsequent version 
(e.g., $A_iv_2$, $A_iv_3$, $A_iv_4$).
Subsequent versions of a query are rewritten 
given the benefit of all opportunistic materialized views from previous versions of the query.

Figure~\ref{fig-we-novf-vs-vf-running-time}(a) shows the performance of
the original query plan (\textsc{no-bfr} in graph) and 
the optimized query plan after rewriting with \WF{} (\textsc{bfr} in graph).
%This figure shows the execution time for each subsequent version of the query 
%is consistently lower when using  our method (\textsc{bfr}).
Figure~\ref{fig-we-novf-vs-vf-running-time}(b) shows the corresponding 
percent improvement in execution time for $\WF{}$ over the baseline 
original plan resulting from 10\% up to 90\% improvement, representing
an average improvement of 61\% and up to two orders of magnitude.
As a concrete data point, $A_5v_4$ requires 54 minutes to execute in the baseline system,
but only  55 seconds after $\WF{}$ finds a suitable rewrite.
The amount of data manipulated (i.e., read/write/shuffle bytes) closely followed the
same trend in Figure~\ref{fig-we-novf-vs-vf-running-time}(a).
% Data moved results are not reported here because later we present the results 
% showing similar data movement trends for the user evolution experiments in 
% Section~\ref{sec-experiments-ue}, 
%Figure~\ref{fig-ue-novf-vs-vf-running-time}(b).
The significant savings in execution time for $\WF{}$ 
can be attributed to moving much less data, 
and avoiding the costly re-extraction of data from raw logs whenever possible, 
due to our algorithm's ability to reuse prior computation from 
all previous query versions, i.e., opportunistic materialized views.
%These results show the benefit of our methods for the query evolution scenario,
%where a user benefits from opportunistic views created during execution
%of 

\subsubsection{User Evolution}\label{sec-experiments-ue}

This section presents results showing the benefit of our methods for the 
user evolution scenario, where a user benefits from opportunistic views 
created during execution of other user's queries.
In this scenario, a new analyst 
arrives and executes the first version of his query given that
all of the other analysts have previously executed their queries in the system.
Our \WF{} algorithm rewrites $A_iv_1$ using the opportunistic materialized 
views from all other analyst queries.

Figure~\ref{fig-ue-novf-vs-vf-running-time}(a) shows the query execution
time while Figure~\ref{fig-ue-novf-vs-vf-running-time}(b) shows the 
data manipulated (read/write/shuffle) for $\WF{}$ and the original plan.
The results demonstrate that query execution time is always lower 
with $\WF{}$, with a similar trend in the amount of data moved.
The percentage improvement in execution time is given in 
Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) where it can be
seen that our system results in an improvement of about 50\%--90\%.


\begin{table}[!h]
\caption{\label{fig-se-novf-vs-vf-time-improvement}
Improvement in execution time of $A_5v_3$ as more
analysts become present in the system}
\centering
\begin{tabular}{| p{2.45cm} | p{0.35cm}| p{0.45cm} | p{0.45cm}| p{0.45cm} | p{0.45cm}|  p{0.45cm} | p{0.45cm}|}
\hline
Analysts  in System & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\ \hline
Improvement    & 0\% & 73\% & 73\% & 75\% & 89\% & 89\% & 89\% \\ \hline
\end{tabular}
\vspace{-0.1in}
\end{table}

As an additional experiment, we show the increasing benefit a user may receive
each time a new analyst arrives and executes their queries.
To show this, first we execute $A_5v_3$ with no opportunistic views in the system,
to create a baseline execution time.
We ``add'' another analyst by executing all four versions of that
analyst's query, creating new opportunistic views. 
Then we re-execute $A_5v_3$ and report the performance 
improvement for  $A_5v_3$ over the baseline as new analysts are added.
We chose $A_5v_3$ as it is a complex query using all three logs. 
Table~\ref{fig-se-novf-vs-vf-time-improvement} reports the 
execution time improvement as analysts are added, 
showing an increasing benefit as more users are present in the system.
The benefit is obviously dependent on similarity to other
analysts' queries.


\subsubsection{Comparison of $\WF{}$ and DPR Algorithms}\label{sec-scalability}

\threefig{fig-ue-bfs-vs-dp-candidates-explored}
{fig-ue-bfs-vs-dp-refine-attempts}
{fig-ue-bfs-vs-dp-time-comparison}
{Algorithm Comparisons for
(a) Candidate views considered, (b) Refine attempts, and (c) Runtime (log-scale)}
{2.15in}

To evaluate the effectiveness of $\WF{}$ to prune the search space of rewrites, 
we compare it against the baseline {\sc dpr} algorithm that exhaustively 
searches the space in order to find the same minimum-cost rewrite. 
First we evaluate the algorithms during the user evolution experiments, 
where the only views in the system are those created by the other users.
This resulted in approximately 100 views for each user evolution experiment.
Next we evaluate the algorithm runtime as we vary the number of views in the system
from 1--1000 to show how the algorithms scale with an increasing number of views.

Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}
compares the performance of the $\WF{}$ and the dynamic programming algorithm ({\sc dpr} in graph)
% by measuring how much of
% the rewrite search space each algorithm explores 
during the user evolution experiment.
While both algorithms find the minimum-cost rewrite $r^*$, these
figures show that $\WF{}$ searches much less of the space to find the 
minimum cost rewrite than does {\sc dpr}.
Candidate views considered in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(a)
corresponds to all the existing views ($V$)  and those views created during 
the rewrite search process (i.e., merged views).
The number of rewrite attempts corresponds to the candidate views examined by
 $\RE{}$ when searching for a valid rewrite with low cost.
%As noted previously this process is computationally expensive.
These results show for many cases it is possible for $\WF{}$ 
to find $r^*$ by considering far fewer candidate views as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(a), 
and orders of magnitude fewer rewrites attempted as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(b),
resulting in significant savings in algorithm  runtime as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(c).
This savings is due to \WF{}'s use of $\ocost{}$ that enables
considering the promising candidate views earlier in the search,
and exploding the space of candidate views incrementally as needed.
% This shows our algorithm results in a significant reduction
% in the rewrite search space.

The next experiment evaluates the runtime performance of $\WF{}$ and 
\textsc{dpr} with an increasing number of materialized views in the system.
We retained about 9,600 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 Analyst scenarios.
% This setup is intended to represent a mature system with many opportunistic 
% views created by previous queries.
We use the $\WF{}$ and \textsc{dpr} algorithms to find rewrites for one 
analyst's query ($A_3v_1$) given a uniform random sampling of subsets of 
the existing 9,600 views to show how the algorithms scale with the number 
of materialized views in the system.
% From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms pruned views at a given target as follows:
a view was pruned if it did not reference the same log as the target,
if it had a predicate condition preventing it from being used in a rewrite for 
the target, or if it was a view that is identical to the target.
Identical views were removed because those do not help to test the scalability
of the algorithms.
After pruning, the number of materialized views available for each target was
slightly more than 1000.  
This experiment was performed many times for each algorithm at a given sample
size.


\onefig{fig-mv-vary-run-time}
{Runtime of $\WF{}$ and DPR for varying number of MVs in the system}{2.5in}

Figure~\ref{fig-mv-vary-run-time} shows the algorithm runtime
for increasing number of materialized views in the system.
\textsc{dpr} becomes prohibitively expensive even when 250 MVs
are present in the system.
$\WF{}$ on the other hand scales much better than \textsc{dpr} and has
a runtime under 1000 seconds even when the system has 1000  views relevant
to the given query. 
% The runtime of \textsc{bfr} may also be too expensive for systems 
% where the execution time of most queries is not more than a few tens of 
% seconds.
While this runtime is not trivial, we note that these are complex queries
involving UDFs that run for thousands of seconds.
%Note that these are complex queries involving UDFs that run for thousands
%of seconds.
The amount of time spent to rewrite the query plus the execution
time of the optimized query is far less than the execution time of unoptimized queries.
For instance, Figure~\ref{fig-ue-novf-vs-vf-running-time}(a) 
reports a query execution time of 451 seconds for $A_5$ optimized versus 
2134 seconds for unoptimized. 
Even if the rewrite time were 1000 seconds (in this case it is actually 3.1 seconds
as seen in Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(c)), 
the end-to-end execution time would be lower by 11 minutes or 32\%. 

However, additional pruning techniques~\cite{Agra2000} can 
be used to reduce the number of views, thereby reducing 
the algorithm search space.
We note that \WF{} will find the minimum cost rewrite in the space it considers.

\subsubsection{Comparison with Caching-based methods}\label{sec-experiments-restore}

Here we compare our approach against caching-based methods 
such as ReStore~\cite{Elgh2012} that only reuse identical answers (i.e.,
existing views that require no compensation).
%i.e., answers generated by identical plans.
Figure~\ref{fig-restore-comparison-execution-improvement} shows the 
query execution time improvements for query evolution of Analyst 1.
The results show that both $\WF{}$ and ReStore are identical for $A_1v_2$, while
ReStore is worse than $\WF{}$ for $A_1v_2$ and significantly worse for $A_1v_3$.
Reusing cached results can  clearly be effective.
However, performance is highly dependent upon the presence of identical 
answers previously generated in the system as cache methods lack
a robust capability to reuse previous results.

\onefig{fig-restore-comparison-execution-improvement}
{Execution time improvement for query evolution using $\WF{}$ 
  and ReStore}{2in}

\begin{table}[h!]
\caption{\label{fig-re-novf-vs-vf-time-improvement}
Improvement in execution time of user evolution using $\WF{}$ without identical views}
{\small
\centering
\begin{tabular}{| p{1.5cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}|p{0.40cm} | p{0.40cm}| p{0.40cm} | p{0.40cm}|}
\hline
Analyst & $A_1$ & $A_2$ & $A_3$ & $A_4$ & $A_5$ & $A_6$ & $A_7$ & $A_8$ \\ \hline
%BFR(with) & 57\% & 64\% & 86\% & 85\% & 78\% & 98\% & 88\% & 84\% \\ \hline
$\WF{}$ & 57\% & 64\% & 83\% & 85\% & 51\% & 96\% & 88\% & 84\% \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}

To illustrate the robustness of our rewrite algorithm beyond caching-based
methods, we present an experiment where we prune away all identical views from 
the solution space.
Removing all identical views represents the worst-case scenario for 
caching-based methods.
Such methods will not be able to find \textit{any} rewrites, resulting in 0\% improvement. 
%caching-based methods are not nearly as effective as our approach.
Table~\ref{fig-re-novf-vs-vf-time-improvement}
reports the percentage improvement using \WF{} when identical views 
have been pruned from consideration.
Our algorithm results in very good performance improvement, and these results 
are comparable to the results in Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) 
that represents the same experiment without pruning identical views.
Table~\ref{fig-re-novf-vs-vf-time-improvement} shows a performance 
drop for $A_5$ compared to the results reported in 
Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) for $A_5$. 
This is because $A_5$ had previously benefited from an identical view corresponding
to restaurant similarity which it has to recompute.
Note that identical views constituted only 7\% of  the view storage space in 
this experiment.
Given that analysts pose different but related queries in an evolutionary scenario,
any method that relies solely on identical matching can have limited benefit.



\subsubsection{Storage Reclamation}\label{sec-experiments-storage-reclamation}

\begin{table}
\caption{\label{fig-ga-improvement-vs-storage-reclaimed}
Execution Time Improvement after reclaiming 10\% to 90\% of the 
view storage space}
{\small
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Reclaimed Storage & $10\%$ & $20\%$ & $30\%$ & $50\%$ & $70\%$ &$90\%$\\ \hline
Improvement & 89\% & 88\% & 86\% & 82\% & 58\% & 30\% \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}

Since storage is not infinite a reclamation policy is necessary.
We demonstrate the robustness of our approach using unsophisticated 
policies, since reclamation is not the focus of this work.
The first simple policy randomly drops views to reclaim 10\%--90\% 
of the view storage space.
%As a baseline, we execute the before dropping any views.
After each reclamation, we run the $A_5v_3$ query 
(used in Section~\ref{sec-experiments-ue})
after applying our rewrite algorithm, and 
compare it to a baseline without our rewrite algorithm.
%and report the percentage improvement in execution time over the baseline
%of \textsc{no-bfr}.
Each test is repeated twice (different randomizations).
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
reports the average execution time improvement for $A_5v_3$ after reclaiming
 various amounts of storage space. % randomly.
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
shows that our system is able to find good rewrites for $A_5v_3$ using the 
remaining views available,
%even when much of the storage space is reclaimed.
until most of the storage space is reclaimed.

Second, Table~\ref{fig-re-novf-vs-vf-time-improvement} provides another perspective 
on how storage reclamation can affect the effectiveness of $\WF{}$. 
Specifically, we observe that $\WF{}$ is able to find good rewrites 
even if the optimal views for each query are removed. 
These results suggest that our approach is robust to ``bad'' 
choices made by the reclamation policy, provided some good views remain in the system.\looseness=-1 
% The best views are those with the ability produce a low cost rewrite, 
% thus such a policy would drop any view that is identical to a target in the plan.
% Table~\ref{fig-re-novf-vs-vf-time-improvement} directly captures the 
% performance of our algorithm given an adversarial policy, showing our 
% algorithm maintains good performance.
% This shows the robustness of our system even with a bad storage reclamation 
% policy that drops all of the best views.
% Best refers to those views that have maximum benefit 
% with lowest cost, 
%, although in the current work we do not consider maintenance cost.
%
% which is exactly the effect measured by the previous experiment
% where our approach shows only slight performance loss after
% dropping the identical views.
% Taken together, the previous two experiments show the
% robustness of our system and rewrite algorithm.

The hardness of designing a good policy is equivalent to the view selection 
problem with a storage constraint.
Certainly better methods~\cite{Mami2012} could be applied but we 
leave this for future work.

\begin{comment}
\subsubsection{Comparison with DB-X}\label{sec-experiments-dbx}

To verify that our system produces good rewrites, we compared our rewrites
to those of a widely-used commercial database system (DB-X)
using data from the TPC-H~\cite{tpcds} benchmark.
DB-X was tuned to its highest optimization level as well as
set to consider all views for query rewriting.
We created two materialized views on the {\tt LINEITEM} table:
group-by--count on {\tt L\_ORDERKEY, L\_SUPPKEY},
and group-by--count on {\tt L\_ORDERKEY, L\_PARTKEY}.
% Our goal was to verify  the rewrites produced by $\WF{}$
% were not significantly worse than those produced by DB-X.
To test the rewrites produced by both systems,
 we use three queries on the {\tt LINEITEM} table:
a) groupby on {\tt L\_ORDERKEY, L\_SUPPKEY, L\_PARTKEY}
b) group-by on {\tt L\_ORDERKEY} with count aggregate, and
c) group-by on {\tt L\_ORDERKEY} with count and max aggregate
on {\tt L\_SUPPKEY}.
The resulting rewrites were given to the DB-X query optimizer,
which provided a cost estimate for each rewrite.

$\WF{}$ made use of both materialized views for the first query while
DB-X did not make use of them which resulted in a rewrite
that was 3$\times$ worse than the rewrite produced by $\WF$.
For the second query both $\WF{}$ and DB-X resulted in identical
rewrites.
For the third query, DB-X did not make use of a materialized view,
whereas $\WF{}$ did resulting in a 5$\times$ improvement over DB-X.
% Our sanity check experiment shows that our rewrite algorithm 
% produces rewrites that are competitive to a state of the art commercial system.
$\WF{}$ produces rewrites competitive to a state-of-the-art commercial DBMS on queries that 
are much simpler than our setup. Using the DBMS to rewrite the complex 
queries in our workload would most likely result in very little improvement. 
\end{comment}


\begin{comment}
\subsubsection{Garbage Collection}

Next how garbage collection does not result in significant loss
of performance. 

Next we briefly consider the effects garbage collection on 
our algorithm performance and workflow execution time.
Garbage collection can be applied to recover storage space
or to reduce the runtime of the rewriting algorithm.
Figure~\ref{fig-mv-vary-num-candidates}(a) shows the space of
candidate views is exponential, thus arguing to keep the
number of views lower.  
Figure~\ref{fig-mv-vary-num-candidates}(b) shows that even 
for higher numbers of available views randomly 'retained' 
among all available views, our algorithm 
only needs to find very few rewrites to obtain $r^*$.

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%% End of File

\begin{comment}
\begin{enumerate}

\item Analyst1 wants to find influential users who are
interested in food with the goal that
these users could be target of a future advertisement campaign.
The evolution of this scenario will propose increasingly
sophisticated interpretations of what it means to be ``influential''.

\item Analyst2 wants to identity 100 wine lovers so that he can 
send them a coupon for a new wine being introduced in the market. 
The evolution of this scenario will investigate 
increasingly sophisticated ways of finding out if a user is a ``wine lover''.

\item Analyst3 wants to start a birthday gift recommendation service where friends
can send a gift certificate to a user $u$ who's birthday is around the corner.
We want to generate 5 restaurant choices based on $u$'s preferences and alert
$u$'s friends to $u$'s upcoming birthday and offer them a choice
of discount certificates to the 5 restaurants.
The evolution in this scenario will investigate how to determine
if a user likes a restaurant enough to visit it on his birthday,
how to suggest a diverse set of recommendations as well as
how to suggest restaurants that would cater to $u$'s close set of friends.

\item Analyst4 wants to provide restaurants with a breakdown of their
customer population. 
In particular, the analyst wants to provide breakdowns in terms of who goes to a
particular restaurant.
The analyst may also want to perform analysis in terms for geographical area.
For instance, for any area which are the popular restaurants by categories etc.
The goal of this scenario is to perform increasingly complicated analytical 
operations on the log.

\item Analyst5 wants give restaurant owners a poaching tool in the 
the following sense.
For each restaurant $r$, we identify customers who go to a ``similar'' 
restaurant in the area but do not visit $r$.
Using the list, the owner of $r$ may send these customers a coupon.
The evolutionary nature of the problem is to find out how to determine
``similar'' restaurants.

\item Analyst6 tries to find out if restaurants are losing their
loyal customers.
In other words, we want to identify those customers 
who used to visit frequently but now slowly
stopped visiting the restaurant, but are still visiting other restaurants in the area.
The restaurant owner can send them a coupon to win them back.
The evolutionary nature of this scenario will focus on 
how to identify prior active users.

\item Analyst7 wants to go by the maxim in business that problems should be caught
as soon as possible. 
For each restaurant in the system, try to identify common problems that
users have reported about the restaurant.
For example, have customers complained about food, service, issues with premises etc.
Moreover, if there is a successful restaurant of the same category, 
what makes it successful.
The evolutionary nature of this scenario will focus on compiling
issues under different categories.

\item Analyst8 wants to identity what category (i.e., american, indian,
chinese, steak) of restaurants is missing from a
certain region. For example, one of the outcome can be that 
Cupertino could really use a Moroccan restaurant. 
The evolutionary nature of this scenario will focus on how to 
find out if there is a need for a good restaurant in a certain
category and if so what is the nature of their clientele etc.

The use-case for our system that it is being used internally
by analysts who work for restaurant marketing company that gets commission
from sending users to restaurants or providing restaurant 
owners analytics support to aid them in their business decisions.
Each analyst starts out with a single log file and expanding
to all the three log files during the course of their
evolutionary workflow.
{\it The idea here is not to get too carried away by the quality
of the answers we get but write workflow structures that capture
the spirit of these scenarios.}


\end{itemize}


The desirable property of the $\cost{}$ is that it must be cheap to compute.
Since a full query optimizer may be too expensive, we use a model of a query optimizer.
We treat this model as a black box, in this way $\RE{}$ and $\ocost{}$ can
utilize any functionality provided by the model or improvements to the model.
%For an RDBMS, a cost model such as in~\cite{x,y} could be used.  
%Because we evaluate our framework in a MapReduce execution system, 

Our cost model is based on the one in~\cite{Nyki2010}, 
which reduces a query $q$ to a set of $m$ jobs $\{J_1, \cdots, J_m\}$. 
The cost of each job is expressed as a linear combination of 
the cost to read the data ($C_{r}$)
the cost of sorting and copying ($C_{s}$),
the cost to transfer data ($C_{t}$).
and the cost to write the output of the job ($C_{w}$).

\begin{equation} \label{eq-cost}
\cost(q,v) = \sum_{i=1}^{m} C_{r}(J_i,v_i) +  C_{s}(J_i,v_i) +  C_{t}(J_i,v_i) +  C_{w}(J_i,v_i)
\end{equation}
where $v_1 = v$, and $v_{i}$ forms the input of $J_i$.

               
To keep the $\cost{}$ function inexpensive, our model does not consider re-ordering 
of joins, predicate push down, or other types of optimizations involved in 
group bys and udfs, but does merge sequential operations (e.g. a sequence of filters)
into the same job whenever possible.


This is a reasonable approach given that we have already committed to creating $v$,
and the $\RE{}$ explores all possible rewrites, such a cost function serves
our purposes here.  

An extension to this basic cost model could consider push downs when computing the cost
to create $v$.  The requirements to including push-downs into the optimization
process would be to employ a cost model $\cost{}$ that is able to 
apply all possible join orderings to creating $v$ along with applying filters 
to all orders.  

Appendix~\ref{appendix-pushdown} provides a proof for using $\RE{}$ and $\ocost$ with an extended 
$\cost{}$ function that considers join ordering and predicate pushdowns,
while still producing a correct lower bound for $\RE{(v,q)}$.

There are 2 reasons we do not consider predicate push downs here.
First $\cost{}$ becomes much more expensive to invoke due to considering all 
of the ordering options. 
Second, we may not wish to push down a filter into $v$ since this could render $v$ 
less useful for answering future queries.  
A more sophisticated algorithm could weigh the cost and benefits of different 
versions of $v$ (with and without filters) given their benefit to other queries 
and their added cost due to avoiding filter push downs.

\subsubsection{Comparison with DB2 and ReStore:}

Show that our $\VF{}$ performs better rewrites compared to 
the DB2 design advisor.
We also need to emphasize that there is a significant ETL time with DB2
which we will not consider for this experiment.

{\em Run the workflow A4-v1 and store the MVs of all targets
  produced by this workflow in DB2. Next, we
give DB2 queries corresponding to $W_n \cdots W_1$ of the A4-v2.
We obtain DB2 cost estimates for the rewrites provided by DB2. 
Next we obtain the rewrite $r^*$that our algorithm provides and 
get it costed using the DB2 cost model.
Hopefully, we can show using the DB2 cost model 
that $r^*$ is cheaper than its own rewrite.

Graph: DB2 optimizer estimated time units (y-axis) against 
DB2 rewrite and $r^*$ for A4-v2 (x-axis).
We may try to do it for all workflows,  A1 thru A8

{
\color{red}
\sout{
Graph2: It would also make sense to take care of ReStore early
on so that we do not have to keep comparing with it through
the rest of the section.} (as per Alkis's comments)
}
}

\item Weakness of $\ocost{}$ on the work efficiency of the
$\VF{}$.
Measure the total rewrites possible (P),
number of rewrites we explored (T),
number of rewrites explored that we should not have explored (E)
(y-axis) vs. three variants of $\ocost{}$ in x-axis.

P here denotes the complexity of a non-incremental algorithm,
T is the total work done by us, E is wasted work among T.

\item Graph on time taken to find $r^*$ (y-axis) vs.
{\em features} of the workflow. Features of the workflow include
$n$, number of joins, udfs etc.

Graph on time taken to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 
  
\item Graph on number of rewrites explored to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 

\item Compare our algorithm with diminished
versions of the algorithm.
Graph on estimated cost of $r^*$ (y-axis) vs. 
remove modules of the $\VF{}$ one by one.
For example, we could reduce the expressivity of $L_R$, joins etc.
This set of experiment will show the benefit of added complexity.\\

{\color{red}

Alkis says: ``I think that this should go first, so that the other experiments utilize the full-featured algorithm''

Response: OK
}

{\color{red}
\sout{We could handle ReStore here as one way of performing equivalent
rewrites}.
}
\end{enumerate}


{\em 
{\color{red}

Alkis: ``Do we know the theoretical complexity of our view-rewrite algorithm?''

Response: Our rough calculation is as follows.

The complexity of the $\WF{}$ is $O(n.l)$, where
$l$ is the number of samplings of the cost range $[0, \cost(W_n)]$.
$l$ can be chosen to be $n$ 
so that the $\WF{}$ algorithm is 
bounded by $O(n^2)$.

The $\VF{}$ is bounded by $O(|V|^{k_1} 2^{k_2})$ where 
$k_1$ represents the maximum number of candidates that
may be explored (generated + existing) by the $\VF{}$, 
while $k_2$ is a small constant 
representing the number of transformation rules in the system.
$k_1$ is bounded by $n$ as in the worse case $W_n$ may
contain $n-1$ joins.
Assuming all joins are of the same cost, the most expensive rewrite
for $W_n$ may contain up to $O(n)$ joins.
Hence, the complexity of the $\VF{}$ for a single target
is bounded by $O(|V|^n 2^{k_2})$.

The complexity of the entire algorithm is bounded by:
$O(n^2 + n \cdot |V|^n 2^{k_2})$, where $k_2 << |V|$.

}

\end{comment}

\begin{comment}
% SJ: Earlier version of the experiments that talked about rewrites etc. We will now
%     deal with RUNNING TIME OF THE algorithms
Secondly after the system has been in use for a few 
months, we show that the existing materialized views in 
the system can aid in rewriting workflows.
We evaluate the rewrites produced by our algorithm with 
increasing numbers of materialized views present in the system.
We retained about 4,800 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 scenarios and our microbenchmark.
This setup is intended to represent a mature system with many views 
left behind from previous execution runs.
Then we try to rewrite one analyst's workflow ($A_3v_1$) given
a random sampling of the existing views.
From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms (``BFR'' and ``DPR'') 
pruned from consideration views that cannot be used in a rewrite 
for a given target for the following reasons. 
A materialized view was pruned if it belonged to a different log, 
if it had a predicate condition that could not be removed,
or if it was a view previously created for any of Analyst3's workflows.
After pruning, the number of materialized views available for each target was
slightly more than 250.  
This experiment was performed ten times for each 
algorithm, and a scatter plot of the results are given in
Figure~\ref{fig-mv-vary-num-candidates}.


\twofig{fig-mv-vary-num-candidates}{fig-mv-vary-rewrites}
{Number of candidates considered (a) and the number of rewrites produced (b) (log-scale)}
{1.75in}

Figure~\ref{fig-mv-vary-num-candidates}(a) shows for each 
experiment performed, BFR creates several times fewer
candidate views.
Because BFR uses \ocost{}, 
it can avoid considering candidate views whose \ocost{}
is more expensive than $\cost(r^*)$.
Clearly the space of newly merged views is exponential in the worst case
as noted in~\cite{Agra2000}.  
These results show that BFR cannot escape this exponential space,
but typically results in creating and searching a smaller space than DPR approach.
Due to the known computational complexity of the problem, any solution that
avoids searching the entire space must resort to pruning which can result in sub-optimal rewrite.
Additional pruning could be applied to reduce the search space, 
but our algorithm will still find the best rewrite in the space it considers.

However, the larger benefit of BFR can be seen in 
Figure~\ref{fig-mv-vary-num-candidates}(b) 
which shows BFR is able to find $r^*$ by obtaining
far fewer rewrites than DPR in each case, and orders of magnitude fewer
for most cases.
The saving from (a) is primarily driven by how \emph{far} $r^*$ is into the space
in relation to the entire space, while the savings from (b)
is driven by \ocost{}'s ability to examine
more promising candidate views before less promising views.

%Furthermore, the more the views that exist, the more likely at least
%some of these will be useful for rewrites. 
%the faster \VF{} can find them, apply them, and terminate early
%by obtaining $r^*$ due to its incremental search behavior.
%we can examine candidates by the potential order of usefulness 
%(i.e. increasing optcost)
\end{comment}



==> old/Experimental_evaluation.tex <==
\section{Experimental Evaluation}\label{sec-experimental-evaluation}

In the following experiments we show the performance
of our system using real social media data and evolutionary queries.
Due to the log nature of the data, the need for data exploration
and the types of analytical functions which can include complex
UDFs, an analyst has significant freedom in revising versions 
of the same workflow.
First, we formally capture the revision \emph{expressions} in our evaluation using 
a microbenchmark that we present here.
Second, we present a microbenchmark that is intended to highlight common types
of revisions that a real analyst would perform.
Third, we evaluate three scenarios:
a) {\em workflow evolution} where 
a user may get benefit from previous version of his workflow,
b) {\em user evolution} where
a new user in the system may get benefit from other users' workflows.
c) {\em system evolution} where a new analyst may get increasing
benefit as the system matures.
We show results for these cases using workflow execution time, 
data moved (bytes),
and percent improvement in execution time of the rewritten workflow compared to
the original workflow. 
Fourth, we show that good rewrites are found even 
when identical materialized views are excluded from
consideration thus showing the advantages of our method compared to
those which only use cached results.
Fifth, we compare our rewrite with those of a state of the art
commercial database system.
Lastly, since storage is not infinite we evaluate the robustness of our rewrite 
algorithm given a view storage reclamation policy.

\subsection{Setup}
% UDF is written in Hive, perl, python, MR but the transformation applied
% by the UDF is expressed in terms of a grammar that describes how an input
% attributes, filter and groupby properties are modified by the UDF.

Our evaluation setup consists of 20 machines running
Hadoop, Hive/Pig, and Oozie.
Our UDFs are implemented in several languages 
such as SQL, Java, Perl and Python.
Some UDFs implemented in our system beyond
basic SQL operators are
text sentiment, sentence tokenizer, lat/lng extractor, 
word count, restaurant menu similarity, and geographical 
tiling, among others.
The workflows are checked against the grammar of the UDFs.
Next, we check data dependencies after which
we parallelize the given workflow based on its 
dependency graph structure.
We then convert this to a Oozie workflow 
which serves as an execution coordinator.
The Oozie workflow nodes are executed on Hive~\cite{Thus2009}
or Hive-CLI for those UDFs that are not expressible by 
HiveQL (e.g., Perl UDFs).

We evaluate our system using three logs totaling over 1TB.
A Twitter log containing 800GB of tweets, 
a Foursquare log containing 250GB of user check-ins, 
and Landmark log containing 7GB of 5 million landmarks including their locations.
The identity of a social network user (\texttt{user\_id}) is common across
the Twitter and Foursquare logs, while
the identity of a landmark (\texttt{location\_id}) 
is common across the Foursquare and Landmarks logs.

Hive currently lacks a mature query optimizer
and a {\em what-if} optimizer functionality to obtain cost
estimates for hypothetical configurations.
Additionally, it cannot consider 
UDFs and their costs properly.
For these reasons, we employ the cost model 
developed for M/R frameworks in~\cite{Nyki2010}
that considers basic data statistics, number of map/reduce 
tasks, and number of jobs.

\subsection{Evolutionary Workflow Scenarios}

The evaluation consists of 8 analysts that write workflows
related to marketing scenarios involving restaurants,
which are described in Table~\ref{tab-experiment-scenarios}.
Each analyst's exploration
consists of 4 evolutionary versions.
Each workflow version captures the analyst's iterative attempt in bringing the
workflow closer to his intended goal.
In the following set of experiments, $A_iv_j$
corresponds to the Analyst $i$ running version $j$ 
of his evolutionary workflow.
We give a high-level description of these workflows in 
Table~\ref{tab-experiment-scenarios} left column, and 
describe one workflow ($A_2v_2$) in Example~\ref{ex-query-a2v2}.
% we will provide all 
%queries as a first step towards a benchmark for evolutionary queries.
We use these 32 workflows in our evaluation, and will provide
them in a subsequent publication.

\begin{example}\label{ex-query-a2v2}
$A_2v_2$:
Find users with affluent friends that tweet 
positively about food, and visit a lot of pubs.

$G_1$: EXTRACT from Foursquare log.
EXTRACT restaurant name from text.
FILTER by check-ins to wine places.
GROUPBY user, compute count.
Find MAX user check-in.
Compute check-in score for each user.

$G_2$: EXTRACT user from Twitter log.
Compute FOOD-SENTIMENT score for each user.

$G_3$: CLASSIFY user's tweets from Twitter log as affluent or not.
GROUPBY affluent users, compute affluent tweet count.
Find MAX count among all users.
COMPUTE an affluent score for each user.

$G_4$: Create social network from Twitter log
using tweet source and dest.
GROUPBY user pair in social network, count tweets. 
Find MAX tweets between a user pair.
Assign friendship strength score to each user pair.

JOIN subgoals $G_1$, $G_2$, and $G_3$ based on user\_id .
JOIN with $G_4$ based on friend\_id .
Threshold based on checkin score, food-sentiment score, 
friendship score, and affluent score.
\end{example}

NO-WFR represents the original execution time
without rewrite, while WFR represents the execution time
after rewrite using $\WF$ and
DPR represents the bottom-up approach that does not make use of \ocost{}.
DPR finds the best rewrite
for each target and then identifies a subset of these to obtain $r^*$ 
using a dynamic programming algorithm.
Furthermore we limit both algorithms from considering more than
$n$-way joins, where we limit $n=4$ simply for practical reasons.

\subsection{Results}

\onefig{fig-slug-illustration}
{Dimensions of change between workflow versions}{2.2in}

\subsubsection{Microbenchmark}

Given the evolutionary nature of our workflow scenarios, we 
capture the changes across the versions by defining and presenting
a {\em micro-benchmark} for the set of evolutionary 
queries evaluated here.

 (P) Parameters: While keeping the structure of the workflow unchanged, 
the parameters of the operations are modified to allow for 
more or less tuples in the results (Figure~\ref{fig-slug-illustration}P).
For example, the analyst may alter a select predicate or a top-k value to allow more
or less data in the output.
Here we evaluate the effect of changing the parameters of the workflow while
keeping the same structure.

 (L) Logs: An analyst may augment a workflow with 
a new log to obtain richer results (Figure~\ref{fig-slug-illustration}L).
Here we evaluate the effect of adding a new log to a workflow.

 (U) UDFs: An analyst may replace a set of operations in the 
workflow with a specialized UDF (Figure~\ref{fig-slug-illustration}U).
The analyst can also add a new UDF to the system which contributes
to the divergence of $L_W$ from $L_R$.
Here we evaluate the effect of replacing possibly multiple
operations with a UDF.

 (G) Sub-Goal Workflows: An analyst writes several sub-workflows
that each achieves a single goal and then joins these to obtain 
the final output (Figure~\ref{fig-slug-illustration}G).
This workflow structure has the benefit that parameters of each sub-goal
can be evolved as in Figure~\ref{fig-slug-illustration}P.
Here we evaluate the effect of adding or removing subgoals from the workflow.

These four dimensions \{P,L,U,G\} inform the 
changes between one workflow version and the next. 

\onefig{fig-mb-execution-time-comparison}
{Microbenchmark results showing execution time}{2.35in}

\twofigrow{fig-we-novf-vs-vf-running-time}
{fig-we-novf-vs-vf-time-improvement}
{Workflow Evolution Comparisons for (a) workflow execution time (log-scale)
and (b) execution time improvement}{3in}

Our microbenchmark starts with a set of simple initial workflows
$P_0, L_0, U_0, G_0$, each representing one of the PLUG dimensions.
Within each dimension, 2-3 evolved 
versions of the initial workflow are evaluated.
Each evolution captures one case of a rewrite-friendly 
change and another case that is not.
The rewrites are restricted to using only the original workflow
(e.g., $P_0$).
The different dimensions and their 
evolutions are meant to show the variations across 
the dimensions as well as variations within a dimension.
Figure~\ref{fig-mb-execution-time-comparison} 
presents the results of the microbenchmark 
experiments, where the y-axis shows the workflow
execution time in seconds and x-axis shows the workflows and their
evolutions.

$P_0$ performs extract, a simple groupby and then a select operation.
$P_1$ modifies $P_0$ by altering the select predicate,
while $P_2$ alters the groupby.
Both changes result in more tuples being output compared to $P_0$.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
$P_1$ is more conducive to rewrite because the rewrite 
is able to use the output from the groupby in $P_0$, while
$P_2$ had to recompute the groupby thus could not benefit
much from $P_0$.
$P$ represents a dimension where
the structure of the workflow remains the same 
while the parameters are varied.
Depending on the nature of the change to $P$,
one can expect opportunities for rewrite using MVs from $P_0$.

$G_0$ contains a single sub-goal.
$G_1$ adds a sub-goal with some commonality with the sub-goal in $G_0$,
while $G_2$ adds a sub-goal that has nothing
in common with $G_0$.
Both changes resulted in a richer answer compared to $G_0$.
$G$ represents a dimension where there is an opportunity
of reusing the entire original subgoal.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
depending on the similarities between the
newly added subgoal $G_1$ and the original $G_0$,
there can be ample opportunities for rewrite 
of the new subgoal using MVs from $G_0$.

$U_0$ contains extract, select, group and project.
$U_1$ replaces the select in $U_0$ with a UDF that is in $L_R$, 
$U_2$ replaces the select in $U_0$ with a UDF that is not in $L_R$, 
$U_3$ replaces the select in $U_0$ with the same UDF that is not in $L_R$.
$U_1$ and $U_3$ place the UDF before
the groupby in $U_0$ while $U_2$ places the UDF after the groupby.
Since the UDF in $U_1$ is in $L_R$, there are opportunities
for rewrite of both the UDF and the groupby from $U_0$.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
 when the UDF is not in $L_R$,
the rewrite becomes sensitive to its position in the workflow.
Thus, due to $U_2$'s position it could reuse 
the groupby in $U_0$, while $U_3$ could not.
$U$ represents a dimension
where UDFs offer opportunities for rewrite if they are in $L_R$,
otherwise the rewrite is sensitive to their position in the workflow.

$L_0$ contains extract, select, project, groupby on a 
single log $l_a$.
$L_1$ replaces $l_a$ with a $2\times$ larger log $l_b$, while
$L_2$ uses both the logs by applying
extract, select, project, groupby on $l_b$
and then joins the result with an extract of $l_a$.
Both changes resulted in a richer answer compared to $L_0$.
Figure~\ref{fig-mb-execution-time-comparison} shows that 
$L$ represents a dimension where there 
may not be opportunities for rewrite 
using the original workflow, unless one log subsumes the other.

Even though the microbenchmark examines the effect
of changing one dimension at a time, in a normal 
use-case the analyst may vary many of the dimensions at 
the same time.  
Table~\ref{tab-experiment-scenarios} right column 
captures the PLUG changes
made from the original workflow $W$ to each of the subsequent
revisions.
For instance, using the PLUG microbenchmark Analyst2's workflow
evolution is be described as:
\begin{center}
$W \rightarrow \{L,G,P\} \rightarrow \{G,P\} \rightarrow \{U,G,P\}$
\end{center}

The analyst begins with initial workflow $W$ (i.e., $A_2v_1$)
then adds a log $L$, modifies sub-goals $G$ and structure parameters $P$ 
to obtain version 2 (i.e., $A_2v_2$), and so on.
The ordering $\{L,G,P\}$ indicates the $L$ dimension 
likely affects the rewrites more than $\{G,P\}$.

\subsubsection{Workflow Evolution}

\threefig{fig-ue-novf-vs-vf-running-time}
{fig-ue-novf-vs-vf-data-moved}
{fig-ue-novf-vs-vf-time-improvement}
{User Evolution Comparisons for (a) workflow execution time (log-scale)(b) data moved
(c) execution time improvement}{2.15in}

% \threefig{fig-we-novf-vs-vf-running-time}
% {fig-we-novf-vs-vf-data-moved}
% {fig-we-novf-vs-vf-time-improvement}
% {Workflow Evolution Comparisons showing (a) execution time (b) data moved
% (c) percentage improvement}{2.2in}
 
Here we present results for the workflow evolution scenario, 
where an analyst $A_i$ executes
the first version of his workflow (e.g., $A_iv_1$) and
follows by posing the subsequent versions (e.g., $A_iv_2$).
Each subsequent version is rewritten given the existence of all 
materialized views created from executing the previous versions.

Figure~\ref{fig-we-novf-vs-vf-running-time}(a) shows the performance of
the rewritten workflow versus the original workflow and 
Figure~\ref{fig-we-novf-vs-vf-running-time}(b) shows the percentage
improvement in workflow execution time.
These figures show that the execution time is always lower for the rewritten
workflow.
Figure~\ref{fig-we-novf-vs-vf-running-time}(b) shows
an execution time improvement of at least 10\%, and up to 90\%.
The amount of data moved (i.e., read/write/shuffle) closely followed the trend
in Figure~\ref{fig-we-novf-vs-vf-running-time}(a).
The data moved results are not reported here
but we present the result for the user evolution case in Section~\ref{sec-experiments-ue}.
The significant savings in execution time can be attributed to moving much less data,
not having to re-ETL the raw logs whenever possible, 
and the ability of WFR{} to reuse and repurpose prior computation from all previous workflow versions.
These results show the benefit of rewriting workflows as well as 
our algorithm's ability  to take advantage of MVs from previous versions 
in the workflow evolution scenario.

While both WFR and DPR produce the optimal workflow rewrite $r^*$,
our WFR algorithm searches a considerably
smaller amount of space and attempts far fewer rewrites 
compared to the DPR algorithm.
We do not present these results here, but show this comparison
next for the user evolution experiments where the search space is 
larger due to the presence of many more materialized views.


\begin{comment}
Next we compare the space searched by both algorithms.
While both WFR and DPR produce the optimal workflow rewrite $r^*$,
it can be seen from Figure~\ref{fig-bfs-vs-dp-merge-attempts}
 that WFR algorithm searches a considerably
smaller amount of space and attempts far fewer rewrites 
compared to the DPR algorithm.
Recall the search for $r^*$ requires examining an exponential space of candidate views
in the worse case.
This search includes all of the existing candidate views and all of the 
views created as part of the rewrite search process (i.e., merged views).
The number of rewrite attempts corresponds to the views guessed to be
complete that we encounter during our search process, which are given to $\RE{}$
to attempt to find a rewrite.
As noted previously this process is computationally expensive.
Notice in most cases our algorithm attempts far fewer rewrites, thus
avoiding that expense.
This is due to our algorithms use of $\ocost{}$ that examines the promising
candidate views earlier.
Our results show for most cases it is possible to 
find $r^*$ by considering far fewer candidates
views in Figure~\ref{fig-bfs-vs-dp-merge-attempts}(a) and
orders of magnitude fewer
rewrites in Figure~\ref{fig-bfs-vs-dp-merge-attempts}(b).

Notice in the worst case our algorithm degenerates into 
the DPR approach when a rewrite does not exist or $r^*$ 
is really expensive, requiring both algorithms to 
examine a large part of the space.
This can be seen in $A_4v_2$, $A_5v_2$, and $A_7v_2$.
It is worthwhile to note that these three cases involved UDFs
that were not part of $L_R$.
From microbenchmark $U_2$ and $U_3$ we saw that UDF rewrites are sensitive
to the position of the UDF in the workflow, especially
those that are not in $L_R$.
Interestingly this only happens in version 2 where the materialized
views that exist are only those from version 1.
But it can be seen that our algorithm does much better for all subsequent iterations
(versions 3 and 4) where there are more materialized views in the system.
Later we will show this effect in the user evolution scenario ---
where any materialized view in the system created by any user may be used for
rewrite --- our algorithm beats DPR by several orders of magnitude
for all cases.
This highlights the utility of \ocost{}.
Even for these degenerative cases we can never search more space than DPR.

\twofig{fig-bfs-vs-dp-merge-attempts}
{fig-bfs-vs-dp-refine-attempts}
{Number of (a) candidate views considered and (b) rewrite
attempts during workflow evolution}
{1.75in}

% 
%\onefig{fig-bfs-vs-dp-merge-attempts}{Number of candidate views 
%examined for each algorithm during workflow evolution}{2.75in}
%\onefig{fig-bfs-vs-dp-refine-attempts}{Number of rewrite
%attempts performed by
%each algorithm during workflow evolution}{2.75in}
%
%Figure~\ref{fig-bfs-vs-dp-merge-attempts}(b) reports the number
%of rewrites attempted by each algorithm.
%Recall from Section~\ref{sec-rewrite-enumeration} that
%finding an equivalent rewrite involves enumerating
%all possible rewrites of a view using $L_R$.  
%Given the known computational complexity of attempting a rewrite,
%the work efficiency of an algorithm can also be evaluated
%by the number of rewrites it attempts.  
%From the figure it can be seen that our algorithm always attempts
%far fewer rewrites than the bottom-up approach, and 
%in many instances at least an order of magnitude fewer.
\end{comment}

\begin{comment}
Note that $r^*$ can be composed of rewrites found
at multiple targets.  
Some of the additional rewrites that our algorithm attempted 
include those where it failed to find an equivalent rewrite and 
those which produced a equivalent rewrite but were not part of $r^*$.
Rewrite attempts in the second case are those that
had a lower \ocost{} than $\ocost(r^*)$
but their \cost{} was actually more than $\cost(r^*)$
thus exposing the limitation of our weak lower bound
of the \ocost{} function.
Yet clearly this result shows even our basic \ocost{} 
function can provide significant savings.
cases.
1. fails to find a rewrite
2. finds a rewrite but is not part of r* as its actual cost is higher
3. it is part of r*
\end{comment}

\subsubsection{User Evolution}\label{sec-experiments-ue}
\threefig{fig-ue-bfs-vs-dp-candidates-explored}
{fig-ue-bfs-vs-dp-refine-attempts}
{fig-ue-bfs-vs-dp-time-comparison}
{User Evolution Comparisons for 
(a) Candidate views considered, (b) Refine attempts, and (c) Runtime (log-scale)}
{2.15in}

Next we evaluate the case of a new analyst entering the system
and executing the first version of his workflow given that
all the other analysts having executed their workflows.
The system rewrites $A_iv_1$ using the existing
materialized views from all other analyst workflows.
Figure~\ref{fig-ue-novf-vs-vf-running-time} shows the performance of
the rewritten workflow versus the original workflow.
Figure~\ref{fig-ue-novf-vs-vf-running-time}(a) shows the workflow execution
time while Figure~\ref{fig-ue-novf-vs-vf-running-time}(b) shows the 
data moved (read/write/shuffle).
It can be seen from these figures that the execution time is always lower for the rewritten
workflow, with a similar trend in the amount of data moved.
The percentage improvement in execution time is given in 
Figure~\ref{fig-ue-novf-vs-vf-running-time}(c) where it can be
seen that our system results in an improvement of about 50\%, 
and up to 90\%.
These results show the benefit of rewriting workflows using
MVs from previous versions in the user evolution scenario.

% Given enough materialized views in the system, 
% intuitively a new analyst can expect some benefit from them
% if there is overlap with at least one other analyst.
% Overlap in this domain is quite common given there is
% a small set of operations that most workflows build upon,
% such as identifying people's friends (social network), 
% their likes (sentiment), 
% and locations they visit (check-in).

Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}
compares the performance of the WFR and DPR algorithms 
by measuring how much of
the rewrite search space each algorithm explores.
The candidate views considered corresponds to 
all the existing candidate views and all the 
views created as part of the rewrite search process (i.e., merged views).
The number of rewrite attempts corresponds to the views guessed to be
complete that we encounter during our search process, 
each of which are given to $\RE{}$ to attempt to find a rewrite.
As noted previously this process is computationally expensive.
These result show for most cases it is possible to 
find $r^*$ by considering far fewer candidates
views as in Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(a),
orders of magnitude fewer
rewrites in Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(b),
resulting in significant savings in runtime as shown in 
Figure~\ref{fig-ue-bfs-vs-dp-candidates-explored}(c)
due to our algorithm's use of $\ocost{}$ that enables
considering the promising candidate views earlier.
% This shows our algorithm results in a significant reduction
% in the rewrite search space.

\subsubsection{System Improvement Over Time}\label{sec-experiments-system-improves}

In our scenario materialized views are artifacts left 
behind from previously executed workflows.
To show that system performance improves over time we present two 
evaluations.
First we execute $A_5v_3$ with no analyst's workflows
in the system, then we repeatedly add another analyst and re-execute 
$A_5v_3$ to show improvements as more analysts are present in the system.
We chose $A_5v_3$ as it uses all three logs as it has
more opportunities to find commonality with other workflows.
Table~\ref{fig-se-novf-vs-vf-time-improvement} reports the 
execution time improvement of $A_5v_3$ using our 
 rewrite algorithm as the number of other analysts increase.
We use the workflow execution time when no
other analysts are present in the system as the baseline, 
and report percentage improvement relative to this baseline.
Table~\ref{fig-se-novf-vs-vf-time-improvement} 
clearly shows an increasing benefit for an
incoming analyst as more users are present in the system.
The benefit is obviously dependent on the amount of similarity to other
analysts workflows, and in this example there is quite a bit of benefit
even when one other analyst is present.

% \onefig{fig-se-novf-vs-vf-time-improvement}{Improvement in execution time of $A_5v_3$ as more
% analysts are present in the system}{2.5in}

\begin{table}
\vspace{-0.10in}
\caption{\label{fig-se-novf-vs-vf-time-improvement}
Improvement in execution time of $A_5v_3$ as more
analysts become present in the system}
\centering
\begin{tabular}{| p{2.5cm} | p{1cm}| p{1cm} | p{1cm}| p{1cm} | p{1cm}|}
\hline
Analyst in System & 1 & 2--3 & 4 & 5--7 \\ \hline
Improvement    & 0\% & 73\% & 75\% & 88\% \\ \hline
\end{tabular}
\vspace{-0.13in}
\end{table}


Secondly after the system has been in use for a few 
months, we show that the existing materialized views in 
the system can aid in rewriting workflows.
We evaluate the rewrites produced by our algorithm with 
increasing numbers of materialized views present in the system.
We retained about 4,800 views that were created during the course
of design and development of our system, including those created
during the process of designing the 8 scenarios and our microbenchmark.
This setup is intended to represent a mature system with many views 
left behind from previous execution runs.
Then we try to rewrite one analyst's workflow ($A_3v_1$) given
a random sampling of the existing views.
From the 4,800 views, only 650 were unique.
Furthermore, both the algorithms (``WFR'' and ``DPR'') 
pruned from consideration views that cannot be used in a rewrite 
for a given target for the following reasons. 
A materialized view was pruned if it belonged to a different log, 
if it had a predicate condition that could not be removed,
or if it was a view previously created for any of Analyst3's workflows.
After pruning, the number of materialized views available for each target was
slightly more than 250.  
This experiment was performed ten times for each 
algorithm, and a scatter plot of the results are given in
Figure~\ref{fig-mv-vary-num-candidates}.


\twofig{fig-mv-vary-num-candidates}{fig-mv-vary-rewrites}
{Number of candidates considered (a) and the number of rewrites produced (b) (log-scale)}
{1.75in}

Figure~\ref{fig-mv-vary-num-candidates}(a) shows for each 
experiment performed, WFR creates several times fewer
candidate views.
Because WFR uses \ocost{}, 
it can avoid considering candidate views whose \ocost{}
is more expensive than $\cost(r^*)$.
Clearly the space of newly merged views is exponential in the worst case
as noted in~\cite{Agra2000}.  
These results show that WFR cannot escape this exponential space,
but typically results in creating and searching a smaller space than DPR approach.
Due to the known computational complexity of the problem, any solution that
avoids searching the entire space must resort to pruning which can result in sub-optimal rewrite.
Additional pruning could be applied to reduce the search space, 
but our algorithm will still find the best rewrite in the space it considers.

However, the larger benefit of WFR can be seen in 
Figure~\ref{fig-mv-vary-num-candidates}(b) 
which shows WFR is able to find $r^*$ by obtaining
far fewer rewrites than DPR in each case, and orders of magnitude fewer
for most cases.
The saving from (a) is primarily driven by how \emph{far} $r^*$ is into the space
in relation to the entire space, while the savings from (b)
is driven by \ocost{}'s ability to examine
more promising candidate views before less promising views.

%Furthermore, the more the views that exist, the more likely at least
%some of these will be useful for rewrites. 
%the faster \VF{} can find them, apply them, and terminate early
%by obtaining $r^*$ due to its incremental search behavior.
%we can examine candidates by the potential order of usefulness 
%(i.e. increasing optcost)

\subsubsection{Comparison with Caching-based methods}\label{sec-experiments-restore}

% \onefig{fig-re-novf-vs-vf-time-improvement}{Improvement in Execution Time of User Evolution 
% when not including identical views}{2.5in}

\begin{table}
\vspace{-0.2in}
\caption{\label{fig-re-novf-vs-vf-time-improvement}
Improvement in execution time of user evolution with 
and without identical views}
{\small
\centering
\begin{tabular}{| p{1cm} | p{0.5cm}| p{0.5cm} | p{0.5cm}| p{0.5cm} | p{0.5cm}|p{0.5cm} | p{0.5cm}| p{0.5cm} | p{0.5cm}|}
\hline
Analyst & $A_1$ & $A_2$ & $A_3$ & $A_4$ & $A_5$ & $A_6$ & $A_7$ & $A_8$ \\ \hline
With & 57\% & 64\% & 86\% & 85\% & 78\% & 98\% & 88\% & 84\% \\ \hline
Without & 57\% & 64\% & 83\% & 85\% & 51\% & 96\% & 88\% & 84\% \\ \hline
\end{tabular}
}
\vspace{-0.15in}
\end{table}

Here we compare our approach against caching-based methods such as ReStore~\cite{Elgh2012} that only
consider reusing identical answers.
Reusing cached results is clearly effective.
However, to illustrate the benefits of our rewrite algorithm beyond simple caching, 
we present an experiment where we prune away all identical views from the solution space.
This setup represents the worst-case for caching-based methods,
as they will not be able to find any rewrites, thus will 
result in no improvement.
%caching-based methods are not nearly as effective as our approach.
Table~\ref{fig-re-novf-vs-vf-time-improvement}
reports the percentage improvement using our algorithm when identical views are present (with), 
and after pruning them all away (without).
Our algorithm results in good improvement
with and without identical views, showing only a slight
performance drop without identical views 
for all analysts except $A_5$.
This is because $A_5$ had previously benefited from an identical view corresponding
to restaurant similarity which it now has to recompute.
Note that identical views constituted only 7\% of 
the view storage space here.
Given that analysts pose different but related queries in an evolutionary scenario,
any method that relies solely on exact matching will
have limited benefit.



\subsubsection{Comparison with DB-X}
To verify that our system produces good rewrites, we compared the rewrites 
produced by our algorithm with a widely-used commercial database system (DB-X) 
and data from the TPC-H \cite{tpcds} benchmark.
DB-X was tuned to its highest optimization level as well as 
set to consider all views for query rewriting.
To represent artifacts from prior executions in our system
we created MVs using  the {\tt LINEITEM} table.
One MV is a groupby-count on {\tt L\_ORDERKEY, L\_SUPPKEY} 
and the other is a groupby-count on {\tt L\_ORDERKEY, L\_PARTKEY}.
We used both systems to produce rewrites for three queries and then compared
their estimated cost using the DB-X query optimizer.
The first query tests if DB-X will produce a rewrite 
that involves a join of the two syntactically relevant MVs.
The second query tests groupby unrolling while reusing the count 
aggregate, while the third query tests a more complicated case of reusing 
count aggregate as well as a max aggregate on one of the keys. 
In the first query, DB-X did not use the MVs for the rewrite 
which made it 3X worse than the rewrite produced by
our system. 
In the second query, both DB-X  and our system produced
identical rewrites, resulting in the same cost. 
In the third query, DB-X did not make use of an MV, 
whereas our rewrite did resulting in a 5X savings. 
This experiment shows 
that our rewrite algorithm produces  rewrites comparable to a
state of the art commercial system. 
%Given that we also allow UDFs in our rewrite 
%language, we will use our rewrite algorithm in the bottom-up (DPR) approach.

\subsubsection{View Storage Maintenance}\label{sec-experiments-gc}

\begin{table}
\caption{\label{fig-ga-improvement-vs-storage-reclaimed}
Execution Time Improvement after reclaiming 10\% to 90\% of the 
view storage space}
{\small
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Reclaimed Storage & $10\%$ & $20\%$ & $30\%$ & $50\%$ & $70\%$ &$90\%$\\ \hline
Improvement & 89\% & 88\% & 86\% & 82\% & 58\% & 30\% \\ \hline
\end{tabular}
}
\vspace{-0.14in}
\end{table}

Since storage is not infinite a reclamation policy is necessary.
Although many policies are possible, we demonstrate the robustness of our approach 
using two unsophisticated policies since this is not focus of our work.
The first randomly drops views to reclaim 10\%--90\% 
of the view (configuration) storage space and then we run the $A_5v_3$ workflow
as used in Section~\ref{sec-experiments-system-improves}. 
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
reports the average workflow execution time improvement when applying our rewrite algorithm after reclaiming 
various amounts of storage space randomly.
Each test is repeated twice (different randomizations) and we report the average improvement.
Table~\ref{fig-ga-improvement-vs-storage-reclaimed} 
shows that our system produces rewrites that give good improvement even as the view storage 
space decreases.

The second policy considered is one that drops all of the \textit{best} views for a 
workflow, representing an adversarial storage reclamation policy.
The best views are those with the ability produce a low cost rewrite, 
thus such a policy would drop any view that is identical to a target in the workflow.
Table~\ref{fig-re-novf-vs-vf-time-improvement}
indirectly captures the performance
of our rewrite algorithm given an adversarial policy showing the robustness of our system even 
when there are no identical views for the workflow.
% Best refers to those views that have maximum benefit 
% with lowest cost, 
%, although in the current work we do not consider maintenance cost.
%
% which is exactly the effect measured by the previous experiment
% where our approach shows only slight performance loss after
% dropping the identical views.
% Taken together, the previous two experiments show the
% robustness of our system and rewrite algorithm.

The hardness of designing a good policy is equivalent to a view selection problem with a storage constraint.
Certainly better methods~\cite{Mami2012} could be applied but we leave this for future work.


\begin{comment}
\subsubsection{Garbage Collection}

Next how garbage collection does not result in significant loss
of performance. 

Next we briefly consider the effects garbage collection on 
our algorithm performance and workflow execution time.
Garbage collection can be applied to recover storage space
or to reduce the runtime of the rewriting algorithm.
Figure~\ref{fig-mv-vary-num-candidates}(a) shows the space of
candidate views is exponential, thus arguing to keep the
number of views lower.  
Figure~\ref{fig-mv-vary-num-candidates}(b) shows that even 
for higher numbers of available views randomly 'retained' 
among all available views, our algorithm 
only needs to find very few rewrites to obtain $r^*$.

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%% End of File

\begin{comment}
\begin{enumerate}

\item Analyst1 wants to find influential users who are
interested in food with the goal that
these users could be target of a future advertisement campaign.
The evolution of this scenario will propose increasingly
sophisticated interpretations of what it means to be ``influential''.

\item Analyst2 wants to identity 100 wine lovers so that he can 
send them a coupon for a new wine being introduced in the market. 
The evolution of this scenario will investigate 
increasingly sophisticated ways of finding out if a user is a ``wine lover''.

\item Analyst3 wants to start a birthday gift recommendation service where friends
can send a gift certificate to a user $u$ who's birthday is around the corner.
We want to generate 5 restaurant choices based on $u$'s preferences and alert
$u$'s friends to $u$'s upcoming birthday and offer them a choice
of discount certificates to the 5 restaurants.
The evolution in this scenario will investigate how to determine
if a user likes a restaurant enough to visit it on his birthday,
how to suggest a diverse set of recommendations as well as
how to suggest restaurants that would cater to $u$'s close set of friends.

\item Analyst4 wants to provide restaurants with a breakdown of their
customer population. 
In particular, the analyst wants to provide breakdowns in terms of who goes to a
particular restaurant.
The analyst may also want to perform analysis in terms for geographical area.
For instance, for any area which are the popular restaurants by categories etc.
The goal of this scenario is to perform increasingly complicated analytical 
operations on the log.

\item Analyst5 wants give restaurant owners a poaching tool in the 
the following sense.
For each restaurant $r$, we identify customers who go to a ``similar'' 
restaurant in the area but do not visit $r$.
Using the list, the owner of $r$ may send these customers a coupon.
The evolutionary nature of the problem is to find out how to determine
``similar'' restaurants.

\item Analyst6 tries to find out if restaurants are losing their
loyal customers.
In other words, we want to identify those customers 
who used to visit frequently but now slowly
stopped visiting the restaurant, but are still visiting other restaurants in the area.
The restaurant owner can send them a coupon to win them back.
The evolutionary nature of this scenario will focus on 
how to identify prior active users.

\item Analyst7 wants to go by the maxim in business that problems should be caught
as soon as possible. 
For each restaurant in the system, try to identify common problems that
users have reported about the restaurant.
For example, have customers complained about food, service, issues with premises etc.
Moreover, if there is a successful restaurant of the same category, 
what makes it successful.
The evolutionary nature of this scenario will focus on compiling
issues under different categories.

\item Analyst8 wants to identity what category (i.e., american, indian,
chinese, steak) of restaurants is missing from a
certain region. For example, one of the outcome can be that 
Cupertino could really use a Moroccan restaurant. 
The evolutionary nature of this scenario will focus on how to 
find out if there is a need for a good restaurant in a certain
category and if so what is the nature of their clientele etc.

The use-case for our system that it is being used internally
by analysts who work for restaurant marketing company that gets commission
from sending users to restaurants or providing restaurant 
owners analytics support to aid them in their business decisions.
Each analyst starts out with a single log file and expanding
to all the three log files during the course of their
evolutionary workflow.
{\it The idea here is not to get too carried away by the quality
of the answers we get but write workflow structures that capture
the spirit of these scenarios.}


\end{itemize}


The desirable property of the $\cost{}$ is that it must be cheap to compute.
Since a full query optimizer may be too expensive, we use a model of a query optimizer.
We treat this model as a black box, in this way $\RE{}$ and $\ocost{}$ can
utilize any functionality provided by the model or improvements to the model.
%For an RDBMS, a cost model such as in~\cite{x,y} could be used.  
%Because we evaluate our framework in a MapReduce execution system, 

Our cost model is based on the one in~\cite{Nyki2010}, 
which reduces a query $q$ to a set of $m$ jobs $\{J_1, \cdots, J_m\}$. 
The cost of each job is expressed as a linear combination of 
the cost to read the data ($C_{r}$)
the cost of sorting and copying ($C_{s}$),
the cost to transfer data ($C_{t}$).
and the cost to write the output of the job ($C_{w}$).

\begin{equation} \label{eq-cost}
\cost(q,v) = \sum_{i=1}^{m} C_{r}(J_i,v_i) +  C_{s}(J_i,v_i) +  C_{t}(J_i,v_i) +  C_{w}(J_i,v_i)
\end{equation}
where $v_1 = v$, and $v_{i}$ forms the input of $J_i$.

               
To keep the $\cost{}$ function inexpensive, our model does not consider re-ordering 
of joins, predicate push down, or other types of optimizations involved in 
group bys and udfs, but does merge sequential operations (e.g. a sequence of filters)
into the same job whenever possible.


This is a reasonable approach given that we have already committed to creating $v$,
and the $\RE{}$ explores all possible rewrites, such a cost function serves
our purposes here.  

An extension to this basic cost model could consider push downs when computing the cost
to create $v$.  The requirements to including push-downs into the optimization
process would be to employ a cost model $\cost{}$ that is able to 
apply all possible join orderings to creating $v$ along with applying filters 
to all orders.  

Appendix~\ref{appendix-pushdown} provides a proof for using $\RE{}$ and $\ocost$ with an extended 
$\cost{}$ function that considers join ordering and predicate pushdowns,
while still producing a correct lower bound for $\RE{(v,q)}$.

There are 2 reasons we do not consider predicate push downs here.
First $\cost{}$ becomes much more expensive to invoke due to considering all 
of the ordering options. 
Second, we may not wish to push down a filter into $v$ since this could render $v$ 
less useful for answering future queries.  
A more sophisticated algorithm could weigh the cost and benefits of different 
versions of $v$ (with and without filters) given their benefit to other queries 
and their added cost due to avoiding filter push downs.

\subsubsection{Comparison with DB2 and ReStore:}

Show that our $\VF{}$ performs better rewrites compared to 
the DB2 design advisor.
We also need to emphasize that there is a significant ETL time with DB2
which we will not consider for this experiment.

{\em Run the workflow A4-v1 and store the MVs of all targets
  produced by this workflow in DB2. Next, we
give DB2 queries corresponding to $W_n \cdots W_1$ of the A4-v2.
We obtain DB2 cost estimates for the rewrites provided by DB2. 
Next we obtain the rewrite $r^*$that our algorithm provides and 
get it costed using the DB2 cost model.
Hopefully, we can show using the DB2 cost model 
that $r^*$ is cheaper than its own rewrite.

Graph: DB2 optimizer estimated time units (y-axis) against 
DB2 rewrite and $r^*$ for A4-v2 (x-axis).
We may try to do it for all workflows,  A1 thru A8

{
\color{red}
\sout{
Graph2: It would also make sense to take care of ReStore early
on so that we do not have to keep comparing with it through
the rest of the section.} (as per Alkis's comments)
}
}

\item Weakness of $\ocost{}$ on the work efficiency of the
$\VF{}$.
Measure the total rewrites possible (P),
number of rewrites we explored (T),
number of rewrites explored that we should not have explored (E)
(y-axis) vs. three variants of $\ocost{}$ in x-axis.

P here denotes the complexity of a non-incremental algorithm,
T is the total work done by us, E is wasted work among T.

\item Graph on time taken to find $r^*$ (y-axis) vs.
{\em features} of the workflow. Features of the workflow include
$n$, number of joins, udfs etc.

Graph on time taken to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 
  
\item Graph on number of rewrites explored to find $r^*$ (y-axis) vs.
  our incremental variant and exhaustive bottom-up approach 

\item Compare our algorithm with diminished
versions of the algorithm.
Graph on estimated cost of $r^*$ (y-axis) vs. 
remove modules of the $\VF{}$ one by one.
For example, we could reduce the expressivity of $L_R$, joins etc.
This set of experiment will show the benefit of added complexity.\\

{\color{red}

Alkis says: ``I think that this should go first, so that the other experiments utilize the full-featured algorithm''

Response: OK
}

{\color{red}
\sout{We could handle ReStore here as one way of performing equivalent
rewrites}.
}
\end{enumerate}


{\em 
{\color{red}

Alkis: ``Do we know the theoretical complexity of our view-rewrite algorithm?''

Response: Our rough calculation is as follows.

The complexity of the $\WF{}$ is $O(n.l)$, where
$l$ is the number of samplings of the cost range $[0, \cost(W_n)]$.
$l$ can be chosen to be $n$ 
so that the $\WF{}$ algorithm is 
bounded by $O(n^2)$.

The $\VF{}$ is bounded by $O(|V|^{k_1} 2^{k_2})$ where 
$k_1$ represents the maximum number of candidates that
may be explored (generated + existing) by the $\VF{}$, 
while $k_2$ is a small constant 
representing the number of transformation rules in the system.
$k_1$ is bounded by $n$ as in the worse case $W_n$ may
contain $n-1$ joins.
Assuming all joins are of the same cost, the most expensive rewrite
for $W_n$ may contain up to $O(n)$ joins.
Hence, the complexity of the $\VF{}$ for a single target
is bounded by $O(|V|^n 2^{k_2})$.

The complexity of the entire algorithm is bounded by:
$O(n^2 + n \cdot |V|^n 2^{k_2})$, where $k_2 << |V|$.

}

\end{comment}


==> old/Introduction-Jagan.tex <==
\section{Introduction}
 
A knowledge-driven enterprise adopts an aggressive strategy of
instrumenting every aspect of their business and encourages
the employees to find value in the large amount of
raw data collected from vastly diverse sources.
The nature of these data explorations begins with
an analyst making a guess and then posing subsequent 
questions, continually revising or \emph{evolving}
the workflow as his intuition leads him toward the desired results.
As analysts are often uncertain about the value of the data
and the best process to identify this value, 
an analytics platform should be able to adapt to the needs of 
many users exploring large diverse data sets.
The process of exploration is iterative as the analyst 
make lack sufficient understanding of the data to be able 
to translate his intent to a workflow in one shot.
Therefore it is to be expected that the exploration will
be reformulated several times 
since this is also a necessary exercise for the user to 
gain better understanding of the data.
This iterative process is time consuming as
workflow revisions are driven by examining the previous results.

The ability of an organization to discover value in the data
is dependent on the speed at which a single analyst
can iterate through successive investigations of the data.
Analysts typically express their data exploration in the 
form of \emph{workflows}, consisting of individual data
access and processing steps. 
Analysts typically express their workflows using a 
high level language, and often apply sophisticated
operations such as text sentiment,
network influence, classification, etc. 
These sophisticated -- and usually domain
specific -- operations can be formulated as User Defined Functions ({\em UDFs}).
Given the compexity of the exploration and the size of the
datasets involved, this exploration process can be extremely time consuming
and there is a need to speed up these explorations.

There is an opportunistic mechasign to reuse prior work..

A platform to support such data explorations should enable users to 
speedup
1) performing increasingly sophisticated analysis 
as they gain better understanding of the data, and
2) possibly benefit from analysis performed by other analysts.
Such a platform that supports {\em Workflow Evolution} and {\em User Evolution},
respectively.
Specifically, workflow evolution is defined as a single analyst adjusting,
modifying, and re-purposing a workflow to better align the results of the workflow
to match the analyst's intent.
User evolution is defined as new analysts arriving that begin querying the
system with new workflows and possibly benefit from 
previous work performed by others. 


The following scenario is an
example of these three evolutionary dimensions:
 
\begin{example}
An analyst wants to identity 100 wine lovers so that he can
send them a coupon for a new wine being introduced in the market.
The evolution of this scenario will investigate
increasingly sophisticated ways of finding out 
if a user is a ``wine lover'' from a
single social networking data source.
Furthermore the analyst may want to make use of
an additional data source, e.g., Foursquare location check-ins,
to obtain more evidence that a user likes wine.
Next, another analyst arrives and wants to identify people
that frequently go to the movies.
She may benefit from some of the answers materialized as part of
the previous analyst's data exploration
such as unique users, their friends, and locations they
check-in to.
\end{example}


%Analysts in these organizations may explore the data using queries
%expressed as {\em workflows} in a high level language, and often
%apply complex operations such as text sentiment,
%network influence, classification, etc.
%A workflow is expressed as a DAG of queries.
%Complex operations are captured by UDFs
%developed by the analyst and used across the organization.
%Recently the role of the data scientist~\cite{Pati2011}
%has been introduced to help organizations identify value
%in their data.

A key technical challenge we address is 
efficiently rewriting the user workflows in a way that effectively 
exploits the results of other workflows from all 
users in the system even as users flexibly
change their workflow structure, 
apply sophisticated functions (UDFs), 
and include additional data sets. 
We address this by formulating it as a query
rewrite problem  for evolutionary workflows. 
We discuss the challenges of this problem
and why state-of-the-art methods would not provide 
satisfactory solutions due to the requirements of the system.
Our contributions are as follows.
 
\begin{itemize}\setlength{\itemsep}{1pt}\setlength{\parsep}{0pt}
  \item A workflow rewriting algorithm \WF{} that finds
  the optimal rewrite of an evolutionary workflow in
  a work-efficient manner.
 
  \item An optimistic cost function \ocost{} that provides a lower
  bound on the cost of a rewrite using a given view.  This
  functionality enables the workflow rewrite algorithm to
  incrementally search the space of rewrites.
 
  \item A gray-box model of a UDF that is expressive yet
  conducive to rewrites.
  This allows any user to add a UDF to the system,
  and the system operator may choose to extend the rewrite language
  to include the UDF.
 
  %\item A set of 8 evolutionary workflows representing realistic scenarios,
 % where each workflow has 4 evolutions resulting in 32 workflows.
  %These types of queries do not appear to be captured by current benchmarks,
  %and we present them as a first step toward a benchmark for evolutionary
  %workflows.
 
  \item A \emph{microbenchmark} to capture and evaluate the flexibility an
analyst has  in revising analytical workflows.
 
  \item Extensive experimental results over large, real data sets and
comprehensive, realistic use-case scenarios that show our rewrites result 
in up to 90\% improvement in workflow execution time, 
 as well as a significant reduction in the rewrite search space considered 
 by our algorithm.
 
 %and the superiority over   
  %reduce workflow execution time by 10\%--90\%
 % and our workflow rewrite algorithm searches much less of the space to
  %find the optimal rewrite than a bottom-up approach.
 
\end{itemize}
 
 


==> old/Introduction-rewrite5.tex <==
\section{Introduction}
Businesses are collecting an increasing amount of data from disparate sources 
and tasking their analysts to find value within the data.  
%New data sources frequently become  available and include social media 
%such as Twitter, Foursquare, Yelp, Pinterest, blogs, 
%user feedback/reviews/comments, among others.  
Much of this new data comes from social media and often has low structure
and can be extremely large. 
The need to identify value in new data has led to an increased interest in data
analysts as well as the new role of the 
data scientist~\cite{Fitz2012, Bowi2012, Pati2011}.
Analysts explore data in the form of complex queries that are revised and 
refined in an iterative manner since the analyst may lack sufficient 
understanding of the data to express and achieve the intended goal 
in the first attempt.
Thus queries evolve during this iterative, exploratory process of identifying 
value in the data.  
As an analyst guides the querying process toward the desired outcome, 
adjustments and modifications may lead to a revised version that retains much 
of the previous query.
%Complex analytical queries often apply sophisticated operations 
%such as text sentiment, network influence, classification, or other processing.
%These sophisticated -- and usually domain specific -- operations can be 
%formulated as User Defined Functions (UDFs) and are a key component of this 
%analysis process.  
The ability of an organization to discover value in the data is dependent on 
the speed a single analyst can iterate through successive explorations 
of the data.  
Thus, reducing the time to insight is an important problem~\cite{Lava2011}.

This type of complex analysis on data with unproven value is well-suited to a 
large-scale data analytics platform such as 
MapReduce~\cite{Dean2004, Ston2010}.
To achieve fault-tolerance, large scale data-analytics platforms create several
artifacts during the execution of a query.  
These artifacts represent the intermediate and final results, and are stored in
the distributed file system. 
Our key insight is to leverage this behaviour by treating artifacts as 
\textit{opportunistic} materialized views that can be used to rewrite queries.
Since queries evolve but retain elements of similarity, we propose a method 
to dramatically improve performance for evolving queries.
Our method rewrites queries based on these opportunistic views that we reuse 
and repurpose to benefit subsequent queries.
In this way, the execution artifacts become part of an 
\emph{opportunistic physical design}.
We note that our opportunistic design does not require any work to proactively 
select good artifacts or views.

The following example illustrates this evolutionary process and indicates 
how users may benefit from opportunistic views.

\begin{example}
An analyst want to identify 100 ``wine-lovers'' for a new marketing campaign. 
The analyst may start with a data source such as Twitter, and search for users 
that like food and/or wine.  
She may then revise the query to include additional evidence a user likes 
wine by also considering the type of restaurants where they check-in frequently.
The execution time of this new query revision can be significantly improved 
through rewriting using opportunistic materialized views generated by the 
previous version.
\end{example}

Improving the performance of complex analytical queries on data with unproven 
value is difficult because the data is not well-curated 
or stable~\cite{Hell2011} and the analysis may include sophisticated operations.
These sophisticated -- and usually domain specific -- operations 
(\textit{e.g.,} text sentiment, network influence, other classification) 
may be formulated as User Defined Functions (UDFs) and are a key component of this 
analysis process.  
It is not straightforward to tune a system for performance when both the data 
and types of operations are fluid.  
Standard tuning methods might be applied if the data were loaded into a 
database using an Extract-Transform-Load process.
However, a formal ETL process may be prohibitively expensive 
(in time and money) for data with unproven value -- constituting as much as 
the majority of a data warehousing project's cost~\cite{Simi2009}. 
Given our scenario, we identify these opportunistic views as an untapped 
source for performance improvements.


Recent methods to reuse complex computations such as ReStore~\cite{Elgh2012}
and MRShare~\cite{Li2011} lack a semantic understanding of the artifacts 
produced during execution and can only reuse/share cached results when 
execution plans are identical.
%The work in ~\cite{Guo2011} recognizes the evolving nature of scientific 
%scripts when exploring data and presents a memoization method to cache
%and reuse previous results, but this is given for a single scripting language 
%(Python) and is limited to code analysis.
Furthermore, methods for rewriting queries using views have not addressed 
complex workflows that may include UDFs due to the opaque nature 
of UDF operations.
Other recent work~\cite{Hues2012} applies static code analysis to UDFs in 
MapReduce to extract limited semantic information that is then used to enable 
reordering of selection and group-by predicates for optimizing a single 
execution plan.
In this work, we present a rewriting algorithm and a semantic model for UDFs 
that take advantage of opportunistic views to more effectively reuse 
previous computations resulting in significant performance improvements.

Our opportunistic retention policy results in many materialized views,  
creating a large search space for rewriting queries.
To address this, we draw inspiration from techniques used in nearest-neighbor 
searches to step through this space in a principled manner.  
Our rewrite algorithm searches the space of rewrites in a best-first manner
to obtain the optimal (lowest cost) rewrite given the views available.

Our specific contributions are as follows.

\begin{itemize}
  \item A gray-box UDF model that is simple but expressive enough to capture
  many common types of UDFs.
   This affords us a limited semantic understanding of UDFs to enable effective
   reuse of previous results.  
   We provide the model and the types of UDFs it admits in 
   Section \ref{sec-preliminaries}.
  
  \item A workflow rewriting algorithm that takes as input a query and a
   set of views  and outputs the optimal rewrite.  
  We show the algorithm is work-efficient in that it considers the minimal
  set  of views necessary to find the optimal rewrite under 
  certain assumptions.
  We describe this further in Section \ref{sec-best-first-workflow-rewrite}.
  
  \item Experimental results showing our methods provide execution time 
  improvements up to  90\% using real-world data and realistic complex 
  queries in Section \ref{sec-experimental-evaluation}.  
  The savings from our method are due to moving much less data, 
  avoiding the high expense of re-reading data from raw logs when possible, 
  and reusing/repurposing results from long-running computations 
  including UDFs.
   
\end{itemize}



==> old/Introduction-rewrite6.tex <==
\section{Introduction}
Data analysts have the crucial task of analyzing the ever increasing volume of data that modern organizations collect and producing actionable insights. As expected, this type of analysis is highly exploratory in nature and involves an iterative process: the data analyst starts with an initial query over the data, examines the results, then reformulates the query and may even bring in additional data sources, and so on. Typically, these queries involve sophisticated, domain-specific operations that are linked to the type of data and the purpose of the analysis, e.g., performing sentiment analysis over tweets or computing the influence of each node within a large social network. 

Not surprisingly, MapReduce (MR), be it the original framework, its open-source incarnation Hadoop or derivative systems such as Pig and Hive that offer a declarative query language, has become a de-facto tool for this type of analysis. Besides offering scalability to large datasets, MR facilitates incorporating new data sources, as there is no need to define a schema upfront and import the data, and provides extensibility through a mechanism of user-defined function (UDFs) that can be applied on the data. Since the computational scope of a single MR job is limited, scientists typically implement a query as an ensemble of MR jobs that feed data to each other. Quite often, such queries are written in a declarative query language, e.g., using HiveQL or PigLatin, and then automatically translated to a set of MR jobs. 

Despite the popularity of MR systems, query performance remains a critical issue which in turn affects directly the ``speed'' at which data analysts can test a hypothesis and converge to a conclusion. Some gains can be achieved by reducing the overheads of MR, but the key impediment to performance is the inherent complexity of queries that ingest large datasets and span several MR jobs, a common class in practice. A-priori tuning, e.g., by reorganizing or preprocessing the data, is quite challenging due to the fluidity and uncertainty of exploratory analysis. 

In this paper, we show that it is possible to dramatically improve query performance by leveraging the built-in fault-tolerance mechanism of MR as an \emph{opportunistic physical design}. Specifically, we make the following observations:
\begin{itemize}
\item Each MR job involves the materialization of intermediate results (the output of mappers, the input of reducers and the output of reducers) for the purpose of failure recovery. More generally, a multi-stage job, such as one that is generated by Pig or Hive, will involve several such materializations. We refer to these materialized results as the artifacts of query execution and note that they are generated automatically as a by-product of query processing. 

\item Given the evolutionary nature of data exploration, it is likely that each query has similarities to previous queries by the same analyst, and even to queries of other analysts who examine the same data. For instance, several data analysts may perform sentiment analysis on a specific class of tweets (e.g., in a specific geographical area) but with a different hypothesis in mind. Hence, the computation performed by previous queries in the system, as captured in the generated artifacts, may be relevant for a new query. 
\end{itemize}
Thus, we propose to treat artifacts as opportunistically-created materialized views and use them to rewrite a new query in the system. The opportunistic nature of our technique has several nice properties: the materialized views are generated as a by-product of query execution, i.e., without additional overhead; the set of views is naturally tailored to the current workload; and, given that large-scale analysis systems typically execute a large number of queries, it follows that there will be an equally large number of materialized views and hence a good chance of finding a good rewrite for a new query. Our results with an implementation of this technique inside an industrial data-analytics system indicates that the savings in query execution time can be dramatic: from 10\% up to an order of magnitude improvement. Testimonies from analysts using the system suggest that these improvements have contributed to a substantial increase in productivity. 

Rewriting a query using views is a well-studied problem in databases, yet its treatment in the context of MR involves a unique combination of technical challenges: there is a huge search space of rewrites due to the large number of materialized views in the opportunistic physical design; queries can be arbitrarily complex; and, views and queries almost certainly involve UDFs. Unfortunately, previous works do not address the problem in its full generality and essentially ignore one or more of the previous dimensions. 
%<Mini review of previous works.> 
Recent methods to reuse MR computations such as ReStore~\cite{Elgh2012}
and MRShare~\cite{Li2011} lack a semantic understanding of the artifacts 
produced during execution and can only reuse/share cached results when 
execution plans are identical.
We strongly believe that any practical solution has to address the query rewrite problem in its full generality. 

Contributions. In this paper we present a novel query-rewrite algorithm that targets the scenario of opportunistic materialized views within an MR system. The algorithm employs techniques inspired by spatial databases (specifically, nearest-neighbor searches in non-metric spaces) in order to aggressively prune the huge space of candidate rewrites and generate the optimal rewrite in an efficient manner. Specifically, our contributions can be summarized as follows:
%- Gray-box model for UDFs.
%- Rewrite algorithm.
%- Experimental study.
\begin{itemize}
  \item A gray-box UDF model that is simple but expressive enough to capture
  many common types of UDFs.
   This affords us a limited understanding of UDFs to enable effective
   reuse of previous results.  
   We provide the model and the types of UDFs it admits in 
   Section \ref{sec-preliminaries}.
  
  \item A rewriting algorithm that takes as input a query and a
   set of views  and outputs the optimal rewrite.  
  We show the algorithm is work-efficient in that it considers the minimal
  set  of views necessary to find the optimal rewrite under 
  certain assumptions.
  We describe this further in Section \ref{sec-best-first-workflow-rewrite}.
  
  \item Experimental results showing our methods provide execution time 
  improvements up to an order of magnitude using real-world data 
  and realistic complex queries in Section \ref{sec-experimental-evaluation}.  
  The savings from our method are due to moving much less data, 
  avoiding the high expense of re-reading data from raw logs when possible, 
  and reusing/repurposing results from long-running computations 
  including UDFs.
   
\end{itemize}



==> old/Introduction-rewrite7.tex <==
\section{Introduction}
Data analysts have the crucial task of analyzing the ever increasing volume of data that modern organizations collect and producing actionable insights. As expected, this type of analysis is highly exploratory in nature and involves an iterative process: the data analyst starts with an initial query over the data, examines the results, then reformulates the query and may even bring in additional data sources, and so on. Typically, these queries involve sophisticated, domain-specific operations that are linked to the type of data and the purpose of the analysis, e.g., performing sentiment analysis over tweets or computing the influence of each node within a large social network. 

Not surprisingly, MapReduce (MR), be it the original framework, its open-source incarnation Hadoop or derivative systems such as Pig and Hive that offer a declarative query language, has become a de-facto tool for this type of analysis. Besides offering scalability to large datasets, MR facilitates incorporating new data sources, as there is no need to define a schema upfront and import the data, and provides extensibility through a mechanism of user-defined function (UDFs) that can be applied on the data. Since the computational scope of a single MR job is limited, scientists typically implement a query as an ensemble of MR jobs that feed data to each other. Quite often, such queries are written in a declarative query language, e.g., using HiveQL or PigLatin, and then automatically translated to a set of MR jobs. 

Despite the popularity of MR systems, query performance remains a critical issue which in turn affects directly the ``speed'' at which data analysts can test a hypothesis and converge to a conclusion. Some gains can be achieved by reducing the overheads of MR, but the key impediment to performance is the inherent complexity of queries that ingest large datasets and span several MR jobs, a common class in practice. A-priori tuning, e.g., by reorganizing or preprocessing the data, is quite challenging due to the fluidity and uncertainty of exploratory analysis. 

In this paper, we show that it is possible to dramatically improve query performance by leveraging the built-in fault-tolerance mechanism of MR as an \emph{opportunistic physical design}. Specifically, we make the following observations:
\begin{itemize}
\item Each MR job involves the materialization of intermediate results (the output of mappers, the input of reducers and the output of reducers) for the purpose of failure recovery. More generally, a multi-stage job, such as one that is generated by Pig or Hive, will involve several such materializations. We refer to these materialized results as the artifacts of query execution and note that they are generated automatically as a by-product of query processing. 

\item Given the evolutionary nature of data exploration, it is likely that each query has similarities to previous queries by the same analyst, and even to queries of other analysts who examine the same data. For instance, several data analysts may perform sentiment analysis on a specific class of tweets (e.g., in a specific geographical area) but with a different hypothesis in mind. Hence, the computation performed by previous queries in the system, as captured in the generated artifacts, may be relevant for a new query. 
\end{itemize}
Thus, we propose to treat artifacts as opportunistically-created materialized views and use them to rewrite a new query in the system. The opportunistic nature of our technique has several nice properties: the materialized views are generated as a by-product of query execution, i.e., without additional overhead; the set of views is naturally tailored to the current workload; and, given that large-scale analysis systems typically execute a large number of queries, it follows that there will be an equally large number of materialized views and hence a good chance of finding a good rewrite for a new query. Our results with an implementation of this technique inside an industrial data-analytics system indicates 
%that the savings in query execution time can be dramatic: from 10\% up to an order of magnitude improvement. 
that the savings in query execution time can be dramatic: a rewrite can reduce execution time by up to two orders of magnitude. 
%Testimonies from analysts using the system suggest that these improvements have contributed to a substantial increase in productivity.

Rewriting a query using views is a well-studied problem in databases, yet its treatment in the context of MR involves a unique combination of technical challenges: there is a huge search space of rewrites due to the large number of materialized views in the opportunistic physical design; queries can be arbitrarily complex; and, views and queries almost certainly involve UDFs. Unfortunately, previous works do not address the problem in its full generality and essentially ignore one or more of the previous dimensions. 
%<Mini review of previous works.> 
Recent methods to reuse MR computations such as ReStore~\cite{Elgh2012}
and MRShare~\cite{Li2011} lack a semantic understanding of the artifacts 
produced during execution and can only reuse/share cached results when 
execution plans are identical.
We strongly believe that any practical solution has to address the query rewrite problem in its full generality. 

Contributions. In this paper we present a novel query-rewrite algorithm that targets the scenario of opportunistic materialized views within an MR system. The algorithm employs techniques inspired by spatial databases (specifically, nearest-neighbor searches in metric spaces~\cite{Hjal03}) in order to aggressively prune the huge space of candidate rewrites and generate the optimal rewrite in an efficient manner. Specifically, our contributions can be summarized as follows:
%- Gray-box model for UDFs.
%- Rewrite algorithm.
%- Experimental study.
\begin{itemize}
  \item A gray-box UDF model that is simple but expressive enough to capture
  many common types of UDFs.
   This affords us a limited understanding of UDFs to enable effective
   reuse of previous results.  
   We provide the model and the types of UDFs it admits in 
   Section \ref{sec-udf-model}.
  
  \item A rewriting algorithm that takes as input a query and a
   set of views  and outputs the optimal rewrite.  
  We show the algorithm is work-efficient in that it considers the minimal
  set  of views necessary to find the optimal rewrite under 
  certain assumptions.
  We describe this further in Section \ref{sec-best-first-workflow-rewrite}.
  
  \item Experimental results showing our methods provide execution time 
  improvements up to two orders of magnitude using real-world data 
  and realistic complex queries in Section \ref{sec-experimental-evaluation}.  
  The savings from our method are due to moving much less data, 
  avoiding the high expense of re-reading data from raw logs when possible, 
  and reusing/repurposing results from long-running computations 
  including UDFs.
   
\end{itemize}



==> old/Introduction-rewrite8.tex <==
\section{Introduction}
Data analysts have the crucial task of analyzing the ever increasing volume of data that modern organizations collect and producing actionable insights. As expected, this type of analysis is highly exploratory in nature and involves an iterative process: the data analyst starts with an initial query over the data, examines the results, then reformulates the query and may even bring in additional data sources, and so on. Typically, these queries involve sophisticated, domain-specific operations that are linked to the type of data and the purpose of the analysis, e.g., performing sentiment analysis over tweets or computing network influence. 
Because a query is often revised multiple times in this scenario, there can 
be significant overlap between queries.

Not surprisingly, MapReduce (MR) has become a de-facto tool for this type of analysis.
It offers scalability to large datasets, easy incorporation of new data sources, 
the ability to query right away without defining a schema upfront, and extensibility 
through user-defined functions (UDFs).
Analyst queries are often written in a declarative query language, e.g., HiveQL or PigLatin, and then automatically translated to a set of MR jobs for execution.


Despite the popularity of MR systems, query performance remains a critical issue which in turn affects directly the ``speed'' at which data analysts can test a hypothesis and converge to a conclusion. Some gains can be achieved by reducing the overheads of MR, but the key impediment to performance is the inherent complexity of queries that may 
contain UDFs, ingest large datasets, and span several MR jobs. 
A-priori tuning, e.g., by reorganizing or preprocessing the data, is quite 
challenging due to the fluidity and uncertainty of exploratory analysis. 

In this paper, we show that it is possible to dramatically improve query performance by leveraging the built-in fault-tolerance mechanism of MR as an \emph{opportunistic physical design}. Specifically, we make the following observations:
\begin{itemize}
\item Each MR job involves the materialization of intermediate results (the output of mappers, the input of reducers and the output of reducers) for the purpose of failure recovery. More generally, a multi-stage job, such as one that is generated by Pig or Hive, will involve several such materializations. We refer to these materialized results as the artifacts of query execution and note that they are generated automatically as a by-product of query processing. 

\item Given the evolutionary nature of data exploration, it is likely that each query has similarities to previous queries by the same analyst, and even to queries of other analysts who examine the same data. For instance, several data analysts may perform sentiment analysis on a specific class of tweets (e.g., in a specific geographical area) but with a different hypothesis in mind. Hence, the computation performed by previous queries in the system, as captured in the generated artifacts, may be relevant for a new query. 
\end{itemize}
Thus, we propose to treat artifacts as opportunistically-created materialized views and use them to rewrite a new query in the system. The opportunistic nature of our technique has several nice properties: the materialized views are generated as a by-product of query execution, i.e., without additional overhead; the set of views is naturally tailored to the current workload; and, given that large-scale analysis systems typically execute a large number of queries, it follows that there will be an equally large number of materialized views (storage space permitting) 
and hence a good chance of finding a good rewrite for a new query. 
Our results indicate the savings in query execution time can be dramatic: 
a rewrite can reduce execution time by up to two orders of magnitude. 
%Testimonies from analysts using the system suggest that these improvements have contributed to a substantial increase in productivity.

Rewriting a query using views is a well-studied problem in databases, 
yet its treatment in the context of MR involves a unique combination of 
technical challenges: 
queries can be arbitrarily complex; 
views and queries almost certainly involve UDFs; 
and there is a huge search space of rewrites due to the large number of 
materialized views in the opportunistic physical design.
Unfortunately, previous works do not address the problem in its full generality and essentially ignore one or more of the previous dimensions. 
%<Mini review of previous works.> 
Recent methods to reuse MR computations such as ReStore~\cite{Elgh2012}
and MRShare~\cite{Li2011} lack a semantic understanding of the artifacts 
produced during execution and can only reuse/share cached results when 
execution plans are identical.
We strongly believe that any truly effective solution will have to address the query 
rewrite problem in its full generality. 

Contributions. In this paper we present a novel query-rewrite algorithm 
that targets the scenario of opportunistic materialized views within an MR 
system and queries that contain UDFs.
The algorithm employs techniques inspired by spatial databases (specifically, nearest-neighbor searches in metric spaces~\cite{Hjal03}) in order to aggressively prune the huge space of candidate rewrites and generate the optimal rewrite in an efficient manner. Specifically, our contributions can be summarized as follows:
%- Gray-box model for UDFs.
%- Rewrite algorithm.
%- Experimental study.
\begin{itemize}
  \item A gray-box UDF model that is simple but expressive enough to capture
  many common types of UDFs.
   This affords us a limited understanding of UDFs to enable effective
   reuse of previous results.  
   We provide the model and the types of UDFs it admits in 
   Section \ref{sec-udf-model}.
  
  \item A rewriting algorithm that takes as input a query and a
   set of views  and outputs the optimal rewrite.  
  We show the algorithm is work-efficient in that it considers the minimal
  set  of views necessary to find the optimal rewrite under 
  certain assumptions.
  We describe this further in Section \ref{sec-best-first-workflow-rewrite}.
  
  \item Experimental results showing that our methods provide execution time 
  improvements of up to an order of magnitude using real-world data 
  and realistic complex queries in Section \ref{sec-experimental-evaluation}.  
  The savings from our method are due to moving much less data, 
  avoiding the high expense of re-reading data from raw logs when possible, 
  and reusing/repurposing results from long-running computations 
  including UDFs.
   
\end{itemize}



==> old/Introduction.original.tex <==
\section{Introduction}


A knowledge-driven enterprise is one that adopts an aggressive strategy of
instrumenting every aspect of their business, and challenges its
employees to explore and evaluate their intuition against the data to ensure better
outcomes for the customers and the company. This data-driven decision making (DDD) \cite{Bryn2011}
leaves no part of the knowledge-driven enterprise immune to changes as long as there is
sufficient evidence in the data to ``prove'' it. 
Any employee in such an enterprise may play the role of analyst, thus there is a
need for a large-scale, cost-effective analytics platform to support the DDD organization.
These types of analysts within an organization may explore the data via queries 
in a {\em workflow} using a higher level language.
If the result of the workflow exposes deficiencies in existing
processes or exposes potential opportunities for the company, it might then be 
made part of the existing {\em business intelligence} (BI) until it is
replaced by a better workflow.   Often this is the case with new data sources of as-yet
 unknown value.  This process stands in contrast to traditional ETL workflows in that ETL is costly and typically requires 
the knowledge of what is of important business value in the data \emph{apriori}.

{\em Evolutionary query workflows} are those written
by analysts as they test hypotheses on the dataset. 
An evolutionary workflow is called so because the analyst knows the hypothesis
that is to be tested but may be unsure of how to write the workflow
that proves or disproves the hypothesis with high confidence.
Hence, the process of writing the workflow becomes evolutionary in the sense 
that the revisions are often applied based on examining the output of the previous query.
Each version of an evolutionary workflow often becomes more and more complicated
until the desired result is achieved.  This concept has been previously noted in \cite{Khou2009} 
as exploratory queries, or continuously changing queries over log data in an environment outside of 
the traditional database setting.


Commercial data warehouses have mature BI analytics and processes to support firms with analytical reporting to maximize the value of their data.  Considering existing warehouse data along with new types of data sources, here we address the question \textsl{what if organizations do not already know exactly where this value is?} This  scenario is representative of organizations that may be inundated with ever-expanding data and as well as new data sources, of which social media is rapidly becoming a large part, and the distinct value within this data is unknown.  Recently, the role of the Data Scientist \cite{Pati2011} \cite{Fayy2011} has been introduced to identify data value in precisely this scenario.

Higher-level languages such as Hive \cite{Thus2009} and Pig \cite{Olst2008} have emerged enabling simpler access for exploring flat data using an MR execution engine. Furthermore, the trends clearly indicate the emergence and incorporation of such low-structured data in traditional \textit{DBMS} systems including Oracle \cite{Hens2011a}, IBM + Netezza, HP + Vertica, EMC + Greenplum, Microsoft \cite{Lobo2010} \cite{Hens2011b}, and Teradata \cite{Xu2010} +AsterData with `SQL-MapReduce' \cite{Frie2009}, which have expanded (or announced) the inclusion of MR-capabilities within or alongside their native \textit{DBMS}.  Possibly motivated by  blind customer demand for `MR capabilities on Big Data', but also clearly motivated by new data sources such as social media where it is obvious that commercial DBMS as well as their customers are uncertain as to where the BI resides  \cite{Groe2011}  \cite{Xu2010}.  
 These data sources may be  somewhat raw having low-structure, often resembling an append-only LOG, thus some effort must clearly be expended to properly understand, clean, and load this new data via a traditional ETL process.  Because the ETL process can be very expensive \cite{Xu2010}, even constituting a high percentage of the cost of a data warehouse project \cite{Simi2009}, applying this complex process to data of unknown value becomes a somewhat risky proposition.  However, if value can be identified within and possibly across new data sources, then traditional  (and costly) ETL methods might be successfully argued for and later applied to that specific data identified as having value.  

\begin{itemize}
\item graph of 3 dimensions here.
\item LOGs have low-structure and are append-only.  relevant examples include clickstream data, sensor data, social media data, telephony data, etc..
\item commodity storage is cheap, about \$0.04/GB
\item other query systems such as hive, pig, and tenzing enable exploration over flat files with \emph{MR} but not seamless answer re-use.  clearly answer re-use is beneficial as Facebook stores all internal user's Hive answers for one week \cite{XX} need ref here.  maybe mention ReStore as an example in this direction
\end{itemize}

\textbf{In this work we propose a system to support answer re-use in evolutionary query workflows.}  Toward this end we introduce an analytical platform and succinct (minimalistic?) data model for performing 
evolutionary queries on large-scale data that speeds up computation by identifying similarities between successive
versions of an evolutionary query issued by a user as well as similarities to evolutionary queries issued by other users in the system.

\begin{itemize}
\item specific contributions here from todays discussion, some of these do not belong in the contributions section, but maybe above.
\item a minimalistic model for describing answers that enables re-use, in contrast to describing answers with fine-grained (tuple-level) data provenance, or a set of queries or even workflow provenance, \textit{(how did i get here vs. what i am)}.  maybe mention provenance size being several times the data size, cite a paper, lipstick on a pig, or identical result reuse such as ReStore.
\item we identify trends (on dimensions above) and describe evolutionary queries.  these do not appear to be captured by tpc benchmarks, and are not directly captured by scientific workflows, nor pig-mix benchmark...
\item emergence of the specialized role of data scientist and organizations are moving toward enabling all employees to be data scientists.  extract value from new data sources such as social media, etc...
\item show how to incorporate answer re-use over log data.  etls costly given usefulness of the data unknown vs. low barrier to entry.  our system enables anyone's exploration of the data to potentially make other's exploration more efficient.
\item a simple viewfinder, with a best-first exploration of useful views.
\item cost-effective workflow plumbing algorithm, also best-first nature.
\end{itemize}
 
It is interesting to note that the result of a workflow $W$ 
may not produce the \textit{desired} answer from the user's point of view.  
As is expected in our use-case, the user lacks the understanding of the data to be able to initially translate his intent to a workflow.
Therefore it is not uncommon for $W$ to be reformulated as $W'$ as the user gains a better understanding of the data.  

Note that $W$ does not necessarily represent wasted work, as $W$ was a necessary exercise for the user to make sense of the data, although 
each evolution of the workflow represents significant time investment for the user given the potentially large data sets involved. 

The ability of an organization to produce useful \emph{BI} is directly tied to the speed which a user can iterate through successive investigations of the data \cite{XX}. 
 Given these iterations are unavoidable in our context, our proposed system provides a means to improve the speed of these iterations for a single user 
posing $W'$ by reusing previous work from $W$.  
Moreover, our design enables $W'$ to benefit from previous work done by other user's workflows in the system. 
We attempt to quantify this effect later in experiment X. 



==> old/Introduction.tex <==
\section{Introduction}
 
A knowledge-driven enterprise adopts an aggressive strategy of
instrumenting every aspect of their business and encourages
the employees to find value in the large amount of
raw data collected from vastly diverse sources.
Data-driven decision making (DDD) \cite{Bryn2011}
leaves no part of the knowledge-driven enterprise
immune to change as long as there is
sufficient evidence in the data to support it. 
Recently the role of the {\em data scientist}
has been introduced to help organizations identify 
value in their data ~\cite{Pati2011}.
Preferably any employee in such an enterprise may play the role of
data analyst, thus there is a need for a 
cost-effective analytics platform to support the DDD organization.
%ok, sounds good, but i already know all of this. are you saying something different? if so, then how does this analysis look?
Analysts typically express their data exploration in the 
form of \emph{workflows}, consisting of individual data
access and processing steps. 
The nature of these data explorations begins with
an analyst making a guess and then posing subsequent 
questions, continually revising or \emph{evolving}
the workflow as his intuition leads him toward the desired results.
As analysts are often uncertain about the value of the data
and the best process to identify this value, 
an analytics platform should be able to adapt to the needs of 
many users exploring large diverse data sets.

A platform to support such data explorations should enable users to 
1) perform increasingly sophisticated analysis 
as they gain better understanding of the data, 
2) automatically benefit from analysis performed by other analysts, 
and 
3) easily add new data sources for their analysis. 
We call a platform that supports these three dimensions 
an {\em Evolutionary Analytics System}, 
that supports {\em Workflow Evolution}, {\em User Evolution}, 
and {\em Data Evolution} to meet these three requirements, respectively.
Specifically, workflow evolution is defined as a single analyst adjusting,
modifying, and re-purposing a workflow to better align the results of the workflow
to match the analyst's intent.
User evolution is defined as new analysts arriving that begin querying the
system with new workflows. 
Data evolution is defined as the process of an analyst
adding a new data source to the system. 
The following scenario is an
example of these three evolutionary dimensions:
 
\begin{example}
An analyst wants to identity 100 wine lovers so that he can
send them a coupon for a new wine being introduced in the market.
The evolution of this scenario will investigate
increasingly sophisticated ways of finding out 
if a user is a ``wine lover'' from a
single social networking data source.
Furthermore the analyst may want to make use of
an additional data source, e.g., Foursquare location check-ins,
to obtain more evidence that a user likes wine.
Next, another analyst arrives and wants to identify people
that frequently go to the movies.
She may benefit from some of the answers materialized as part of
the previous analyst's data exploration
such as unique users, their friends, and locations they
check-in to.
\end{example}


An {\em evolutionary analytics workflow} is a query written
by an analyst as she iteratively explores the data. 
The result of an evolutionary workflow $W$ 
may not initially produce the desired answer
as the user lacks sufficient understanding of the data to be able 
to translate his intent to a workflow.
Therefore it is to be expected that  $W$ will 
be reformulated as a new workflow $W'$, and this process repeats.
Note that $W$ does not necessarily represent wasted work, 
since it was a necessary exercise for the user to 
gain better understanding of the data.
This iterative process is time consuming as
workflow revisions are driven by examining the previous results.
Thus the ability of an organization to discover value in the data
is dependent on the speed at which a single analyst
can iterate through successive investigations of the data 
as well as the benefit the analyst derives from 
previous work performed by others. 
Furthermore an analyst should be able to easily add new data sources for 
investigation without incurring the expense of a formal ETL process
which can be very expensive, often consuming a high percentage of the cost
of a data warehouse project~\cite{Simi2009}.
Analysts typically express their workflows using a 
high level language, and often apply sophisticated
operations such as text sentiment,
network influence, classification, etc. 
These sophisticated -- and usually domain
specific -- operations can be formulated as User Defined Functions ({\em UDFs}). 

  
%Analysts in these organizations may explore the data using queries
%expressed as {\em workflows} in a high level language, and often
%apply complex operations such as text sentiment,
%network influence, classification, etc.
%A workflow is expressed as a DAG of queries.
%Complex operations are captured by UDFs
%developed by the analyst and used across the organization.
%Recently the role of the data scientist~\cite{Pati2011}
%has been introduced to help organizations identify value
%in their data.

We propose an evolutionary analytics system that supports 
these three dimensions through
\emph{rewriting}
workflows to improve performance.
A key technical challenge in realizing such a system is 
efficiently rewriting the user workflows in a way that effectively 
exploits the results of other workflows from all 
users in the system even as users flexibly
change their workflow structure, 
apply sophisticated functions (UDFs), 
and include additional data sets. 
We address this by formulating it as a query rewrite problem using views  
for evolutionary workflows that may include complex arbitrary UDFs. 
We are not aware of any known work on rewriting such workflows, 
although some recent work~\cite{Hues2012, Simi2009} has addressed optimizing workflows 
with UDFs.
Our contributions are as follows.
 
\begin{itemize}\setlength{\itemsep}{1pt}\setlength{\parsep}{0pt}
  \item A workflow rewriting algorithm \WF{} that finds
  the optimal rewrite of an evolutionary workflow in
  a work-efficient manner.
  WFR{} is work-efficient as it examines only the views that may potentially produce an optimal
  rewrite, but never examines a view that cannot.
  
  \item An optimistic cost function \ocost{} that provides a lower
  bound on the cost of a rewrite using a given view.  This
  functionality enables the workflow rewrite algorithm to
  incrementally search the space of rewrites.

  \item A gray-box model of a UDF that is expressive yet
  conducive to rewrites.
  This allows any user to add a UDF to the system,
  and the system operator may choose to extend the rewrite language
  to include the UDF.
 
  %\item A set of 8 evolutionary workflows representing realistic scenarios,
 % where each workflow has 4 evolutions resulting in 32 workflows.
  %These types of queries do not appear to be captured by current benchmarks,
  %and we present them as a first step toward a benchmark for evolutionary
  %workflows.
 
  \item A \emph{microbenchmark} to capture and evaluate the flexibility an
analyst has  in revising analytical workflows.
 
  \item Extensive experimental results over large, real data sets and
comprehensive, realistic use-case scenarios that show our rewrites result 
in up to 90\% improvement in workflow execution time, 
 as well as a significant reduction in the rewrite search space considered 
 by our algorithm.
 
 %and the superiority over   
  %reduce workflow execution time by 10\%--90\%
 % and our workflow rewrite algorithm searches much less of the space to
  %find the optimal rewrite than a bottom-up approach.
 
\end{itemize}
 
 


==> old/Preliminaries-rewrite0.tex <==
\section{Preliminaries}\label{sec-preliminaries}
Here we present the architecture of our system
and briefly describe its individual components and how they interact.
Then we describe our cost model and definitions.


\subsection{System Architecture}\label{sec-system-architecture}
Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of the system we have implemented.

\onefig{fig-odyssey-system-diagram}
{System diagram of Odyssey that shows control flows}{3.25in}
%% New outline.
%%Input Q.
%%Q goes to optimizer.
%%optimizer returns physical plan, representing by MR jobs.
%We annotate each job in the plan with the operators to which it corresponds.\
%%We annotate jobs in the plan using our UDF model (Section~\ref{sec-udf-model})
%%A single UDF can correspond to mulitple jobs.
%We parallelize the annotated plan based on data dependencies.
%We use oozie workflow coordinator to handle parallel execution of jobs.
%Each node is an MR job.
%I would encourage you to restructure the text to be more narrative instead of essentially using bullets. E.g.,

We assume that the analyst submits a query $q$ in some declarative query language, 
which is then translated to an execution plan by a query optimizer. 
We treat the optimizer as a black-box provided by the execution engine, 
that returns a plan and its expected cost for an input query.
Our rewriter, presented in Section~\ref{sec-best-first-workflow-rewrite},
utilizes the optimizer to obtain a plan and estimated cost for a candidate rewrite during its search of the space of rewrites 
given the views in our system.
Once the rewriter is finished with its search, it selects a rewrite to forward to the execution engine.
During query execution, all by-products of query processing are retained as opportunistic 
materialized views, and stored in the system becoming part of its opportunistic 
physical design configuration.
A primary data source in our scenario are large logs, which can
have a high extraction cost when the data is flat with low structure.
Extraction can include unpacking (deserializing), formatting, type-checking, re-encoding,
and tokenizing, to name a few.
One of the motivations for our system to retain processed log data as materialized views is to
 avoid re-extraction from logs when possible due to this high cost.
The materialized view metadata store contains information about the existing materialized views 
and base data currently in the system such as the view definitions, and standard data statistics used in query optimization.



\subsection{Definitions}
We use $W$ to denote a plan generated by the query optimizer,
represented as a DAG containing $n$ nodes and is ordered topologically.
$W_i$ is a sub-graph that contains all vertices up to and including $i$, $i \in [1,n]$.
We refer to $W_i$ as one of the rewritable \emph{targets} of plan $W$.
A property of $W_i$ is that it represents a materialization point in plan $W$.
\node{k} corresponds to the $i^{th}$ vertex of $W$.
An outgoing edge from \node{j} to \node{k} represents data flow from $j$ to $k$.
%The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which is a cost estimate provided by the query optimizer.
We make two assumptions about the optimizer, first that it can provide
a cost estimate for relational operators, and second that it can provide a cost
estimate for a UDF.
The optimizer considers execution plans for
$q$ and returns the cheapest plan that implements $q$ and the plan's cost estimate.
\cost(\node{k}) is the cost of the physical operator at \node{k}, given its input data,
and \cost($W_i$) $ = \sum_{\forall \node{k} \in W_i} \cost(\node{k})$.

$V$ is the set of all existing materialized views (MVs) in the system.
%corresponding to the artifacts from prior execution runs.
\textit{Candidate views} $C$ are those views that rewriter component considers for rewriting a target $W_i$.
$C$ may include all views in $V$ and additional views created by merging views in $V$ to create new views.
Additional views are created using a \textsc{merge} function 
(Section~\ref{sec-viewfinder}) that can apply a standard view-merging procedure 
(e.g.,~\cite{Agra2000,Hale2001}).


$L_W$ represents the language of the queries, which is also the language of the views,
and $L_R$ represents the rewrite language.
Queries may contain UDFs, and thus $L_W$ includes any UDF admitted to the system
by our UDF model (presented in Section~\ref{sec-udf-model}).
$L_R$ represents the transformation rules used during rewriting.
In this implementation, $L_R$ includes select, project, join, groupby, and aggregation (SPJGA).
%$L_R$ does not contain UDFs, thus is a subset of $L_W$.
$L_R \subseteq L_W$ indicates that the rewrite language is less expressive than the query language.


A rewrite $r$, is an equivalent rewrite of target $W_i$ using only candidate views.
$r$ is considered an equivalent rewrite of $W_i$ \textsl{iff}
it produces an identical output to $W_i$ given the same database instance $D$.
A rewrite $r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
%In this work we only consider equivalent rewrites.



\subsection{C\fakesc{ost} Function -- oldversion}

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which corresponds to a cost estimate provided by the query optimizer
(see Figure~\ref{fig-odyssey-system-diagram}).
We make two assumptions about the optimizer, first that it can provide
a cost estimate for relational operators, and second that it can provide a cost
estimate for a UDF.
The optimizer considers execution plans for
$q$ and returns the cost of the cheapest plan that implements $q$.
%We while require the query optimizer to estimate the cost of applying a UDF,
%we recognize that its ability to reorder and push-down UDFs may be very limited.
%A further optimization that the query optimizer considers is to combine operations,
%thereby amortizing their combined cost.
The ability to cost a query is required by our rewriter (Section~\ref{sec-best-first-workflow-rewrite}),
as it searches for rewrites considering the available views.

Thus we assume the following weak property about the nature of the
operations and the $\cost{}$ function, which forms the basis of
our \ocost{} presented in Section~\ref{sec-viewfinder}.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be a set of operations \sout{drawn from the three operations
given by the UDF model}{\small --This is not defined yet, which leaves `operations' under-specified at this point, 
what do you think?--}.
Let $\cost(S,D)$ be defined as the total cost of performing all operations in $S$, on database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
Taking the minimum cost of an operation in $S$ provides a lower bound on the
cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must assume the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter $F$
with high selectivity and a group-by operation $G$ with higher cost than $F$
when considering the operations independently on database $D$.
Let $S'$ contain only $G$.
Suppose that applying $F$ before $G$ results in few or no tuples streamed to $G$.
Then applying $G$ can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.



\subsection{UDF Model}\label{sec-udf-model}

Workflows commonly include complex analytical operations expressed as UDFs, thus
our system requires a way to model them semantically.
UDFs may be modeled using a white, grey, or black box approach with varying levels
of overhead and complexity to the system.
A white box approach requires a complete description of the UDF so that the system
understands \textit{how} the UDF transforms the inputs.
This is too much of an overhead for an analyst adding a new UDF to the system.
A black box approach produces an output that is completely opaque to the
system (similar to a stored procedure)
thus may not be suitable for our goal of reusing results.
Since UDFs can involve fairly complex operations on the data, our system adopts a gray-box approach
that only captures the \textit{end-to-end transformations} performed by a UDF.
This requires little overhead when adding a new UDF, yet
allows the system to understand the UDF's transformations in a useful way.
Alternatively, a method such as \cite{Hues2012} could be applied to automatically extract
some of the semantic properties of the UDFs we are interested in capturing,
thereby reducing the burden on the user.
The end-to-end transformations allowed by our gray-box model are limited to the following operations.

%%Given an input $I$ the end to end transformation allowed by our model are limited to the following
%%operations on $I$ to produce and output $O$.

\vspace{-0.05in}
\begin{enumerate}
\setlength{\itemsep}{3pt}%
\setlength{\parskip}{0mm}%
\item Discard or add attributes, e.g., \textsc{projection, aggregate, sentiment-score, word-count}, etc.
\item Discard tuples, e.g., \textsc{filter}
\item Perform grouping of tuples, e.g., \textsc{groupby}
\end{enumerate}
\vspace{-0.01in}

Given these operations, our UDF model only captures the end-to-end transformation from
an input $I$ to an output $O$
as reflected by the change in attributes, the addition of filters, and the change in group-by.

Accordingly,
$I$ is expressed as a set $A$ of attributes, a set $F$ of filters, and the current grouping $G$ of attributes.
After applying any end-to-end transformation,
$O$ is expressed as a set $A$ of attributes (additional or fewer than $I$), a conjunction of
the filters $F$ in $I$ and any additional filters applied, and any re-grouping $G$ of attributes.

If any new attributes are produced, then those attributes in $O$ record their dependency on $I$
as small signature containing the required
attributes in $I$, the Filters in $I$, and Groupby
of $I$. For uniqueness the signature also includes the UDF name, and an optional modifier
(e.g., $k$ in \textsc{top-k}).
Note there is no facility to update attributes in place, which is not unreasonable here given
that our primary data source is logs.
Any modification to a required attribute in $I$ is recorded as a new attribute.


\begin{example}\label{ex-food-sentiment}
UDF implementation:
For each user, gather all of their tweets.
%Discard those tweets that do not refer to food or any of its closely related terms.
Apply a classifier that determines if a tweet refers to food or a closely-related concept,
and then computes a food sentiment score for each user.
Output only those users with score above a given threshold.
The UDF Model for this UDF is given by:  \\
Inputs: required-attrs<\texttt{userid}, \texttt{tweet}>, modifier<$t$ (threshold)>,
 UDF-name<\texttt{FOOD-SENTIMENT}>\\
Output: new-attribute<\texttt{score}>, add-filter<\texttt{`score > $t$'}>, re-groupby<\texttt{userid}>
\end{example}

Suppose that $I$ is represented by $A$=\{\texttt{userid}, \texttt{tweet}, \texttt{tweetid}\},
$F$=$\emptyset$, and $G$=$\emptyset$.
After invoking the example UDF with $t$=0.5, output $O$ is represented by
$A$=\{\texttt{userid}, \texttt{score}\},
with $F$=\{\texttt{`score > $0.5$'}\},
and $G$=\{\texttt{userid}\}.
The new attribute \texttt{score} has a unique signature that is dependent on $I$ and is given by
required-attrs<\texttt{userid}, \texttt{tweet}>,
%%$\{\texttt{userid}, \texttt{tweet}\}$,
$F$=$\emptyset$, $G$=$\emptyset$, $t$, and \texttt{FOOD-SENTIMENT}.
This signature is a minimal form of provenance that captures a functional dependency on its immediate inputs.

UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured using our model
can be \emph{admitted} to the system.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two identical UDFs with different names, their new attributes will result in different signatures.
This deficiency can only be overcome if we resort to a white-box approach.




==> old/Preliminaries-rewrite1.tex <==
\section{Preliminaries}\label{sec-preliminaries}
Here we present the architecture of our system
and briefly describe its individual components and how they interact.
Then we describe our cost model and definitions.


\subsection{System Architecture}\label{sec-system-architecture}
Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of the system we have implemented.

\onefig{fig-odyssey-system-diagram}
{System diagram of Odyssey that shows control flows}{3.25in}
%% New outline.
%%Input Q.
%%Q goes to optimizer.
%%optimizer returns physical plan, representing by MR jobs.
%We annotate each job in the plan with the operators to which it corresponds.\
%%We annotate jobs in the plan using our UDF model (Section~\ref{sec-udf-model})
%%A single UDF can correspond to mulitple jobs.
%We parallelize the annotated plan based on data dependencies.
%We use oozie workflow coordinator to handle parallel execution of jobs.
%Each node is an MR job.
%I would encourage you to restructure the text to be more narrative instead of essentially using bullets. E.g.,

We assume that the analyst submits a query $q$ in some declarative query language, 
which is then translated to an execution plan by a query optimizer. 
We treat the optimizer as a black-box provided by the execution engine, 
that returns a plan and its expected cost for an input query.
Our rewriter, presented in Section~\ref{sec-best-first-workflow-rewrite},
utilizes the optimizer to obtain a plan and estimated cost for a candidate rewrite during its search of the space of rewrites 
given the views in our system.
Once the rewriter is finished with its search, it selects a rewrite to forward to the execution engine.
During query execution, all by-products of query processing are retained as opportunistic 
materialized views, and stored in the system becoming part of its opportunistic 
physical design configuration.
A primary data source in our scenario are large logs, which can
have a high extraction cost when the data is flat with low structure.
Extraction can include unpacking (deserializing), formatting, type-checking, re-encoding,
and tokenizing, to name a few.
One of the motivations for our system to retain processed log data as materialized views is to
 avoid re-extraction from logs when possible due to this high cost.
The materialized view metadata store contains information about the existing materialized views 
and base data currently in the system such as the view definitions, and standard data statistics used in query optimization.



\subsection{Definitions}
We use $W$ to denote a plan generated by the query optimizer,
represented as a DAG containing $n$ nodes and is ordered topologically.
$W_i$ is a sub-graph that contains all vertices up to and including $i$, $i \in [1,n]$.
We refer to $W_i$ as one of the rewritable \emph{targets} of plan $W$.
A property of $W_i$ is that it represents a materialization point in plan $W$.
\node{k} corresponds to the $i^{th}$ vertex of $W$.
An outgoing edge from \node{j} to \node{k} represents data flow from $j$ to $k$.
%The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which is a cost estimate provided by the query optimizer.
We make two assumptions about the optimizer, first that it can provide
a cost estimate for relational operators, and second that it can provide a cost
estimate for a UDF.
The optimizer considers execution plans for
$q$ and returns the cheapest plan that implements $q$ and the plan's cost estimate.
\cost(\node{k}) is the cost of the physical operator at \node{k}, given its input data,
and \cost($W_i$) $ = \sum_{\forall \node{k} \in W_i} \cost(\node{k})$.

$V$ is the set of all existing materialized views (MVs) in the system.
%corresponding to the artifacts from prior execution runs.
\textit{Candidate views} $C$ are those views that rewriter component considers for rewriting a target $W_i$.
$C$ may include all views in $V$ and additional views created by merging views in $V$ to create new views.
Additional views are created using a \textsc{merge} function 
(Section~\ref{sec-viewfinder}) that can apply a standard view-merging procedure 
(e.g.,~\cite{Agra2000,Hale2001}).


$L_W$ represents the language of the queries, which is also the language of the views,
and $L_R$ represents the rewrite language.
Queries may contain UDFs, and thus $L_W$ includes any UDF admitted to the system
by our UDF model (presented in Section~\ref{sec-udf-model}).
$L_R$ represents the transformation rules used during rewriting.
In this implementation, $L_R$ includes select, project, join, groupby, and aggregation (SPJGA).
%$L_R$ does not contain UDFs, thus is a subset of $L_W$.
$L_R \subseteq L_W$ indicates that the rewrite language is less expressive than the query language.


A rewrite $r$, is an equivalent rewrite of target $W_i$ using only candidate views.
$r$ is considered an equivalent rewrite of $W_i$ \textsl{iff}
it produces an identical output to $W_i$ given the same database instance $D$.
A rewrite $r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
%In this work we only consider equivalent rewrites.



\subsection{C\fakesc{ost} Function -- oldversion}

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which corresponds to a cost estimate provided by the query optimizer
(see Figure~\ref{fig-odyssey-system-diagram}).
We make two assumptions about the optimizer, first that it can provide
a cost estimate for relational operators, and second that it can provide a cost
estimate for a UDF.
The optimizer considers execution plans for
$q$ and returns the cost of the cheapest plan that implements $q$.
%We while require the query optimizer to estimate the cost of applying a UDF,
%we recognize that its ability to reorder and push-down UDFs may be very limited.
%A further optimization that the query optimizer considers is to combine operations,
%thereby amortizing their combined cost.
The ability to cost a query is required by our rewriter (Section~\ref{sec-best-first-workflow-rewrite}),
as it searches for rewrites considering the available views.

Thus we assume the following weak property about the nature of the
operations and the $\cost{}$ function, which forms the basis of
our \ocost{} presented in Section~\ref{sec-viewfinder}.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be a set of operations \sout{drawn from the three operations
given by the UDF model}{\small --This is not defined yet, which leaves `operations' under-specified at this point, 
what do you think?--}.
Let $\cost(S,D)$ be defined as the total cost of performing all operations in $S$, on database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
Taking the minimum cost of an operation in $S$ provides a lower bound on the
cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must assume the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter $F$
with high selectivity and a group-by operation $G$ with higher cost than $F$
when considering the operations independently on database $D$.
Let $S'$ contain only $G$.
Suppose that applying $F$ before $G$ results in few or no tuples streamed to $G$.
Then applying $G$ can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.



\subsection{UDF Model}\label{sec-udf-model}

Workflows commonly include complex analytical operations expressed as UDFs, thus
our system requires a way to model them semantically.
UDFs may be modeled using a white, grey, or black box approach with varying levels
of overhead and complexity to the system.
A white box approach requires a complete description of the UDF so that the system
understands \textit{how} the UDF transforms the inputs.
This is too much of an overhead for an analyst adding a new UDF to the system.
A black box approach produces an output that is completely opaque to the
system (similar to a stored procedure)
thus may not be suitable for our goal of reusing results.
Since UDFs can involve fairly complex operations on the data, our system adopts a gray-box approach
that only captures the \textit{end-to-end transformations} performed by a UDF.
This requires little overhead when adding a new UDF, yet
allows the system to understand the UDF's transformations in a useful way.
Alternatively, a method such as \cite{Hues2012} could be applied to automatically extract
some of the semantic properties of the UDFs we are interested in capturing,
thereby reducing the burden on the user.
The end-to-end transformations allowed by our gray-box model are limited to the following operations.

%%Given an input $I$ the end to end transformation allowed by our model are limited to the following
%%operations on $I$ to produce and output $O$.

\vspace{-0.05in}
\begin{enumerate}
\setlength{\itemsep}{3pt}%
\setlength{\parskip}{0mm}%
\item Discard or add attributes, e.g., \textsc{projection, aggregate, sentiment-score, word-count}, etc.
\item Discard tuples, e.g., \textsc{filter}
\item Perform grouping of tuples, e.g., \textsc{groupby}
\end{enumerate}
\vspace{-0.01in}

Given these operations, our UDF model only captures the end-to-end transformation from
an input $I$ to an output $O$
as reflected by the change in attributes, the addition of filters, and the change in group-by.

Accordingly,
$I$ is expressed as a set $A$ of attributes, a set $F$ of filters, and the current grouping $G$ of attributes.
After applying any end-to-end transformation,
$O$ is expressed as a set $A$ of attributes (additional or fewer than $I$), a conjunction of
the filters $F$ in $I$ and any additional filters applied, and any re-grouping $G$ of attributes.

If any new attributes are produced, then those attributes in $O$ record their dependency on $I$
as small signature containing the required
attributes in $I$, the Filters in $I$, and Groupby
of $I$. For uniqueness the signature also includes the UDF name, and an optional modifier
(e.g., $k$ in \textsc{top-k}).
Note there is no facility to update attributes in place, which is not unreasonable here given
that our primary data source is logs.
Any modification to a required attribute in $I$ is recorded as a new attribute.


\begin{example}\label{ex-food-sentiment}
UDF implementation:
For each user, gather all of their tweets.
%Discard those tweets that do not refer to food or any of its closely related terms.
Apply a classifier that determines if a tweet refers to food or a closely-related concept,
and then computes a food sentiment score for each user.
Output only those users with score above a given threshold.
The UDF Model for this UDF is given by:  \\
Inputs: required-attrs<\texttt{userid}, \texttt{tweet}>, modifier<$t$ (threshold)>,
 UDF-name<\texttt{FOOD-SENTIMENT}>\\
Output: new-attribute<\texttt{score}>, add-filter<\texttt{`score > $t$'}>, re-groupby<\texttt{userid}>
\end{example}

Suppose that $I$ is represented by $A$=\{\texttt{userid}, \texttt{tweet}, \texttt{tweetid}\},
$F$=$\emptyset$, and $G$=$\emptyset$.
After invoking the example UDF with $t$=0.5, output $O$ is represented by
$A$=\{\texttt{userid}, \texttt{score}\},
with $F$=\{\texttt{`score > $0.5$'}\},
and $G$=\{\texttt{userid}\}.
The new attribute \texttt{score} has a unique signature that is dependent on $I$ and is given by
required-attrs<\texttt{userid}, \texttt{tweet}>,
%%$\{\texttt{userid}, \texttt{tweet}\}$,
$F$=$\emptyset$, $G$=$\emptyset$, $t$, and \texttt{FOOD-SENTIMENT}.
This signature is a minimal form of provenance that captures a functional dependency on its immediate inputs.

UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured using our model
can be \emph{admitted} to the system.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two identical UDFs with different names, their new attributes will result in different signatures.
This deficiency can only be overcome if we resort to a white-box approach.




==> old/Preliminaries-rewrite2.tex <==
\section{Preliminaries}\label{sec-preliminaries}
Here we present the architecture of our system
and briefly describe its individual components and how they interact, 
followed by our definitions.


\subsection{System Architecture}\label{sec-system-architecture}
\onefig{fig-odyssey-system-diagram}
{System diagram of Odyssey that shows control flows}{3.25in}
%% New outline.
%%Input Q.
%%Q goes to optimizer.
%%optimizer returns physical plan, representing by MR jobs.
%We annotate each job in the plan with the operators to which it corresponds.\
%%We annotate jobs in the plan using our UDF model (Section~\ref{sec-udf-model})
%%A single UDF can correspond to mulitple jobs.
%We parallelize the annotated plan based on data dependencies.
%We use oozie workflow coordinator to handle parallel execution of jobs.
%Each node is an MR job.
%I would encourage you to restructure the text to be more narrative instead of essentially using bullets. E.g.,
Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of the system we have implemented.
We assume that an analyst submits a query $q$ in some declarative query language, 
which is then translated to an execution plan by a query optimizer. 
The optimizer outputs a plan and its expected cost for an input query.
The execution plan is for an MR engine, and represents a sequence of MR jobs.
We treat the optimizer as a black-box provided by the execution engine.

Our rewriter takes the plan generated by the optimizer, and searches for a rewrite of the plan
using the materialized views in the system.
The rewriter, presented in Section~\ref{sec-best-first-workflow-rewrite},
utilizes the optimizer to obtain a plan and estimated cost for a candidate rewrite during its search of the space of rewrites 
given the views in our system.
Once the rewriter is finished with its search, it selects a rewrite to forward to the execution engine.

During query execution, all by-products of query processing are retained as opportunistic 
materialized views, and stored in the system becoming part of its opportunistic 
physical design configuration.
The materialized view metadata store contains information about the materialized views 
currently in the system such as the view definitions, and standard data statistics used in query optimization.
The base data in our system consists of large logs.


\subsection{Definitions}
We use $W$ to denote a plan generated by the query optimizer,
represented as a DAG containing $n$ nodes and is ordered topologically.
Each node  represents an MR job.
The plan has a single sink that computes the result of the query.
Under the topological order assumption, this is node $n$.
$W_i$ is a sub-graph that contains all nodes up to and including $i$, $i \in [1,n]$.
We refer to $W_i$ as one of the rewritable \emph{targets} of plan $W$.
A property of $W_i$ is that it represents a materialization point in plan $W$.
\node{k} corresponds to the $i^{th}$ vertex of $W$.
An outgoing edge from \node{j} to \node{k} represents data flow from $j$ to $k$.

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which is a cost estimate provided by the query optimizer.
We make two assumptions about the optimizer, first that it can provide
a cost estimate for relational operators, and second that it can provide a cost
estimate for a UDF.
\cost(\node{k}) is the cost of the MR job at \node{k}, given its input data.
\cost($W_i$) $ = \sum_{\forall \node{k} \in W_i} \cost(\node{k})$.

$V$ is the set of all existing materialized views (MVs) in the system.
%corresponding to the artifacts from prior execution runs.
%\textit{Candidate views}  are those views that rewriter component considers for rewriting a target $W_i$.
%Candidate views includes all views in $V$ and additional views created by merging views in $V$ to create new views.
%Additional views are created using a \textsc{merge} function 
%(Section~\ref{sec-viewfinder}) that can apply a standard view-merging procedure (e.g.,~\cite{Agra2000,Hale2001}).


$L_W$ represents the language of the queries, which is the declarative query language used by an analyst.
This is also the language of the views.
Queries may contain UDFs, and thus $L_W$ includes any UDF admitted to the system
by our UDF model (presented in Section~\ref{sec-udf-model}).

$L_R$ represents the rewrite language.
This includes only the transformation rules used during rewriting, 
i.e., when searching for a valid rewrite of a query using views.
$L_R$ includes select, project, join, groupby, and aggregation (SPJGA).
%$L_R$ does not contain UDFs, thus is a subset of $L_W$.
$L_R \subset L_W$ indicates that the rewrite language is less expressive than the query language.
This implies that it might not be possible to find an equivalent rewrite of a query in $L_W$ using the 
transformation rules in $L_R$ and the available views.


A rewrite $r$ is an equivalent rewrite of target $W_i$ using only candidate views.
$r$ is considered an equivalent rewrite of $W_i$ \textsl{iff}
it produces an identical output to $W_i$ given the same database instance $D$.
A rewrite $r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
%In this work we only consider equivalent rewrites.



==> old/Preliminaries-rewrite3.tex <==
\section{Preliminaries}\label{sec-preliminaries}
Here we present the architecture of our system
and briefly describe its individual components and how they interact, 
followed by our definitions.

\subsection{System Architecture}\label{sec-system-architecture}
\onefig{fig-odyssey-system-diagram}
{System diagram of Odyssey that shows control flows}{3.25in}

Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of the system we have implemented.
We assume that an analyst submits a query $q$ in some declarative query 
language, which is then translated to an execution plan by a query optimizer.
The optimizer outputs a plan and its expected cost for an input query.
The execution plan is for an MR engine, and represents a sequence of MR jobs.
We treat the optimizer as a black-box provided by the execution engine.

Our rewriter takes the plan generated by the optimizer, and searches for a 
low-cost rewrite of the plan using the materialized views in the system.
The rewriter, presented in Section~\ref{sec-best-first-workflow-rewrite},
utilizes the optimizer to obtain a plan and estimated cost for a candidate 
rewrite during its search of the space of rewrites given the views 
in our system.
Once the rewriter is finished with its search, it selects a rewrite to forward
 to the execution engine.

During query execution, all by-products of query processing are retained 
as opportunistic 
materialized views, and stored in the system becoming part of its 
opportunistic physical design configuration.
The materialized view metadata store contains information about the
materialized views 
currently in the system such as the view definitions, and standard data 
statistics used in query optimization.
The base data in our system consists of large logs.


\subsection{Definitions}
We use $W$ to denote a plan generated by the query optimizer,
represented as a DAG containing $n$ nodes, ordered topologically.
Each node represents an MR job.
We denote the $i^{th}$ node of $W$ as \node{i}, $i \in [1,n]$.
The plan has a single sink that computes the result of the query.
Under the topological order assumption, this is \node{n}.
%$W_i$ is a sub-graph that contains all nodes up to and including \node{i}.
$W_i$ is a sub-graph of $W$ containing \node{i} and all ancestor nodes of 
\node{i} in $W_i$.
We refer to $W_i$ as one of the rewritable \emph{targets} of plan $W$.
A property of $W_i$ is that it represents a materialization point in plan $W$.
%\node{i} corresponds to the $i^{th}$ node of $W$.
An outgoing edge from \node{k} to \node{i} represents data flow 
from $k$ to $i$.

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which is a cost estimate provided by the query optimizer.
We make several assumptions about the optimizer, first that it can provide
a cost estimate for relational operators, and second that it can provide a cost
estimate for a UDF, and third that it cannot do a very good job of optimizing
a query containing UDFs.
\cost(\node{i}) is the cost of the MR job at \node{i}, given its input data.
\cost($W_i$) $ = \sum_{\forall \node{k} \in W_i} \cost(\node{k})$.

$V$ is the set of all existing materialized views (MVs) in the system.
%corresponding to the artifacts from prior execution runs.
%\textit{Candidate views}  are those views that rewriter component considers 
%for rewriting a target $W_i$.
%Candidate views includes all views in $V$ and additional views created by 
%merging views in $V$ to create new views.
%Additional views are created using a \textsc{merge} function 
%(Section~\ref{sec-viewfinder}) that can apply a standard view-merging 
%procedure (e.g.,~\cite{Agra2000,Hale2001}).

$L_W$ represents the language of the queries, which is the declarative query
language used by an analyst when submitting a query to our system.
This is also the language of the views.
Queries may contain UDFs, and thus $L_W$ includes any UDF admitted to 
the system by our UDF model (presented in Section~\ref{sec-udf-model}).

$L_R$ represents the rewrite language.
This includes only the transformation rules used during rewriting, 
i.e., when searching for a valid rewrite of a query using views.
The transformation rules in $L_R$ are: select, project, join, 
group-by, and aggregation (SPJGA).
However, our system is designed to easily extend $L_R$ by including
new rules (e.g., UDFs from $L_W$) without changing our techniques.
%$L_R$ does not contain UDFs, thus is a subset of $L_W$.
$L_R \subseteq L_W$ indicates that the rewrite language may be less expressive 
than the query language.
This implies that it may not be possible to find an equivalent rewrite of a
query in $L_W$ using the transformation rules in $L_R$ and the available views.

A rewrite $r$ is an equivalent rewrite of target $W_i$ using only candidate
views.
$r$ is considered an equivalent rewrite of $W_i$ \textsl{iff}
it produces an identical output to $W_i$ given the same database instance $D$.
A rewrite $r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
%In this work we only consider equivalent rewrites.



==> old/Preliminaries-rewrite4.tex <==
\section{Preliminaries}\label{sec-preliminaries}
Here we present the architecture of our system
and briefly describe its individual components and how they interact, 
followed by our definitions.

\subsection{System Architecture}\label{sec-system-architecture}

Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of the generic system framework we have developed.
Our system integrates our query rewriting component with
an existing query execution engine that is used by analysts.

We make the following observations about our system and the nature
of the queries.
First, the optimizer takes a query written in some declarative language
and translates it into an execution plan that consists of MR jobs.
Second, queries are expressed against the base data, which are
large logs and queries contain UDFs.
% (which implies that a query typically contains various
% UDFs to extract useful information from logs).
Third, each MR job materializes its output to the stable
storage (e.g., HDFS in Hadoop).
% Intermediate outputs are the by-products of query processing 
% that we exploit as opportunistic materialized views.
Fourth, we provide a way to provide cost estimates for 
UDFs admitted to the system.




We extend the target execution engine by integrating
our rewriter, presented in Section~\ref{sec-best-first-workflow-rewrite},
as well as a materialized view metadata store. In order to
let the rewriter communicate with the optimizer of the target engine,
we extend the optimizer to generate a plan with two types of
annotations on each plan node: (1) the logical expression of its
computation and (2) the estimated execution cost.

\onefigtop{fig-odyssey-system-diagram}
{System diagram showing control flows}{3.25in}

The rewriter uses the logical expression in the annotation when searching for
rewrites for the output of a node. The expression consists of
relational operators or UDFs. For each rewrite found
during the search, the rewriter utilizes the optimizer to obtain
a plan and estimated cost.

%
%
%We assume that an analyst submits a query $q$ in some declarative query 
%language, which is then translated to an execution plan by a query optimizer.
%The query is expressed against the base data, which are large logs.
%The optimizer outputs a plan and its expected cost for an input query.
%The execution plan is for an MR engine, and represents a sequence of MR jobs.
%We treat the optimizer as a black-box provided by the execution engine.

%Our rewriter, presented in Section~\ref{sec-best-first-workflow-rewrite},
%takes the plan generated by the optimizer, and searches for a 
%low-cost rewrite of the plan using the materialized views in the system.
%We assume the optimizer provides the logical annotations for nodes in the plan.
%This annotated plan requires a small modification to the query optimizer such 
%that every node in the plan is annotated with the logical expression of the 
%computation.
%Therefore each node in the plan is annotated with either a relational 
%expression that was optimized in some way or represents a UDF.
%In this way a node represents an indivisible unit of computation
%from the perspective of our rewriter.
%Our rewrite algorithm uses this annotated plan as the input. 

%Note that had the rewriter been incorporated inside the query optimizer, 
%the resulting rewrites would be at least good as the rewrites that we find 
%using the already optimized plan.
%We chose to put our rewriter outside the optimizer in order to provide easy 
%integration with an existing optimizer.
%
%
%Incorporating the rewriter and the UDF model inside a query optimizer would 
%require changing the internal mechanisms of the optimizer for each specific  
%MR execution engine, thus failing  our goal of making our solution easy to 
%integrate.
%
%The rewriter utilizes the optimizer to obtain a plan and estimated cost for a
% candidate rewrite during its search of the space of rewrites.
%Once the rewriter is finished with its search, it selects a rewrite to forward
% to the execution engine.

During query execution, all by-products of query processing are retained 
as opportunistic 
materialized views, and stored in the system becoming part of its 
opportunistic physical design configuration.
The materialized view metadata store contains information about the
materialized views 
currently in the system such as the view definitions, and standard data 
statistics used in query optimization.

\subsection{Notations}\label{sec-preliminaries-definitions}

We use $W$ to denote a plan generated by the query optimizer,
represented as a DAG containing $n$ nodes, ordered topologically.
Each node represents an MR job.
We denote the $i^{th}$ node of $W$ as \node{i}, $i \in [1,n]$.
The plan has a single sink that computes the result of the query.
Under the topological order assumption, this is \node{n}.
%$W_i$ is a sub-graph that contains all nodes up to and including \node{i}.
$W_i$ is a sub-graph of $W$ containing \node{i} and all of its ancestor nodes.
We refer to $W_i$ as one of the rewritable \emph{targets} of plan $W$.
%A property of $W_i$ is that it represents a materialization point in plan $W$.
Following standard MR semantics, we assume that the output of each job is
materialized to disk.
Hence, a property of $W_i$ is that it represents a materialization point 
in $W$.
An outgoing edge from \node{k} to \node{i} represents data flow 
from $k$ to $i$.
$V$ is the set of all existing materialized views (MVs) in the system.

The function  $\cost(W_i)$ takes as input $W_i$ and returns its estimated cost
 provided by the query optimizer.
% We make two assumptions about the optimizer.
% First that it can provide a cost estimate for relational operators, and second 
% that it can provide a cost estimate for a UDF.
\cost(\node{i}) is the cost of the MR job at \node{i}, given its input data.
\cost($W_i$) $ = \sum_{\forall \node{k} \in W_i} \cost(\node{k})$.

We use $r_i$ to denote an equivalent rewrite of target $W_i$ using only views in $V$.
$r_i$ is considered an equivalent rewrite of $W_i$ \textsl{iff}
it produces an identical output to $W_i$ given the same database instance $D$.
A rewrite $r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
%In this work we only consider equivalent rewrites.


\subsection{Problem Definition}
Given these basic definitions, we introduce the problem we solve in this paper.

\textbf{Problem Statement.}
\textit{Given a plan $W$ for an input query $q$, and a set of materialized 
views $V$, find the minimum cost rewrite $r^*$ of $W$.}\looseness=-1  

Our rewrite algorithm considers views in $V$ and the rewrite language $L_R$
to search for $r^*$.  
Since some views may contain UDFs, we require an understanding of UDFs in order 
for the rewriter to utilize those views during its search.
Next we will describe our UDF model and then present our rewrite algorithm 
that solves this problem.



==> old/Preliminaries-rewrite5.tex <==
\section{Preliminaries}\label{sec-preliminaries}
Here we present the architecture of our system
and briefly describe its individual components and how they interact, 
followed by our definitions.

\subsection{System Architecture}\label{sec-system-architecture}

Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of our system and its components.
Our system is built on top of Hive, and the queries are written in HiveQL.
Queries are posed directly over the log data stored in Hadoop.
In our system, MapReduce UDFs are expressed in a language supported by HiveQL, 
such as Java, Perl, Python, etc.
To reduce execution cost, the system automatically rewrites queries based on 
the existing views.
A query execution plan in Hive consists of a series of MR jobs, 
and each MR job materializes its output to HDFS.
As Hive lacks a mature query optimizer and cannot cost UDFs, 
we implemented an optimizer based on the cost model 
from~\cite{Nyki2010} and extended it to cost UDFs in our system.

During query execution, all by-products of query processing 
(i.e., intermediate and final results) are retained as opportunistic 
materialized views.
These are stored in the system (space permitting) as the opportunistic 
physical design.
The materialized view metadata store contains information about the
materialized views currently in the system such as the view definitions, 
and standard data statistics used in query optimization.
For each view stored, we collect statistics by running a lightweight Map 
job that samples the data.
This constitutes a small overhead to our opportunistic approach, but as we show
experimentally, this time denotes a small fraction of query execution time but 
provides significant benefits.

Our rewriter presented in Section~\ref{sec-best-first-workflow-rewrite} 
uses the materialize view metadata store to rewrite queries based on the 
existing views.
In order to let the rewriter communicate with the optimizer of the execution 
engine, our optimizer generates plans with two types of
annotations on each plan node: (1) the logical expression of its
computation and (2) the estimated execution cost.

\onefigtop{fig-odyssey-system-diagram}
{System diagram showing control flows}{3.25in}

The rewriter uses the logical expression in the annotation when searching for
rewrites for the output of a node. The expression consists of
relational operators or UDFs. For each rewrite found
during the search, the rewriter utilizes the optimizer to obtain
a plan and estimated cost.



\subsection{Notations}\label{sec-preliminaries-definitions}

We use $W$ to denote a plan generated by the query optimizer,
represented as a DAG containing $n$ nodes, ordered topologically.
Each node represents an MR job.
We denote the $i^{th}$ node of $W$ as \node{i}, $i \in [1,n]$.
The plan has a single sink that computes the result of the query.
Under the topological order assumption, this is \node{n}.
%$W_i$ is a sub-graph that contains all nodes up to and including \node{i}.
$W_i$ is a sub-graph of $W$ containing \node{i} and all of its ancestor nodes.
We refer to $W_i$ as one of the rewritable \emph{targets} of plan $W$.
%A property of $W_i$ is that it represents a materialization point in plan $W$.
As is standard in Hive, the output of each job is materialized to disk.
Hence, a property of $W_i$ is that it represents a materialization point 
in $W$, in this way, materializations are free except for the statistics 
collection.
An outgoing edge from \node{k} to \node{i} represents data flow 
from $k$ to $i$.
$V$ is the set of all existing materialized views (MVs) in the system, which 
includes the base data.

The function  $\cost(W_i)$ takes as input $W_i$ and returns its estimated cost
 provided by the query optimizer.
% We make two assumptions about the optimizer.
% First that it can provide a cost estimate for relational operators, and second 
% that it can provide a cost estimate for a UDF.
\cost(\node{i}) is the cost of the MR job at \node{i}, given its input data.
\cost($W_i$) $ = \sum_{\forall \node{k} \in W_i} \cost(\node{k})$.

We use $r_i$ to denote an equivalent rewrite of target $W_i$ using views in $V$.
$r_i$ is considered an equivalent rewrite of $W_i$ \textsl{iff}
it produces an identical output to $W_i$ given the same database instance $D$.
A rewrite $r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
%In this work we only consider equivalent rewrites.


\subsection{Problem Definition}
Given these basic definitions, we introduce the problem we solve in this paper.

\textbf{Problem Statement.}
\textit{Given a plan $W$ for an input query $q$, and a set of materialized 
views $V$, find the minimum cost rewrite $r^*$ of $W$.}\looseness=-1  

Our rewrite algorithm considers views in $V$ to search for $r^*$.  
Since some views may contain UDFs, for the rewriter to utilize those views 
during its search, some understanding of UDFs is required.
Next we will describe our UDF model and then present our rewrite algorithm 
that solves this problem.



==> old/Preliminaries.tex <==
\section{Preliminaries}\label{sec-preliminaries}

Here we present the architecture of our system 
and briefly describe its individual components and how they interact.
Figure~\ref{fig-odyssey-system-diagram} provides a high level
overview of the system we have implemented.
Then we describe our UDF model, our cost model, and definitions.

\subsection{System Architecture}\label{sec-system-architecture}

\onefig{fig-odyssey-system-diagram}
{System diagram of Odyssey that shows control flows}{3.25in}

\textbf{\textit{Input.}}
In our system, users (i.e., analysts) compose a workflow $W$ 
%%xxx change diagram WF->W xxx
as a DAG from a library of shared UDFs (that includes standard SQL operators) and base data (e.g., \textit{logs}).
Each UDF is a node in the DAG, and is annotated appropriately as per our UDF model 
described next in Section~\ref{sec-udf-model}.
The annotated workflow $W$ is given as input to the {\em workflow compiler}.

\textbf{\textit{Workflow Compiler.}}
Verifies the DAG structure, then creates a dependency graph which it uses to parallelize the DAG nodes where possible.

\textbf{\textit{Artifact Metadata Store.}}
This contains information about the existing materialized views and base data
currently in the system.  
Metadata includes the view ids, their descriptions, and some
data statistics about the views and base data.

\textbf{\textit{Rewriter.}}
The {\em workflow rewriter} has two inputs: 
1) the annotated, verified, and parallelized version of DAG $W$ from the workflow compiler, and 
2) materialized view metadata from the Artifact Metadata Store.
The rewriter uses our workflow rewrite algorithm, \WF{} 
to obtain a low-cost rewrite of $W$.
\WF{} which is presented in Section~\ref{sec-best-first-workflow-rewrite},
utilizes the \ocost{} functionality described in Section~\ref{sec-viewfinder}.

\textbf{\textit{Optimizer.}}
Each valid candidate rewrite produced by the rewriter is given to the optimizer which returns
a logical plan and its expected cost.  
We treat the optimizer as a black-box, provided by the execution engine.
%Finally, the rewrite of $W$ yielding the lowest cost plan found among all candidate 
%rewrites is then given to the {\em execution engine}.

\textbf{\textit{Execution Engine.}}
The logical plan for the lowest-cost rewrite found for $W$ by the Rewriter 
is given to the execution engine,
which is then launched as a job for that specific engine.

\textbf{\textit{Artifacts.}}
The output of workflow nodes are artifacts of execution and
are retained and stored as materialized views (MVs), 
with their metadata added to the artifact store.
%xxx The logical plan (rewrite of $W$) is received and then a physical plan for the 
%Since the output of our rewrite algorithm is a logical plan, the engine is free to implement a 
%low-cost physical plan specific to its own engine xxx.
%% xxxremove DFS term from the figure.??xxx

\begin{comment}
Then it is given to {\em rewriter} which automatically   
{\em rewrites} $W$ to make 
it more efficient by using the base data and any artifacts
from prior workflow executions that 
obtained from the {\em artifact store}.
The rewriter generates rewrites of $W$, which are given to 
the {\em optimizer} to obtain their cheapest execution plans
and costs.
From all the {\em valid} rewrites, the one with the cheapest plan cost
is given to the {\em execution engine}, which executes it.
An artifact is the result of an execution,
which is stored in the distributed file system {\em DFS}, and its meta data is
added to the artifact store.

In our system an analyst (i.e., user) composes a workflow by
dragging and dropping boxes from a library of UDFs.
The query language of the workflow encompasses all UDFs that have been
added to the system.
The system automatically {\em rewrites} the given workflow to make 
it more efficient by reusing previous work.
During workflow execution we retain all workflow outputs as artifacts.
Our system reuses these artifacts (i.e., materialized views--MVs) 
to make subsequent queries more efficient.

An analyst in our use case typically revises the workflow
iteratively by examining previous results and modifying 
the original workflow.
This way the analyst has the freedom to explore
their intuition in any direction as they move toward 
their desired answer.
Workflow modifications can include adding a new base data source,
changing a \textit{sub-goal}, 
changing parameters,
or replacing some operations in the workflow with a UDF.
We capture these types of modifications in our microbenchmark
in Section~\ref{sec-experimental-evaluation}.
Analysts extend the language of the workflow
by adding a new UDF to the system then the 
UDF becomes available to all the other analysts.  

%This may sometimes require the provider to take decisions that affect a single
%user for the benefit of the community of users.
The system must consider tradeoffs between maximizing performance for a single
user versus performance for the community of the users.
The system can extend the language of the rewrites by adding more UDFs.
Extending the rewrite language with a UDF can benefit the analysts
by finding better rewrites, but makes the rewrite search space larger
which increases the time taken to find a good rewrite. 
Even though the rewrite language includes a rich and
extensible set of transformations,
it is to be expected that the language of the rewrite
is less expressive than the language of the workflow.
The system also has to decide which materialized views to retain.
Because storage space is not infinite 
a garbage collector is required.
%We present some results on the effect of garbage collection
%on query performance in Section~\ref{sec-experimental-evaluation}.
\end{comment}

%Our system does not make any assumption about the structure of 
%the data sources.
\textbf{\textit{Base data.}}
A primary data source in our scenario are large logs, which can
have a high extraction cost when the data is flat with low structure.
Extraction can include unpacking (deserializing), formatting, type-checking, re-encoding, 
and tokenizing, to name a few. 
The ETL process can require further data cleaning methodologies such as replacing missing values, 
nominalize values, exception handling, logical ETL modeling, as well as the time required 
for all analysts to agree on these.
%This type of large-scale base data in an evolutionary scenario maps most naturally to
%an M/R system due to its low barrier to entry (e.g., hardware, software, 
%no formal ETL process need defined initially, etc.).
This type of large-scale base data in an evolutionary scenario maps most naturally to
a system that operates on flat files and has a low barrier to entry (e.g., hardware, software, 
no formal ETL process need defined initially, etc.) such as a MapReduce platform.

\textbf{\textit{MapReduce.}}
Because this log data is large and its utility unproven,
an M/R framework provides a flexible system
that allows users freedom to start exploring the data early and try complex 
analytics, often as UDFs, to find value.
UDFs in an M/R system may be implemented in many supported languages
(e.g., Hive-QL, Pig, Python, Perl, Java) allowing a reasonable amount of flexibility.
In a traditional M/R framework, a job can often spawn a sequence of sub-jobs. 
This sequence typically communicates inputs
and outputs via reads and writes on the distributed file system,
allowing our system to retain the artifacts created during execution 
with little additional overhead.
Our system and rewrite algorithm are not specific to MapReduce, but for these
reasons we consider the M/R framework as the primary {\em execution engine}
in this work without precluding other analytical stores.

\subsection{UDF Model}\label{sec-udf-model}

Workflows commonly include complex analytical operations expressed as UDFs, thus
our system requires a way to model them semantically.
UDFs may be modeled using a white, grey, or black box approach with varying levels 
of overhead and complexity to the system. 
A white box approach requires a complete description of the UDF so that the system 
understands \textit{how} the UDF transforms the inputs.
This is too much of an overhead for an analyst adding a new UDF to the system.
A black box approach produces an output that is completely opaque to the
system (similar to a stored procedure)
thus may not be suitable for our goal of reusing results.
Since UDFs can involve fairly complex operations on the data, our system adopts a gray-box approach
that only captures the \textit{end-to-end transformations} performed by a UDF.
This requires little overhead when adding a new UDF, yet
allows the system to understand the UDF's transformations in a useful way.
Alternatively, a method such as \cite{Hues2012} could be applied to automatically extract
some of the semantic properties of the UDFs we are interested in capturing, 
thereby reducing the burden on the user.
The end-to-end transformations allowed by our gray-box model are limited to the following operations.

%%Given an input $I$ the end to end transformation allowed by our model are limited to the following
%%operations on $I$ to produce and output $O$.

\vspace{-0.05in}
\begin{enumerate}
\setlength{\itemsep}{3pt}%
\setlength{\parskip}{0mm}%
\item Discard or add attributes, e.g., \textsc{projection, aggregate, sentiment-score, word-count}, etc.
\item Discard tuples, e.g., \textsc{filter}
\item Perform grouping of tuples, e.g., \textsc{groupby}
\end{enumerate}
\vspace{-0.01in}

Given these operations, our UDF model only captures the end-to-end transformation from 
an input $I$ to an output $O$
as reflected by the change in attributes, the addition of filters, and the change in group-by.

Accordingly, 
$I$ is expressed as a set $A$ of attributes, a set $F$ of filters, and the current grouping $G$ of attributes.
After applying any end-to-end transformation,
$O$ is expressed as a set $A$ of attributes (additional or fewer than $I$), a conjunction of 
the filters $F$ in $I$ and any additional filters applied, and any re-grouping $G$ of attributes.

If any new attributes are produced, then those attributes in $O$ record their dependency on $I$ 
as small signature containing the required 
attributes in $I$, the Filters in $I$, and Groupby
of $I$. For uniqueness the signature also includes the UDF name, and an optional modifier 
(e.g., $k$ in \textsc{top-k}).
Note there is no facility to update attributes in place, which is not unreasonable here given
that our primary data source is logs.
Any modification to a required attribute in $I$ is recorded as a new attribute.  
 
\begin{comment}
The model captures these transformations as a set of operations on attributes
filters and groupby on the input
The end-to-end transformations is expressed as the 
on the input.  
We represent the transformation performed by a UDF as the set of 
attributes, filter, groupbys.
You can hide very expensive computation inside the box.
The model is annotated with a UDF name, required-attributes, modifier, and 
output attributes which together denotes the end-to-end transformation performed.
UDFs are common in this space, thus we need a model as a way to 
understand them semantically.
Many complex analytical operations are performed as UDFs, thus our system requires
a way to model UDF processing in order to take advantage of previous computation based
on logical data semantics rather than exact plan-level input and output matching.
A UDF modeled by our system allows the following types of processing:

The model captures many standard SQL operations such as Select, Project, Join, Groupby,
and Aggregation as well as UDFs that can fit within this representation.  
For instance, a UDF that computes and outputs a text-sentiment score falls into the category
of $(2)$, where the input data is used to output a score value representing the sentiment, 
or a nominal value such as `positive', where either can be represented as an additional output
attribute with a label such as `sentiment-score'.
Another example is an \textsc{extract} operation over a log that might include a specific
user's cleaning method to replace a log attribute value (e.g., \textsc{null}) with a new value ($-1$).  
This \textsc{extract} function is written as a UDF, and can be shared, modified, or 
repurposed by other users later.

Choosing this model represents a tradeoff, as it creates several limitations to our system, 
and our workflow language $L_W$.
Because we primarily process log data sources, there is no provision to update-in-place.  
Our workflow language does not include negation or recursion.  
Our model allows us to understand UDFs within the language of conjunctive queries
with aggregation, (SPJG+A).

A UDF is represented by a simple grammar, requiring the following 
annotations to be provided when adding a new UDF.
\begin{itemize}
  \item Required-attributes: includes those which influence the output in any way, and the `*' symbol
  is used for pass-thru (non-required) attributes.
  \item Output-attributes: may include the newly created attributes, the subset of required attributes
  that are output, and the `*' symbol for pass-thru (non-processed) attributes.
  \item Function-name:  for uniqueness and re-usability by others
  \item Modifier (optional): for uniqueness re-usability of UDFs that may be changed with a simple
  argument parameter
\end{itemize}

The Modifier attribute can be used to re-purpose UDFs with simple changes such as the k-value in \textsc{top-k} 
or the threshold for a nominal positive sentiment value in \textsc{sentiment-score}, rather
than adding a completely new UDF.
Any newly created attributes in the Output-attributes list are considered a derived attribute,
and can be mapped back to the UDF by its signature.  
A derived attribute's signature 

Each derived attribute produced by an operation in a UDF records a \textit{signature}.
This is a minimal form of provenance that captures the nature of the
operation's input in terms of attributes, group-bys, and filters.
The dependency of the derived attributes on a subset of the 
properties of the input is captured by the signature.
Notice there is no provision to modify attributes in-place
meaning that modifications are reflected as new attributes.

This UDF model maps well to a M/R execution framework in the sense that the map and/or reduce phase
can filter tuples based on a condition (1), transform single attributes or groups of attributes
to produce derived attributes (2),
and the reduce phase can group attributes (3).
Moreover, complex UDFs consisting of several operations can be expressed as multiple jobs with
several map and reduce phases.

UDFs can be modeled using a white, grey, or black box approach with varying levels of overhead for the user 
as well as adding varying levels of complexity to the system. 
A white box approach requires a complete description of the UDF so that the system 
understands the UDF's transformations of the input as well as the interaction of the UDF with all other UDFs
in the system, which is too much of an overhead for an analyst in our system.
The black box approach produces an output that is completely opaque to the
system (similar to a stored procedure)
thus may not be suitable for our expressed goal of reusing results.
Thus our modeling of a UDF takes a grey box approach,
requiring little overhead when a user adds a UDF to the system,
while still allowing the system to understand the UDF's input transformations
 and interactions in a limited way.
\end{comment}

%Our model is expressive enough to capture many types of UDFs, including classifiers.
Consider an example UDF called \texttt{FOOD-SENTIMENT} that uses a classifier to 
compute a sentiment score on users who talk about food items.
One possible instance of this UDF can be implemented in a supported language (e.g., Java, Perl,...) and
is described in Example \ref{ex-food-sentiment}.


\begin{example}\label{ex-food-sentiment}
UDF implementation: 
For each user, gather all of their tweets.  
%Discard those tweets that do not refer to food or any of its closely related terms.
Apply a classifier that determines if a tweet refers to food or a closely-related concept,
and then computes a food sentiment score for each user.
Output only those users with score above a given threshold. 
The UDF Model for this UDF is given by:  \\
Inputs: required-attrs<\texttt{userid}, \texttt{tweet}>, modifier<$t$ (threshold)>,
 UDF-name<\texttt{FOOD-SENTIMENT}>\\
Output: new-attribute<\texttt{score}>, add-filter<\texttt{`score > $t$'}>, re-groupby<\texttt{userid}>
\end{example}

Suppose that $I$ is represented by $A$=\{\texttt{userid}, \texttt{tweet}, \texttt{tweetid}\},  
$F$=$\emptyset$, and $G$=$\emptyset$.
After invoking the example UDF with $t$=0.5, output $O$ is represented by
$A$=\{\texttt{userid}, \texttt{score}\},
with $F$=\{\texttt{`score > $0.5$'}\}, 
and $G$=\{\texttt{userid}\}.
The new attribute \texttt{score} has a unique signature that is dependent on $I$ and is given by 
required-attrs<\texttt{userid}, \texttt{tweet}>, 
%%$\{\texttt{userid}, \texttt{tweet}\}$, 
$F$=$\emptyset$, $G$=$\emptyset$, $t$, and \texttt{FOOD-SENTIMENT}.
This signature is a minimal form of provenance that captures a functional dependency on its immediate inputs.

UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured using our model
can be \emph{admitted} to the system.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations. 
For instance, given two identical UDFs with different names, their new attributes will result in different signatures.
This deficiency can only be overcome if we resort to a white-box approach.


\begin{comment}
--
For each \texttt{user\_id}, \texttt{tweet}, discard those tweets that do not refer to
food or any of its closely related terms.
Then group-by the remaining tweets by the \texttt{user\_id}, and compute using a classifier
a \texttt{food\_sentiment\_score} for each group of tweets for a \texttt{user\_id}.
Finally, retain those \texttt{user\_id} that scored above a threshold
$t$, which is a tunable parameter in the UDF.
--
UDF Model:  Required-attrs: $u$,$t$, modifier: $r$, UDF-name: \texttt{FOOD-SENTIMENT},
new attribute: $s$, add-filters: \texttt{`$t$ contains food'},\texttt{`$s > r$'} and re-groupby: $u$.
\end{example}
An analyst adds a new UDF to the system by providing
an implementation of the UDF in
at least one of the languages the system supports,
identifying the tunable parameters,
and a {\em grammar} that describes how the
UDF transforms the inputs.
A UDF is expressed by a combination of the following operations.
\vspace{-0.05in}
\begin{enumerate}
\setlength{\itemsep}{3pt}%
\setlength{\parskip}{0mm}%
\item Discard tuples based on certain condition
\item Create one or more attributes based on transformation of a set of attributes from
a single tuple or a group of tuples
\item Group tuples based on a common property
\end{enumerate}
\vspace{-0.01in}
\end{comment}

\subsection{C\fakesc{ost} Function}

The cost function $\cost{}$ takes as input a query $q$ and returns $\cost(q)$
which corresponds to a cost estimate provided by the {\em query optimizer}
(see Figure~\ref{fig-odyssey-system-diagram}),
which we treat as a black-box.
The optimizer considers execution plans for
$q$ and returns the cost of the cheapest plan that implements $q$.
We require the query optimizer to estimate the cost of applying a UDF,
but its ability to reorder and push-down UDFs may be restricted
to simple UDFs that implement relational operators.
A further optimization that the query optimizer considers is to combine operations,
thereby amortizing their combined cost.
Thus we assume the following weak property about the nature of the
operations and the $\cost{}$ function, which forms the basis of
our \ocost{} presented in Section~\ref{sec-viewfinder}.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be a set of operations drawn from the three operations
given by the UDF model.  Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality

The reason we must assume the weak min property is because 
a stronger max property requires 
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter ($F$)
with high selectivity and a group-by ($G$) operation 
that is more expensive than $F$,
 and $S'$ contains only $G$.
Suppose that applying $F$ before $G$ 
results in few or no tuples being given to $G$.
Then applying $G$ can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.

\subsection{Definitions}
$W$ is a workflow which is represented as a DAG, containing $n$ vertices and ordered topologically.
$W_1 \cdots W_n$ are sub-workflows of $W$ such that $W_i$
contains all vertices up to and including $i$, $i \in [1,n]$.  
$W_i$ is also referred to as one of the rewritable \emph{targets} of $W$.
% The language of the workflow (including UDFs as given by the model) belongs to SPJGA.

\node{i} corresponds to the $i^{th}$ vertex, representing 
the last transformation  applied by sub-workflow $W_i$. 
An incoming edge to \node{i} from \node{j} represents data flow from $j$ to $i$,
and an outgoing edge from \node{i} to \node{k} denotes data flow from $i$ to $k$.
The output of a \textsc{node} is stored as an \emph{Artifact}.

\cost(\node{i}) is the cost to produce its output from its inputs, and 
\cost($W_i$) $ = \sum_{\forall \node{j} \in W_i} \cost(\node{j})$.

$V$ is the set of all existing materialized views (MV) in the system,
corresponding to the artifacts from prior execution runs.
\textit{Candidate views} describes all views in $V$ and those additional
views created by merging views in $V$.
Candidate views are those views
that are considered for rewriting a workflow.

$r$ is a rewrite of $W_i$ using candidate views.
Furthermore, $r$ is considered an equivalent rewrite of $W_i$ \textsl{iff} 
it produces an identical output to $W_i$ given the same database instance $D$.
$r^*$ represents the minimum cost rewrite of $W$ (i.e., $W_n$).
In this work we only consider equivalent rewrites.


$L_W$ represents the language of the workflow, which is also the language of the views, 
and $L_R$ represents the rewrite language.
$L_W$ includes any UDF admitted to the system,
while $L_R$ is a restricted subset of the UDFs which form the transformation rules used during rewriting.
$L_R \subseteq L_W$ indicates that the rewrite language is less expressive than the
workflow language.


\begin{comment}
%Given the allowable operations, a result can be modeled as a set of Attributes (\textsf{A}),
%a set of filters (\textsf{F}), and group by attributes (\textsf{G}).
%We consider \textsf{F} to contain conjunctions of simple selection predicates.
%In this model, the result of a equijoin operation appears as an additional filter representing the join predicate.
%A result is considered a materialized view in our system (a view extension).
\end{comment}


==> old/Preliminaries_old_comments.tex <==
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given this high computation cost, we use a model of a query optimizer such that
$\cost(q)$ approximates the cost of performing the operations in $q$
in the order specified without exploring reordering these operations.
This model is sufficient as we only require a cost to execute $q$ as given.
The task of reordering operations in $q$ is performed by the $\VF{}$ which
generates all possible orderings of operations when enumerating rewrites for $q$.
Since each rewrite considered by $\VF{}$ is given to the cost function $\cost{}$,
the application of $\cost{}$ should be inexpensive.
A further optimization that a query optimizer considers is to combine operations,
thereby amortizing their combined cost.
We assume the following weak property about the nature of the
operations and the cost model.

We now define the grammar of the UDFs that takes an input and produces an output.
The input is described in terms of {\sf A, G, F} fields in the sense
what are the set of attributes in the input, what is the group-bys
applied to the system, and the set of filters that have been applied
to the system.
A UDF is expressed as a chain of one or more of these operations.
\begin{enumerate}
\item Discard tuples based on certain condition

\item Group tuples based on a common property

\item Create one or more attributes based on transformation of a set of attributes from
a single tuple or a group of tuples

\end{enumerate}
For the attributes produced by the UDFs we record the box that produced
the attribute {\sf B} field, group-by of the input {\sf G},
filters on the input {\sf F}, input attributes {\sf I} and other
properties of the inputs that created it.

\begin{example}
The food-sentiment udf takes as inputs user\_id, tweets written by the user
and outputs the user\_id as well as food\_sentiment\_score for those
users who expressed sufficient knowledge about food.
Such a UDF can be expressed as followed.
One implementation of the UDF can be as follows.
For each user\_id, tweet, we discard those tweets that do not refer to
food or any of its closely related terms.
Then we group-by the remaining tweets by the user\_id, and compute
a score food\_sentiment\_score for each group of tweets for a user\_id.
Finally, we threshold those user\_id that scored below a threshold
$t$, which is a tunable parameter in the UDF.
If the input to the box is given by {\sf A: \{user\_id, tweet\}},
{\sf F: $\emptyset$}, and {\sf G: $\emptyset$}.
The grammar will transform the output to
{\sf A: \{user\_id, food\_sentiment\_score\}},
{\sf F: \{tweet not contains food\_terms, food\_sentiment\_score $<$ t\}}, and
{\sf G: \{user\_id\}}.
The {\sf food\_sentiment\_score} is given by
{\sf B: food-sentiment}, {\sf F: \{tweet not contains food\_terms\}},
{\sf G: \{user\_id\}}, {\sf I: \{tweet\}}, where
{\sf B} captures the UDF name that created the attribute,
{\sf F} filters applied to the input to the inputs,
{\sf G} group-bys of the input, and
{\sf I} input attribute over which the score has been computed.
\end{example}

\item Log data is large, and flat. Because of this previous computations
should be reused whenever possible as they can denote a substantial
investment in terms of computation in machine hours from the provider's perspective.

\item Extraction of data from logs is expensive.  Extraction can
include unpacking (deserializing), formatting, type-checking, re-encoding,
or tokenizing just to name a few.

\end{enumerate}

% SJ: Need to write it in words
% \item $L_W$ is the language of the workflow consist of all user contributed UDFs
% \item $L_R$ is the language of the rewrite workflow consisting of some of the
%       user contributed UDFs
% \item $L_R \subseteq L_W$ means that $L_r$ is less expressive than $L_W$
% \item Any vertex $q_i$ in $W$ is drawn from $L_W$
% \item Any vertex $q_j$ in $r$ is drawn from $L_R$
% However, this is only true if the
% language of the rewrite is as {\em expressive}
% than the language of the user workflow.
% not to mention
% assuming that the $\ViewFinder{}$ examines the space of all
% possible plans for $t_n$ which can be very large and infeasible to search.

However, this signature of our grey box approach is limited in that a white box approach could determine
two derived attributes to be equivalent because their transformations are identical, even though their signatures are different.
When adding a UDF a user may specify how it interacts with some other UDFs
in the system, making a limited progression toward a white box approach.
But this requires significant additional overhead while here we focus on the usefulness of our model
even on the level of understanding a UDF as a grey box.

\begin{table}[t]
\centering
\small
\begin{tabular}{| l || l |}
    \hline
    \textbf{Map Phase Operations} & \textbf{Reduce Phase Operations} \\
    \hline
    Project - Extract LOG Attributes       & Groupby\\
    \hline
    Select - Apply Filters                 & Aggregations\\
    \hline
    Transform - Add Derived Attributes     & Transform - Add Derived Attributes\\
    \hline
  \end{tabular}
 \normalsize
\caption{Operations possible during distinct Map and Reduce phases}
\label{tab:mrops}
\end{table}
\end{comment}


==> old/Problem_definition-rewrite1.tex <==
\section{Solution Outline}\label{sec-problem-definition}

% Why is this problem hard?
%  Why is this problem hard?
%  Determining if a rewrite exists
%  Determining a candidate rewrite
%  Containment 

Answering queries using views is a long-studied problem~\cite{Hale2001,Abit1998,Levy1995}.
% It is primarily considered in the context of data integration or data warehouse
% design (query optimization)~\cite{Hale2001}.
% Data integration is often interested in maximally-contained rewrites while
% query optimization is concerned with equivalent rewrites.
% Our interest is the latter.
The complexity of finding an {\em equivalent} rewrite is described with respect to the
expressivity of the languages used for both the queries
and the view definitions~\cite{Abit1998}.
Even when both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete
both for determining whether a rewrite exists~\cite{Levy1995} and
checking the correctness of a rewrite.
Checking the correctness of the rewrite is the same problem as
determining containment (i.e. $ Q_1 \subseteq Q_2$), which is
NP-complete~\cite{Chan1977} for conjunctive queries.
Here we must consider a rich query language that may include any UDF admitted by the system.
A \textit{complete} rewriting of $Q$ using $V$ is said to be one
that only uses $V$, and does not use any of the base relations.
Determining whether there is a complete rewriting of $Q$ using $V$
(again for the class of conjunctive queries) is NP-complete~\cite{Levy1995}.
Furthermore, when $Q$ and $V$ are disjunctions of conjunctive queries,
finding a complete rewriting is NP-complete~\cite{Levy1995}.
Producing a \textit{minimal} rewrite entails using the minimal number
of views in the rewrite such that no view can be removed
without invalidating the rewrite.
This problem is also NP-complete~\cite{Levy1995}.
We only consider complete rewrites, those using
the existing views, without extracting new views from the log.

% Finding a optimal rewrite for a single target is NP-hard
Given as input a plan $W$ with a single target, and a set of existing
materialized views $V$, we want to find a rewrite of $W$ that
minimizes the total execution cost of $W$.
% As $W$ is a query, this problem can be formulated
% as the query rewrite problem using materialized views, which is
% known to be NP-complete even considering a language
% for both queries and views belonging to the simple class
% of conjunctive queries~\cite{Levy1995}.
\begin{comment}
We decompose this problem into two sub-problems.
First, we introduce a $\VF{}$ which
given a query, a set of candidate artifacts,
and a set of transformational rules finds the cheapest rewrite workflow of the target,
if such a plan exists.
Next, utilizing the $\VF{}$ at each target,
we introduce a workflow rewrite algorithm $\WF{}$ that obtains the
lowest cost workflow rewrite plan of $W$, while performing minimum amount of work.
\end{comment}
% The problem of finding a rewrite of a query using materialized views
% is known to be NP-complete even considering a language
% for both queries and views belonging to the simple class
% of conjunctive queries~\cite{Levy1995}.
% Here we must consider a rich workflow language that may include any UDF admitted by the system.
% Furthermore, existing candidates may only be {\em partial} solutions with
% respect to the target, thus we have to consider creating new candidates by {\em merging}
% existing candidates, which explodes the space further.
Finding an optimal rewrite of $W$ requires considering all
combinations of materialized views and transformation rules, which
makes the solution search space exponential both in 1) the
number of materialized views ($|V|$) and 2) the number of transformation rules ($|L_R|$).
Thus finding a rewrite for a single target
in a workflow is computationally expensive.

% Naive Solution: Bottom up solution
When searching for the optimal rewrite $r^*$ of a plan $W$ containing multiple
targets, $L_R \subseteq L_W$ has the following implications on any search 
 process that finds the optimal rewrite.
A first consequence of $L_R \subseteq L_W$ is that searching for 
an optimal rewrite of only $W_n$ does not suffice.
This is because the inability to find a rewrite for $W_n$ 
does not mean that one cannot find a rewrite at a different target $W_i$ in $W$.
If a rewrite $r$ is found at $W_i$, $r$ can be expressed as a rewrite
for $W_n$ by combining $r$ with the remaining part of the workflow
indicated by $\node{i+1} \cdots \node{n}$.
The second consequence of $L_R \subseteq L_W$ is that
the search process cannot stop once it finds a rewrite 
at any target in $W$.
For instance, if a rewrite $r$ is found for some target $W_i$,
a rewrite $r'$ of
$W_{i-1}$ may exist and it may be cheaper to use $r'$  
to obtain a rewrite for $W_i$ than $r$.
Thus the search process must happen at all targets in $W$.

Given these implications, a bottom-up algorithm is a natural fit.
This algorithm searches for rewrites at all targets 
in the workflow in a bottom-up fashion.
It obtains the best rewrite for each target, if one exists,
and chooses a subset of these to obtain $r^*$ using a dynamic programming
approach.  We call this algorithm bottom-up, although 
strictly bottom-up  is not  necessary since it must search at all targets.

One drawback of the bottom-up approach is that there is  
no easy way of early terminating the search at a single target.
Even with an early termination property,
the algorithm may search for a long time at a target only to find 
an expensive rewrite, 
when it could have found a cheap rewrite much sooner 
at the target above.
This is illustrated in Example~\ref{example-greedy-plumbing}.

\begin{minipage}{0.60\linewidth}
\vspace{0.1in}
\begin{example}\label{example-greedy-plumbing}
The figure alongside shows an example of
a plan $W$ containing 3 targets.
The space of rewrite is shown
alongside each target, where candidate views
that results in a rewrite are shown in triangles
that records their costs, while the filled rectangles
corresponds to those that did not yeild an equivalent rewrite.
A bottom-up algorithm would have examined all
the rewrites for $n_3$ choosing the rewrite with a cost of $12$,
then examining both $n_1$ and $n_3$ to obtain a lesser
cost rewrite of $2$ at $n_1$, $1$ at $n_2$, and
retaining the target  $n_3$.
The algorithm would have performed much better had
we known that the best possible rewrites at each target
and we would have started with $n_1$ and $n_2$, and
avoided looking at $n_3$.
\end{example}
\end{minipage}%
\hspace{0.1cm}%
\begin{minipage}{0.35\linewidth}
\centering
\includegraphics[width=1.5in]{fig-running-example-1}
\end{minipage}
\vspace{0.1in}

\begin{comment}
\begin{minipage}{0.70\linewidth}
\vspace{0.1in}
\begin{example}\label{example-greedy-plumbing}
The figure alongside shows an example of
a workflow $W$ containing 4 targets.
Suppose that the bottom-up algorithm 
could not find a rewrite for
targets $W_n$ and $W_{n-2}$ in spite of searching
the entire space,
yet was able to find an expensive rewrite for $W_{n-1}$.
The algorithm would have performed much better had
it first looked for rewrites at $W_{n-3}$,
thus obviating the need to search too long 
at $W_{n-2} \cdots W_{n}$.
\end{example}
\end{minipage}%
\hspace{0.1cm}%
\begin{minipage}{0.25\linewidth}
\centering
\includegraphics[width=1in]{fig-greedy-plumbing-fails}
\end{minipage}
\vspace{0.1in}
\end{comment}

The bottom-up approach described
is not {\em work efficient} in the sense that
a) it did not start the search with $n_1$ and $n_2$ which
would have avoided looking for rewrites exhaustively at $n_3$,
b) use the rewrite found at $n_1$ and $n_2$ to bound the search
space at $n_3$.
Note that searching for all possible rewrites at a node
is extremely time consuming especially if there are many
materialized views in the system.
The inefficiency of a bottom-up approach is partly due to
not considering the rich interactions possible between the
$n$ search problems at each of the targets in $W$.

Suppose that we had an {\em oracle} that would identify the lowest
cost rewrite at each target without having to exhaustively 
enumerate the search space at each target.
For example, in Example~\ref{example-greedy-plumbing}
it would identify that $n_1$ contains a rewrite at a cost
of 2, $n_2$ at a cost of 1, and $n_3$ at a cost of 12.
Given such an oracle, an hypothetical algorithm would examine
the rewrites at differrent targets in a global ordering 
of its ability to produce a low cost rewrite for $W$.
First, it would examine the rewrite at $n_2$ at cost of 1 with a 
hypothetical rewrite at $n_1$ at a cost of $\geq 1$ followed
by $n_3$ for a cost of $\geq 3$.
Next, it would compose the next low cost rewrite by using 
the rewrite at $n_2$ at a cost of 1, rewrite at $n_1$ at a cost of 2,
followed by $n_3$ at a cost of 1 for a rewrite that costs $4$.
Having obtained a rewrite at a cost of 4 means that $n_3$ need not
be examined as its best rewrite of 12 is much more expensive than
the cost of 4 we know about.

This algorithm using the oracle is work-efficient as unlike
the bottom-up algorithm, it looks at
the most promising target capable of producing the low-cost rewrite
first or can avoid exhaustive enumeration of rewrites at a target
that does not have the potential to produce a low-cost rewrite.

% Note that being able to take advantage of the interactions
% between the $n$ rewrite search problems at each of the targets
% requires the design of the $\VF{}$
% to be {\em incremental} in that it can find
% cheaper plans first and expensive plans later as well as
% has the ability to stop early if a cheaper plan is found
% at some other target that obviates the need to search
% further at a particular target.

Ofcourse, an oracle to identify the best rewrite 
at each target does not exist but we have developed a method by 
which we can arrange the candidate views at each target by
their ability to produce a  low-cost rewrite.
In particular, for a given target $W_i$, the candidate views by the 
{\em lower bound} on the cost of a rewrite they may produce without
having to enumerate all the possible rewrites they may produce.
The lower-bound merely orders the candidate views merely based
on their ability to produce a rewrite but the actual cost of the
rewrite itself if one exists still needs an exhaustively 
searching as detailed above.

As we will see in the following sections,
ordering the candidate views based on their ability to produce
low-cost rewrites has a similar effect as an oracle.
First, it allows examining targets based on their ability to
produce a low-cost rewrites for $W$.
Next, it avoids examining all the candidate views in some of 
the targets 

==============================================

In this paper we propose a work efficient
rewrite algorithm for finding the optimal rewrite $r^*$ of $W$
by breaking the problem into two components:
1) $\VF{}$ provides of enumerating the candidate views 
for a single target based on their ability to produce
a low-cost rewrite for the rewrite and 2) $\WF{}$
% that tries to combine the rewrites found for all the $n$ targets into
performs an efficient search of rewrites for all targets in $W$
and outputs a globally optimal rewrite for $W_n$.
The $\WF{}$ concurrently searches for rewrites
at each of the $n$ targets in $W$, while maintaining the
cheapest ({\em best}) rewrite for $W$ found thus far.
Additionally, by communicating the success or failure in finding
a rewrite at a target $W_i$ with other the targets in the workflow,
our approach obviates the need to look in sub-spaces
where it is not possible to find a cheaper rewrite for $W$.
This forms the \textbf{best-first} nature of our proposed algorithm.
In the following sections we present an algorithm which finds 
the {\em optimal rewrite} for a given plan, 
while also being {\em work efficient}.

\begin{comment}
% OLDER TExT REMOVED DUE TO LACK OF SPACE...
The design of our $\VF{}$ is inspired by nearest neighbor finding problems
in metric spaces (e.g., road networks) where computing the distances between
objects can be computationally expensive.
For instance, in the case of road networks the distance between two vertices
requires the invocation of a shortest path algorithm
to find the shortest path between two vertices.
Next, the network distance between
the two vertices can be determined by summing up the edge weights along the shortest path.
In such metric spaces, a common strategy to avoid expensive
network distance computations between vertices is by making
use of an alternate distance function (e.g., Euclidean or the geodesic distance function)
that is easy to compute (i.e., not requiring a search process)
with the desirable property it is always less than or equal to
the network distance function.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the network distance between vertices.

Our current problem domain has a similar properties to
nearest neighbor searches in metric spaces, such as the one described above.
We are given a materialized view $v$ and a query $q$
such that the cost function $\cost()$
corresponds to the amount of time or effort required
in transforming $v$ so that it produces an output that is
identical to that produced by $q$.
As will be discussed later, this problem is known to be NP-hard,
which means that finding a rewrite
workflow for $q$ using $v$ requires examining all possible
rewrites involving $v$ and testing their {\em equivalence} with $q$.
This is expensive as the number of possible rewrites of $q$ involving
$v$ is exponential in the number of transformation rules in the system.
In other words, computing the rewrite plan for $q$ using $v$
first requires finding a rewrite plan for $q$, which is a search
process similar to the shortest computation in road networks.
The intuition here is that we want to make use of another distance
function, which is easy to compute and has some desirable with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$
that takes as input $v$ and $q$ and always provides a
lower-bound on $\cost()$ without enumerating
all possible rewrites of $q$ involving $v$.
In other words, if $r$ is the cheapest rewrite plan
of $q$ involving $r$, we have that $\cost(r) \leq \ocost(v,q)$.
\end{comment}

\begin{comment}
% CUT DUE TO LACK OF SPACE.... :(
Our design of a $\VF{}$ is inspired by nearest neighbor finding problems
in metric and non-metric spaces where computing distances between
objects can be computationally expensive.
In such spaces, a common strategy to avoid expensive distance computations is to
use of an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the actual distance between the objects.
\end{comment}

Our design of a $\VF{}$ is inspired by nearest neighbor finding problems
in metric spaces where computing distances between
objects can be computationally expensive, thus
preferring an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
In our problem domain we are given a materialized view $v$ and a target $W_i$,
and we want to find a rewrite $r$ that
transforms $v$ such that it produces an output that is
identical to that produced by $W_i$.
%This problem is known to be NP-complete,
%which means that finding a rewrite
%workflow for $q$ using $v$ requires generating all possible
%rewrites involving $v$ and testing their {\em equivalence} with $q$.
Because this process is known to be computationally hard,
we wish to utilize an alternative distance function (e.g., \textit{dist}($v,W_i$))
% TODO: \cost is defined as yet?
that is easy to compute and has some desirable property with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$
that takes $v$ and $W_i$ as inputs and always provides a
lower-bound on any possible rewrite of $W_i$ using $v$, without enumerating
all possible rewrites.
The property of the alternative distance function is that
$\ocost(v,W_i) \leq \cost(r)$.

The $\WF$ uses an instance of the $\VF$ at each target.
The $\WF$ treats $\VF$ as a black-box and exploits its $\ocost$ functionality
to incrementally search the space of rewrites for $W$.
After every step of the incremental search at some target $W_i$ the following two properties are true.

\begin{enumerate}
\item The $\VF$ at target $W_i$ performs an incremental expansion to some
 cost value $d$ as requested by the $\WF{}$, and there are no remaining
 rewrites to be found for \textbf{sub-workflow} $W_i$ that has a cost less than $d$.
\item After the $\WF$ performs an incremental expansion of the $\VF$ at $W_i$ to cost $d$,
there are no remaining rewrites to be found for \textbf{workflow} $W$ 
with cost less than $d'$, where $d' \leq d$.

\end{enumerate}

The key feature of our method is the $\ocost$ functionality that allows the $\WF{}$
to incrementally search the space of rewrites of $W$, such that $\WF$
finds the optimal rewrite of $W$ in a work efficient manner.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
While the details of the $\VF{}$ algorithm and the cost
functions will will be provided in a later section,
for the sake of developing the $\WF{}$ algorithm,
it is sufficient to model $\VF{}$ as a black-box
$\VF(W_i, d, d',\cost(), \ocost())$, $d < d'$, that takes
as input a workflow $W_i$, two thresholds $d, d'$,
a cost function $\cost()$, an optimistic cost function $\ocost{}$
and outputs a single rewrite $r$ of $W_i$ with the following properties:

\begin{enumerate}

\item $r$ is a rewrite workflow for $W_i$ using $V$ and the transformation rules

\item The invocation of the $\VF(W_i,d,d')$ such that $d < d'$
examines all rewrites of $W_i$ whose optimistic cost is less than or equal to $d'$.
Moreover, any subsequent invocation of
$\VF(t_i, d', d", \cost(), \ocost())$, such that $d' < d"$,
will not produce a rewrite whose optimistic cost is less than or equal to $d'$.

\item $d < \ocost(r) \leq d'$ such that $r$ has the lowest
cost among all the plans found by $\VF{}$ in this invocation.

% \item The time taken (or cost) to answer $\VF(t_i,d,d")$ is
% just a little more than the time taken to answer
% $\VF(t_1, d, d')$ and $\VF(t_1, d', d")$.
\end{enumerate}
\end{comment}



\begin{comment}
\begin{algorithm}[htp]\label{algn-main-setup}
\begin{algorithmic}[1]
\State {\sf sub} $\WF$($W$)\\
\Comment{Produces an optimal rewrite of $W$ using $\VF$}
\State $p^* \qlet W_n$\Comment{Original workflow}
\If{{\bf {\em simple/traditional} variant}}
   \State $p$ \qlet $\VF(t_n)$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
\ElsIf{{\bf {\em bottom-up greedy} variant}}
   \ForAll{$t_i$ in $\{t_n \cdots t_1\}$}
    \State $p \qlet \VF(t_i) \cup \{\node{i+1} \cdots \node{n}\}$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
   \EndFor
\EndIf
\State Rewrite $W$ using $p^*$
\end{algorithmic}
\end{algorithm}

Given the $\VF{}$ only finds a rewrite of a single target,
a workflow rewrite algorithm is required in order to
to find an optimal rewrite plan for the entire workflow
in the most efficient manner with the aid of the $\VF{}$.
To show that finding an optimal rewrite plan for the workflow is
not straightforward, consider two simple approaches,
namely {\em simple} and {\em greedy}, as shown in
the procedure $\WF$.
The simple variant queries the $\VF{}$ for a rewrite plan for
$t_n$, using it as the workflow rewrite plan of $W$.
The intuition here that
the {\em optimal} rewrite plan of $t_n$ produced by the
$\VF{}$ is also the optimal rewrite plan for $W$.
So, the most likely outcome of applying the simple variant is
that we may not find any rewrite plans for $t_n$.
\end{comment}


==> old/Problem_definition-rewrite2.tex <==
\section{Problem Overview}\label{sec-problem-definition}

% Why is this problem hard?
%  Why is this problem hard?
%  Determining if a rewrite exists
%  Determining a candidate rewrite
%  Containment 

Answering queries using views is a long-studied problem
~\cite{Hale2001,Abit1998,Levy1995}.
When both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete
both for determining whether a rewrite exists~\cite{Levy1995} and
checking the correctness of a rewrite~\cite{Chan1977}.
A \textit{complete} rewriting of a query using views is one that only uses 
views and does not use any of the base relations.
Determining whether there is a complete rewriting of a query using a set of 
views is also NP-complete~\cite{Levy1995} for conjuctive queries.
In this work we consider only complete rewrites, those using
the existing views, without extracting new views from the log.

%Given as input a plan $W$ with a single target, and a set of existing
%materialized views $V$, we want to find a rewrite of $W$ that minimizes 
%the total execution cost of $W$.
When searching for a rewrite of a target $W_i \in W$,
existing views in $V$ may only be {\em partial} solutions with
respect to the target, thus we have to consider creating new candidates by 
{\em merging} views, which explodes the space further.
Finding the minimum cost equivalent rewrite of $W$ requires considering all
combinations of materialized views and operations in $L_R$,
making the solution search space exponential both in 1) the
number of materialized views and 2) the size of $L_R$.
Thus finding a rewrite for a single target in $W$ is computationally expensive.

% Naive Solution: Bottom up solution
As noted in Section~\ref{sec-preliminaries-definitions}, $L_R \subseteq L_W$
has implications for a rewrite algorithm.
A first consequence is that searching for 
an optimal rewrite of only $W_n$ does not suffice.
This is because the inability to find a rewrite for $W_n$ 
does not mean that one cannot find a rewrite at a different target in $W$.
If a rewrite $r_i$ is found for $W_i$, $r_n$ can be expressed as a rewrite
for $W_n$ by combining $r_i$ with the remaining nodes in $W$
indicated by $\node{i+1} \cdots \node{n}$.
The second consequence is that the search process cannot stop once a rewrite 
is found for a target in $W$.
For instance, if a rewrite $r_i$ is found for some target $W_i$,
a rewrite $r_{i-1}$ of $W_{i-1}$ may exist, and it may be cheaper to use 
$r_{i-1}$ followed by $\node{i}$ to obtain a rewrite for $W_i$.
Thus the search process must happen at all targets in $W$.

Given these implications, a solution that searches for rewrites of all targets 
in a bottom-up fashion (i.e., start with $W_n$) is a natural fit.
It obtains the best rewrite for each target, if one exists,
and chooses a subset of these to obtain $r^*$ using a dynamic programming
approach.  
Although we refer to this as bottom-up, strictly bottom-up is not necessary 
since the algorithm must search for rewrites at all targets.

One drawback of this bottom-up approach is that due to the known hardness of 
the problem, there is no easy way of early terminating the search at a single 
target.
Another drawback is that even with an early termination property, the algorithm
 may search for a long time at a target (e.g., $W_i$) only to find an expensive 
 rewrite, when it could have found a better (lower-cost) rewrite at an upstream 
 target (e.g., $W_{i-1}$).
This is illustrated in Example~\ref{example-greedy-plumbing}.

\begin{example}\label{example-greedy-plumbing}
$W$ contains 3 nodes, $n_1$, $n_2$, $n_3$,
each with their individual costs indicated, where cost of $W=12$.
Alongside each node is the space of views to consider for rewriting.
Views that result in a rewrite are indicated by triangles with the rewrite cost.
Views that fail to yield a rewrite are indicated by the empty triangles.
\begin{wrapfigure}{r}{1.15in}
\centering
\hspace*{-0.25in}\includegraphics[width=1.5in]{fig-running-example-1}\hspace*{2cm}
\end{wrapfigure}
A bottom-up algorithm could have examined all the views at $W_3$ finally 
identifying the rewrite with a cost of $12$.
However, as noted, this algorithm cannot stop.
Notice that by searching for rewrites of $W_1$ and $W_2$, the algorithm would 
find a rewrite of cost 2 for $W_1$, and of cost 1 for $n_2$.
It could then combine these with the cost of 1 for the node $n_3$,
resulting in a rewrite of $W_3$ with a total cost of 4.
This is much less than the rewrite found for $n_3$ with a cost of 12.
\end{example}

This approach is clearly inefficient.
Suppose there is an oracle that could reveal the best rewrite for each target, as well as its cost.
An algorithm could make use of the oracle in two ways.
First it could determine the correct order of visiting targets.
For instance, rewrites for $n_1$ and $n_2$ should be considered before $n_3$
as they have the potential to create a low cost rewrite for $n_3$, as shown in the example.
Second it could prune some of the targets from consideration.
For instance, there is no need to search for rewrites at $n_3$ that have a cost greater than 4.
Since the oracle knows the best rewrite of $n_3$ has a cost of 12,
the algorithm can prune $n_3$ from the search space.

\subsection{Outline of our Approach}

We can approximate such an oracle to achieve similar results.
We can order the search space at each target if we can obtain a lower 
bound on the cost of a rewrite using a view.
The lower bound should not require finding a valid rewrite, as this is computationally expensive.
Thus we wish to utilize an alternative cost function that is easy to compute 
and has some desirable property with respect to  the actual cost of a rewrite.

We define an optimistic cost function $\ocost(v,W_i)$ that takes a view $v$ and target $W_i$ 
as inputs and provides a lower-bound on a rewrite of $W_i$ using $v$.
The property of the lower bound is
$$\ocost(v,W_i) \leq \cost(r_i)$$
which we will describe in Section~\ref{sec-ocost}.

The use of a lower-bound cost is inspired by nearest neighbor finding problems
in metric spaces where computing distances between
objects can be computationally expensive, thus
preferring an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
Next we describe how we use the lower bound to approximate the functionality
 of the oracle.

\subsubsection{Pruning at a Single Target}

\onefig{fig-running-example-2}{Candidate views 
  ordered by their \ocost{} with respect to a target $n$}{2in}

We can use our lower bound to order candidate views by their ability to 
produce a low-cost rewrite for a single target node  as illustrated in 
Figure~\ref{fig-running-example-2}.
The triangles correspond to candidate views, and their labels
correspond to the cheapest possible rewrite that each of the
views can produce.
The {\em scale} refers to the lower-bound cost that we assigned
using a suitable method sucht that the candidate views of $n$
are ordered based on this distance.
The utility of the lower bound cost can be immediately seen
as after the algorithm visits the first candidate view, the
cost of best rewrite found so far is set to 6, which reduces
to $5$ after visiting the second candidate view.
The algorithm can terminate early skipping having to look at
the remaining candidate views starting with those candidate
views (i.e., the fourth) whose lower bound distance is greater
than or equal to best rewrite found so far(i.e., 6).



\subsection{Multi-Target Example}

\onefig{fig-running-example-3}{A multi-target example
illustrating utility of $\ocost{}$}{2.5in}

Consider an example shown in Figure~\ref{fig-running-example-3} containing
3 targets $n_1$, $n_2$ and $n_3$ of cost 6,5, and 2, respectively.
The candidate views at each target is ordered by their $\ocost{}$ value.
Similar to the hypothetical oracle, a best-first search algorithm would
first examine a rewrite composed of the candidate view at $n_1$ at $\ocost{}$ of 1 and
the candidate view $n_2$ at a $\ocost{}$ of $2$ and the node $n_3$ at $\cost{}$
of 2, with a $\ocost{}$ of the rewrite at 5.
However, upon obtaining the actual rewrite of the candidate views at $n_1$
and $n_2$, we can see that the actual cost of the rewrite is 10.
The algorithm examines the candidate view at a $\ocost{}$ of $3$ as
it has the potential to produce a rewrite of $\ocost$ of $3$ at $n_1$, \cost{}
$4$ at $n_1$, and $n_3$ at a cost of $2$, but when we found the actual
rewrite of candidate view at $n_1$ its cost was $6$ and hence the rewrite
is discarded.
Now, the algorithm need not examine $n_3$ as the $\ocost{}$ of its
candidate view (i.e., 12) is greater than the cost of best rewrite
found so far.
The algorithm terminates without examining any additional candidate views.
As one can see that the algorithm performs close to the oracle 
in the sense that it starts with the candidate views at different
targets that have the potential to form the lowest cost rewrites
in an incremental fashion.


\subsection{Algorithm Structure}
\onefig{fig-rewriter-block-diagram}{Figure shows the block diagram of a)
rewriter module consisting of an instance of \VF{} (labelled VF) and \WF{}
module that manages the \VF{} using the three operations shown in
(b)}{2.0in}

Our rewrite algorithm takes as input $W$ and the set of materialized views
in the system. It spawns one instance of $\VF{}$ per target in $W$ which
is invoked using the \WF{} algorithm.
Figure~\ref{fig-rewriter-block-diagram}a shows a block diagram of our
rewriter, while Figure~\ref{fig-rewriter-block-diagram}b shows the defined
operations on the $\VF{}$, which we consider a black-box until
Section~\ref{sec-vf}.

In this paper we propose a work efficient
rewrite algorithm for finding the optimal rewrite $r^*$ of $W$
by breaking the problem into two components:
1) $\VF{}$ provides of enumerating the candidate views 
for a single target based on their ability to produce
a low-cost rewrite for the rewrite and 2) $\WF{}$
% that tries to combine the rewrites found for all the $n$ targets into
performs an efficient search of rewrites for all targets in $W$
and outputs a globally optimal rewrite for $W_n$.
The $\WF{}$ concurrently searches for rewrites
at each of the $n$ targets in $W$, while maintaining the
cheapest ({\em best}) rewrite for $W$ found thus far.
Additionally, by communicating the success or failure in finding
a rewrite at a target $W_i$ with other the targets in the workflow,
our approach obviates the need to look in sub-spaces
where it is not possible to find a cheaper rewrite for $W$.
This forms the \textbf{best-first} nature of our proposed algorithm.
In the following sections we present an algorithm which finds 
the {\em optimal rewrite} for a given plan, 
while also being {\em work efficient}.

\begin{comment}
% OLDER TExT REMOVED DUE TO LACK OF SPACE...
The design of our $\VF{}$ is inspired by nearest neighbor finding problems
in metric spaces (e.g., road networks) where computing the distances between
objects can be computationally expensive.
For instance, in the case of road networks the distance between two vertices
requires the invocation of a shortest path algorithm
to find the shortest path between two vertices.
Next, the network distance between
the two vertices can be determined by summing up the edge weights along the shortest path.
In such metric spaces, a common strategy to avoid expensive
network distance computations between vertices is by making
use of an alternate distance function (e.g., Euclidean or the geodesic distance function)
that is easy to compute (i.e., not requiring a search process)
with the desirable property it is always less than or equal to
the network distance function.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the network distance between vertices.

Our current problem domain has a similar properties to
nearest neighbor searches in metric spaces, such as the one described above.
We are given a materialized view $v$ and a query $q$
such that the cost function $\cost()$
corresponds to the amount of time or effort required
in transforming $v$ so that it produces an output that is
identical to that produced by $q$.
As will be discussed later, this problem is known to be NP-hard,
which means that finding a rewrite
workflow for $q$ using $v$ requires examining all possible
rewrites involving $v$ and testing their {\em equivalence} with $q$.
This is expensive as the number of possible rewrites of $q$ involving
$v$ is exponential in the number of transformation rules in the system.
In other words, computing the rewrite plan for $q$ using $v$
first requires finding a rewrite plan for $q$, which is a search
process similar to the shortest computation in road networks.
The intuition here is that we want to make use of another distance
function, which is easy to compute and has some desirable with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$
that takes as input $v$ and $q$ and always provides a
lower-bound on $\cost()$ without enumerating
all possible rewrites of $q$ involving $v$.
In other words, if $r$ is the cheapest rewrite plan
of $q$ involving $r$, we have that $\cost(r) \leq \ocost(v,q)$.
\end{comment}

\begin{comment}
% CUT DUE TO LACK OF SPACE.... :(
Our design of a $\VF{}$ is inspired by nearest neighbor finding problems
in metric and non-metric spaces where computing distances between
objects can be computationally expensive.
In such spaces, a common strategy to avoid expensive distance computations is to
use of an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the actual distance between the objects.
\end{comment}


The $\WF$ uses an instance of the $\VF$ at each target.
The $\WF$ treats $\VF$ as a black-box and exploits its $\ocost$ functionality
to incrementally search the space of rewrites for $W$.
After every step of the incremental search at some target $W_i$ the following two properties are true.

\begin{enumerate}
\item The $\VF$ at target $W_i$ performs an incremental expansion to some
 cost value $d$ as requested by the $\WF{}$, and there are no remaining
 rewrites to be found for \textbf{sub-workflow} $W_i$ that has a cost less than $d$.
\item After the $\WF$ performs an incremental expansion of the $\VF$ at $W_i$ to cost $d$,
there are no remaining rewrites to be found for \textbf{workflow} $W$ 
with cost less than $d'$, where $d' \leq d$.

\end{enumerate}

The key feature of our method is the $\ocost$ functionality that allows the $\WF{}$
to incrementally search the space of rewrites of $W$, such that $\WF$
finds the optimal rewrite of $W$ in a work efficient manner.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
While the details of the $\VF{}$ algorithm and the cost
functions will will be provided in a later section,
for the sake of developing the $\WF{}$ algorithm,
it is sufficient to model $\VF{}$ as a black-box
$\VF(W_i, d, d',\cost(), \ocost())$, $d < d'$, that takes
as input a workflow $W_i$, two thresholds $d, d'$,
a cost function $\cost()$, an optimistic cost function $\ocost{}$
and outputs a single rewrite $r$ of $W_i$ with the following properties:

\begin{enumerate}

\item $r$ is a rewrite workflow for $W_i$ using $V$ and the transformation rules

\item The invocation of the $\VF(W_i,d,d')$ such that $d < d'$
examines all rewrites of $W_i$ whose optimistic cost is less than or equal to $d'$.
Moreover, any subsequent invocation of
$\VF(t_i, d', d", \cost(), \ocost())$, such that $d' < d"$,
will not produce a rewrite whose optimistic cost is less than or equal to $d'$.

\item $d < \ocost(r) \leq d'$ such that $r$ has the lowest
cost among all the plans found by $\VF{}$ in this invocation.

% \item The time taken (or cost) to answer $\VF(t_i,d,d")$ is
% just a little more than the time taken to answer
% $\VF(t_1, d, d')$ and $\VF(t_1, d', d")$.
\end{enumerate}
\end{comment}



\begin{comment}
\begin{algorithm}[htp]\label{algn-main-setup}
\begin{algorithmic}[1]
\State {\sf sub} $\WF$($W$)\\
\Comment{Produces an optimal rewrite of $W$ using $\VF$}
\State $p^* \qlet W_n$\Comment{Original workflow}
\If{{\bf {\em simple/traditional} variant}}
   \State $p$ \qlet $\VF(t_n)$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
\ElsIf{{\bf {\em bottom-up greedy} variant}}
   \ForAll{$t_i$ in $\{t_n \cdots t_1\}$}
    \State $p \qlet \VF(t_i) \cup \{\node{i+1} \cdots \node{n}\}$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
   \EndFor
\EndIf
\State Rewrite $W$ using $p^*$
\end{algorithmic}
\end{algorithm}

Given the $\VF{}$ only finds a rewrite of a single target,
a workflow rewrite algorithm is required in order to
to find an optimal rewrite plan for the entire workflow
in the most efficient manner with the aid of the $\VF{}$.
To show that finding an optimal rewrite plan for the workflow is
not straightforward, consider two simple approaches,
namely {\em simple} and {\em greedy}, as shown in
the procedure $\WF$.
The simple variant queries the $\VF{}$ for a rewrite plan for
$t_n$, using it as the workflow rewrite plan of $W$.
The intuition here that
the {\em optimal} rewrite plan of $t_n$ produced by the
$\VF{}$ is also the optimal rewrite plan for $W$.
So, the most likely outcome of applying the simple variant is
that we may not find any rewrite plans for $t_n$.
\end{comment}

\begin{comment}

Suppose that we had an {\em oracle} that would identify the lowest
cost rewrite at each target without having to exhaustively 
enumerate the search space at each target.
For example, in Example~\ref{example-greedy-plumbing}
it would identify that $n_1$ contains a rewrite at a cost
of 2, $n_2$ at a cost of 1, and $n_3$ at a cost of 12.
Given such an oracle, an hypothetical algorithm would examine
the rewrites at differrent targets in a global ordering 
of its ability to produce a low cost rewrite for $W$.
First, it would examine the rewrite at $n_2$ at cost of 1 with a 
hypothetical rewrite at $n_1$ at a cost of $\geq 1$ followed
by $n_3$ for a cost of $\geq 3$.
Next, it would compose the next low cost rewrite by using 
the rewrite at $n_2$ at a cost of 1, rewrite at $n_1$ at a cost of 2,
followed by $n_3$ at a cost of 1 for a rewrite that costs $4$.
Having obtained a rewrite at a cost of 4 means that $n_3$ need not
be examined as its best rewrite of 12 is much more expensive than
the cost of 4 we know about.
\end{comment}

\begin{comment}
This approach is clearly inefficient.
The algorithm would have performed much better had it known something 
about the cost of the rewrites at each target.
Then it would have started with $n_1$ and $n_2$, and possibly avoided searching
for all rewrites at $n_3$.
Additionally, it could use the cost of the rewrites found for $n_1$ and $n_2$ 
(2 and 1 respectively) to bound the search space at $n_3$.
For example, knowledge of those rewrites for $n_1$ and $n_2$, means that 
we can obtain a rewrite of $n_3$ for cost $2+1+1=5$.
Thus there is no reason to keep searching for rewrites at $n_3$ that have a
cost greater than $5$.
This would help prune the search space at $n_3$, thus never needing to 
find the expensive rewrite of $n_3$ for a cost of 12.
Searching for all possible rewrites at a node is extremely time consuming 
especially if there are many materialized views in the system.
The inefficiency of a bottom-up approach is partly due to not considering the 
rich interactions possible between the $n$ search problems ($n$ targets) in $W$.
\end{comment}

==> old/Problem_definition-rewrite3.tex <==
\section{Problem Overview}\label{sec-problem-definition}

% Why is this problem hard?
%  Why is this problem hard?
%  Determining if a rewrite exists
%  Determining a candidate rewrite
%  Containment 
%\subsection{Challenges in the Problem}
Two factors make our problem
challenging: (1) the complexity of answering queries
using views, and (2) the property that $L_R \subseteq L_W$.

First, answering queries using views is a long-studied problem
~\cite{Hale2001,Abit1998,Levy1995} and known to be hard.
When both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete.
% both for determining whether a rewrite exists~\cite{Levy1995} and
% checking the correctness of a rewrite~\cite{Chan1977}.
A \textit{complete} rewriting of a query using views is one that only uses 
views and does not use any of the base relations.
Determining whether there is a complete rewriting of a query using a set of 
views is also NP-complete~\cite{Levy1995} for conjunctive queries.
In this work we consider only complete rewrites.
% , those using the existing views, without extracting new views from the log.

%Given as input a plan $W$ with a single target, and a set of existing
%materialized views $V$, we want to find a rewrite of $W$ that minimizes 
%the total execution cost of $W$.
When searching for a rewrite of a target, % $W_i \in W$,
existing views in $V$ may only represent {\em partial} solutions~\cite{Hale2001} with
respect to the target. 
Partial solutions can be repeatedly merged to produce {\em complete} solutions, 
which explodes the space further~\cite{Hale2001,Agra2000}.
\textit{Candidate views} are those considered by the rewriter, which
  includes all views in $V$ and all hypothetical 
views obtained by merging views in $V$   
during the process of creating complete solutions.
% using a merge procedure described in Section~\ref{sec-viewfinder}.
Finding the minimum cost equivalent rewrite of $W$ requires considering
merging views in $V$ and operations in $L_R$,
making the solution search space exponential both in 1) the
number of views in $V$ and 2) the size of $L_R$.
Thus finding a rewrite for a single target in $W$ is computationally expensive.

% Naive Solution: Bottom up solution
Second, 
as noted in Section~\ref{sec-preliminaries-definitions}, $L_R \subseteq L_W$
has the following implication that make a rewrite algorithm more challenging.
% A first consequence is that 
Searching for 
an optimal rewrite of only $W_n$ does not suffice.
This is because the inability to find a rewrite for $W_n$ 
does not mean that one cannot find a rewrite at a different target in $W$.
If a rewrite $r_i$ is found for $W_i$, $r_n$ can be expressed as a rewrite
for $W_n$ by combining $r_i$ with the remaining nodes in $W$
indicated by $\node{i+1} \cdots \node{n}$.
% The second consequence is that the search process cannot stop once a rewrite 
% is found for a target in $W$.
% For instance, if a rewrite $r_i$ is found for some target $W_i$,
% a rewrite $r_{i-1}$ of $W_{i-1}$ may exist, and it may be cheaper to use 
% $r_{i-1}$ followed by $\node{i}$ to obtain a rewrite for $W_i$.
Thus the search process must happen at all targets in $W$.

A straightforward solution is to search for rewrites at all targets of $W$.
It obtains the best rewrite for each target, if one exists,
and chooses a subset of these to obtain $r^*$ using a dynamic programming approach.  
% Although we refer to this as bottom-up, strictly bottom-up is not necessary 
% since the algorithm must search for rewrites at all targets.
One drawback of this approach is that
% that due to the known hardness of the problem, 
there is no easy way of early terminating the search at a single target.
Another drawback is that even with an early termination property, the algorithm
may search for a long time at a target (e.g., $W_i$) only to find an expensive 
rewrite, when it could have found a better (lower-cost) rewrite at an upstream 
target (e.g., $W_{i-1}$) more quickly.
This is illustrated in Example~\ref{example-greedy-plumbing}.


\begin{example}\label{example-greedy-plumbing}
$W$ contains 3 nodes, $n_1$, $n_2$, $n_3$,
each with their individual costs as indicated, where cost of $W=13$.
Alongside each node is the space of views to consider for rewriting.
\begin{wrapfigure}{r}{1.15in}
\centering
\vspace{-0.1in}
\hspace*{-0.25in}\includegraphics[width=1.5in]{fig-running-example-1}\hspace*{2cm}
\vspace{-0.1in}
\end{wrapfigure}
Candidate views that result in a rewrite 
are indicated by triangles with the rewrite cost and
those that fail to yield a rewrite are indicated by the empty triangles.
An algorithm could have examined all the views at $W_3$ finally 
identifying the rewrite with a cost of $12$.
However, as noted, this algorithm cannot stop.
Notice that by searching for rewrites of $W_1$ and $W_2$, the algorithm would 
find a rewrite of cost 2 for $W_1$, and of cost 1 for $W_2$.
It could then combine these with the cost of 2 for the node $n_3$,
resulting in a rewrite of $W_3$ with a total cost of 5.
This is much less than the rewrite found for $W_3$ with a cost of 12.
Had the algorithm known about the low-cost rewrites at $n_1$
and $n_2$, it could have searched less of the space at $n_3$.
\end{example}

Now assume that, during the search for rewrites of a given target,
we can somehow obtain the lower bound of the cost of possible rewrites.
Such information would be useful to stop the search earlier in two ways.
First, if we know the lowest cost of rewrites in the unexplored space
of a single target is
higher than the cost of a rewrite already found, there is no use to continue
searching the remaining space. 
Second, the failures and successes at finding
a rewrite at one target can be used to inform the search at a different target.
For example, if we already found the best rewrites for $n_1$ and $n_2$, we can
stop search at $n_3$ when all remaining rewrites for $n_3$ have a cost greater than 5.
Assuming that lower bounds are available,
a challenging question then is how to best utilize such information
to search this complex space of query rewriting.


%This approach is clearly inefficient.
%Suppose there is an oracle that could reveal the best rewrite for each target, 
%as well as its cost.
%An algorithm could make use of the oracle in two ways.
%First it could determine the correct order of visiting targets.
%For instance, rewrites for $n_1$ and $n_2$ should be considered before $n_3$
%as they have the potential to create a low cost rewrite for $n_3$, as shown in 
%the example.
%Second it could prune some of the targets from consideration.
%For instance, there is no need to search for rewrites at $n_3$ that have a cost
%greater than 4.
%Since the oracle knows the best rewrite of $n_3$ has a cost of 12,
%the algorithm can prune $n_3$ from the search space.

\subsection{Outline of our Approach}\label{sec-solution-outline}

%We can approximate such an oracle to achieve similar results.
We propose a work efficient query rewriting algorithm that searches the
space at each target ordered by a lower bound on the cost
of a rewrite using a view.
%can do this by ordering the search space at each target if we can obtain a lower 
%bound on the cost of a rewrite using a view.
The lower bound should not require finding a valid rewrite, as this is 
computationally expensive.
Thus we wish to utilize an alternative cost function that is easy to compute 
and has some desirable property with respect to  the actual cost of a rewrite.

We define an optimistic cost function $\ocost(W_i,v)$ that takes 
a candidate view $v$ 
and target $W_i$ as inputs and provides a lower-bound on a rewrite $r_i$ of $W_i$ 
using $v$.
$r_i$ is a rewrite of $W_i$ that uses the candidate view $v$.
The property of the lower bound is $$\ocost(W_i,v) \leq \cost(r_i)$$
which we will describe further in Section~\ref{sec-ocost}.  
For the purposes of discussion here we assume the existence of this function
and it can be employed as a black-box.
The use of a lower-bound cost is inspired by nearest neighbor finding problems
in metric spaces where computing distances between objects can be 
computationally expensive, thus preferring an alternate distance function 
that is easy to compute with the desirable property that it is always less 
than or equal to the actual distance.

%In this paper we propose a 
Given $\ocost{}$ function,
our rewrite algorithm finds the 
optimal rewrite $r^*$ of $W$ by breaking the problem into two components:
\begin{enumerate}
\item $\WF{}$ (Section~\ref{sec-best-first-workflow-rewrite})
% that tries to combine the rewrites found for all the $n$ targets into
performs an efficient search of rewrites for all targets in $W$ and outputs a
globally optimal rewrite for $W_n$.
\item $\VF{}$ (Section~\ref{sec-viewfinder}) enumerates candidate views 
for a single target based on their potential to produce a low-cost rewrite of 
the target, and is utilized by $\WF{}$.
\end{enumerate}

The \VF{} orders candidate views at a target as illustrated in the example 
alongside.
These graphics show candidate views as triangles arranged by their 
$\ocost{}$ to a target as indicated by the scaled line below the views.
The $\ocost{}$ of all views can be obtained quickly, which determines their
placement along the line.
The top graphic shows the initial state of $\VF{}$ before searching
for rewrites.
The bottom graphic shows the state of $\VF{}$ after examining two
candidate views for rewrite.
The cost of the rewrite for each candidate view is
indicated inside the triangle.
\begin{wrapfigure}{r}{1in}
\centering
\vspace{-0.1in}
\hspace*{-0.25in}\includegraphics[width=1.25in]{fig-running-example-2}\hspace*{2cm}
\vspace{-0.1in}
\end{wrapfigure}
The \VF{} began by examining the view at $\ocost{}$ of 1 as this view
had the potential to produce the lowest-cost rewrite of the target.  
It obtains the actual cost of a rewrite using this view, found to be 6 as marked.
The next candidate view was at $\ocost$ of 3, which 
is examined and its rewrite cost was found to 
be 5.
So, the best rewrite found for the target is now 5. 
The utility of the lower bound cost can be immediately seen now
as there is no reason to examine the next candidate 
view which has an $\ocost{}$ of 7.
Thus any remaining views can be pruned 
from consideration, and the $\VF{}$ at this target can terminate early.

%cost of best rewrite found so far is set to 6, which reduces
%to $5$ after visiting the second candidate view.
%The algorithm can terminate early skipping having to look at
%the remaining candidate views starting with those candidate
%views (i.e., the fourth) whose lower bound distance is greater
%than or equal to best rewrite found so far (i.e., 6).


The $\WF{}$ spawns one instance of $\VF{}$ per target in $W$ and 
uses the information from the search at a target to  
inform and control the search at other targets.
By exploiting $\ocost{}$ our algorithm 
performs an incremental search with a $\VF{}$ at each target.
It starts with the candidate views at different targets that have the potential 
to form the lowest cost rewrite of $W$ and continues its search in an 
incremental fashion until termination.
In this way our approach obviates the need to 
look in sub-spaces where it is not possible to find a cheaper rewrite for $W$.
This forms the {\em best-first} nature of our solution.
Note that due to the known hardness of the problem, in the worst case it must
examine all candidate views at each target.
% In the following sections we present our algorithm which finds the optimal 
% rewrite $r^*$ of $W$, while also being {\em work efficient} by performing its 
% search in the manner just described.


\begin{comment}
Our algorithm exploits the lower bound, $\ocost{}$,
by using $\VF{}$ 
and $\WF{}$ to perform an incremental search. % wisely.
It starts with the candidate views at different targets that have the potential 
to form the lowest cost rewrite of $W$ and continues its search in an 
incremental fashion until termination.
Note that due to the known hardness of the problem, in the worst case it must
examine all candidate views at each target.
In the following sections we present our algorithm which finds the optimal 
rewrite $r^*$ of $W$, while also being {\em work efficient} by performing its 
search in the manner just described.

Our rewrite algorithm spawns one instance of $\VF{}$ per target in $W$
and $\WF{}$ maintains the best ({\em lowest-cost}) rewrite for $W$ found 
during the search process.
Because there are $n$ search problems, $\WF{}$ can use
the information from 
rewrites attempted at one target to inform the search at another target.
By communicating the success or failure in finding a rewrite at a target
with the other targets in the workflow, our approach obviates the need to 
look in sub-spaces where it is not possible to find a cheaper rewrite for $W$.
This forms the {\em best-first} nature of our proposed algorithm.
\end{comment}

To illustrate \WF{} process, the example shown alongside again shows $W$ 
containing 3 targets $n_1$, $n_2$ and $n_3$ with cost 6, 5, and 2, 
respectively.
The candidate views at each target are ordered by their $\ocost{}$ value as
described previously.

%Similar to the hypothetical oracle,
Our best-first algorithm would
first examine a rewrite composed of the next candidate view at $n_1$ 
($\ocost{}$ of 1), the next candidate view at $n_2$ 
($\ocost{}$ of $2$) and node $n_3$ ($\cost{}$ of 2).
This combination has the {\em potential} to produce a rewrite of $W_3$ with an 
$\ocost{}$ of 1+2+2=5.
However, upon obtaining the actual rewrite of the candidate views at $n_1$
and $n_2$, we can see that the actual cost of this rewrite is 10.
\begin{wrapfigure}{r}{1.75in}
\vspace{-0.1in}
\hspace*{-0.25in}\includegraphics[width=2.25in]{fig-running-example-3}
\vspace{-0.1in}
\end{wrapfigure}
The algorithm continues by examining the next
candidate view at $n_1$ ($\ocost{}$ of $3$).
This can potentially produce a rewrite of $W_3$ by composing: 
$\ocost$ of $3$ at $n_1$, plus rewrite with \cost{} $4$ 
at $n_2$, plus $n_3$ with $\cost{}$ $2$ (3+4+2=9).
However, this candidate view at $n_1$ was found to have an
actual cost of $6$.
Hence, this rewrite of $W$ has a $\cost{}$ of 12 (6+4+2) 
and can be discarded since $\WF{}$ already has found a rewrite of $W$
with $\cost{}$ 10.
The algorithm need not examine any remaining candidate views in $n_1$ and $n_3$
as they do not have the potential to produce a cheaper rewrite.


% \onefig{fig-rewriter-block-diagram}{Figure shows the block diagram of a)
% rewriter module consisting of an instance of \VF{} (labelled VF) and \WF{}
% module that manages the \VF{} using the three operations shown in
% (b)}{2.0in}

\begin{comment}
% OLDER TExT REMOVED DUE TO LACK OF SPACE...
The design of our $\VF{}$ is inspired by nearest neighbor finding problems
in metric spaces (e.g., road networks) where computing the distances between
objects can be computationally expensive.
For instance, in the case of road networks the distance between two vertices
requires the invocation of a shortest path algorithm
to find the shortest path between two vertices.
Next, the network distance between
the two vertices can be determined by summing up the edge weights along the shortest path.
In such metric spaces, a common strategy to avoid expensive
network distance computations between vertices is by making
use of an alternate distance function (e.g., Euclidean or the geodesic distance function)
that is easy to compute (i.e., not requiring a search process)
with the desirable property it is always less than or equal to
the network distance function.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the network distance between vertices.

Our current problem domain has a similar properties to
nearest neighbor searches in metric spaces, such as the one described above.
We are given a materialized view $v$ and a query $q$
such that the cost function $\cost()$
corresponds to the amount of time or effort required
in transforming $v$ so that it produces an output that is
identical to that produced by $q$.
As will be discussed later, this problem is known to be NP-hard,
which means that finding a rewrite
workflow for $q$ using $v$ requires examining all possible
rewrites involving $v$ and testing their {\em equivalence} with $q$.
This is expensive as the number of possible rewrites of $q$ involving
$v$ is exponential in the number of transformation rules in the system.
In other words, computing the rewrite plan for $q$ using $v$
first requires finding a rewrite plan for $q$, which is a search
process similar to the shortest computation in road networks.
The intuition here is that we want to make use of another distance
function, which is easy to compute and has some desirable with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$
that takes as input $v$ and $q$ and always provides a
lower-bound on $\cost()$ without enumerating
all possible rewrites of $q$ involving $v$.
In other words, if $r$ is the cheapest rewrite plan
of $q$ involving $r$, we have that $\cost(r) \leq \ocost(v,q)$.
\end{comment}

\begin{comment}
% CUT DUE TO LACK OF SPACE.... :(
Our design of a $\VF{}$ is inspired by nearest neighbor finding problems
in metric and non-metric spaces where computing distances between
objects can be computationally expensive.
In such spaces, a common strategy to avoid expensive distance computations is to
use of an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the actual distance between the objects.
\end{comment}

\begin{comment}
The $\WF$ uses an instance of the $\VF$ at each target.
The $\WF$ treats $\VF$ as a black-box and exploits its $\ocost$ functionality
to incrementally search the space of rewrites for $W$.
After every step of the incremental search at some target $W_i$ the following two properties are true.

\begin{enumerate}
\item The $\VF$ at target $W_i$ performs an incremental expansion to some
 cost value $d$ as requested by the $\WF{}$, and there are no remaining
 rewrites to be found for \textbf{sub-workflow} $W_i$ that has a cost less than $d$.
\item After the $\WF$ performs an incremental expansion of the $\VF$ at $W_i$ to cost $d$,
there are no remaining rewrites to be found for \textbf{workflow} $W$ 
with cost less than $d'$, where $d' \leq d$.

\end{enumerate}

The key feature of our method is the $\ocost$ functionality that allows the $\WF{}$
to incrementally search the space of rewrites of $W$, such that $\WF$
finds the optimal rewrite of $W$ in a work efficient manner.
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
While the details of the $\VF{}$ algorithm and the cost
functions will will be provided in a later section,
for the sake of developing the $\WF{}$ algorithm,
it is sufficient to model $\VF{}$ as a black-box
$\VF(W_i, d, d',\cost(), \ocost())$, $d < d'$, that takes
as input a workflow $W_i$, two thresholds $d, d'$,
a cost function $\cost()$, an optimistic cost function $\ocost{}$
and outputs a single rewrite $r$ of $W_i$ with the following properties:

\begin{enumerate}

\item $r$ is a rewrite workflow for $W_i$ using $V$ and the transformation rules

\item The invocation of the $\VF(W_i,d,d')$ such that $d < d'$
examines all rewrites of $W_i$ whose optimistic cost is less than or equal to $d'$.
Moreover, any subsequent invocation of
$\VF(t_i, d', d", \cost(), \ocost())$, such that $d' < d"$,
will not produce a rewrite whose optimistic cost is less than or equal to $d'$.

\item $d < \ocost(r) \leq d'$ such that $r$ has the lowest
cost among all the plans found by $\VF{}$ in this invocation.

% \item The time taken (or cost) to answer $\VF(t_i,d,d")$ is
% just a little more than the time taken to answer
% $\VF(t_1, d, d')$ and $\VF(t_1, d', d")$.
\end{enumerate}
\end{comment}



\begin{comment}
\begin{algorithm}[htp]\label{algn-main-setup}
\begin{algorithmic}[1]
\State {\sf sub} $\WF$($W$)\\
\Comment{Produces an optimal rewrite of $W$ using $\VF$}
\State $p^* \qlet W_n$\Comment{Original workflow}
\If{{\bf {\em simple/traditional} variant}}
   \State $p$ \qlet $\VF(t_n)$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
\ElsIf{{\bf {\em bottom-up greedy} variant}}
   \ForAll{$t_i$ in $\{t_n \cdots t_1\}$}
    \State $p \qlet \VF(t_i) \cup \{\node{i+1} \cdots \node{n}\}$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
   \EndFor
\EndIf
\State Rewrite $W$ using $p^*$
\end{algorithmic}
\end{algorithm}

Given the $\VF{}$ only finds a rewrite of a single target,
a workflow rewrite algorithm is required in order to
to find an optimal rewrite plan for the entire workflow
in the most efficient manner with the aid of the $\VF{}$.
To show that finding an optimal rewrite plan for the workflow is
not straightforward, consider two simple approaches,
namely {\em simple} and {\em greedy}, as shown in
the procedure $\WF$.
The simple variant queries the $\VF{}$ for a rewrite plan for
$t_n$, using it as the workflow rewrite plan of $W$.
The intuition here that
the {\em optimal} rewrite plan of $t_n$ produced by the
$\VF{}$ is also the optimal rewrite plan for $W$.
So, the most likely outcome of applying the simple variant is
that we may not find any rewrite plans for $t_n$.
\end{comment}

\begin{comment}
Suppose that we had an {\em oracle} that would identify the lowest
cost rewrite at each target without having to exhaustively 
enumerate the search space at each target.
For example, in Example~\ref{example-greedy-plumbing}
it would identify that $n_1$ contains a rewrite at a cost
of 2, $n_2$ at a cost of 1, and $n_3$ at a cost of 12.
Given such an oracle, an hypothetical algorithm would examine
the rewrites at different targets in a global ordering 
of its ability to produce a low cost rewrite for $W$.
First, it would examine the rewrite at $n_2$ at cost of 1 with a 
hypothetical rewrite at $n_1$ at a cost of $\geq 1$ followed
by $n_3$ for a cost of $\geq 3$.
Next, it would compose the next low cost rewrite by using 
the rewrite at $n_2$ at a cost of 1, rewrite at $n_1$ at a cost of 2,
followed by $n_3$ at a cost of 1 for a rewrite that costs $4$.
Having obtained a rewrite at a cost of 4 means that $n_3$ need not
be examined as its best rewrite of 12 is much more expensive than
the cost of 4 we know about.
\end{comment}

\begin{comment}
This approach is clearly inefficient.
The algorithm would have performed much better had it known something 
about the cost of the rewrites at each target.
Then it would have started with $n_1$ and $n_2$, and possibly avoided searching
for all rewrites at $n_3$.
Additionally, it could use the cost of the rewrites found for $n_1$ and $n_2$ 
(2 and 1 respectively) to bound the search space at $n_3$.
For example, knowledge of those rewrites for $n_1$ and $n_2$, means that 
we can obtain a rewrite of $n_3$ for cost $2+1+1=5$.
Thus there is no reason to keep searching for rewrites at $n_3$ that have a
cost greater than $5$.
This would help prune the search space at $n_3$, thus never needing to 
find the expensive rewrite of $n_3$ for a cost of 12.
Searching for all possible rewrites at a node is extremely time consuming 
especially if there are many materialized views in the system.
The inefficiency of a bottom-up approach is partly due to not considering the 
rich interactions possible between the $n$ search problems ($n$ targets) in $W$.
\end{comment}


==> old/Problem_definition-rewrite4.tex <==
\section{Problem Overview}\label{sec-problem-definition}


%  Why is this problem hard?
%  Determining if a rewrite exists
%  Determining a candidate rewrite
%  Containment 


Our UDF model enables better reuse of views to improve query performance,
even when queries contain complex functions.
However, reusing an existing view toward rewriting a query with any arbitrary UDF
requires the rewrite language to include all UDFs in the system.
Hence any UDF admitted to the system becomes part of the rewrite language.
However, given that any user can add a new UDF to the system, including all UDFs 
in the rewrite language makes the process of finding a rewrite impractical for
any realistic workload and number of views.  
This is because the search space of finding a rewrite is exponential in both 
1) the number of views in $V$ and 2) the size of the rewrite language.
The problem is known to be hard even when both the queries and the 
views are expressed in a language that
only includes conjunctive queries~\cite{Hale2001,Abit1998,Levy1995}.

For practical reasons, it is necessary that only a small subset of all UDFs
be included in the rewrite language.  
In this work we include select, project, join, group-by,
and several UDFs that compute aggregates (e.g., min, max, count, sum) in
rewrite language but others are possible.
Our system provides an easy way of adding new UDFs, but they do not automatically
become part of the rewrite language.  
Selecting the right subset of UDFs for the rewrite language is an interesting 
problem.
It must consider the tradeoff between the added expressiveness of the rewrite language
versus the additional exponential cost incurred to search for rewrites. 
For instance, it may be worthwhile to add a popular UDF to the rewrite language
if it enables much better reuse of views in spite of making the rewrite search 
take longer.




However, an implication of the rewrite language being a subset of the query 
language means that finding the optimal rewrite for $W$ requires that we 
solve $n$ rewrite search problems.
This is because finding an optimal rewrite of only $W_n$ does not suffice.
The inability to find a rewrite for $W_n$ 
does not mean that one cannot find a rewrite at a different target in $W$.
Furthermore, even if a rewrite is found for $W_n$, this does not mean that  
a cheaper rewrite of $W$ does not exist at a different target $W_i$.
For example, a rewrite $r_i$ found for $W_i$  can be expressed as a rewrite
for $W_n$ by combining $r_i$ with the remaining nodes in $W$
indicated by $\node{i+1} \cdots \node{n}$.
Thus the search process for the optimal rewrite must happen at all $n$ targets 
in $W$, which complicates a solution since solving even a single instance of the 
problem is hard.


A straightforward solution is to search independently for rewrites at all 
$n$ targets of $W$.
This approach finds the best rewrite for each target, if one exists,
and chooses a subset of these to obtain the optimal rewrite $r^*$.
One drawback of this approach is that
there is no way of terminating early the search at a single target.
Another drawback is that even with an early termination property, the algorithm
may search for a long time at a target (e.g., $W_i$) only to find an expensive 
rewrite, when it could have found a better (lower-cost) rewrite at an upstream 
target (e.g., $W_{i-1}$) more quickly if it had known where to look first. 
This is illustrated in Example~\ref{ex-greedy-plumbing}.

\begin{example}\label{ex-greedy-plumbing}
$W$ contains 3 nodes, $n_1$, $n_2$, $n_3$,
each with their individual costs as indicated, where cost of $W=13$.
Alongside each node is the space of views to consider for rewriting.
\begin{wrapfigure}{r}{1.15in}
\centering
\vspace{-0.1in}
\hspace*{-0.25in}\includegraphics[width=1.5in]{fig-running-example-1}\hspace*{2cm}
\vspace{-0.1in}
\end{wrapfigure}
Candidate views that result in a rewrite 
are indicated by triangles with the rewrite cost and
those that fail to yield a rewrite are indicated by the empty triangles.
An algorithm could have examined all the views at $W_3$ finally 
identifying the rewrite with a cost of $12$.
However, as noted, this algorithm cannot stop.
Notice that by searching for rewrites of $W_1$ and $W_2$, the algorithm would 
find a rewrite of cost 2 for $W_1$, and of cost 1 for $W_2$.
It could then combine these with the cost of 2 for the node $n_3$,
resulting in a rewrite of $W_3$ with a total cost of 5.
This is much less than the rewrite found for $W_3$ with a cost of 12.
Had the algorithm known about the low-cost rewrites at $n_1$
and $n_2$, it could have searched less of the space at $n_3$.
\end{example}

\subsection{Overview of our Approach}\label{sec-solution-outline}
We significantly improve the search for the optimal rewrite 
by making use of the lower bound function $\ocost{}$ introduced in 
Section~\ref{sec-costing-udfs}.
During the search for rewrites at each of the $n$ targets, 
the lower bound 
can be used to help terminate the search earlier in two ways.
First, for any rewrite $r$ found at a given target, if 
the lower-bound on the cost of any possible  rewrites remaining in the 
unexplored space is greater than the cost of $r$, there is no need 
to continue searching the remaining space. 
This enables us to terminate the search early at a single target.
Second, we can use $r$ and the lower bound on the remaining unexplored 
space at one target to inform the search at a different target.
For instance, in Example~\ref{ex-greedy-plumbing}, after finding 
the best rewrites for $n_1$ and $n_2$ of cost 2 and 1 respectively, 
we can stop searching at $n_3$ when the lower-bound on the cost of the
unexplored space is greater than 5, since we already have found a rewrite
of $W$ with cost 5.


%This approach is clearly inefficient.
%Suppose there is an oracle that could reveal the best rewrite for each target, 
%as well as its cost.
%An algorithm could make use of the oracle in two ways.
%First it could determine the correct order of visiting targets.
%For instance, rewrites for $n_1$ and $n_2$ should be considered before $n_3$
%as they have the potential to create a low cost rewrite for $n_3$, as shown in 
%the example.
%Second it could prune some of the targets from consideration.
%For instance, there is no need to search for rewrites at $n_3$ that have a cost
%greater than 4.
%Since the oracle knows the best rewrite of $n_3$ has a cost of 12,
%the algorithm can prune $n_3$ from the search space.



We propose a work efficient query rewriting algorithm that uses $\ocost{}$ to
order the search space at each target.
Since  a property of $\ocost{}$ is that it is easy to compute, it enables us
to quickly order the candidate views at each target by the lower-bound
on their ability to produce a rewrite (if one exists).
This allows our algorithm to step through the space at each target in an 
incremental fashion.
Our approach is inspired by nearest neighbor finding problems
in metric spaces where computing distances between objects can be 
computationally expensive, thus preferring an alternate distance function (e.g., $\ocost{}$)
that is easy to compute with the desirable property that it is always less 
than or equal to the actual distance.


Using the $\ocost{}$ function to order the space, our rewrite algorithm finds the 
optimal rewrite $r^*$ of $W$ by breaking the problem into two components:
\begin{enumerate}
\item $\WF{}$ (Section~\ref{sec-best-first-workflow-rewrite})
% that tries to combine the rewrites found for all the $n$ targets into
performs an efficient search of rewrites for all targets in $W$ and outputs a
globally optimal rewrite for $W_n$.
\item $\VF{}$ (Section~\ref{sec-viewfinder}) enumerates candidate views 
for a single target based on their potential to produce a low-cost rewrite of 
the target, and is utilized by $\WF{}$.
\end{enumerate}


==> old/Problem_definition-rewrite5.tex <==
\section{Problem Overview for Rewriting Queries Containing UDFs}\label{sec-problem-definition}


%  Why is this problem hard?
%  Determining if a rewrite exists
%  Determining a candidate rewrite
%  Containment 


Our UDF model enables reuse of views to improve query performance,
even when queries contain complex functions.
However, reusing an existing view toward rewriting a query with any arbitrary UDF
requires the rewrite process to include all UDFs in the system.
%Hence any UDF admitted to the system becomes part of the rewrite language.
Given that any user can add a new UDF to the system, including all UDFs 
in the rewrite process makes searching for the optimal rewrite impractical for
any realistic workload and number of views.  
This is because the search space of finding a rewrite is exponential in both 
1) the number of views in $V$ and 2) the number of operations considered by 
the rewrite process.
The problem is known to be hard even when both the queries and the 
views are expressed in a language that only includes conjunctive queries~\cite{Hale2001,Abit1998,Levy1995}.
In our system, both the queries and the views can contain any arbitrary UDF.


Our rewriter considers relational operators  select, project, join, group-by,
aggregations (SPJGA), and a few of the most popular UDFs, as these offer 
frequent opportunities for reuse. 
For practical reasons, it is necessary that only a small subset of all UDFs 
be considered by the rewrite process.  
Even though including additional UDFs  increases opportunities for reusing 
results, it exponentially increases the search space for the rewrite process.
Our system provides an easy way of adding new UDFs, but these are not 
automatically known to the rewriter; 
selecting the right subset of UDFs to include in the rewrite process 
is an interesting open problem.
%It must consider the tradeoff between the added expressiveness of the rewrite 
% language
%versus the additional exponential cost incurred to search for rewrites. 
For instance, it may be worthwhile to include a popular UDF 
if it enables much better reuse of views even though it makes the rewrite 
process longer.


However, an implication of limiting the rewrite process to include only a 
small subset of UDFs means that finding the optimal 
rewrite for $W$ requires that we solve $n$ rewrite search problems.
This is because finding an optimal rewrite of only $W_n$ does not suffice.
Since the rewriter does not consider all UDFs, even if one cannot find a 
rewrite for $W_n$, one \textit{may} be able to find a rewrite at a 
different target in $W$.
Furthermore, even if a rewrite is found for $W_n$, there may be a 
\textit{cheaper} rewrite of $W$ using a rewrite found for a different 
target $W_i$.
For example, a rewrite $r_i$ found for $W_i$  can be expressed as a rewrite
for $W_n$ by combining $r_i$ with the remaining nodes in $W$
indicated by $\node{i+1} \cdots \node{n}$.
Thus the search process for the optimal rewrite must happen at all $n$ targets 
in $W$, which complicates a solution since solving even a single instance of 
the problem is hard.


A naive solution is to search independently for rewrites at all 
$n$ targets of $W$.
This approach finds the best rewrite for each target, if one exists,
and chooses a subset of these to obtain the optimal rewrite $r^*$.
One drawback of this approach is that
there is no way of terminating early the search at a single target.
Another drawback is that even with an early termination property, the algorithm
may search for a long time at a target (e.g., $W_i$) only to find an expensive 
rewrite, when it could have found a better (lower-cost) rewrite at an upstream 
target (e.g., $W_{i-1}$) more quickly if it had known where to look first. 
This is illustrated in Example~\ref{ex-greedy-plumbing}.

\begin{example}\label{ex-greedy-plumbing}
$W$ contains 3 MR job nodes, $n_1$, $n_2$, $n_3$,
each with their individual node cost as indicated, where the total cost of $W$=13 (6+5+2).
Alongside each node is the space of views ($V$) to consider for rewriting.
\begin{wrapfigure}{r}{1.15in}
\centering
\vspace{-0.1in}
\hspace*{-0.25in}\includegraphics[width=1.5in]{fig-running-example-1}\hspace*{2cm}
\vspace{-0.1in}
\end{wrapfigure}
Candidate views that fail to yield a rewrite are indicated by the empty triangles,  
and those that result in a rewrite are indicated by cost of the rewrite found.
A naive algorithm would first examine \emph{exhaustively} the views at $n_3$ finally 
identifying the rewrite of $W$ with a cost of $12$.
However, as noted, to find the optimal rewrite it cannot stop at this point,
and must continue searching for rewrites at $n_1$ and $n_2$.
The algorithm would then find a rewrite at $n_1$ of cost 2, and at $n_2$ of cost 1.
It then combines these with the node $n_3$ (node cost 2), 
resulting in a rewrite of $W$ with a total cost of 5 (2+1+2).
This is much less than the earlier rewrite found at $n_3$ with a cost of 12.
This example shows the algorithm cannot stop even when it finds a rewrite for 
$n_n$.
Also, had the algorithm known about the low-cost rewrites at $n_1$
and $n_2$, it need not have exhaustively searched the space at $n_3$.
\end{example}

\subsection{Overview of our Approach}\label{sec-solution-outline}
We significantly improve the search overhead for the optimal rewrite 
by making use of the lower bound function $\ocost{}$ introduced in 
Section~\ref{sec-costing-udfs}.
During the search for rewrites at each of the $n$ targets, 
the lower bound 
can be used to help terminate the search earlier in two ways.
First, for any rewrite $r$ found at a given target, if 
the lower-bound on the cost of any possible  rewrites remaining in the 
unexplored space is greater than the cost of $r$, there is no need 
to continue searching the remaining space. 
This enables us to terminate the search early at a single target.
Second, we can use $r$ and the lower bound on the remaining unexplored 
space at one target to inform the search at a different target.
For instance, in Example~\ref{ex-greedy-plumbing}, after finding 
the best rewrites for $n_1$ and $n_2$ of cost 2 and 1 respectively, 
we can stop searching at $n_3$ when the lower-bound on the cost of the
unexplored space is greater than 5, since we already have found a rewrite
of $W$ with cost 5.


%This approach is clearly inefficient.
%Suppose there is an oracle that could reveal the best rewrite for each target, 
%as well as its cost.
%An algorithm could make use of the oracle in two ways.
%First it could determine the correct order of visiting targets.
%For instance, rewrites for $n_1$ and $n_2$ should be considered before $n_3$
%as they have the potential to create a low cost rewrite for $n_3$, as shown in 
%the example.
%Second it could prune some of the targets from consideration.
%For instance, there is no need to search for rewrites at $n_3$ that have a cost
%greater than 4.
%Since the oracle knows the best rewrite of $n_3$ has a cost of 12,
%the algorithm can prune $n_3$ from the search space.



We propose a work-efficient query rewriting algorithm that uses $\ocost{}$ to
order the search space at each target.
Since  a property of $\ocost{}$ is that it is easy to compute, it enables us
to quickly order the candidate views at each target by the lower-bound
on their ability to produce a rewrite (if one exists).
This allows our algorithm to step through the space at each target in an 
incremental fashion.
Our approach is inspired by nearest neighbor finding problems
in metric spaces where computing distances between objects can be 
computationally expensive, thus preferring an alternate distance function (e.g., $\ocost{}$)
that is easy to compute with the desirable property that it is always less 
than or equal to the actual distance.


Using the $\ocost{}$ function to order the space, our rewrite algorithm finds the 
optimal rewrite $r^*$ of $W$ by breaking the problem into two components:
\begin{enumerate}
\item $\WF{}$ (Section~\ref{sec-best-first-workflow-rewrite})
% that tries to combine the rewrites found for all the $n$ targets into
performs an efficient search of rewrites for all targets in $W$ and outputs a
globally optimal rewrite for $W_n$.
\item $\VF{}$ (Section~\ref{sec-viewfinder}) enumerates candidate views 
for a single target based on their potential to produce a low-cost rewrite of 
the target, and is utilized by $\WF{}$.
\end{enumerate}


==> old/Problem_definition.tex <==
\section{Problem Definition}\label{sec-problem-definition}

Given as input a workflow $W$, and a set of existing
materialized views $V$, we want to find a rewrite of $W$ that
minimizes the total execution cost of $W$.
% As $W$ is a query, this problem can be formulated
% as the query rewrite problem using materialized views, which is
% known to be NP-complete even considering a language
% for both queries and views belonging to the simple class
% of conjunctive queries~\cite{Levy1995}.
\begin{comment}
We decompose this problem into two sub-problems.
First, we introduce a $\VF{}$ which
given a query, a set of candidate artifacts,
and a set of transformational rules finds the cheapest rewrite workflow of the target,
if such a plan exists.
Next, utilizing the $\VF{}$ at each target,
we introduce a workflow rewrite algorithm $\WF{}$ that obtains the
lowest cost workflow rewrite plan of $W$, while performing minimum amount of work.
\end{comment}
The problem of finding a rewrite of a query using materialized views
is known to be NP-complete even considering a language
for both queries and views belonging to the simple class
of conjunctive queries~\cite{Levy1995}.
Here we must consider a rich workflow language that may include any UDF admitted by the system.
% Furthermore, existing candidates may only be {\em partial} solutions with
% respect to the target, thus we have to consider creating new candidates by {\em merging}
% existing candidates, which explodes the space further.
Finding an optimal rewrite of a query $q$ requires considering all
combinations of materialized views and transformation rules, which
makes the solution search space exponential both in 1) the
number of materialized views ($|V|$) and 2) the number of transformation rules ($|L_R|$).
Thus finding a rewrite for a single target
in a workflow is computationally expensive.


When searching for the optimal rewrite $r^*$ of a workflow $W$,
 $L_R \subseteq L_W$ has the following implications on any search 
 process that finds the optimal rewrite.
A first consequence of $L_R \subseteq L_W$ is that searching for 
an optimal rewrite of only $W_n$ does not suffice.
This is because the inability to find a rewrite for $W_n$ 
does not mean that one cannot find a rewrite at a different target $W_i$ in $W$.
If a rewrite $r$ is found at $W_i$, $r$ can be expressed as a rewrite
for $W_n$ by combining $r$ with the remaining part of the workflow
indicated by $\node{i+1} \cdots \node{n}$.
The second consequence of $L_R \subseteq L_W$ is that
the search process cannot stop once it finds a rewrite 
at any target in $W$.
For instance, if a rewrite $r$ is found for some target $W_i$,
a rewrite $r'$ of
$W_{i-1}$ may exist and it may be cheaper to use $r'$  
to obtain a rewrite for $W_i$ than $r$.
Thus the search process must happen at all targets in $W$.

Given these implications, a bottom-up algorithm is a natural fit.
This algorithm searches for rewrites at all targets 
in the workflow in a bottom-up fashion.
It obtains the best rewrite for each target, if one exists,
and chooses a subset of these to obtain $r^*$ using a dynamic programming
approach.  We call this algorithm bottom-up, although 
strictly bottom-up  is not  necessary since it must search at all targets.

One drawback of the bottom-up approach is that there is  
no easy way of early terminating the search at a single target.
Even with an early termination property,
the algorithm may search for a long time at a target only to find 
an expensive rewrite, 
when it could have found a cheap rewrite much sooner 
at the target above.
This is illustrated in Example~\ref{example-greedy-plumbing}.

\begin{minipage}{0.70\linewidth}
\vspace{0.1in}
\begin{example}\label{example-greedy-plumbing}
The figure alongside shows an example of
a workflow $W$ containing 4 targets.
Suppose that the bottom-up algorithm 
could not find a rewrite for
targets $W_n$ and $W_{n-2}$ in spite of searching
the entire space,
yet was able to find an expensive rewrite for $W_{n-1}$.
The algorithm would have performed much better had
it first looked for rewrites at $W_{n-3}$,
thus obviating the need to search too long 
at $W_{n-2} \cdots W_{n}$.
\end{example}
\end{minipage}%
\hspace{0.1cm}%
\begin{minipage}{0.25\linewidth}
\centering
\includegraphics[width=1in]{fig-greedy-plumbing-fails}
\end{minipage}
\vspace{0.1in}

The bottom-up approach described
is not {\em work efficient} in the sense that
it does not make use of a rewrite found for $W_i$
to bound the search space at another target $W_j$ in the workflow.
For example, had the bottom-up strategy first found the cheap
rewrite at $W_{n-3}$ in Example \ref{example-greedy-plumbing}
it may not have needed to exhaustively
search the space at $W_n$ and at $W_{n-2}$, and even perhaps
may have stopped sooner at $W_{n-1}$.
Note that searching for all possible rewrites at $W_n$ and $W_{n-2}$
is extremely time consuming especially if there are many
materialized views in the system.
% Do we need to say that the complexity is exp in #views and #rules?
The inefficiency of a bottom-up approach is partly due to
not considering the rich interactions possible between the
$n$ search problems at each of the targets in $W$.

% Note that being able to take advantage of the interactions
% between the $n$ rewrite search problems at each of the targets
% requires the design of the $\VF{}$
% to be {\em incremental} in that it can find
% cheaper plans first and expensive plans later as well as
% has the ability to stop early if a cheaper plan is found
% at some other target that obviates the need to search
% further at a particular target.

In this paper we propose a work efficient workflow 
rewrite algorithm for finding $r^*$ 
by breaking the problem into two components:
1) $\VF{}$ finds the best possible rewrite
for a single workflow input and 2) $\WF{}$
% that tries to combine the rewrites found for all the $n$ targets into
performs an efficient search of rewrites for all targets in $W$
and outputs a globally optimal rewrite for $W_n$.
The $\WF{}$ concurrently searches for rewrites
at each of the $n$ targets in $W$, while maintaining the
cheapest ({\em best}) rewrite for $W$ found thus far.
Additionally, by communicating the success or failure in finding
a rewrite at a target $W_i$ with other the targets in the workflow,
our approach obviates the need to look in sub-spaces
where it is not possible to find a cheaper rewrite for $W$.
This forms the \textbf{best-first} nature of our proposed algorithm.
In the following sections we present an algorithm which finds 
the {\em optimal rewrite} for a given workflow, 
while also being {\em work efficient}.

\begin{comment}
% OLDER TExT REMOVED DUE TO LACK OF SPACE...
The design of our $\VF{}$ is inspired by nearest neighbor finding problems
in metric spaces (e.g., road networks) where computing the distances between
objects can be computationally expensive.
For instance, in the case of road networks the distance between two vertices
requires the invocation of a shortest path algorithm
to find the shortest path between two vertices.
Next, the network distance between
the two vertices can be determined by summing up the edge weights along the shortest path.
In such metric spaces, a common strategy to avoid expensive
network distance computations between vertices is by making
use of an alternate distance function (e.g., Euclidean or the geodesic distance function)
that is easy to compute (i.e., not requiring a search process)
with the desirable property it is always less than or equal to
the network distance function.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the network distance between vertices.

Our current problem domain has a similar properties to
nearest neighbor searches in metric spaces, such as the one described above.
We are given a materialized view $v$ and a query $q$
such that the cost function $\cost()$
corresponds to the amount of time or effort required
in transforming $v$ so that it produces an output that is
identical to that produced by $q$.
As will be discussed later, this problem is known to be NP-hard,
which means that finding a rewrite
workflow for $q$ using $v$ requires examining all possible
rewrites involving $v$ and testing their {\em equivalence} with $q$.
This is expensive as the number of possible rewrites of $q$ involving
$v$ is exponential in the number of transformation rules in the system.
In other words, computing the rewrite plan for $q$ using $v$
first requires finding a rewrite plan for $q$, which is a search
process similar to the shortest computation in road networks.
The intuition here is that we want to make use of another distance
function, which is easy to compute and has some desirable with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$
that takes as input $v$ and $q$ and always provides a
lower-bound on $\cost()$ without enumerating
all possible rewrites of $q$ involving $v$.
In other words, if $r$ is the cheapest rewrite plan
of $q$ involving $r$, we have that $\cost(r) \leq \ocost(v,q)$.
\end{comment}

\begin{comment}
% CUT DUE TO LACK OF SPACE.... :(
Our design of a $\VF{}$ is inspired by nearest neighbor finding problems
in metric and non-metric spaces where computing distances between
objects can be computationally expensive.
In such spaces, a common strategy to avoid expensive distance computations is to
use of an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
In other words, the alternate distance function, while quick to compute,
is always a lower-bound on the actual distance between the objects.
\end{comment}

Our design of a $\VF{}$ is inspired by nearest neighbor finding problems
in metric spaces where computing distances between
objects can be computationally expensive, thus
preferring an alternate distance function that is easy to compute
with the desirable property that it is always less than or equal to
the actual distance.
In our problem domain we are given a materialized view $v$ and a target $W_i$,
and we want to find a rewrite $r$ that
transforms $v$ such that it produces an output that is
identical to that produced by $W_i$.
%This problem is known to be NP-complete,
%which means that finding a rewrite
%workflow for $q$ using $v$ requires generating all possible
%rewrites involving $v$ and testing their {\em equivalence} with $q$.
Because this process is known to be computationally hard,
we wish to utilize an alternative distance function (e.g., \textit{dist}($v,W_i$))
% TODO: \cost is defined as yet?
that is easy to compute and has some desirable property with respect to $\cost{}$.
We define an optimistic distance function, $\ocost{}$
that takes $v$ and $W_i$ as inputs and always provides a
lower-bound on any possible rewrite of $W_i$ using $v$, without enumerating
all possible rewrites.
The property of the alternative distance function is that
$\ocost(v,W_i) \leq \cost(r)$.

The $\WF$ uses an instance of the $\VF$ at each target.
The $\WF$ treats $\VF$ as a black-box and exploits its $\ocost$ functionality
to incrementally search the space of rewrites for $W$.
After every step of the incremental search at some target $W_i$ the following two properties are true.

\begin{enumerate}
\item The $\VF$ at target $W_i$ performs an incremental expansion to some
 cost value $d$ as requested by the $\WF{}$, and there are no remaining
 rewrites to be found for \textbf{sub-workflow} $W_i$ that has a cost less than $d$.
\item After the $\WF$ performs an incremental expansion of the $\VF$ at $W_i$ to cost $d$,
there are no remaining rewrites to be found for \textbf{workflow} $W$ 
with cost less than $d'$, where $d' \leq d$.

\end{enumerate}

The key feature of our method is the $\ocost$ functionality that allows the $\WF{}$
to incrementally search the space of rewrites of $W$, such that $\WF$
finds the optimal rewrite of $W$ in a work efficient manner.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
While the details of the $\VF{}$ algorithm and the cost
functions will will be provided in a later section,
for the sake of developing the $\WF{}$ algorithm,
it is sufficient to model $\VF{}$ as a black-box
$\VF(W_i, d, d',\cost(), \ocost())$, $d < d'$, that takes
as input a workflow $W_i$, two thresholds $d, d'$,
a cost function $\cost()$, an optimistic cost function $\ocost{}$
and outputs a single rewrite $r$ of $W_i$ with the following properties:

\begin{enumerate}

\item $r$ is a rewrite workflow for $W_i$ using $V$ and the transformation rules

\item The invocation of the $\VF(W_i,d,d')$ such that $d < d'$
examines all rewrites of $W_i$ whose optimistic cost is less than or equal to $d'$.
Moreover, any subsequent invocation of
$\VF(t_i, d', d", \cost(), \ocost())$, such that $d' < d"$,
will not produce a rewrite whose optimistic cost is less than or equal to $d'$.

\item $d < \ocost(r) \leq d'$ such that $r$ has the lowest
cost among all the plans found by $\VF{}$ in this invocation.

% \item The time taken (or cost) to answer $\VF(t_i,d,d")$ is
% just a little more than the time taken to answer
% $\VF(t_1, d, d')$ and $\VF(t_1, d', d")$.
\end{enumerate}
\end{comment}



\begin{comment}
\begin{algorithm}[htp]\label{algn-main-setup}
\begin{algorithmic}[1]
\State {\sf sub} $\WF$($W$)\\
\Comment{Produces an optimal rewrite of $W$ using $\VF$}
\State $p^* \qlet W_n$\Comment{Original workflow}
\If{{\bf {\em simple/traditional} variant}}
   \State $p$ \qlet $\VF(t_n)$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
\ElsIf{{\bf {\em bottom-up greedy} variant}}
   \ForAll{$t_i$ in $\{t_n \cdots t_1\}$}
    \State $p \qlet \VF(t_i) \cup \{\node{i+1} \cdots \node{n}\}$
    \If{$p$ exists and $\cost(p) < \cost(p^*)$}
      \State $p^* \qlet p$
    \EndIf
   \EndFor
\EndIf
\State Rewrite $W$ using $p^*$
\end{algorithmic}
\end{algorithm}

Given the $\VF{}$ only finds a rewrite of a single target,
a workflow rewrite algorithm is required in order to
to find an optimal rewrite plan for the entire workflow
in the most efficient manner with the aid of the $\VF{}$.
To show that finding an optimal rewrite plan for the workflow is
not straightforward, consider two simple approaches,
namely {\em simple} and {\em greedy}, as shown in
the procedure $\WF$.
The simple variant queries the $\VF{}$ for a rewrite plan for
$t_n$, using it as the workflow rewrite plan of $W$.
The intuition here that
the {\em optimal} rewrite plan of $t_n$ produced by the
$\VF{}$ is also the optimal rewrite plan for $W$.
So, the most likely outcome of applying the simple variant is
that we may not find any rewrite plans for $t_n$.
\end{comment}


==> old/Relatedwork-v1.tex <==
\section{Related Work}

\textbf{\textit{Query Rewriting Using Views.}}
As noted in Section~\ref{sec-viewfinder} there has been much previous 
work on rewriting queries using views.
MiniCon~\cite{Pott2001} and~\cite{Konst2011} both consider 
rewriting a single query using existing materialized views, 
while~\cite{Konst2012} extends~\cite{Konst2011} to consider multiple queries.
MiniCon extends the bucket-algorithm to be more general, and
~\cite{Konst2011} uses a graph approach and applies a form of
sub-graph matching among queries and views.
In these cases both the queries and views are restricted to the class
of conjunctive queries (SPJ).
Furthermore these methods consider maximally contained rewrites
as their context is data integration.
Our context is cost-based query optimization thus we are interested in 
equivalent rewrites, not maximally contained rewrites.
We consider the rewrite problem when the queries and views can contain UDFs.  
Our unique problem setup creates $n$ rewrite problems, which we solve 
concurrently and incrementally in a work-efficient manner.

%%\cite{Pott2001} discusses extensions to cost-based rewriting
%%and notes that optimal rewrite for their case is also
%%exponential in the number of views present in the system.
%%The ability to incrementally search the space of views by their costs \VF{}
%%coupled with the workflow rewriting algorithm \WF{} that solves $n$ search
%%problems concurrently and incrementally is the key contribution of our work.

\textbf{\textit{Online Index Selection.}}
Methods such as \cite{Schn2007} adapt the physical configuration to benefit a dynamically 
changing workload by actively creating or dropping indexes/views.
Our work is opportunistic, and simply relies on the by-products of query execution.
%During query rewriting, our \WF{} algorithm produces exactly 
%those views required for the optimal rewrite of a workflow
%by exploring the space of existing views as well as new candidate views.
However, view selection methods could be applicable during storage reclamation to retain only those views that provide maximum benefit within a given space budget constraint.

\begin{comment}
\textbf{\textit{View Selection.}}
The view selection problem addresses how to choose views that provide a good
benefit for a representative workload.
Benefit is computed by the reduction in workload cost minus the cost to maintain the views.
In this work we are concerned with the view rewriting problem which determines how
to use any of the existing views to benefit a query.
View maintenance and updates impact the view selection problem rather than
the view rewriting problem we address in this work.
%Although in our system there are no updates-in-place, views
%may need to be maintained as new log data arrives.
\end{comment}

\textbf{\textit{Reusing Computations in MapReduce.}}
Other methods for optimizing MapReduce jobs have been introduced 
such as those that support incremental computations \cite{Li2011},
sharing computation or scans \cite{Nyki2010}, 
and re-using previous results \cite{Elgh2012}.  
% These approaches operate on lower-level constructs 
% (e.g.,plans) 
% than our system.  
As shown in Section~\ref{sec-experiments-restore},
caching-style sharing methods 
are effective but provide limited benefit compared to our approach.

\begin{comment}
\textbf{\textit{Evolutionary queries.}}
% These types of queries do not appear to be well-captured by current benchmarks.
Two similar ideas are the interactive OLAP queries included in the TPC-DS~\cite{tpcds}
benchmark and \emph{exploratory} queries in \cite{Khou2009}.
\cite{Khou2009} notes that many users would like to pose 
related queries on a shared data set and subsequently revise and them.
The interactive query class in TPC-DS represents a scenario with
ad-hoc analytic queries designed to mimic
a user analyzing a result before posing a new related query.
%refers to continuously changing queries over 
%log data in an environment outside of the traditional database setting
\end{comment}

\textbf{Multi-query optimization (MQO).}
The goal of MQO \cite{Sell1988} (and similar approaches \cite{Nyki2010}) is to maximize resource sharing, 
particularly common intermediate data, by producing a scheduling strategy for a set of queries in-flight.  
%Thus the output  of MQO is a scheduling strategy that minimizes the amount of duplicate work for the query set.
%Our goal is to rewrite a workflow to take advantage of the available materialized views, 
%thus the output of our work is a low-cost rewrite rather than a scheduling policy for multiple queries.
Our work produces a low-cost rewrite rather than a scheduling policy for concurrent query plans.
% Our workflow compiler (Section \ref{sec-system-architecture}) does parallelize the nodes
% In the workflow to the extent possible.
% An MQO strategy could be applied to improve the performance of
% parallel nodes if they contain redundant work.
 
\begin{comment} 
\textbf{UDFs in data flows.}
The work in \cite{Hues2012} addresses data flows that contain arbitrary UDFs, the case we
consider as well.  
A static code analysis is applied to the UDF to extract its read set and write set, along with 
its execution signature (M/R jobs) which they use to determine conflicts that affect reordering
UDFs with a fixed signature.
In our work the \textit{outputs} of a UDF have a unique signature, which is then used to perform
semantic matching for rewriting using views.  
Qo-X\cite{Simi2009} also performs optimization of data flows with UDFs for different objectives
(e.g.,cost, recoverability,etc.).  
All of these approaches address plan-level optimizations by considering reordering 
flows that contain UDFs.
Our approach is not concerned with reordering a UDF but rather finding a rewrite among the 
available views that produces the same output of the UDF at a lower cost.
Both \cite{Hues2012} and \cite{Elgh2012} consider an execution path unique if it has the same input files and M/R plan.
A unique execution path is not required for our semantic representation and signature.
\end{comment}


==> old/Udf-model-rewrite2.tex <==
\section{UDF Model}\label{sec-udf-model}
Queries in our scenario are likely to include complex analytical operations 
expressed as UDFs.
In order to reuse previous computation in our system effectively, we require a
way to model UDFs semantically.

Possibilities for modeling UDFs may include white, gray, or black-box 
approaches with varying levels of overhead and complexity to the system.
A white box approach requires a complete description of the UDF such that the 
system understands \textit{how} the UDF transforms the inputs.
This approach has high overhead for an analyst when adding a new UDF to the 
system.
A black box approach has very low overhead for an analyst but produces an 
output that is completely opaque to the system 
%(similar to a stored procedure)
thus may not be suitable for our goal of reusing results.
%
Since UDFs can involve fairly complex operations on the data, our system
adopts a gray-box approach that only captures the 
\textit{end-to-end transformations} performed by a UDF.
By \textit{end-to-end transformations}, we imply
that our model can capture
fine-grain dependencies between the input and output tuples, although 
our UDF model does not know anything more about the computation.
%
This requires additional work to provide the gray-box model when adding a new UDF, 
yet allows the system to understand the UDF's transformations in a useful way.
A black-box model, on the other hand,
can only track coarse-grain dependency between input and output as a whole.

The end-to-end transformations allowed by our gray-box model are limited to 
the following operations.

\vspace{-0.05in}
\begin{enumerate}
\setlength{\itemsep}{3pt}%
\setlength{\parskip}{0mm}%
\item Discard or add attributes using a \emph{local} function
\item Discard tuples by applying \emph{local} filter predicate
\item Perform grouping of tuples by attribute values
\end{enumerate}
\vspace{-0.01in}
\emph{Local} functions/predicates refer to those
that operate on a single tuple or a single group of tuples.
By combining these with grouping, our model  
can express rich UDFs, as well as relational operators such as select, project, join, group-by and aggregation.
Joins are modelled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.


Following our gray-box model, the input and output of
every node in the plan
is modeled by three properties:  attributes $A$, filters $F$, 
and group-by $G$.
$F$ is the conjunction of all filters applied to the input data,
$G$ is the current grouping applied, and
$A$ captures the schema.
A UDF must specify its transformation of the input to the output
in terms of these three properties.

% Notice that these three basic operations represent those 
% performed in a map or a reduce phase of a MR job, but compositions
% of these can express many complex data manipulations.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select, project, join, group-by 
% and aggregation.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select (2), project (1), join (2), group-by (3) 
%  and aggregation (3,1), where the numbers in the parenthesis 
%refers to the applicable operations above.
% This model can also represent a UDF with a single input or multiple inputs.  
% If multiple inputs are specified, the UDF input becomes a cross-product of the inputs.
% This is how a join operation can be represented by the model.
%This model describes the output of each $W_i$ in the following way.
% For instance, a \node{i} may have several UDFs applied to its input.
% The transformations of each UDF are composed in order to 
% derive the output signature of \node{i} in terms of 
% attributes, filters, and group-bys.
% This signature is equivalent to the output signature of $W_i$.


The following example illustrates how the model captures one possible 
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a classifier 
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF:
For each user, gather all of their tweets from the Twitter log;
Apply a classifier that determines if a tweet refers to food or a 
closely-related concept, and then computes a food sentiment score for 
each user;
Output only those users with score above a given threshold, $0.5$.
The representation of this UDF in the gray-box model is as follows.
Suppose the inputs are defined as attributes $A$=\{\texttt{userid},
\texttt{tweet}\}, filters $F$=$\emptyset$, group-by $G$=$\emptyset$, 
and the UDF name is \texttt{FOOD-SENTIMENT}.
Then the output includes the new attribute \texttt{score} and an additional 
filter, given by $A'$=\{\texttt{userid}, \texttt{score}\}, 
$F'$=\{\texttt{score>$0.5$}\},
and $G'=$\{\texttt{userid}\}.
\end{example}

Note from the three operations described, there is no facility to update 
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a 
new attribute.
When a new attribute is produced by a UDF, its dependencies on the 
subset of the input are recorded as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{userid}, \texttt{tweet}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.


%UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured by the model
can be admitted to the system.
We use this model to capture UDFs such as classifiers, lat/lon extractor,
sentiment analysis, log extractor and others 
as we show later in our experimental evaluation.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two UDFs with different names but identical inputs and 
functionality, the new attributes they produce will have different meta-data.
This deficiency can only be overcome by resorting to a white-box approach.



==> old/Udf-model-rewrite3.tex <==
\section{UDF Model}\label{sec-udf-model}
Queries in our scenario are likely to include complex analytical operations 
expressed as UDFs.
In order to reuse previous computation in our system effectively, we require a
way to model UDFs semantically.

Possibilities for modeling UDFs may include white, gray, or black-box 
approaches with varying levels of overhead and complexity to the system.
A white box approach requires a complete description of the UDF such that the 
system understands \textit{how} the UDF transforms the inputs.
This approach has high overhead for an analyst when adding a new UDF to the 
system.
A black box approach has very low overhead for an analyst but produces an 
output that is completely opaque to the system 
%(similar to a stored procedure)
thus may not be suitable for our goal of reusing results.
Since UDFs can involve fairly complex operations on the data, our system
adopts a gray-box approach that only captures the 
\textit{end-to-end transformations} performed by a UDF.
By \textit{end-to-end transformations}, we imply
that our model can capture
fine-grain dependencies between the input and output tuples, although 
our UDF model does not know anything more about the computation.
This requires additional work to provide the gray-box model when adding a new UDF, 
yet allows the system to understand the UDF's transformations in a useful way.
A black-box model, on the other hand,
can only track coarse-grain dependency between input and output as a whole.

% \onefig{fig-composition-udf-local-function}
% {A UDF is composed of local functions showing end-to-end transformation}{2in}

A UDF in our gray-box model is written as a {\em composition} of {\em local functions}.
A local function refers to a function 
that operates on a single tuple or a single group of tuples.
We restrict a local function to perform the following operations.

\begin{enumerate}
\item Discard or add attributes
\item Discard tuples by applying filters
\item Perform grouping of tuples
\end{enumerate}
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.

The gray-box model does not understand the nature of the transformation
performed by the local functions however it understands the 
transformation afforded by each local function.
The end-to-end transformation of the UDF can be obtained by
composing the operations performed by each local function in the UDF
% , which
% is captured in Figure~\ref{fig-composition-udf-local-function}.

Following our gray-box model, 
the input and output of
every node in the plan
is captured by three properties:  attributes $A$, filters $F$, 
and group-by $G$.
$F$ is the conjunction of all filters applied to the input data,
$G$ is the current grouping applied, and
$A$ captures the schema.
The end-to-end transformation of a UDF can be expressed as the
transformation of the input to the output using the composition
of the local functions.
Note that the composition captures the {\em semantics}
of the end-to-end transformation using the three operations, but not
the actual computation.
and not to describe the internal procedure.
By combining these with grouping, our model  
can express rich UDFs, as well as relational operators such as select, project, join, group-by and aggregation.
Joins are modelled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).

% Notice that these three basic operations represent those 
% performed in a map or a reduce phase of a MR job, but compositions
% of these can express many complex data manipulations.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select, project, join, group-by 
% and aggregation.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select (2), project (1), join (2), group-by (3) 
%  and aggregation (3,1), where the numbers in the parenthesis 
%refers to the applicable operations above.
% This model can also represent a UDF with a single input or multiple inputs.  
% If multiple inputs are specified, the UDF input becomes a cross-product of the inputs.
% This is how a join operation can be represented by the model.
%This model describes the output of each $W_i$ in the following way.
% For instance, a \node{i} may have several UDFs applied to its input.
% The transformations of each UDF are composed in order to 
% derive the output signature of \node{i} in terms of 
% attributes, filters, and group-bys.
% This signature is equivalent to the output signature of $W_i$.

\subsection{UDF Example}


The following example illustrates how the model captures one possible 
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a classifier 
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF is expressed as a composition of 
the following local functions:
For each user, gather all of their tweets from the Twitter log;
Apply a classifier that determines if a tweet refers to food or a 
closely-related concept, and then computes a food sentiment score for 
each user;
Output only those users with score above a given threshold, $0.5$.
The representation of this UDF in the gray-box model is as follows.
Suppose the inputs are defined as attributes $A$=\{\texttt{userid},
\texttt{tweet}\}, filters $F$=$\emptyset$, group-by $G$=$\emptyset$, 
and the UDF name is \texttt{FOOD-SENTIMENT}.
Then the output includes the new attribute \texttt{score} and an additional 
filter, given by $A'$=\{\texttt{userid}, \texttt{score}\}, 
$F'$=\{\texttt{score>$0.5$}\},
and $G'=$\{\texttt{userid}\}.
\end{example}

Note from the three operations described, there is no facility to update 
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a 
new attribute.
When a new attribute is produced by a UDF, its dependencies on the 
subset of the input are recorded as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{userid}, \texttt{tweet}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.

%UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured by the model
can be admitted to the system.
We use this model to capture UDFs such as classifiers, lat/lon extractor,
sentiment analysis, log extractor and others 
as we show later in our experimental evaluation.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two UDFs with different names but identical inputs and 
functionality, the new attributes they produce will have different meta-data.
This deficiency can only be overcome by resorting to a white-box approach.

\subsection{Cost of UDF}

We now briefly describe how the optimizer costs a UDF given its gray-box
description and its composition in terms of local functions.
We assume that a mapping between each local function to the number of MR jobs,
map and reduces phases are known to the optimizer. 
The optimizer costs a UDF by summing up the cost of 
performing the local functions to reasonably estimate cost.

Suppose that a local function performs a set $S$ of operations 
given by the three UDF model.
Without a mapping of the operations to the number of jobs, maps and reduce,
we use the following weak property of a cost optimizer.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be any set of operations represented by the UDF model.
Let $\cost(S,D)$ be defined as the total cost of performing all operations 
in $S$ on a database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
%Taking the minimum cost of an operation in $S$ provides a lower bound on the
%cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
%Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
%of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must rely on the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter 
with high selectivity and a group-by operation with higher cost than 
applying the filter,
when considering the operations independently on database $D$.
Let $S'$ contain only group-by.
Suppose that applying the filter before group-by results in few or no tuples streamed to 
group-by.
Then applying group-by can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.


==> old/Udf-model-rewrite4.orig.tex <==
\section{UDF Model}\label{sec-udf-model}
Since queries will frequently include UDFs, we require a
way to model UDFs semantically in order to reuse previous 
computation in our system effectively.
This can be challenging as UDFs can be written in many languages, performing
arbitrary functions.
To address this problem we provide a model for UDFs that allows the system
to capture a UDF as  a {\em composition} of {\em local functions}, which will 
be described next.
In this way, our model only captures the 
\textit{end-to-end transformations} performed by a UDF, which are represented 
as fine-grain dependencies between the input and output tuples.
Note that this does not require the model to know anything more about 
the computation performed by the UDF,
yet allows the system to understand the UDF's transformations in a useful way.
This represents a gray-box approach to modeling UDFs, in contrast with a 
white-box approach that understands the nature of the transformations, or a 
black-box model that only tracks coarse-grain dependency between input and 
output as a whole.

% \onefig{fig-composition-udf-local-function}
% {A UDF is composed of local functions showing end-to-end transformation}{2in}


A local function refers to a function that operates on a single tuple or 
a single group of tuples.
We restrict a local function to perform the following operations.

\begin{enumerate}
\item Discard or add attributes
\item Discard tuples by applying filters
\item Perform grouping of tuples
\end{enumerate}
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.

These operations correspond exactly to the type of operations that can be 
performed by \textit{map} and \textit{reduce} tasks.
By capturing these operations, the model can understand the 
transformation performed by each local function.
Then, the end-to-end transformation of the UDF can be obtained by
composing the operations performed by each local function in the UDF.
% , which
% is captured in Figure~\ref{fig-composition-udf-local-function}.

The input and output of a UDF is captured by three properties corresponding
to the three operations in the model:  
attributes $A$, filters $F$, and group-by $G$.
$A$ captures the input and output schema,
$F$ is the conjunction of all filters applied to the input data,
and $G$ is the current grouping applied.
Note that aggregations are composed of a grouping and a new attribute, which
is a modification of the schema.
The composition of local functions into an end-to-end transformation captures 
the {\em semantics} of the end-to-end transformation using the three operations, 
but does not describe the internal procedure by any local function.
By combining these with grouping, our model  
can express rich UDFs, as well as relational operators such as select, project, join, group-by and aggregation.
Joins are modelled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).

% Notice that these three basic operations represent those 
% performed in a map or a reduce phase of a MR job, but compositions
% of these can express many complex data manipulations.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select, project, join, group-by 
% and aggregation.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select (2), project (1), join (2), group-by (3) 
%  and aggregation (3,1), where the numbers in the parenthesis 
%refers to the applicable operations above.
% This model can also represent a UDF with a single input or multiple inputs.  
% If multiple inputs are specified, the UDF input becomes a cross-product of the inputs.
% This is how a join operation can be represented by the model.
%This model describes the output of each $W_i$ in the following way.
% For instance, a \node{i} may have several UDFs applied to its input.
% The transformations of each UDF are composed in order to 
% derive the output signature of \node{i} in terms of 
% attributes, filters, and group-bys.
% This signature is equivalent to the output signature of $W_i$.

\subsection{UDF Example}


The following example illustrates how the model captures one possible 
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a classifier 
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF is expressed as a composition of 
the following local functions:
For each user, gather all of their tweets from the Twitter log;
Apply a classifier that determines if a tweet refers to food or a 
closely-related concept, and then computes a food sentiment score for 
each user;
Output only those users with score above a given threshold, $0.5$.
The representation of this UDF in the gray-box model is as follows.
Suppose the inputs are defined as attributes $A$=\{\texttt{userid},
\texttt{tweet}\}, filters $F$=$\emptyset$, group-by $G$=$\emptyset$, 
and the UDF name is \texttt{FOOD-SENTIMENT}.
Then the output includes the new attribute \texttt{score} and an additional 
filter, given by $A'$=\{\texttt{userid}, \texttt{score}\}, 
$F'$=\{\texttt{score>$0.5$}\},
and $G'=$\{\texttt{userid}\}.
\end{example}

Note from the three operations described, there is no facility to update 
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a 
new attribute.
When a new attribute is produced by a UDF, its dependencies on the 
subset of the input are recorded as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{userid}, \texttt{tweet}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.

%UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured by the model
can be admitted to the system.
We use this model to capture UDFs such as classifiers, lat/lon extractor,
sentiment analysis, log extractor and others 
as we show later in our experimental evaluation.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two UDFs with different names but identical inputs and 
functionality, the new attributes they produce will have different meta-data.
This deficiency can only be overcome by resorting to a white-box approach.

\subsection{Cost of UDF}

We now briefly describe how the optimizer costs a UDF given its gray-box
description and its composition in terms of local functions.
We assume that a mapping between each local function to the number of MR jobs,
map and reduces phases are known to the optimizer. 
The optimizer costs a UDF by summing up the cost of 
performing the local functions to reasonably estimate cost.

Suppose that a local function performs a set $S$ of operations 
given by the three UDF model.
Without a mapping of the operations to the number of jobs, maps and reduce,
we use the following weak property of a cost optimizer.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be any set of operations represented by the UDF model.
Let $\cost(S,D)$ be defined as the total cost of performing all operations 
in $S$ on a database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
%Taking the minimum cost of an operation in $S$ provides a lower bound on the
%cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
%Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
%of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must rely on the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter 
with high selectivity and a group-by operation with higher cost than 
applying the filter,
when considering the operations independently on database $D$.
Let $S'$ contain only group-by.
Suppose that applying the filter before group-by results in few or no tuples streamed to 
group-by.
Then applying group-by can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.


==> old/Udf-model-rewrite4.tex <==
% all relational operators are modeled in 
given that hive implements all these relational ops, they can also be exressed with our UDF model.

everything is expressed by the same model.
a udf in perl is handled no differently than a relational op in hive.
everyhting is a udf/terms.

now that everything is a udf, we can take a set of inputs, the 
given a view and a query, checking for equivalence can be done by 
comparing the a, f, g, sets.
furthermore, if a view and a query are not equivalent, if the view
contains the query, then we can at least try to apply a compensation.


no you can define equivalent if they have the same attr, f, g, as captured by the model.  

\section{UDF Model}\label{sec-udf-model}

\textbf{Queries have a lot of UDFs}
In our scenario, queries are likely to include UDFs  express complex 
analytical operations. 
In order to reuse previous computation in our system effectively, we require a
way to model UDFs semantically.

\textbf{How are UDFs implemented}
Typically in the Hive environment, the UDFs are written in either perl, python or
Java and invoked by the query using the Hive CLI feature.
The UDF usually contains several cascaded functions that implements
a sequence of map and reduce functions.
We refer to these functions as {\em local} to indicate that they operate
on a small portion of the dataset.
A local function here refers to a map or a reduce function 
that operates on a single tuple or a single group of tuples.
The nature of the M/R framework, reduces the local functions to
perform a combination of these operations.

\textbf{Given the nature of MR framework, this all you could in a local function}
\onefig{fig-composition-udf-local-function}
{A UDF is composed of local functions showing end-to-end transformation}{2in}

\begin{enumerate}
\item Discard or add attributes
\item Discard tuples by applying filters
\item Perform grouping of tuples
\end{enumerate}
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.

\textbf{example.}
The following example illustrates how the model captures one possible 
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a classifier 
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF is expressed as a composition of 
the following local functions:

Map: For each ({\it tweet\_id}, {\it user\_id}, {\it tweet\_text}), 
apply food sentiment classifier function that produces user\_id as key, and 
({\it tweet\_id}, {\it sentiment\_score}) as value. 
The sentiment classifer applies a NLP and
a sentiment classifier on the tweet\_text to represent  
the postive or negative sentiment towards food as the {\it sentiment\_score}.

Reduce: For each user\_id, sum up the sentiment score. Emit only those
users who have a sentiment score of greater than 0.5.

% For each user, gather all of their tweets from the Twitter log;
% Apply a classifier that determines if a tweet refers to food or a 
% closely-related concept, and then computes a food sentiment score for 
% each user;
% Output only those users with score above a given threshold, $0.5$.
\end{example}

\textbf{end to end is easy to model}
A UDF in our gray-box model is written as a {\em composition} of {\em local functions}.
Each local functions can be quite complex in the way it transforms data (e.g.,
apply a sentiment analysis function).
However, our model does not 
capture the nature of the computation 
performed by the local functions.
However the operations performed by them is recorded by each local function. 
For instance, the application of a sentiment analysis function is captured
by the creation of a new attribute from a specified set of inputs.
The end-to-end transformation of the UDF can be obtained by
composing the operations performed by each local function in the UDF, which
is captured in Figure~\ref{fig-composition-udf-local-function}.

By \textit{end-to-end transformations}, we imply
that our model can capture
fine-grain dependencies between the input and output tuples, although 
our UDF model does not know anything more about the computation.

Following our gray-box model, 
the input and output of
every node in the plan
is captured by three properties:  attributes $A$, filters $F$, 
and group-by $G$.
$F$ is the conjunction of all filters applied to the input data,
$G$ is the current grouping applied, and
$A$ captures the schema.
The end-to-end transformation of a UDF can be expressed as the
transformation of the input to the output using the composition
of the local functions.
Note that the composition captures the {\em semantics}
of the end-to-end transformation using the three operations, but not
the actual computation.
and not to describe the internal procedure.
By combining these with grouping, our model  
can express rich UDFs, as well as relational operators such as 
select, project, join, group-by and aggregation.
Joins are modelled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).

% Notice that these three basic operations represent those 
% performed in a map or a reduce phase of a MR job, but compositions
% of these can express many complex data manipulations.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select, project, join, group-by 
% and aggregation.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select (2), project (1), join (2), group-by (3) 
%  and aggregation (3,1), where the numbers in the parenthesis 
%refers to the applicable operations above.
% This model can also represent a UDF with a single input or multiple inputs.  
% If multiple inputs are specified, the UDF input becomes a cross-product of the inputs.
% This is how a join operation can be represented by the model.
%This model describes the output of each $W_i$ in the following way.
% For instance, a \node{i} may have several UDFs applied to its input.
% The transformations of each UDF are composed in order to 
% derive the output signature of \node{i} in terms of 
% attributes, filters, and group-bys.
% This signature is equivalent to the output signature of $W_i$.

\begin{example}
The representation of this UDF in the gray-box model is either provided
by the UDF creator or can be automatically deduced is as follows:

If the input attributes are 
\{\texttt{user\_id}, \texttt{tweet\_id}, and \texttt{tweet\_text}\}, 
applied filters $F$=$\emptyset$, and applied group-by $G$=$\emptyset$. 

The output includes the new attribute \texttt{sentiment\_score} and an additional 
filter.
The attributes in the output are \{\texttt{userid}, \texttt{sentiment\_score}\}, 
filter \{\texttt{sentiment\_score>$0.5$}\},
and group-by \{\texttt{userid}\}.

As the UDF can be used with any arbitrary input with additional attributes, 
arbitrary filters and group-by, the UDF representation is written in a way
that it can produce the output representation from the provided input represenation.
\end{example}


\textbf{why is this desirable}
everything is a udf.

\textbf{equiavlance check is easy}
containtment is hard.
we provide a method to guess containment, formalized sectionXX.
its a heuristic but
this modeling allows us to perform a quick test for possible equivalence.
equivalence testing is a known hard problem, since it is the same as the
containment problem, which is NP-hard \cite{xx}.
However, while checking actual containment is hard, 
we can be certain that something is not contained quite easily.
i.e., an atom is missing or something?? \cite{xx}.
then we can make a conservative guess that containment might be possible,
and then apply more effort to check containment only for these promising 
cases, avoiding effort for hopeless cases. 
           

Note from the three operations described, there is no facility to update 
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a 
new attribute.
When a new attribute is produced by a UDF, its dependencies on the 
subset of the input are recorded as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{userid}, \texttt{tweet}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.

%UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured by the model
can be admitted to the system.
We use this model to capture UDFs such as classifiers, lat/lon extractor,
sentiment analysis, log extractor and others 
as we show later in our experimental evaluation.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two UDFs with different names but identical inputs and 
functionality, the new attributes they produce will have different meta-data.
This deficiency can only be overcome by resorting to a white-box approach.

\subsection{Cost of UDF}

We now briefly describe how the optimizer costs a UDF given its gray-box
description and its composition in terms of local functions.
We assume that a mapping between each local function to the number of MR jobs,
map and reduces phases are known to the optimizer. 
The optimizer costs a UDF by summing up the cost of 
performing the local functions to reasonably estimate cost.

Suppose that a local function performs a set $S$ of operations 
given by the three UDF model.
Without a mapping of the operations to the number of jobs, maps and reduce,
we use the following weak property of a cost optimizer.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be any set of operations represented by the UDF model.
Let $\cost(S,D)$ be defined as the total cost of performing all operations 
in $S$ on a database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
%Taking the minimum cost of an operation in $S$ provides a lower bound on the
%cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
%Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
%of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must rely on the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter 
with high selectivity and a group-by operation with higher cost than 
applying the filter,
when considering the operations independently on database $D$.
Let $S'$ contain only group-by.
Suppose that applying the filter before group-by results in few or no tuples streamed to 
group-by.
Then applying group-by can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.



% Possibilities for modeling UDFs may include white, gray, or black-box 
% approaches with varying levels of overhead and complexity to the system.
% A white box approach requires a complete description of the UDF such that the 
% system understands \textit{how} the UDF transforms the inputs.
% This approach has high overhead for an analyst when adding a new UDF to the 
% system.
% A black box approach has very low overhead for an analyst but produces an 
% output that is completely opaque to the system 
% %(similar to a stored procedure)
% thus may not be suitable for our goal of reusing results.
% Since UDFs can involve fairly complex operations on the data, our system
% adopts a gray-box approach that only captures the 
% \textit{end-to-end transformations} performed by a UDF.
% By \textit{end-to-end transformations}, we imply
% that our model can capture
% fine-grain dependencies between the input and output tuples, although 
% our UDF model does not know anything more about the computation.
% This requires additional work to provide the gray-box model when adding a new UDF, 
% yet allows the system to understand the UDF's transformations in a useful way.
% A black-box model, on the other hand,
% can only track coarse-grain dependency between input and output as a whole.


==> old/Udf-model-rewrite5.tex <==
\section{UDF Model}\label{sec-udf-model}
Since queries will frequently include UDFs, we require a
way to model UDFs semantically in order to reuse previous 
computation in our system effectively.
This is challenging as UDFs can be written in many languages, performing
arbitrary functions.
In Hive, this can include Java, Perl, Python, and these are invoked via the
Hive command line interface.
Hive ``performs'' these UDFs as external functions and thus has little 
knowledge or control over the operations perforned.

\subsection{Modeling a UDF}

To address this problem we provide a model for UDFs that allows the system
to capture a UDF as  a {\em composition} of {\em local functions}.
Each UDF is composed of a sequence of local map and reduce functions, as 
shown in Figure~\ref{fig-composition-udf-local-function}.
We refer to these functions as {\em local} to indicate that they each operate
on a small portion of the dataset: a single tuple or a single group of tuples.
In this way, our model only captures the 
\textit{end-to-end transformations} performed by a UDF, which are represented 
as fine-grain dependencies between the input and output tuples.
Note that this does not require the model to know anything more about 
the computation performed by the UDF,
yet allows the system to understand the UDF's transformations in a useful way.
This represents a gray-box approach to modeling UDFs, in contrast with a 
white-box approach that requires a complete understanding of the transformations, 
or a black-box model that only tracks coarse-grain dependency between input and
output as a whole.

\onefig{fig-composition-udf-local-function}
{A UDF is composed of a sequence of local functions ($lf_1, lf_2,\dots, lf_k$) showing the end-to-end transformation of the input to the output.}{2in}


Due to the nature of the M/R framework, local functions can only 
perform a combination of the following three operations.
%We restrict a local function to perform the following operations.

\begin{enumerate}
\item Discard or add attributes
\item Discard tuples by applying filters
\item Perform grouping of tuples
\end{enumerate}
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.

These operations correspond exactly to the type of operations that can be 
performed by \textit{map} and \textit{reduce} tasks.
By capturing these operations, the model can understand the 
transformation performed by each local function.
Then, the end-to-end transformation of the UDF can be obtained by
composing the operations performed by each local function in the UDF.
Note from the three operations described, there is no facility to update
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a
new attribute.
When a new attribute is produced, its dependencies on the
subset of the input are recorded.  

The input and output of a UDF is captured by three properties corresponding
to the three operations in the model:  
attributes $A$, filters $F$, and group-by $G$ as shown in Figure~\ref{fig-composition-udf-local-function}.
Property $A$ captures the input and output schema,
property $F$ is the conjunction of all filters applied to the input data,
and property $G$ is the current grouping applied.
Note that aggregations are composed of a grouping ($G$) and producing new attribute, 
which is a modification of the schema ($A$).
Whenever a UDF is applied, the properties $A$, $F$, and $G$ are recorded for the 
inputs and outputs, as well as the \textit{unique} UDF name.
The composition of local functions into an end-to-end transformation captures 
the {\em semantics} of the end-to-end transformation using the three operations, 
but does not describe the internal procedure by any local function.
%%By combining these with grouping, 

Any UDF or relational operation with end-to-end transformations correctly 
captured by the model can be \textit{admitted} to the system.
As we show later in our experimental evaluation, we use the model to capture 
relational operations in Hive as well as common 
UDFs such as classifiers, lat/lon extractor, sentiment analysis, log extractor and others.
Note the model only needs specified the first time a particular UDF is added,
and the \textit{unique} UDF name is recorded.

The properties modelled are straightforward and map directly to the local functions
performed.
Thus the properties can be provided as annotations by the 
UDF creator with minimal overhead, or may be automatically deduced via some
code analysis method such as that in~\cite{Hues2012}.
In this work, we have the user provide the annotations when a UDF is admitted
to the system.  
This is a reasonable compromise since the properties only need provided one
time for any UDF, and our model annotations are very simple.


% Notice that these three basic operations represent those 
% performed in a map or a reduce phase of a MR job, but compositions
% of these can express many complex data manipulations.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select, project, join, group-by 
% and aggregation.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select (2), project (1), join (2), group-by (3) 
%  and aggregation (3,1), where the numbers in the parenthesis 
%refers to the applicable operations above.
% This model can also represent a UDF with a single input or multiple inputs.  
% If multiple inputs are specified, the UDF input becomes a cross-product of the inputs.
% This is how a join operation can be represented by the model.
%This model describes the output of each $W_i$ in the following way.
% For instance, a \node{i} may have several UDFs applied to its input.
% The transformations of each UDF are composed in order to 
% derive the output signature of \node{i} in terms of 
% attributes, filters, and group-bys.
% This signature is equivalent to the output signature of $W_i$.

\subsection{Example of Applying the UDF Model}

The following example illustrates how the model captures one possible
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a
classifier
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF is expressed as a composition of
the following local functions:

Map: For each ({\it tweet\_id}, {\it user\_id}, {\it tweet\_text}),
apply food sentiment classifier function that produces user\_id as key, and
({\it tweet\_id}, {\it sentiment-score}) as a value.
The sentiment classifer applies a NLP and
a sentiment classifier on the tweet\_text to represent
the postive or negative sentiment towards food as the  \texttt{sentiment\_score}.

Reduce: For each user\_id, sum up the  \texttt{sentiment-score}. Emit only those
users who have a sentiment score of greater than 0.5.
\end{example}


In terms of the model, the inputs to this UDF are 
$\langle A$=\{\texttt{user\_id}, \texttt{tweet\_id}, \texttt{tweet\_text}\},
$F$=$\emptyset$,
$G$=$\emptyset$ $\rangle$,
assuming the input does not have any previous filters or groupings here.
Then the outputs are 
$\langle A$=\{\texttt{user\_id}, \texttt{sentiment\_score}\},
$F$=$\texttt{sentiment\_score}>0.5$,
$G$=\texttt{user\_id}$\rangle$.
Notice this UDF produces a new attribute,  \texttt{sentiment\_score}. 
As mentioned previously, whenever a new attribute is produced, 
its dependencies on the subset of the input are recorded by the model as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{sentiment\_score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{user\_id}, \texttt{tweet\_text}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.




\subsection{Benefits and Limitations of the Model}

This model can express rich UDFs as well as standard relational
operators such as select (2), project (1), join (2), group-by (3) 
and aggregation (3,1), where the numbers in the parenthesis 
refers to the applicable operations above.
Operations modeled may have a single input or multiple inputs. 
Joins are modeled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).
For our system, this provides the benefit that both UDFs and relational 
operations can be captured by the model.


The main benefit of the model is that it enables a simple test to check 
equivalence between any two functions that are both described in terms of this 
model.
This allows the system to leverage any previously computed results that can 
be reused toward answering a new query. 
To reuse results in our system, the previous results must either be 
semantically equivalent in terms of our model, or the previous results 
must \textit{contain} the new query.
While an equivalance check becomes quick and easy using the model by comparing
the properties $A$, $F$, and $G$, a \textit{containtment} check is a known 
hard problem even for conjunctive 
queries under bag or set semantics~\cite{Jayr2006}.
However, by guessing containment, we can use the model to determine if a 
previous result has a high potential to produce a complete rewrite for a 
new query.
Later in Section~\ref{sec-guess-rewrite} we provide a conservative heuristic 
to guess containment.
Because the containment problem is hard, the guess only serves as a quick 
conservative approximation.
%this modeling allows us to perform a quick test for possible equivalence.
%equivalence testing is a known hard problem, since it is the same as the
%containment problem, which is NP-hard \cite{xx}.
However, while checking actual containment is hard,
we can make a rough guess that something is likely \textit{not} contained 
quite easily, e.g., an attribute is missing or an unwanted filter is present.
When attempting to rewrite a new query, 
this conservative guess that containment might be possible allows us to focus 
computational efforts toward checking containment on the most promising previous 
results and avoid computational effort for likely hopeless cases.

Another benefit of the model is that it allows us to provide a rough estimate
of the cost of a potential rewrite given an existing previous result.
For results that pass the containment guess we can quickly calculate a minimum 
difference between a previous result and a new query in terms of the model, 
e.g., one attribute and filter are different.
Since each difference might be \textit{fixed} through the application of a local
function, it is possible to provide a lower bound on the cost of a potential 
rewrite (should one actually exist), without actually finding a valid rewrite, 
which is a hard problem as mentioned.
This is done by costing a summation of local function costs for the computed 
difference, and is described in more detail in Section~\ref{}.
Our approach avoids the significant computational effort of finding an actual 
rewrite and then obtaining its true cost.
Using the model to make a quick conservative guess and quick lower bound cost
of a potential rewrite, our rewriter can focus on those previous results with
the best potential and the lowest cost first during its search for rewrites.
This approach is what enables the best-first nature of our rewrite search 
which is described in Section~\ref{sec-best-first-workflow-rewrite}. 
As we demonstrate later in Section~\ref{sec-scalability}, this results in significant
computational savings by allowing the rewriter to search the exponential space 
in an ordered way, potentially stopping early in some cases.


The gray-box model has certain limitations.
For instance, given two UDFs with different names but identical inputs and
functionality, the new attributes they produce will have different
meta-data.
This deficiency can only be overcome by resorting to a white-box approach,
requiring more system overhead 
(potentially in the form of transformational rules for all possible operations) 
and may not offer much additional benefit in our scenario.











==> old/Udf-model-rewrite6.tex <==
\section{UDF Model}\label{sec-udf-model}
Since queries will frequently include UDFs, we require a
way to model UDFs semantically in order to reuse previous 
computation in our system effectively.
This is challenging as UDFs can be written in many languages, performing
arbitrary functions.
In Hive, this can include Java, Perl, Python, and these are invoked via the
Hive command line interface.
Hive ``performs'' these UDFs as external functions and thus has little 
knowledge or control over the operations performed.

\subsection{Modelling a UDF}

To address this problem we provide a model for UDFs that allows the system
to capture a UDF as  a {\em composition} of {\em local functions}.
Each UDF is composed of a sequence of local map and reduce functions, as 
shown in Figure~\ref{fig-composition-udf-local-function}.
We refer to these functions as {\em local} to indicate that they each operate
on a small portion of the dataset: a single tuple or a single group of tuples.
In this way, our model only captures the 
\textit{end-to-end transformations} performed by a UDF, which are represented 
as fine-grain dependencies between the input and output tuples.
Note that this does not require the model to know anything more about 
the computation performed by the UDF,
yet allows the system to understand the UDF's transformations in a useful way.
This represents a gray-box approach to modelling UDFs, in contrast with a 
white-box approach that requires a complete understanding of the transformations, 
or a black-box model that only tracks coarse-grain dependency between input and
output as a whole.

\onefig{fig-composition-udf-local-function}
{A UDF is composed of a sequence of local functions ($lf_1, lf_2,\dots, lf_k$) showing the end-to-end transformation of the input to the output.}{2in}


Due to the nature of the M/R framework, local functions can only 
perform a combination of the following three operations.
%We restrict a local function to perform the following operations.

\begin{enumerate}
\item Discard or add attributes
\item Discard tuples by applying filters
\item Perform grouping of tuples
\end{enumerate}
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.

These operations correspond exactly to the type of operations that can be 
performed by \textit{map} and \textit{reduce} tasks.
By capturing these operations, the model can understand the 
transformation performed by each local function.
Then, the end-to-end transformation of the UDF can be obtained by
composing the operations performed by each local function in the UDF.
Note from the three operations described, there is no facility to update
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a
new attribute.
When a new attribute is produced, its dependencies on the
subset of the input are recorded.  

The input and output of a UDF is captured by three properties corresponding
to the three operations in the model:  
attributes $A$, filters $F$, and group-by $G$ as shown in Figure~\ref{fig-composition-udf-local-function}.
Property $A$ captures the input and output schema,
property $F$ is the conjunction of all filters applied to the input data,
and property $G$ is the current grouping applied.
Note that aggregations are composed of a grouping ($G$) and producing new attribute, 
which is a modification of the schema ($A$). 
Any UDF modelled may have a single input or multiple inputs.
For each UDF, the properties $A$, $F$, and $G$ are recorded for the 
inputs and outputs, as well as the \textit{unique} UDF name.
The composition of local functions into an end-to-end transformation captures 
the {\em semantics} of the end-to-end transformation using the three operations, 
but does not describe the internal procedure by any local function.
%%By combining these with grouping, 

Any UDF or relational operation with end-to-end transformations correctly 
captured by the model can be \textit{admitted} to the system.
As we show later in our experimental evaluation, we use the model to capture 
relational operations in Hive as well as common 
UDFs such as classifiers, lat/lon extractor, sentiment analysis, log extractor and others.
Note the model only needs specified the first time a particular UDF is added,
and the \textit{unique} UDF name is recorded.

The properties modelled are straightforward and map directly to the local functions
performed.
Thus the properties can be provided as annotations by the 
UDF creator with minimal overhead, or may be automatically deduced via some
code analysis method such as that in~\cite{Hues2012}.
In this work, we have the user provide the annotations when a UDF is admitted
to the system.  
This is a reasonable compromise since the properties only need provided one
time for any UDF, and our model annotations are very simple.


% Notice that these three basic operations represent those 
% performed in a map or a reduce phase of a MR job, but compositions
% of these can express many complex data manipulations.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select, project, join, group-by 
% and aggregation.
% Morover, the UDF model can also be used to expresss standard relational
% operators such as select (2), project (1), join (2), group-by (3) 
%  and aggregation (3,1), where the numbers in the parenthesis 
%refers to the applicable operations above.
% This model can also represent a UDF with a single input or multiple inputs.  
% If multiple inputs are specified, the UDF input becomes a cross-product of the inputs.
% This is how a join operation can be represented by the model.
%This model describes the output of each $W_i$ in the following way.
% For instance, a \node{i} may have several UDFs applied to its input.
% The transformations of each UDF are composed in order to 
% derive the output signature of \node{i} in terms of 
% attributes, filters, and group-bys.
% This signature is equivalent to the output signature of $W_i$.

\subsection{Example of Applying the UDF Model}

The following example illustrates how the model captures one possible
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a
classifier
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF is expressed as a composition of
the following local functions:

Map: For each ({\it tweet\_id}, {\it user\_id}, {\it tweet\_text}),
apply food sentiment classifier function that produces user\_id as key, and
({\it tweet\_id}, {\it sentiment-score}) as a value.
The sentiment classifer applies a NLP and
a sentiment classifier on the tweet\_text to represent
the postive or negative sentiment towards food as the  \texttt{sentiment\_score}.

Reduce: For each user\_id, sum up the  \texttt{sentiment-score}. Emit only those
users who have a sentiment score of greater than 0.5.
\end{example}


In terms of the model, the inputs to this UDF are 
$\langle A$=\{\texttt{user\_id}, \texttt{tweet\_id}, \texttt{tweet\_text}\},
$F$=$\emptyset$,
$G$=$\emptyset$ $\rangle$,
assuming the input does not have any previous filters or groupings here.
Then the outputs are 
$\langle A$=\{\texttt{user\_id}, \texttt{sentiment\_score}\},
$F$=$\texttt{sentiment\_score}>0.5$,
$G$=\texttt{user\_id}$\rangle$.
Notice this UDF produces a new attribute,  \texttt{sentiment\_score}. 
As mentioned previously, whenever a new attribute is produced, 
its dependencies on the subset of the input are recorded by the model as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{sentiment\_score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{user\_id}, \texttt{tweet\_text}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.




\subsection{Benefits of the Model}

The first benefit of the model is that it provides a unified way of 
capturing both UDFs and relational operations.
For example, it can model standard relational
operators such as select (2), project (1), join (2), group-by (3) 
and aggregation (3,1), where the numbers in the parenthesis 
refers to the applicable operations above.
Joins are modelled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).

A second benefit of the model is that it enables a simple test to check 
equivalence of queries.
This check allows the system to leverage any previously computed results that can 
be reused toward answering a new query. 
An equivalence check becomes quick and easy using the model by comparing
the properties $A$, $F$, and $G$. 
Furthermore, previous results can also be reused if they \textit{contain} 
the new query.
We describe our method to check for equivalence as well as containment 
 in the next section.

The third benefit of the model is to provide a way of costing a UDF.  
By decomposing UDFs into local functions, this makes costing a UDF possible.
Through these local functions, we can also determine a lower bound 
on the cost of a potential 
rewrite (should one actually exist), without actually finding a valid rewrite, 
which is a hard problem as mentioned. 






==> old/Udf-model-rewrite7.tex <==
\section{UDF Model}\label{sec-udf-model}
Since queries will frequently include UDFs, we require a
way to model UDFs semantically in order to reuse previous 
computation in our system effectively.
This is challenging as UDFs can be written in many languages, performing
arbitrary functions.
In Hive, this can include Java, Perl, Python, and these are invoked via the
Hive command line interface.



We propose a UDF  model that provides a unified way of capturing both UDFs and 
common relational operations.
The model captures a class of UDFs that includes many common operators such as classifiers, social network, spatial, NLP and text processors.
If the analyst is able to describe their UDF in terms of the model, it will enable
the system to reuse artifacts more effectively.
However, if the UDF does not use this model, then it is treated as a black-box
and there are limited opportunities to reuse previous results  --- i.e.,
only when there is an exact match of inputs and outputs.



\subsection{Modelling a UDF}

To address this problem we provide a model for UDFs that allows the system
to capture a UDF as  a {\em composition} of {\em local functions}.
Each UDF is composed of a sequence of local map and reduce functions, as 
shown in Figure~\ref{fig-composition-udf-local-function}.
We refer to these functions as {\em local} to indicate that they each operate
on a small portion of the dataset: a single tuple or a single group of tuples.
Due to the nature of the M/R framework, local functions can only 
perform a combination of the following three operations.
%We restrict a local function to perform the following operations.
\begin{enumerate}
\item Discard or add attributes ($A$)
\item Discard tuples by applying filters ($F$)
\item Perform grouping of tuples ($G$)
\end{enumerate}
% Notice also that the semantics of these local functions and filters
% are opaque unlike a white-box model.

\onefig{fig-composition-udf-local-function}
{A UDF is composed of local functions ($lf_1, lf_2,\dots, lf_k$) shows 
  the end-to-end transformation of input to output.}{2in}


These operations correspond exactly to the type of operations that can be 
performed by \textit{map} and \textit{reduce} tasks.
The end-to-end transformation of the UDF can be obtained by
composing the operations performed by each local function $lf$ in the UDF.
In this way, our model only captures the 
\textit{end-to-end transformations} performed by a UDF, which are represented 
as fine-grain dependencies between the input and output tuples.
Note that this does not require the model to know anything more about 
the computation performed by the local functions,
yet allows the system to understand the UDF's transformations in a useful way.
This represents a gray-box approach to modelling UDFs, giving the system
a limited view of the UDF's functionality.
In contrast, a white-box approach would require a complete understanding of the way 
the transformations are performed, and a black-box model would only captures the 
coarse-grain dependency between input and output as a whole.



The input and output of a UDF is captured by three properties corresponding
to the three operations in the model:  
attributes $A$, filters $F$, and group-by $G$ as shown in Figure~\ref{fig-composition-udf-local-function}.
Property $A$ captures the input and output schema,
property $F$ is the conjunction of all filters applied to the input data,
and property $G$ is the current grouping applied.
Note that aggregations are composed of a grouping ($G$) that produces a new attribute, 
which is reflected as a modification of the schema ($A$). 
Any UDF modelled may have a single input or multiple inputs.
The inputs and outputs of each UDF are recorded in terms of $A$, $F$, and $G$ 
and a reference to the UDF name.
In this model, the filter $F$ (similarly $A$/$G$) can apply an arbitrary function on the input to discard (add/group) tuples.  

\subsection{Example of Applying the UDF Model}

The following example illustrates how the model captures one possible
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a
classifier
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF is expressed as a composition of
the following local functions:

Map: For each ({\it tweet\_id}, {\it user\_id}, {\it tweet\_text}),
apply food sentiment classifier function that produces user\_id as key, and
({\it tweet\_id}, {\it sentiment-score}) as a value.
The sentiment classifer applies a NLP and
a sentiment classifier on the tweet\_text to represent
the postive or negative sentiment towards food as the  \texttt{sentiment\_score}.

Reduce: For each user\_id, sum up the  \texttt{sentiment-score}. Emit only those
users who have a sentiment score of greater than 0.5.
\end{example}


In terms of the model, the inputs to this UDF are 
$\langle A$=\{\texttt{user\_id}, \texttt{tweet\_id}, \texttt{tweet\_text}\},
$F$=$\emptyset$,
$G$=$\emptyset$ $\rangle$,
assuming the input does not have any previous filters or groupings here.
Then the outputs are 
$\langle A$=\{\texttt{user\_id}, \texttt{sentiment\_score}\},
$F$=$\texttt{sentiment\_score}>0.5$,
$G$=\texttt{user\_id}$\rangle$.
Notice this UDF produces a new attribute,  \texttt{sentiment\_score}. 
As mentioned previously, whenever a new attribute is produced, 
its dependencies on the subset of the input are recorded by the model as well as the UDF name.
For instance, the meta-data describing the new attribute \texttt{sentiment\_score} in 
Example~\ref{ex-food-sentiment} is:
$\langle A$=\{\texttt{user\_id}, \texttt{tweet\_text}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
%This signature captures the dependency of the output attribute on its
% immediate inputs.

Note the model also captures standard relational
operators such as select (2), project (1), join (2), group-by (3) 
and aggregation (3,1), where the numbers in the parenthesis 
refers to the three applicable operations.
Joins are modelled in the standard way in MapReduce which is to group
multiple relations on a common key (as in Pig~\cite{Olst2008}).
Note from the three operations described, there is no facility to update
attributes in place, which is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a
new attribute.
When a new attribute is produced, its dependencies on the
subset of the input are recorded. 

The properties modelled are straightforward and correspond directly to the local functions
performed.
The properties can be provided as annotations by the 
UDF creator with minimal overhead, or may be automatically deduced via some
code analysis method such as that in~\cite{Hues2012}.
In this work, we have the user provide the annotations when a UDF is admitted
to the system.  
This is a reasonable compromise since the properties only need provided the first
time the UDF is added to the system, and our model annotations are very simple.




==> old/Udf-model.tex <==
\section{UDF Model}\label{sec-udf-model}
Queries in our scenario are likely to include complex analytical operations 
expressed as UDFs.
In order to reuse previous computation in our system effectively, we require a
way to model UDFs semantically.
Possibilities for modeling UDFs may include white, gray, or black-box 
approaches with varying levels of overhead and complexity to the system.
A white box approach requires a complete description of the UDF such that the 
system understands \textit{how} the UDF transforms the inputs.
This approach has high overhead for an analyst when adding a new UDF to the 
system.
A black box approach has very low overhead for an analyst but produces an 
output that is completely opaque to the system (similar to a stored procedure)
thus may not be suitable for our goal of reusing results.
Since UDFs can involve fairly complex operations on the data, our system
adopts a gray-box approach that only captures the 
\textit{end-to-end transformations} performed by a UDF.
This requires a small amount of overhead when adding a new UDF, 
yet allows the system to understand the UDF's transformations in a useful way.
The end-to-end transformations allowed by our gray-box model are limited to 
the following operations.

\vspace{-0.05in}
\begin{enumerate}
\setlength{\itemsep}{3pt}%
\setlength{\parskip}{0mm}%
\item Discard or add attributes 
\item Discard tuples
\item Perform grouping of tuples
\end{enumerate}
\vspace{-0.01in}

%In the model, a UDF must describe its output attributes, based on their 
%relation to the input attributes.
We provide a grammar for UDFs, which is used as a program that takes 
an input to the gray-box model of a UDF and provides output.
The output of the model represents the end-to-end transformation of the inputs
performed by the UDF.

Specifically, the input to the model is a set of attributes $A$, 
a set of filters $F$, and the current grouping attributes $G$.
The output is given as a set of attributes $A'$, a set of filters $F'$, 
and the new grouping attributes $G'$.
For example, given input $A,F,G$, the output is $A',F',G'$ with 
$A'=\{(A-X) \cup Y\}$, $F'=\{F\cup Z\}$, $G'\subseteq\{G \cup A \cup Y\}$, 
where $X \subseteq A$,
$Y$ is the set of all new attributes produced by the UDF, and
$Z$ is the set of new filters applied by the UDF.
Note from the 3 operations described, there is no facility to update 
attributes in place, which we believe is reasonable given that our primary
data source is logs.
Any modification to an input attribute must be reflected as a new attribute 
appearing in $A'$.
%The filters in $F'$ are a conjunction of the input filters $F$ with any 
%additional filters applied by the UDF.
%$G'$ represents the new grouping attributes (if any) after applying the UDF.
When a new attribute $y \in Y$ is produced, its dependencies (if any) on 
 $A$, $F$, $G$ are recorded as a small signature, described shortly.

%Our model is expressive enough to capture many common types of UDFs, 
%including classifiers.
The following example illustrates how the model captures one possible 
implementation of a UDF called \texttt{FOOD-SENTIMENT} that uses a classifier 
to compute a sentiment score on users who talk about food items.

\begin{example}\label{ex-food-sentiment}
\texttt{FOOD-SENTIMENT} UDF:
For each user, gather all of their tweets from the Twitter log.
%Discard those tweets that do not refer to any terms closely related to food.
Apply a classifier that determines if a tweet refers to food or a 
closely-related concept, and then computes a food sentiment score for 
each user.
Output only those users with score above a given threshold, $0.5$.
The representation of this UDF in the gray-box model is as follows.
Suppose the inputs are defined as attributes $A$=\{\texttt{userid},
\texttt{tweet}\}, filters $F$=$\emptyset$, group-by $G$=$\emptyset$, 
and the UDF name is \texttt{FOOD-SENTIMENT}.
Then the output includes the new attribute \texttt{score} and an additional 
filter, given by $A'$=\{\texttt{userid}, \texttt{score}\}, 
$F'$=\{\texttt{score>$0.5$}\},
and $G'=$\{\texttt{userid}\}.
\end{example}

The new attribute \texttt{score} has a signature, which is the inputs required
for the UDF as indicated by the model and the UDF name.  
In this example the signature would be 
$\langle A$=\{\texttt{userid}, \texttt{tweet}\},
$F$=$\emptyset$,
$G$=$\emptyset$, 
name=\texttt{FOOD-SENTIMENT}$\rangle$.
This signature is a minimal form of provenance that captures a functional 
dependency of the output attribute on its immediate inputs.

%UDFs in the system can be as expressive as the execution engine permits.
Any UDF with end-to-end transformations correctly captured using the model
can be \emph{admitted} to the system.
Note the model only needs to be provided the first time the UDF is added.
This gray-box model has certain limitations.
For instance, given two identical UDFs with different names but otherwise 
identical inputs, their new attributes will result in different signatures.
This deficiency can only be overcome if we resort to a white-box approach.



==> old/Viewfinder-rewrite1.tex <==
\section{ViewFinder}\label{sec-viewfinder}

The key feature of $\VF{}$ is its ability to order
candidate views by their lower-bound cost thereby
allowing it to incrementally explore the the space of rewrites using
the views in $V$.
This functionality is used by $\WF{}$ to explore 
the space in an incremental manner and prune unneccessary sub-spaces
as shown in Section~\ref{sec-solution-outline}.
% Thus we incorporate $\ocost{}$ with the traditional approach
% which consists of finding {\em complete} candidate views and enumerating
% rewrites for each candidate.

As noted in Section~\ref{sec-problem-definition} rewriting queries
using views is known to be a hard problem.
Traditionally, methods for rewriting queries using views for the
class of SPJG queries use a two stage approach~\cite{Hale2001, Agra2000}.
The prune stage determines which views are \emph{relevant} to the query,
and among the relevant views those that contain
all the required join predicates  are termed as \emph{complete},
otherwise they are called {\em partial} solutions.
This is typically followed by a merge stage that joins the partial
solutions using all possible equijoin methods on all join orders to form
additional relevant views.
The algorithm repeats until only those views that are
useful for answering the query remain.

We take a similar approach in that we identify partial and
complete solutions, then follow with a merge phase.
The $\VF{}$ considers candidate views $C$ when 
searching for rewrite of a target.
$C$ includes views in $V$ as well as views
formed by ``merging'' views in $V$ using a
\textsc{Merge} function, which is an implementation of a 
standard view-merging procedure (e.g.,~\cite{Agra2000,Hale2001}).

% However, the direct applicability of existing approach
% to our problem is limited.
With no early termination condition existing approaches 
explore the space exhaustively,  degenerating into the 
bottom-up approach.
Thus we desire a rewriting algorithm  that can
enumerate the space and incrementally explore
only as much as required, frequently stopping
and resuming the search as requested by \WF.
We note that while an equivalent rewrite for a target may exist,
the \VF may never be asked to find it,
as illustrated by Example~\ref{example-greedy-plumbing}.

\subsection{V\fakesc{iew}F\fakesc{inder} Algorithm}

The $\VF{}$ maintains a priority queue for each target containing candidate views.
% The \VF{} finds a rewrite for a target in $W$ given a set of materialized views $V$.
% This problem is referred to as \emph{query} rewriting, hence our 
% input is a query $q$ representing the target, and $V$.
% Given our problem formulation, we require one instance of the \VF{} per target in $W$.
The $\VF{}$ is {\em stateful} which
enables the $\WF$ to start, stop and resume the incremental searches at each target.
Moreover, the space of candidate views $C$ can be very large due to merging
views in $V$. Our approach allows for a gradual explosion of the space as needed.
% Here we will describe the functionality of the \VF{}, and later in
% Section~\ref{sec-best-first-workflow-rewrite} we
% will present the \WF{} which exploits the \VF's{} ability to incrementally examine
% the space of solutions for each target.
The lower bound provided by $\ocost{}$ enables the \VF{} to explore the space
incrementally, at every step examining any potentially lower-cost rewrites before exploding the
space further to produce candidate views that have higher potential cost.

\begin{comment}
% Good text but got rid of it in the Alkis rewrite
Answering queries using views is a long-studied problem.
It is primarily considered in the context of data integration or data warehouse
design (query optimization)~\cite{Hale2001}.
Data integration is often interested in maximally-contained rewrites while
query optimization is concerned with equivalent rewrites.
Our interest is the latter.
The complexity of the problem is described with respect to the
expressivity of the languages used for both the queries
and the view definitions~\cite{Abit1998}.
Even when both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete
both for determining whether a rewrite exists~\cite{Levy1995} and
checking the correctness of a rewrite.
Checking the correctness of the rewrite is the same problem as
determining containment (i.e. $ Q_1 \subseteq Q_2$), which is
NP-complete~\cite{Chan1977} for conjunctive queries.
A \textit{complete} rewriting of $Q$ using $V$ is said to be one
that only uses $V$, and does not use any of the base relations.
Determining whether there is a complete rewriting of $Q$ using $V$
(again for the class of conjunctive queries) is NP-complete~\cite{Levy1995}.
Furthermore, when $Q$ and $V$ are disjunctions of conjunctive queries,
finding a complete rewriting is NP-complete~\cite{Levy1995}.
Producing a \textit{minimal} rewrite entails using the minimal number
of views in the rewrite such that no view can be removed
without invalidating the rewrite.
This problem is also NP-complete~\cite{Levy1995}.
We only consider complete rewrites, those using
the existing views, without extracting new views from the log.
\end{comment}

\begin{comment}
% CUT due to lack of space.
The reason we do not return to the log (i.e., base relation) is that
more and more views become materialized in the system as analysts
perform their data exploration and furthermore log extraction is expensive.
The rewrites are expressions in $L_R$ which may include
additional transformations on $V$ in order to produce an equivalent rewrite.
\end{comment}

\begin{comment}

\begin{enumerate}
\item {\bf Prune Step}:  Retain only those views that are relevant 
to the query (have the required attributes, have a mapping to the 
same base relations, logically-weaker selection and join predicates).

Find {\em all} relevant views $v$ to the query $q$.
Views that are not relevant to the query are pruned.

Determining a relevant view $v$ involves
(a) $v$ shares common base relations with $q$,
(b) $v$ must not have projected out any attributes required by $q$, and
(c) $v$ must contain a subset of the join predicates in $q$ and (d) must have
identical or logically weaker selection predicates.

The views in $V$ that pass the prune step are called {\em relevant} views.

Among the relevant views those that contain all the join predicates in $q$
are termed as \emph{complete}, otherwise they are called {\em partial} solutions.
%% Note that the {\em complete} solutions are added to the {\em winner} pile,whereas the partial solutions are added to the {\em loser} pile.
Next, a {\em  dominance} pruning is performed by comparing all pairs of relevant views, from each pair
discard the view with lower contribution or higher cost.

%%For all the complete solutions, it tries to find an equivalent rewrite using the views, which we term as {\em chain forming}.
% SJ: Need to figure out what the hardness result of "chain formation"

\item {\bf Merge Step}: Join all partial solutions using all
possible equijoin methods on all join orders to form
additional relevant views. Return to prune step.
\end{enumerate}
\end{comment}

To determine if a view $v$ is partial or complete with respect to a
query $q$, we take an optimistic approach.
This approach represents a \emph{guess} that a complete rewrite exists using $v$.
A guess requires the following necessary conditions
as described in~\cite{Hale2001} (SPJ) and~\cite{Gold2001} (SPJG)
that a view must satisfy to participate in a rewrite of $q$, 
although these conditions are not sufficient to
confirm the existence of an equivalent rewrite using $v$.

\begin{itemize}
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item $v$ contains all the attributes required by $q$; or contains all the 
    necessary attributes to produce those attributes in $q$ that are not in $v$
\item $v$ contains weaker selection predicates than $q$
\item $v$ is less aggregated than $q$
\end{enumerate}
\end{itemize}

The function $\complete(q,v)$ performs these checks and returns true if $v$
satisfies the properties i--iii with respect to $q$.
Note these conditions under-specify the requirements for
determining that a valid rewrite exists, thus a guess may
result in a false positive, but will never result in a false negative.

% The lower bound provided by $\ocost{}$ allows the \VF{} to search the space
% incrementally, exploring any potentially
% lower-cost rewrites first before exploding the
% space unnecessarily to find and enumerate them all.
%The $\VF{}$ takes as inputs
%a query $q$, the set of existing materialized views $V$,
%two values $d',d$, s.t., $d' < d$ and outputs an equivalent
%rewrite $r$ of $q$ using a set of views in $V$, such that
%$d' < \ocost(r) \leq d$ if $r$ exists.
%Note that $V$ is only required in the initialization step,
%and in subsequent invocations $d'$ is implicit in the sense that it records
%the value of $d$ from the previous invocation.


\begin{comment}
% SJ: Given that we now use Surajit Chaudhuri's method, this text is not needed 
%
The $\VF{}$ maintains a priority queue $\PQ$ which contains all candidate views.
The candidate views include those in $V$ as well as views
formed by ``merging'' of views in $V$.
To merge a pair of candidate views $v_1$ and $v_2$,
we consider all possible equi-join methods based on common keys,
as well as trying all possible subsets of join predicates that are present in $q$
which is similar to the approaches in~\cite{Agra2000,Hale2001}.
In~\cite{Hale2001} partial views are only considered for merging if they satisfy join
predicates in $q$, while~\cite{Agra2000} merges views to create parent
views that can answer the same or larger subset of queries
in the given workload than their constituent views (i.e, $v_1$ and $v_2$).
We adapt both approaches as a way of making partial views complete with respect to $q$.
As in~\cite{Agra2000}, we generate new views by a series of pair-wise merges.
This process is captured in the procedure $\merge(v_1, v_2)$, 
where $v_1$ and $v_2$ are candidate views
and the output is a new candidate view $v_{12}$.
Because the merging process adds exponentially more
views for consideration, we should avoid growing the space larger than necessary.
Thus we control the candidate generation process by merging a candidate view with those
candidates views that have a lesser $\ocost{}$.
The use of the $\PQ$ enables the merge process to be resumed later when the
$\VF{}$ is invoked in the next iteration, if it is needed.

While~\cite{Agra2000} only retains candidate views that the optimizer considers 
 useful for answering queries and their merge step only considers
merging based on the join condition specified in $p$,
we consider merging views when they share a common key.
The utility of merging views based on a common key can 
be seen from the following example.
Consider a query $q$ that requires the key $\{A,D\}$.
Suppose that $v_1$ contains key $\{A,B\}$, $v_2$ contains key $\{B,C\}$ and $v_3$ contains
key $\{C,D\}$.
A typical pruning step would discard $v_2$ as it does not contain any attributes
syntactically relevant to $q$.
We note that merging $v_1$ with $v_2$, followed by a merge with $v_3$ will obtain a superset
of keys needed by $q$.
This merged view is complete with respect to $q$.
\end{comment}


\begin{algorithm}[h!]
\caption{$\VF$\label{alg-viewfinder}}
{\small
\begin{algorithmic}[1]
\Function{\sc Init}{$query$, $V$}\label{alg-vf-init}
 \State Priority Queue $PQ$ \qlet $\emptyset$; $Seen$ \qlet $\emptyset$; Query $q$ 
  \State $q$ \qlet $query$
  \ForAll{$v \in V$}
     \State $PQ$.\texttt{add}($v$, $\ocost(q,v))$
  \EndFor
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Peek}{}\label{alg-vf-peek}
%\State \Return ($PQ$.\texttt{peek}().$\ocost$: $\infty$) ? 
\State {\bf if} $PQ$ is not empty {\bf return} $PQ$.\texttt{peek}().$\ocost$ {\bf else} $\infty$
%   \If{not $PQ$.\texttt{empty}()}
%   \State \Return $PQ$.\texttt{peek}().$\ocost$ 
%   \Else 
%   \State \Return $\infty$
%   \EndIf  
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Refine}{}\label{alg-vf-refine}
  \If{\texttt{not} $PQ$.\texttt{empty}()}
    \State $v$ \qlet $PQ$.\texttt{pop}()
    \State $M$ \qlet \merge($v$, $Seen$) \Comment{Ensure $Seen \cap M = \emptyset$}
    \ForAll{$v' \in M$}
      \State $PQ$.\texttt{add}($v'$, $\ocost(q,v')$)
    \EndFor
    \State $Seen$.\texttt{add}($v$)
    \If{\complete($q$, $v$)}
      \State \Return $\RE(q, v)$
    \EndIf
  \EndIf \\
  \Return {\sc null}
\EndFunction
\end{algorithmic}}
\end{algorithm}

The $\VF{}$  is given in Algorithm~\ref{alg-viewfinder} and described below.

The \Init{} function instantiates an instance of the $\VF{}$ 
with a $query$ which a logical representation of a target $W_i \in W$
and a set of materialized views $V$ present in the system.
Next, $query$ is assigned to $q$ and $V$ is added to a priority queue $\PQ$
that orders candidate views by their $\ocost{}$.
At the end of \Init{}, the candidate views in $\PQ$ includes only those views in $V$.

The $\Peek{}$ function is used by $\WF{}$ to obtain the $\ocost{}$ of the head item
in the $\PQ$.

The $\Refine{}$ function is invoked when $\WF{}$ asks the $\VF{}$
to examine the next candidate view.
At this stage, the $\VF{}$ pops the head item $v$ out of $\PQ$.
The $\VF{}$ then generates a set of new candidate views $M$
by merging $v$ with previously popped  candidate views (i.e., views in $Seen$),
thereby incrementally exploding the space of candidate views.
Note that $Seen$ contains candidate views that have an $\ocost{}$ 
less than or equal to that of $v$.
$M$ only retains those candidate  that are
not already in $Seen$, which are then inserted into $\PQ$.
% TODO: Need a proof for that statement
A property of $\ocost{}$ provided as a theorem later is that
the candidate views  in $M$ have an
$\ocost{}$ that is greater than that of $v$.
Then, $v$ is added to $Seen$.
If $v$ is guessed to be complete,  we try to find rewrites of $q$
using $v$ by invoking the $\RE$ function.
Among the rewrites found by $\RE{}$, the cheapest rewrite is returned to $\WF{}$ as the result.
% TODO: Do we need to talk about join ordering?


\subsection{Rewrite Enumeration}\label{sec-rewrite-enumeration}

% Suppose that a candidate view $v$ is guessed to be complete.
% To determine if an equivalent rewrite exists requires finding at
% least one valid rewrite among all possible rewrites,
% is known to be a hard problem~\cite{Levy1995}.
In our system the \RE{} algorithm attempts to produce a valid rewrite
of a query using a view that is guessed to be complete, if one exists.
% \RE{} takes as input a query $q$ and a view $v$ that is guessed to be complete
% and outputs a rewrite $r$ if one exists.
The rewrite returned represents the cheapest among
all possible equivalent rewrites of $q$ using $v$.
The cost of a rewrite is evaluated by the \cost{} function,
and corresponds to the cheapest execution \textit{plan} that
implements the rewrite.
Equivalence is determined by ensuring
that the rewrite and query contain the same attributes,
filters, and groupby.
%This type of equivalence testing is simple but effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%Although this type of equivalence testing may seem simple it is effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%We replace an SPJ+G expression with a single view.  as in GL2001


We search for equivalent rewrites of $q$ by applying compensations
to $v$ using $L_R$.
%A transformational rule is a UDF in the system that may
%modify any set of the properties in our UDF model
%which are attributes, filters, and groupbys.
% Given the complex interactions possible 
% for any arbitrary set of $k$ rules in $L_R$,
% it may require generating all possible rewrites of $r$ using $L_R$
% before identifying an equivalent rewrite if one exists.
We do this by generating all permutations of required compensations and
testing for equivalence, which
% which can also include multiple applications of the same rule.
amounts to a brute force enumeration of all possible rewrites given $L_R$.
This makes case for the system to keep $|L_R|$ small.
When $L_R$ is restricted to a known, fixed 
set of operators it may suffice to examine a polynomial number of 
rewrites attempts, as in~\cite{Grum2003} for the specific case 
of simple aggregations involving group-bys.
Such approaches are not applicable to our case as 
the system should have the flexibility of extending $L_R$ with 
UDFs from $L_W$ when it results in overall system benefit.

Given the computational complexity of finding valid rewrites,
we limit the invocation of $\RE{}$ algorithm using two strategies.
% we employ the following two strategies.
First,  we avoid having to apply $\RE{}$ on every $v$ by making
a guess for the completeness of a view based
on the three properties described earlier.
Second, we delay the application of $\RE$ to every complete view 
by determining a lower bound on the cost of a rewrite using $v$ should one exist.
For the lower bound we use the $\ocost$, which is described in the next section.
% The goal of guessing completeness and estimating a lower bound is
% to quickly distinguish between potentially low cost rewrite from those with higher cost.

\subsection{Determining O\fakesc{pt}C\fakesc{ost}}\label{sec-ocost}
The utility of  a lower bound we develop in this section is that it 
provides a ``spread''  of candidate views based their potential 
to provide a low cost rewrite.
Our expectation of the lower bound is only that it should be able to quickly distinguish between 
candidate views with potential to produce cheap versus very expensive rewrites.
Given a candidate view $v$ and a query $q$,
we wish to determine a lower bound on the cost of \textit{any} plan yielded by
an equivalent rewrite of $q$ using $v$ if one exists without enumerating all possible rewrites,
checking for equivalence and examining their plan costs.
We refer to this lower bound as the optimistic cost, or \ocost.
\ocost relies on the following property about the nature of the $\cost{}$ function.

\begin{definition}\label{definition-non-subsumable-property}
Non-subsumable cost property:
Let $S$ be any set of operations given by the UDF model.
Let $\cost(S,D)$ be defined as the total cost of performing all operations 
in $S$ on a database instance $D$.
Let $\cost(x,D) = \infty$ for those operations $x \in S$ that
cannot be applied on $D$.
Then the following property states the
cost of performing $S$ on a database instance $D$ is at least
as much as performing the cheapest operation in $S$ on $D$.
$$\cost(S,D) \geq \min(\cost(x,D), \forall x \in S)$$
\end{definition}

% Could use MR-cost model or a RDBMS cost model depending on the underlying store
% SJ: Need to extend it to support \ocost functionality
%Taking the minimum cost of an operation in $S$ provides a lower bound on the
%cost of $S$ given $D$.
Because the lower bound is derived from the minimum operation cost, it provides a weak lower bound.
%Noting the fact that at least one operation in $S$ must be applied to $D$ allows us to use the cost
%of the least expensive operation in $S$.
A tighter bound might be provided if we could use the cost of the most expensive operation in $S$,
i.e., $\max(\cost(x,D), \forall x \in S)$.
The reason we must rely on the weak min property is because
a stronger max property requires
$\cost(S', D) \leq \cost(S,D)$, where $S' \subseteq S$.
This requirement is difficult to meet in practice.
As a simple counter-example, suppose $S$ contains a filter $F$
with high selectivity and a group-by operation $G$ with higher cost than $F$
when considering the operations independently on database $D$.
Let $S'$ contain only $G$.
Suppose that applying $F$ before $G$ results in few or no tuples streamed to $G$.
Then applying $G$ can have nearly zero cost and it is plausible that
$\cost(S', D) > \cost(S,D)$.

%There are two possible approaches we can take here.
%One approach assumes that  $v$ will be materialized in the process of rewriting the query
%and then any necessary compensation will be applied.
%Another approach is for compensations
%to be pushed down into $v$ before the join when possible, 
%thereby creating $v'$ which may be cheaper to materialize than $v$.
%The optimizer

Given that $v$ is guessed to be complete with respect to $q$, 
a set difference between the attributes, filters and group-bys representation 
of $q$ and $v$ 
is referred to as the {\em fix}.
Fix denotes the  set of non-subsumable cost operations
by Definition~\ref{definition-non-subsumable-property}
needed to transform $v$'s representation into $q$'s.
%\ocost{} uses the attributes, filters, and group-by representation 
%of $q$ and $v$ to take a set difference between each of these properties.
%This denotes a minimum set of non-subsumable operations
%by Definition~\ref{definition-non-subsumable-property}
%needed to transform $v$'s representation into $q$'s.
Note that this does not guarantee that $v$ will result in a valid rewrite 
for the same reason that  guessed to be complete can result in a false positive.
Both assume that the required
compensation operations can be applied independently of each other to $v$.
% resolve the differences  in the attributes, filters, and group-bys of $q$ and $v$.
%compensate these properites independently.
% is possible to compensate $v$ using operations in $L_r$
%independently of the others.

%We refer to this set as the {\em fix} of $v$ with respect to $q$.
%The non-subsumable property allows \ocost{} 
%to consider operations in the fix as independent of one another,
%although they can still affect each other's cost.
% \ocost{} then returns the sum of the create cost $c'_1$, access cost $c'_2$, and the
% minimum operation cost $c'_3$ in the fix as the
% lower bound on the cost of \textit{any} plan.

%\ocost takes an optimistic approach in determining the minimum possible plan cost.
If a candidate view $v$ is not yet materialized (i.e., to be created by merging),
$\RE{}$ might consider
materializing it first before applying all necessary compensation.
%If $v$ is not materialized in the process of rewriting a query and then any
%neccessary compensation is applied. 
Then, intuitively it can be seen that any plan yielded by an equivalent rewrite would incur at
the least the sum of
the cost $c_1$ for accessing all the constituent views in $v$ (i.e., access cost),
the cost $c_2$ for materializing any new views it requires (i.e., creation cost), and
the cost $c_3$ 
of applying the least expensive compensation operation on the view $v$.
\ocost{} invokes \cost{} to obtain the cost of 
performing each of the operations in the fix on $v$.
It chooses the least expensive operation in the fix
as the third component $c_3$ of the \ocost, where
$c_3$ is given by $\min(\cost(x, v))$ such that
$x$ is an operation in {\em fix}.
We define \ocost{} as $c_1 + c_2 + c_3$, which has the property 
that it is a lower bound on the cost of \textit{any} plan returned by $\RE(q,v)$
and inexpensive to compute.
If $v$ is partial (i.e., not guessed to be complete) with respect to $q$,
then $c_3 = 0$ since no compensation should be applied.

%Note that if using the push-down approach, 
%when the view is partial then \ocost{} is only $c'_1$,
%since push-down predicates may change the join ordering.
%Further details  of this \ocost{} function 
%and our proof of the lower bound property when considering predicate pushdown is 
%omitted here due to lack of space.


\begin{comment}
There are certain benefits to both approaches.
The choice to create $v$ is similar to the approach that a view recommender~\cite{Agra2000} might take,
while pushing down predicates into $v$ to create $v'$ is an approach that a query optimizer may take for
answering a single query $q$.
One way to think about this is that $v$ is a recommended view by the $\VF{}$ and here we
decide to piggyback its creation as a part of execution of query $q$.
Given the use case of the system, we prefer this approach as we
wish for the artifacts created (i.e., $v$) as part of answering $q$ to
be as beneficial as possible to the subsequent queries by future users.

The $\VF{}$ could be modified to support predicate pushdown by
modifying $\ocost$ to order partial views by their access cost for $v$ (i.e., $c'_1$).
The pushdown predicates can potentially change the cost of all the joins and their orderings.
\end{comment}


% RETAIN THE REMAINDER OF THIS PROOF HERE. -- REFERS TO APPENDIx
% An $\ocost{}$ function that considers predicate pushdown 
% is given in Appendix~\ref{appendix-pushdown}.


$\RE{}$ might consider push-down of compensations into a candidate view $v$ before materializing it.
%thereby creating $v'$ which may be cheaper to materialize than $v$.
The $\ocost{}$ function for this case has a weaker lower bound property
as it can only consider the cost ($c_1$) of accessing all the consitituent views of $v$ 
plus the minimum cost of applying the least expensive operation 
in the fix on any consitituent views of $v$.

\begin{comment}
\begin{theorem}
$c'$ is a lower-bound on on the cost of \textit{any} plan yielded by
an equivalent rewrite of $q$ using $v$ if one exists.
\end{theorem}

\begin{proof}
Let $c$ be the minimum cost plan generated by the $\RE(q,v)$ corresponding
to the rewrite $r$.
$c$ is composed of
the cost $c_1$ for accessing all the views, and
the cost $c_2$ for materializing any new views it requires,
the cost $c_3$ for least expensive ordering of transformation 
rules in $L_R$ applied to $v$.
As $v$ is guessed to be complete for the query $q$,
both $\RE$ and $\ocost$ use $\cost$ to obtain the cost to create and access $v$,
then $c_1 = c'_1$ and $c_2 = c'_2$.

In order to find the lowest cost $r$, $\RE{}$ will have
to enumerate all permutations of rules in $L_R$ required
to achieve the fix.
If \RE{} finds a rewrite, $r$ will have covered all operations in fix,
choosing the cheapest rewrite found to be $c_3$.
$\ocost{}$ uses \cost{} once per each operation in fix
choosing the cheapest as $c'_3$.
As $c'_1$ and $c'_2$ are common to both $c$ and $c'$,
it suffices to show that $c_3 \geq c'_3$.

Recall that \emph{fix} is made up of non-subsumable operations.
A property of two non-subsumable operations as mentioned
earlier in Definition~\ref{definition-non-subsumable-property} is that:
$\cost(xy, D) \geq \min(\cost(x, D),
\cost(y, D))$, where $v$ is an instance of a database $D$, and
$x$, $y$ are operators in fix, and $xy$ performs both $x$ and $y$.

By induction we can show that the cost of the cheapest
rewrite that applies  the fix to $v$
is greater than or equal to $\cost(op^*, v)$, 
where $op^* \in \mbox{\em fix}$
and is the cheapest operator present in the {\em fix} but we
omit the remainder of the induction for lack of space.\qed

-- RETAIN THE REMAINDER OF THIS PROOF HERE. -- 
Base Case: Let the fix be denoted by the operators $x$, $y$, $z$,
such that $op^* = z$ is the cheapest operator in fix.
A rewrite $r$  using {\em fix} can
apply operators in the following sequence:
a) apply one operator followed by another or both,
b) apply two operators (e.g., $xz$) followed by a third
operator (e.g., $y$), or
c) apply operators $xyz$ all at once.
For case a) the cost of $r$ is greater than or equal to
either $\cost(x,v)$ or $\cost(y,v)$  or $\cost(z,v)$.
For case b) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(z,v))$ if the first operation
is given by $xz$.
For case c) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$.
As $r^*$ represents the lowest cost rewrite across
all rewrites denoted by the three cases, it is bounded by:
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$, which proves
the base case of {\em fix} with 3 operators.

Induction Step:
Let $y$ be the cheapest operation in the set denoted by $\mbox{\em fix}-x$, such that
$\cost(r^*,v) \geq \cost(y,v)$ where $r^*$ corresponds
to lowest cost rewrite on $\mbox{\em fix}-x$.
In other words, the cost of $r^*$ is at least the cost of applying
the cheapest operator in $\mbox{\em fix} -x$.

Add $x$ back to the {\em fix}.
Now, let $r^*$ be the lowest cost rewrite
using {\em fix}.
Suppose that $r^*$ is composed of sets operators $p_1, p_2 \cdots p_k$, such that
$p_1 \cup p_2 \cdots \cup p_k = \mbox{\em fix}$ and
the output of $p_1$ forms the input to $p_2$ and so on.
Then, $\cost(r^*,v) = \cost(p_1, v) + \cost(p_2, v|p_1) + \cdots + \cost(p_k, v|p_1\cdots{}p_{k-1})$,
where $v|p_1$ means that operators in $p_1$ have been applied to $v$.
This means that $\cost(r^*,v) \geq \cost(p_1, v)$ given that $\cost{}$ is always non-negative.
The lowest value of $\cost(p_1,v)$ occurs when $op^*$ is present in
$p_1$ possibly along with other operators in the {\em fix}.
Thus, $op^*$ must either be $y$ which was the cheapest operator in $\mbox{\em fix} - x$
or $op^*$ must equal to $x$.
Then, $\cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$.
Finally, $\cost(r^*,v) \geq \cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$. \qed
\end{proof}
\end{comment}

%The $\ocost{}$ does not cause the algorithm to lose its optimality property,
%regardless of considering an even larger (or pruned)
%rewrite space  than the one we consider here.


\begin{comment}
The lower bound provided by our $\ocost{}$ function could be tightened if we are
willing to commit to a particular execution environment and a specific query optimizer.
For example in an MR environment with a Hive query processor,
given the set of operations in the fix, one could
estimate the minimum number of maps, reduces, and jobs it would take to
apply all operations in fix to $v$.
Such an approach requires intimate knowledge of a specific system,
and thus loses the desired generality of a lower bound estimator.
\end{comment}

%Finally, we provide the following lemma describing the $\ocost{}$ property
%for any new candidate view created in $M$ during Algorithm~\ref{alg-viewfinder}.

The following theorem describes the $\ocost{}$ property for newly
merged candidates in $M$.
This enables Algorithm~\ref{alg-viewfinder}
in order to generate candidate views as needed to avoid a pre-explosion
of the space of all candidates.

\begin{theorem}
The $\ocost{}$ of every candidate view in $M$ that is not in $Seen$
is greater than or equal to the $\ocost{}$ of $v$.
\end{theorem}
\begin{proof}
The proof sketch is as follows. The theorem is trivially true for 
$v \in V$ as all candidate views in $M$ cannot be in $Seen$
and have $\ocost$ greater than $v$. 
If $v \notin V$, it is sufficient to point out
that all constituent views of $v$ are already in $Seen$
since they must have had $\ocost{}$ lesser or equal to $v$
Hence all candidate views in $M$ with $\ocost{}$ smaller than $v$ are
 already in $Seen$, and those with $\ocost{}$ greater than $v$ will be added to $PQ$
if they are not already in $PQ$.
 %all the 
%candidate views in $M$ are already present in $Seen$ if smaller, or if greater,
%are still in $\PQ$.
\end{proof}

\begin{comment}
% RETAIN THE REMAINDER OF THIS PROOF HERE.
\begin{proof}
Suppose that $v'$ is a new candidate  that is created by merging $v$ with $Seen$.
Then we need only consider the case of $v$ being a base view or a composite view.
If $v$ is a base view (i.e., already materialized), then the $\ocost{}$ of $v'$  cannot be
less than $v$ as $\ocost(v)$ only considers its access cost, while $\ocost(v')$
is at least the cost of accessing $v$ as well as accessing the other candidate view that $v$ is joining with.
If $v$ is a composite view (i.e., $v$ is composed of multiple base views),
then the $\ocost{}$ of $v'$ cannot be less than $v$.
To show that by contradiction,
consider the case where $v'$ is not in $Seen$
and $v'$has a lesser $\ocost{}$ than $v$.
As $v$ is a composite view, then all of its constituent views would already
have been joined with all the candidate views in $Seen$.
Thus, $v'$ must already have been created.
If $v'$ has a lesser $\ocost{}$ than $v$,
it would have already been popped out of $\PQ$ and in $Seen$ before we got to $v$.
\end{proof}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}


\begin{itemize}
\item Two queries $Q_1$, $Q_2$
are said to be {\em equivalent} if $Q_1 \subseteq Q_2$ and $Q_2 \subseteq Q_1$.
From a query answering perspective,
the set of tuples in the result set of $Q_1$ are identical
to the set of tuples in the result set of $Q_2$.
To determine if an equivalent rewriting using views exists has been already
shown to be in NP even for the class of conjunctive queries~\cite{Hale01}.

\item A query $Q_1$ is said to be {\em contained } by $Q_2$
if $Q_1 \subseteq Q_2$.
From a query answering perspective,
all the tuples in the result set of $Q_1$ are contained in
the result set of $Q_2$, although the result set of $Q_2$ can contain additional
tuples that is not present in the result set of $Q_1$.
The problem finding contained rewriting is also known to NP-complete
even for conjunctive queries~\cite{Hale01-18}.

\end{itemize}

\item A candidate $c$ is said to be {\em complete} with respect to a $Q$ iff $c$ has
has a superset of the attributes and a subset of the filters and
superset of the groupby keys.
If there are attributes in $Q$ that are not present in $c$, $c$ has
the necessary ingredients (i.e., attributes) to obtain $Q$.
Of course, even if $c$ is complete,  it does not mean that
there exists an equivalent rewrite of $Q$ using $c$.
Thus, this provides a necessary but not sufficient
condition that equivalent rewrite exists.
The sufficient condition is when an equivalent
rewrite of $Q$ using $c$ exists.

\item We provide a set of $k$ transformational rules for
query rewriting using a candidate $c$. We call the
rewrite of complete candidate $c$ to a target $t$ using
our transformational rules a {\em chain}.

\item There are three classes of transformational rules that
we allow in the system.



\begin{itemize}
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item Rules that transform \{A\}, \{F\}, \text{or} \{G\}
\item Rules that transform \{A,F\}, \{F, G\}, \text{or} \{A, G\}
\item Rules that transform \{A, F, G\}
\end{enumerate}
\end{itemize}
\renewcommand{\labelenumi}{\theenumi}


% SJ: Let us add an example here
\item We have 4 transformation rules in our system:
\begin{enumerate}
\item $P$ \textendash Project (class \textsl{i})
\item $F$ \textendash Filter (class \textsl{i})
\item $G$ \textendash Groupby (class \textsl{i} and \textsl{ii})
\item $D$ \textendash Derived (class \textsl{i}, \textsl{ii}, \textsl{iii})
\end{enumerate}

In our $\MinDist$ function presented later, we make the assumption
that each rule can be applied independently.
Furthermore, our algorithm (described later) makes the assumption that the
 Filter rule applies all missing filters, one at a time before completing.
This prevents a large explosion of rule permutations
to apply when searching for a valid rewrite.  However, it presents a limitation on the
ability of our algorithm to find a successful rewrite if one exists.
It may be that no valid rewrite exists using a permutation
of these 4 rules, but one might exist if we consider each missing filter a separate
application of our $F$ transformation rule and thus could produce a successful rewrite such as
$F \rightarrow G \rightarrow F$ whereas due to our restriction of applying all missing filters
with the  $F$ rule before moving to another rule would not be able to produce such a re-write.

The \emph{Derived} rule allows for easy extensions, which is useful for attributes
created by UDFs that can easily be manipulated into other attributes.  For instance, one could add
a derivation that transforms lat-lon into a grid, or positive sentiment with a scoring value of
0.5 to 0.6, or word-count into (approximate) character-count.  Currently we have implemented
several derived attr transformations such as Groupby stats...

\item Determining if a solution $c$ is {\em complete} is  NP-hard
as it involves enumerating all possible chains using the transformation
rules

\item If a candidate is complete we can ``guess''
the minimum number of
transformational rules that go into the chain.
It is minimum ``guess'' as it based on the necessary
condition but not the sufficient condition, so no valid
chain may exist.

\item Why we cannot directly apply the traditional view finding:
  \begin{itemize}
  \item Discarding the non-relevant views using common base relations is not an effective pruning strategy as all queries are posed on a small set of logs, thus many views have the same base relation, a log.
  \end{itemize}
\end{itemize}

\subsection{View Finding Algorithm}

\begin{itemize}

\item Idea of a guess or mindist of a candidate to a target.
\begin{enumerate}
\item Also determine (optimistic guess) complete (winners) vs. partial candidates (losers)
\item Helps prune away the space quickly
\end{enumerate}

\item Describe chain data structure
\begin{enumerate}
\item Series of cmerged or joined candidates, where joined candidates
are restricted to those join predicates that appears in $t$
\item cmerge are keyed equijoins between candidates that shares
common keys
\item joins are equi across different keys or non-keys
\end{enumerate}

\item How to determine mindist?
\item mindist(chain c, t)
\begin{enumerate}
\item Really quick computation
\item Committed cost(c) + guess\_remaining\_cost(c.tail, t)
\item Decouples search from distance computation by assuming independence
\item Magical UDF
\item Claim: Guess is always <= actual cost
\item Finite mindist does not mean existence of chain which
is known to be NP-hard.. (because necessary condition only)
\end{enumerate}

\end{itemize}

Because we explore the solution space incrementally using our MINDIST, we
initialize the viewfinder by registering a target view and a set of candidate
views as follows in Algorithm \ref{viewfinderinit}:

\begin{algorithm}
\caption{ $\VF$-\textsc{initialize}($t$, $C$)}
\label{viewfinder-init}
\begin{algorithmic}[1]
\Require target $t$, candidate pool $C$ % some input
\State {Initialize WinnersPriorityQ, LosersPriorityQ}
\ForAll{$c \in C$}
  \State chain $c' \Leftarrow c$
  \State $d \qlet \MinDist(c', t)$
  \If{$d$ is $\infty$}
    \State LosersPQ.add($c'$, $d$)
  \Else
    \State WinnersPQ.add($c'$, $d$)
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\caption{ $\VF$($t$,\textit{MinCost})}
\label{viewfinder}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ
\State \textsc{mergeables}.\textit{clear()} \\
\Comment {\scriptsize Grow candidate space by merging all (partial view) pairs until the \textsc{committed\_cost} of all Losers is greater than the requested MinCost \normalsize}
\State $m \qlet $ \textit{MinCost}
\While{LosersPQ.peek().committed\_cost $ < m$}
  \State \textsc{mergeables}.\textit{add}( LosersPQ.pop() )
\EndWhile
\State \viewfinderCMerge(\textsc{mergeables})
\While{$ \MinDist$ (Winners.peek()$, t) < m$}
  \State $chain$ $\qlet$ Winners.pop()
  \State   \answer $\qlet$ \viewfinderRefine($chain$, $t$)
  \If {\answer}
    \State $\result$.\textit{add}($\ans$)
  \EndIf
\EndWhile
\State return $\result $

\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{ \viewfinderCMerge(\textsc{mergeables}) }
\label{viewfinder-cmerge}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ \\
\Comment \scriptsize attempt to merge all pairs of views, join order is not considered here \normalsize \\
\Comment \scriptsize This is a keyed equi-join \normalsize
\ForAll{$i \in $ \textsc{mergeables}}
	\ForAll{$j \in $ \textsc{mergeables}}
	  \State $tmp \qlet$\textsl{ColumnMerge}($chain_i$, $chain_j$)
	  \If{$tmp$}
	    \State $newchain \qlet chain_i + chain_j$
	    \State $d \qlet \MinDist(newchain, t)$
	    \State $totalDist \qlet d + newchain$.\textsc{committed\_cost}
        \If{$d$ is $\infty$}
          \State LosersPQ.add($newchain$, $totalDist$)
        \Else
          \State WinnersPQ.add($newchain$,$totalDist$)
        \EndIf
      \EndIf
	\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{ \viewfinderRefine($chain$, $t$)}
\label{viewfinder-refine}
\begin{algorithmic}[1]
\Require transformation rules (P, F, G, D)
\State $P \qlet permutations$(transformation\_rules)
\ForAll{$p \in P$}
  \For {rule $\in p$}
   \State  $newchain \qlet$ \textsc{ApplyRule}(rule, $chain$, $t$)
   \If{$newchain$.\textsl{isEquivalent}($t$)}
     \State return $newchain$
   \EndIf
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\begin{itemize}
\item Mindist allows to look at the existence of shorter chain
first before exploring the longer chains

\item Why best first? Each iteration of the loser pile
keeps merging the chains cost up to $n$ way joins.
We do only two way of joins


\item cmerge is expensive so the cost grows very quickly.
A best first nature means you do not explode your space too much
because the remaining cost fo the minimum people is less than $m$.


\item Don't know there is a rewrite but have to look for  them all
to see which is the cheapest but we take advantage of the fact
that there are multiple opportunities for plumbing at different
targets, which means that if you find a valid rewrite at one target
it immediately bounds the search space of all the targets in the workflow.

\item Mindist allows the incremental exploration of the space in two place
a) Is it winner or loser?
b) Look for short rewrites if they exist
c) Grow the loser partial candidates slowly

\end{itemize}

\subsection{Artifacts}
We call a Materialized View that is created as the output of any query $q \in Q$ an artifact.  We make the assumption that this output is
always written to stable storage in the DFS.

We model an artifact in a minimalistic way as follows.  An artifact is considered to have 3 properties:
\begin{enumerate}
\item Attributes
\item Filters
\item Groupbys
\end{enumerate}


\end{comment}



\begin{comment}
Our system considers every operation as a UDF.
Given that our execution framework is a simple MR system, we identify the types of operations that are possible.
Table \ref{tab:mrops} shows these operations and indicates which phase (Map or Reduce) they can occur.
UDFs may apply any of the operations shown.
Clearly this framework limits the expressivity of UDFs.
Yet many complex UDFs such as ... can still be applied in this framework as shown in example X.
Thus the framework is sufficient for many analytics we consider.
An execution (MapReduce job) may apply filters,
apply projections,
create new attributes via transformations,
or perform aggregations to produce the result.
Given the allowable operations, a result can be modeled as a set of Attributes (\textsf{A}),
a set of filters (\textsf{F}), and group by attributes (\textsf{G}).
We consider \textsf{F} to contain conjunctions of simple selection predicates.
In this model, the result of a equijoin operation appears as an additional filter representing the join predicate.
A result is considered a materialized view in our system (a view extension).

Because UDFs can perform complicated transformations any derived attribute produced must contain
some metadata about itself.
Consequently each attribute has a \textit{signature}, which is a minimal form of provenance that captures the nature of the
view's direct input in terms of \textsf{A}, \textsf{F}, \textsf{G} along with some other small metadata such as the operation applied
(UDF name) to the input to produce the view.

This representation enables us to easily understand UDF as a grey box, rather than a black box.
It is considered to be grey since we don't really understand what the function actually does,
we only understand the label of the function and what the input and output look like.
This means that two identical functions with different labels will not appear identical to our model.
Or UDFs that may subsume each other will not be identified.
Our method is extensible toward a more fine-grained understanding of the function where some UDFs may become a white box.
This requires additional complexity while here we focus on the usefulness of our method
even on the level of understanding a UDF as a grey box.

We now define our grammar that is used by all UDFs.
All UDFs operations are described in this grammar.
A UDF takes at least one view as input and produces a view as output.
To understand a UDF as a grey box, each attribute created by a
UDF records the following metadata describing itself.
\begin{enumerate}
\item {\sf B} - the name of the UDF that produced the attribute
\item {\sf M} - a modifier argument given to the UDF (if any)
\item {\sf A} - the input attributes to the UDF
\item {\sf F} - the filters previously applied to the input
\item {\sf G} - the group-bys previously applied to the input
\end{enumerate}

The output of the UDF is a materialized view which is described
in terms of \textsf{A}, \textsf{F}, \textsf{G}.
The grammar of the UDF must describe the transformations from
{\sf B, M, A, F, G} to {\sf A, F, G}.
\end{comment}



==> old/Viewfinder-rewrite2.tex <==
\section{ViewFinder}\label{sec-viewfinder}

The key feature of $\VF{}$ is its $\ocost{}$ functionality
% that enables it to incrementally explore the the space of rewrites using
% the views in $V$.
%This functionality is used by $\WF{}$ to explore 
which is used by the $\WF{}$ to explore
the space in an incremental manner and prune unnecessary sub-spaces
as shown in Section~\ref{sec-solution-outline}.
% Thus we incorporate $\ocost{}$ with the traditional approach
% which consists of finding {\em complete} candidate views and enumerating
% rewrites for each candidate.
% As noted in Section~\ref{sec-problem-definition} rewriting queries
As noted earlier, rewriting queries
using views is known to be a hard problem.
Traditionally, methods for rewriting queries using views for the
class of SPJG queries use a two stage approach~\cite{Hale2001, Agra2000}.
The prune stage determines which views are \emph{relevant} to the query,
and among the relevant views those that contain
all the required join predicates  are termed as \emph{complete},
otherwise they are called {\em partial} solutions.
This is typically followed by a merge stage that joins the partial
solutions using all possible equijoin methods on all join orders to form
additional relevant views.
The algorithm repeats until only those views that are
useful for answering the query remain.

We take a similar approach in that we identify partial and
complete solutions, then follow with a merge phase.
The $\VF{}$ considers candidate views $C$ when 
searching for rewrite of a target.
$C$ includes views in $V$ as well as views
formed by ``merging'' views in $V$ using a
\textsc{Merge} function, which is an implementation of a 
standard view-merging procedure (e.g.,~\cite{Agra2000,Hale2001}).
Traditional approaches merge all partial solutions to create complete solutions,
and continues until no partial solutions remain.
This ``explodes'' the space of candidate views exponentially.
Our approach allows for a gradual explosion of the space as needed,
which results in far fewer candidates views from being considered.

% Here we will describe the functionality of the \VF{}, and later in
% Section~\ref{sec-best-first-workflow-rewrite} we
% will present the \WF{} which exploits the \VF's{} ability to incrementally examine
% the space of solutions for each target.
% However, the direct applicability of existing approach
% to our problem is limited.
With no early termination condition existing approaches 
would have explore the space exhaustively at all targets.
Thus we desire a rewriting algorithm  that can
enumerate the space and incrementally explore
only as much as required, frequently stopping
and resuming the search as requested by \WF.
% We note that while an equivalent rewrite for a target may exist,
% the \VF may never be asked to find it,
% as illustrated by Example~\ref{example-greedy-plumbing} for
% the case of the candidate view with cost 12 at $n_3$. 

%\subsection{V\fakesc{iew}F\fakesc{inder} Algorithm}
\subsection{Algorithm}

The $\VF{}$ is presented in Algorithm~\ref{alg-viewfinder}.
At a high level, the $\VF{}$ is {\em stateful} which
enables the $\WF$ to start, stop and resume the incremental searches at each target.
The $\VF{}$ maintains state using 
a priority queue of candidate views. % for each target.
The $\VF{}$ implements three functions {\sc Init}, {\sc Peek} and {\sc Refine} which 
we describe next.

The \Init{} function instantiates an instance of the $\VF{}$ 
with a $query$ which a logical representation of a target $W_i \in W$
and a set of materialized views $V$ present in the system.
Next, $query$ is assigned to $q$ and each view in $V$ is added to priority queue
using $\ocost(q,v)$ as the sorting key.
At the end of \Init{}, the candidate views in $\PQ$ includes only those views in $V$.

The $\Peek{}$ function is used by $\WF{}$ to obtain the $\ocost{}$ of the head item
in the $\PQ$.

The $\Refine{}$ function is invoked when $\WF{}$ asks the $\VF{}$
to examine the next candidate view.
At this stage, the $\VF{}$ pops the head item $v$ out of $\PQ$.
The $\VF{}$ then generates a set of new candidate views $M$
by merging $v$ with previously popped  candidate views (i.e., views in $Seen$),
thereby incrementally exploding the space of candidate views.
Note that $Seen$ contains candidate views that have an $\ocost{}$ 
less than or equal to that of $v$.
$M$ only retains those candidate  that are
not already in $Seen$, which are then inserted into $\PQ$.
% TODO: Need a proof for that statement
A property of $\ocost{}$ provided as a theorem later is that
the candidate views in $M$ have an
$\ocost{}$ that is greater than that of $v$ and hence none
of these views should have been examined before $v$.
This property enables a gradual explosion of the space of candidate views.
Then, $v$ is added to $Seen$.

If $v$ is guessed to be complete (described in Section~\ref{sec-guess-rewrite}),  
we try to find rewrites of $q$ using $v$ by invoking the $\RE$ function
      (described in Section~\ref{sec-rewrite-enumeration}).
Among the rewrites found by $\RE{}$,
the cheapest rewrite is returned to $\WF{}$ as the result.
% TODO: Do we need to talk about join ordering?


% The \VF{} finds a rewrite for a target in $W$ given a set of materialized views $V$.
% This problem is referred to as \emph{query} rewriting, hence our 
% input is a query $q$ representing the target, and $V$.
% Given our problem formulation, we require one instance of the \VF{} per target in $W$.
% The space of candidate views $C$ can be very large due to merging
% views in $V$. 
% Our approach allows for a gradual explosion of the space as needed.
% Here we will describe the functionality of the \VF{}, and later in
% Section~\ref{sec-best-first-workflow-rewrite} we
% will present the \WF{} which exploits the \VF's{} ability to incrementally examine
% the space of solutions for each target.
% The lower bound provided by $\ocost{}$ enables the \VF{} to explore the space
% incrementally, at every step examining any potentially lower-cost rewrites before exploding the
% space further to produce candidate views that have higher potential cost.

\begin{comment}
% Good text but got rid of it in the Alkis rewrite
Answering queries using views is a long-studied problem.
It is primarily considered in the context of data integration or data warehouse
design (query optimization)~\cite{Hale2001}.
Data integration is often interested in maximally-contained rewrites while
query optimization is concerned with equivalent rewrites.
Our interest is the latter.
The complexity of the problem is described with respect to the
expressivity of the languages used for both the queries
and the view definitions~\cite{Abit1998}.
Even when both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete
both for determining whether a rewrite exists~\cite{Levy1995} and
checking the correctness of a rewrite.
Checking the correctness of the rewrite is the same problem as
determining containment (i.e. $ Q_1 \subseteq Q_2$), which is
NP-complete~\cite{Chan1977} for conjunctive queries.
A \textit{complete} rewriting of $Q$ using $V$ is said to be one
that only uses $V$, and does not use any of the base relations.
Determining whether there is a complete rewriting of $Q$ using $V$
(again for the class of conjunctive queries) is NP-complete~\cite{Levy1995}.
Furthermore, when $Q$ and $V$ are disjunctions of conjunctive queries,
finding a complete rewriting is NP-complete~\cite{Levy1995}.
Producing a \textit{minimal} rewrite entails using the minimal number
of views in the rewrite such that no view can be removed
without invalidating the rewrite.
This problem is also NP-complete~\cite{Levy1995}.
We only consider complete rewrites, those using
the existing views, without extracting new views from the log.
\end{comment}

\begin{comment}
% CUT due to lack of space.
The reason we do not return to the log (i.e., base relation) is that
more and more views become materialized in the system as analysts
perform their data exploration and furthermore log extraction is expensive.
The rewrites are expressions in $L_R$ which may include
additional transformations on $V$ in order to produce an equivalent rewrite.
\end{comment}

\begin{comment}

\begin{enumerate}
\item {\bf Prune Step}:  Retain only those views that are relevant 
to the query (have the required attributes, have a mapping to the 
same base relations, logically-weaker selection and join predicates).

Find {\em all} relevant views $v$ to the query $q$.
Views that are not relevant to the query are pruned.

Determining a relevant view $v$ involves
(a) $v$ shares common base relations with $q$,
(b) $v$ must not have projected out any attributes required by $q$, and
(c) $v$ must contain a subset of the join predicates in $q$ and (d) must have
identical or logically weaker selection predicates.

The views in $V$ that pass the prune step are called {\em relevant} views.

Among the relevant views those that contain all the join predicates in $q$
are termed as \emph{complete}, otherwise they are called {\em partial} solutions.
%% Note that the {\em complete} solutions are added to the {\em winner} pile,whereas the partial solutions are added to the {\em loser} pile.
Next, a {\em  dominance} pruning is performed by comparing all pairs of relevant views, from each pair
discard the view with lower contribution or higher cost.

%%For all the complete solutions, it tries to find an equivalent rewrite using the views, which we term as {\em chain forming}.
% SJ: Need to figure out what the hardness result of "chain formation"

\item {\bf Merge Step}: Join all partial solutions using all
possible equijoin methods on all join orders to form
additional relevant views. Return to prune step.
\end{enumerate}
\end{comment}

\subsubsection{Determining Partial or Complete solutions}\label{sec-guess-rewrite}

To determine if a view $v$ is partial or complete with respect to a
query $q$, we take an optimistic approach.
This approach represents a \emph{guess} that a complete rewrite exists using $v$.
A guess requires the following necessary conditions
as described in~\cite{Hale2001} (SPJ) and~\cite{Gold2001} (SPJG)
that a view must satisfy to participate in a rewrite of $q$, 
although these conditions are not sufficient to
confirm the existence of an equivalent rewrite using $v$.

\begin{itemize}
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item $v$ contains all the attributes required by $q$; or contains all the 
    necessary attributes to produce those attributes in $q$ that are not in $v$
\item $v$ contains weaker selection predicates than $q$
\item $v$ is less aggregated than $q$
\end{enumerate}
\end{itemize}

The function $\complete(q,v)$ performs these checks and returns true if $v$
satisfies the properties i--iii with respect to $q$.
Note these conditions under-specify the requirements for
determining that a valid rewrite exists, thus a guess may
result in a false positive, but will never result in a false negative.

% The lower bound provided by $\ocost{}$ allows the \VF{} to search the space
% incrementally, exploring any potentially
% lower-cost rewrites first before exploding the
% space unnecessarily to find and enumerate them all.
%The $\VF{}$ takes as inputs
%a query $q$, the set of existing materialized views $V$,
%two values $d',d$, s.t., $d' < d$ and outputs an equivalent
%rewrite $r$ of $q$ using a set of views in $V$, such that
%$d' < \ocost(r) \leq d$ if $r$ exists.
%Note that $V$ is only required in the initialization step,
%and in subsequent invocations $d'$ is implicit in the sense that it records
%the value of $d$ from the previous invocation.


\begin{comment}
% SJ: Given that we now use Surajit Chaudhuri's method, this text is not needed 
%
The $\VF{}$ maintains a priority queue $\PQ$ which contains all candidate views.
The candidate views include those in $V$ as well as views
formed by ``merging'' of views in $V$.
To merge a pair of candidate views $v_1$ and $v_2$,
we consider all possible equi-join methods based on common keys,
as well as trying all possible subsets of join predicates that are present in $q$
which is similar to the approaches in~\cite{Agra2000,Hale2001}.
In~\cite{Hale2001} partial views are only considered for merging if they satisfy join
predicates in $q$, while~\cite{Agra2000} merges views to create parent
views that can answer the same or larger subset of queries
in the given workload than their constituent views (i.e, $v_1$ and $v_2$).
We adapt both approaches as a way of making partial views complete with respect to $q$.
As in~\cite{Agra2000}, we generate new views by a series of pair-wise merges.
This process is captured in the procedure $\merge(v_1, v_2)$, 
where $v_1$ and $v_2$ are candidate views
and the output is a new candidate view $v_{12}$.
Because the merging process adds exponentially more
views for consideration, we should avoid growing the space larger than necessary.
Thus we control the candidate generation process by merging a candidate view with those
candidates views that have a lesser $\ocost{}$.
The use of the $\PQ$ enables the merge process to be resumed later when the
$\VF{}$ is invoked in the next iteration, if it is needed.

While~\cite{Agra2000} only retains candidate views that the optimizer considers 
 useful for answering queries and their merge step only considers
merging based on the join condition specified in $p$,
we consider merging views when they share a common key.
The utility of merging views based on a common key can 
be seen from the following example.
Consider a query $q$ that requires the key $\{A,D\}$.
Suppose that $v_1$ contains key $\{A,B\}$, $v_2$ contains key $\{B,C\}$ and $v_3$ contains
key $\{C,D\}$.
A typical pruning step would discard $v_2$ as it does not contain any attributes
syntactically relevant to $q$.
We note that merging $v_1$ with $v_2$, followed by a merge with $v_3$ will obtain a superset
of keys needed by $q$.
This merged view is complete with respect to $q$.
\end{comment}


\begin{algorithm}[h!]
\caption{$\VF$\label{alg-viewfinder}}
{\small
\begin{algorithmic}[1]
\Function{\sc Init}{$query$, $V$}\label{alg-vf-init}
 \State Priority Queue $PQ$ \qlet $\emptyset$; $Seen$ \qlet $\emptyset$; Query $q$ 
  \State $q$ \qlet $query$
  \ForAll{$v \in V$}
     \State $PQ$.\texttt{add}($v$, $\ocost(q,v))$
  \EndFor
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Peek}{}\label{alg-vf-peek}
%\State \Return ($PQ$.\texttt{peek}().$\ocost$: $\infty$) ? 
\State {\bf if} $PQ$ is not empty {\bf return} $PQ$.\texttt{peek}().$\ocost$ {\bf else} $\infty$
%   \If{not $PQ$.\texttt{empty}()}
%   \State \Return $PQ$.\texttt{peek}().$\ocost$ 
%   \Else 
%   \State \Return $\infty$
%   \EndIf  
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Refine}{}\label{alg-vf-refine}
  \If{\texttt{not} $PQ$.\texttt{empty}()}
    \State $v$ \qlet $PQ$.\texttt{pop}()
    \State $M$ \qlet \merge($v$, $Seen$) \Comment{Discard from $M$ those in $Seen \cap M$}
    \ForAll{$v' \in M$}
      \State $PQ$.\texttt{add}($v'$, $\ocost(q,v')$)
    \EndFor
    \State $Seen$.\texttt{add}($v$)
    \If{\complete($q$, $v$)}
      \State \Return $\RE(q, v)$
    \EndIf
  \EndIf \\
  \Return {\sc null}
\EndFunction
\end{algorithmic}}
\end{algorithm}


\subsection{Rewrite Enumeration}\label{sec-rewrite-enumeration}

% Suppose that a candidate view $v$ is guessed to be complete.
% To determine if an equivalent rewrite exists requires finding at
% least one valid rewrite among all possible rewrites,
% is known to be a hard problem~\cite{Levy1995}.
In our system the \RE{} algorithm attempts to produce a valid rewrite
of a query using a view that is guessed to be complete.
% \RE{} takes as input a query $q$ and a view $v$ that is guessed to be complete
% and outputs a rewrite $r$ if one exists.
The rewrite returned represents the cheapest among
all possible equivalent rewrites of $q$ using $v$.
The cost of a rewrite is evaluated by the \cost{} function,
and corresponds to the cheapest execution \textit{plan} that
implements the rewrite.
Equivalence is determined by ensuring
that the rewrite and query contain the same attributes,
filters, and group-by.
%This type of equivalence testing is simple but effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%Although this type of equivalence testing may seem simple it is effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%We replace an SPJ+G expression with a single view.  as in GL2001


We enumerate equivalent rewrites of $q$ by applying {\em compensations}~\cite{Zaha2000}
to a guessed to be complete view $v$ using $L_R$.
%A transformational rule is a UDF in the system that may
%modify any set of the properties in our UDF model
%which are attributes, filters, and groupbys.
% Given the complex interactions possible 
% for any arbitrary set of $k$ rules in $L_R$,
% it may require generating all possible rewrites of $r$ using $L_R$
% before identifying an equivalent rewrite if one exists.
We do this by generating all permutations of required compensations and
testing for equivalence, which
% which can also include multiple applications of the same rule.
amounts to a brute force enumeration of all possible rewrites given $L_R$.
This makes case for the system to keep $|L_R|$ small.
When $L_R$ is restricted to a known, fixed 
set of operators it may suffice to examine a polynomial number of 
rewrites attempts, as in~\cite{Grum2003} for the specific case 
of simple aggregations involving group-bys.
Such approaches are not applicable to our case as 
the system should have the flexibility of extending $L_R$ with 
UDFs from $L_W$ when it results in overall system benefit.

Given the computational cost of finding valid rewrites,
$\WF{}$ limits the invocation of $\RE{}$ algorithm using two strategies.
% we employ the following two strategies.
First,  we avoid having to apply $\RE{}$ on every candidate view making
a guess for the completeness of a view based
on the three properties described earlier.
Second, we delay the application of $\RE$ to every complete view 
by determining a lower bound on the cost of a rewrite using $v$ should one exist.
For the lower bound we use the $\ocost$, which is described in the next section.
% The goal of guessing completeness and estimating a lower bound is
% to quickly distinguish between potentially low cost rewrite from those with higher cost.

\subsection{Determining O\fakesc{pt}C\fakesc{ost}}\label{sec-ocost}
The utility of  a lower bound we develop in this section enables
the enumeration of the candidate views based their potential 
to provide a low cost rewrite.
% Our expectation of the lower bound is only that it should be able to quickly distinguish between 
% candidate views with potential to produce cheap versus very expensive rewrites.
% Given a candidate view $v$ and a query $q$,
% we wish to determine a lower bound on the cost of \textit{any} plan yielded by
% an equivalent rewrite of $q$ using $v$ if one exists without enumerating all possible rewrites,
% checking for equivalence and examining their plan costs.
% We refer to this lower bound as the optimistic cost, or \ocost.
\ocost relies on the non-subsumable cost property of the $\cost{}$ function
to arrive at a lower-bound.

Given that $v$ is guessed to be complete with respect to $q$, 
a set difference between the attributes, filters and group-bys representation 
of $q$ and $v$ is referred to as the {\em fix}.
Fix denotes a hypothetical local function that can
transform $v$'s representation into $q$'s.
Note that a UDF containing such a local function may not really exist.
We have to invoke $\RE{}$ which produces a rewrite
containing compensations from $L_R$.
The composition of the local functions in the compensation
transforms $v$'s representation to $q$.
%\ocost{} uses the attributes, filters, and group-by representation 
%of $q$ and $v$ to take a set difference between each of these properties.
%This denotes a minimum set of non-subsumable operations
%by Definition~\ref{definition-non-subsumable-property}
%needed to transform $v$'s representation into $q$'s.
Finally, note that the existence of fix guarantee that $v$ will result in a valid rewrite 
for the same reason that  guessed to be complete can result in a false positive.
Both assume that the required
compensation operations can be applied independently of each other to $v$.
% resolve the differences  in the attributes, filters, and group-bys of $q$ and $v$.
%compensate these properties independently.
% is possible to compensate $v$ using operations in $L_r$
%independently of the others.

%We refer to this set as the {\em fix} of $v$ with respect to $q$.
%The non-subsumable property allows \ocost{} 
%to consider operations in the fix as independent of one another,
%although they can still affect each other's cost.
% \ocost{} then returns the sum of the create cost $c'_1$, access cost $c'_2$, and the
% minimum operation cost $c'_3$ in the fix as the
% lower bound on the cost of \textit{any} plan.

%If $v$ is not materialized in the process of rewriting a query and then any
%necessary compensation is applied. 
We now describe a $\ocost{}$ function with the two properties 
that it is a lower bound on the cost of \textit{any} plan returned by $\RE(q,v)$
and inexpensive to compute.
If $v$ is a materialized view then $c_1$ is equal to the cost of accessing $v$. 
Otherwise, if $v$ results from the merging of views, 
then $c_1$ is the total cost to access the constituent views of $v$. 
% We denote $c_1$ as the cost of accessing all the constituent views in $v$ (i.e., access cost).
We denote $c_2$ as the cost of merging the constituent views in $v$ (i.e., creation cost)
if $v$ is already not materialized, else $c_2$ = 0 if it is already materialized.
We denote $c_3$ as the cost of applying the least expensive operation in the fix on $v$,
obtained by invoking the \cost{} to obtain the cost of 
performing each of the operations in the fix on $v$.
$c_3$ is obtained by $\min(\cost(x, v))$ such that $x$ is an operation in {\em fix}.

% If a plan of the rewrite using $v$, materializes $v$ before applying
% all the applicable compensation, then 
The \ocost{} of $v$ with respect to $q$ is given
by: $c = c_1 + c_2 + c_3$, where $c$ is less than the cost of any
plan of the rewrite using $v$.
If $v$ is partial with respect to $q$,
then $c_3 = 0$ since no compensation should be applied.

Suppose that the optimizer can generate plans where some of compensations
can be pushed into the candidate view $v$ before materializing it.
In this case, $\ocost{}$ can provide a weaker lower bound
as it can only consider the cost ($c_1$) of accessing all the constituent views of $v$ 
plus the minimum cost $c'_3$ of applying the least expensive operation 
in the fix on any constituent views of $v$ or on any intermediate view
that can be created in the process of creating $v$.
If $v$ is partial with respect to $q$, then $\ocost{}$ only includes $c_1$.

We provide the following proof sketch to capture the correctness of the 
$\ocost{}$ function.

\begin{comment}
%\ocost takes an optimistic approach in determining the minimum possible plan cost.
If a candidate view $v$ is not yet materialized (i.e., to be created by merging),
$\RE{}$ might consider
materializing it first before applying all necessary compensation.
%If $v$ is not materialized in the process of rewriting a query and then any
%neccessary compensation is applied. 
Then, intuitively it can be seen that any plan yielded by an equivalent rewrite would incur at
the least the sum of
the cost $c_1$ for accessing all the constituent views in $v$ (i.e., access cost),
the cost $c_2$ for materializing any new views it requires (i.e., creation cost), and
the cost $c_3$ 
of applying the least expensive compensation operation on the view $v$.
\ocost{} invokes \cost{} to obtain the cost of 
performing each of the operations in the fix on $v$.
It chooses the least expensive operation in the fix
as the third component $c_3$ of the \ocost, where
$c_3$ is given by $\min(\cost(x, v))$ such that
$x$ is an operation in {\em fix}.
We define \ocost{} as $c = c_1 + c_2 + c_3$, which has the property 
that it is a lower bound on the cost of \textit{any} plan returned by $\RE(q,v)$
and inexpensive to compute.
If $v$ is partial (i.e., not guessed to be complete) with respect to $q$,
then $c_3 = 0$ since no compensation should be applied.
\end{comment}

%Note that if using the push-down approach, 
%when the view is partial then \ocost{} is only $c'_1$,
%since push-down predicates may change the join ordering.
%Further details  of this \ocost{} function 
%and our proof of the lower bound property when considering predicate pushdown is 
%omitted here due to lack of space.


\begin{comment}
There are certain benefits to both approaches.
The choice to create $v$ is similar to the approach that a view recommender~\cite{Agra2000} might take,
while pushing down predicates into $v$ to create $v'$ is an approach that a query optimizer may take for
answering a single query $q$.
One way to think about this is that $v$ is a recommended view by the $\VF{}$ and here we
decide to piggyback its creation as a part of execution of query $q$.
Given the use case of the system, we prefer this approach as we
wish for the artifacts created (i.e., $v$) as part of answering $q$ to
be as beneficial as possible to the subsequent queries by future users.

The $\VF{}$ could be modified to support predicate pushdown by
modifying $\ocost$ to order partial views by their access cost for $v$ (i.e., $c'_1$).
The pushdown predicates can potentially change the cost of all the joins and their orderings.
\end{comment}


% RETAIN THE REMAINDER OF THIS PROOF HERE. -- REFERS TO Appendix
% An $\ocost{}$ function that considers predicate pushdown 
% is given in Appendix~\ref{appendix-pushdown}.

\input{scenario-no-plug}

\begin{theorem}
$c$ is a lower-bound on on the cost of \textit{any} plan yielded by
an equivalent rewrite $r$ of $q$ using $v$ if one exists.
\end{theorem}

\begin{proof}
Any plan of the rewrite $r$ will have to access all the constituent views in $v$
and materialize it. So, $c_1$ and $c_2$ is common to $\ocost{}$
and the cost of any plan of $r$.

In order to find the lowest cost $r$, $\RE{}$ applies all 
permutations of compensation operations to achieve 
an equivalent rewrite.
% that achieves the same
% effect as the fix, although each operation in the compensations
% can ``cover'' more than one operations in fix.
% The end-to-transformation produced by the compensation 
% is the same as that denoted by fix, regardless of whether
% there is a one-to-one correspondence between the operators in the compensation
% and fix, or a single operation in the compensation covers all of fix.
Regardless of how many operations are used in the compensation,
by Definition~\ref{definition-non-subsumable-property}, the cost
of applying the compensations has to be at least as expensive as 
the cheapest operation $c_3$ in the fix.

Next we consider the $\ocost{}$ function 
for the case involving push-down of compensations.
For this case, both the ordering of the merges of the
constituent views of $v$ as well as the applicable compensations are as yet unknown.
Our lower-bound holds as it does not make any assumptions about
the ordering of the constituent views in $v$ (i.e., by using $c_1$) as well as 
the position of any compensation operator in any plan of $r$ (i.e., $c'_3$) . \qed
\end{proof}

\begin{comment}
Base Case: Let the fix be denoted by the operators $x$, $y$, $z$,
such that $op^* = z$ is the cheapest operator in fix.
A rewrite $r$  using {\em fix} can
apply operators in the following sequence:
a) apply one operator followed by another or both,
b) apply two operators (e.g., $xz$) followed by a third
operator (e.g., $y$), or
c) apply operators $xyz$ all at once.
For case a) the cost of $r$ is greater than or equal to
either $\cost(x,v)$ or $\cost(y,v)$  or $\cost(z,v)$.
For case b) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(z,v))$ if the first operation
is given by $xz$.
For case c) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$.
As $r^*$ represents the lowest cost rewrite across
all rewrites denoted by the three cases, it is bounded by:
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$, which proves
the base case of {\em fix} with 3 operators.

Induction Step:
Let $y$ be the cheapest operation in the set denoted by $\mbox{\em fix}-x$, such that
$\cost(r^*,v) \geq \cost(y,v)$ where $r^*$ corresponds
to lowest cost rewrite on $\mbox{\em fix}-x$.
In other words, the cost of $r^*$ is at least the cost of applying
the cheapest operator in $\mbox{\em fix} -x$.

Add $x$ back to the {\em fix}.
Now, let $r^*$ be the lowest cost rewrite
using {\em fix}.
Suppose that $r^*$ is composed of sets operators $p_1, p_2 \cdots p_k$, such that
$p_1 \cup p_2 \cdots \cup p_k = \mbox{\em fix}$ and
the output of $p_1$ forms the input to $p_2$ and so on.
Then, $\cost(r^*,v) = \cost(p_1, v) + \cost(p_2, v|p_1) + \cdots + \cost(p_k, v|p_1\cdots{}p_{k-1})$,
where $v|p_1$ means that operators in $p_1$ have been applied to $v$.
This means that $\cost(r^*,v) \geq \cost(p_1, v)$ given that $\cost{}$ is always non-negative.
The lowest value of $\cost(p_1,v)$ occurs when $op^*$ is present in
$p_1$ possibly along with other operators in the {\em fix}.
Thus, $op^*$ must either be $y$ which was the cheapest operator in $\mbox{\em fix} - x$
or $op^*$ must equal to $x$.
Then, $\cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$.
Finally, $\cost(r^*,v) \geq \cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$. \qed
\end{comment}


\begin{comment}
\begin{theorem}
$c'$ is a lower-bound on on the cost of \textit{any} plan yielded by
an equivalent rewrite of $q$ using $v$ if one exists.
\end{theorem}

\begin{proof}
Let $c$ be the minimum cost plan generated by the $\RE(q,v)$ corresponding
to the rewrite $r$.
$c$ is composed of
the cost $c_1$ for accessing all the views, and
the cost $c_2$ for materializing any new views it requires,
the cost $c_3$ for least expensive ordering of transformation 
rules in $L_R$ applied to $v$.
As $v$ is guessed to be complete for the query $q$,
both $\RE$ and $\ocost$ use $\cost$ to obtain the cost to create and access $v$,
then $c_1 = c'_1$ and $c_2 = c'_2$.

In order to find the lowest cost $r$, $\RE{}$ will have
to enumerate all permutations of rules in $L_R$ required
to achieve the fix.
If \RE{} finds a rewrite, $r$ will have covered all operations in fix,
choosing the cheapest rewrite found to be $c_3$.
$\ocost{}$ uses \cost{} once per each operation in fix
choosing the cheapest as $c'_3$.
As $c'_1$ and $c'_2$ are common to both $c$ and $c'$,
it suffices to show that $c_3 \geq c'_3$.

Recall that \emph{fix} is made up of non-subsumable operations.
A property of two non-subsumable operations as mentioned
earlier in Definition~\ref{definition-non-subsumable-property} is that:
$\cost(xy, D) \geq \min(\cost(x, D),
\cost(y, D))$, where $v$ is an instance of a database $D$, and
$x$, $y$ are operators in fix, and $xy$ performs both $x$ and $y$.

By induction we can show that the cost of the cheapest
rewrite that applies  the fix to $v$
is greater than or equal to $\cost(op^*, v)$, 
where $op^* \in \mbox{\em fix}$
and is the cheapest operator present in the {\em fix} but we
omit the remainder of the induction for lack of space.\qed

-- RETAIN THE REMAINDER OF THIS PROOF HERE. -- 
Base Case: Let the fix be denoted by the operators $x$, $y$, $z$,
such that $op^* = z$ is the cheapest operator in fix.
A rewrite $r$  using {\em fix} can
apply operators in the following sequence:
a) apply one operator followed by another or both,
b) apply two operators (e.g., $xz$) followed by a third
operator (e.g., $y$), or
c) apply operators $xyz$ all at once.
For case a) the cost of $r$ is greater than or equal to
either $\cost(x,v)$ or $\cost(y,v)$  or $\cost(z,v)$.
For case b) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(z,v))$ if the first operation
is given by $xz$.
For case c) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$.
As $r^*$ represents the lowest cost rewrite across
all rewrites denoted by the three cases, it is bounded by:
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$, which proves
the base case of {\em fix} with 3 operators.

Induction Step:
Let $y$ be the cheapest operation in the set denoted by $\mbox{\em fix}-x$, such that
$\cost(r^*,v) \geq \cost(y,v)$ where $r^*$ corresponds
to lowest cost rewrite on $\mbox{\em fix}-x$.
In other words, the cost of $r^*$ is at least the cost of applying
the cheapest operator in $\mbox{\em fix} -x$.

Add $x$ back to the {\em fix}.
Now, let $r^*$ be the lowest cost rewrite
using {\em fix}.
Suppose that $r^*$ is composed of sets operators $p_1, p_2 \cdots p_k$, such that
$p_1 \cup p_2 \cdots \cup p_k = \mbox{\em fix}$ and
the output of $p_1$ forms the input to $p_2$ and so on.
Then, $\cost(r^*,v) = \cost(p_1, v) + \cost(p_2, v|p_1) + \cdots + \cost(p_k, v|p_1\cdots{}p_{k-1})$,
where $v|p_1$ means that operators in $p_1$ have been applied to $v$.
This means that $\cost(r^*,v) \geq \cost(p_1, v)$ given that $\cost{}$ is always non-negative.
The lowest value of $\cost(p_1,v)$ occurs when $op^*$ is present in
$p_1$ possibly along with other operators in the {\em fix}.
Thus, $op^*$ must either be $y$ which was the cheapest operator in $\mbox{\em fix} - x$
or $op^*$ must equal to $x$.
Then, $\cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$.
Finally, $\cost(r^*,v) \geq \cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$. \qed
\end{proof}
\end{comment}

%The $\ocost{}$ does not cause the algorithm to lose its optimality property,
%regardless of considering an even larger (or pruned)
%rewrite space  than the one we consider here.


\begin{comment}
The lower bound provided by our $\ocost{}$ function could be tightened if we are
willing to commit to a particular execution environment and a specific query optimizer.
For example in an MR environment with a Hive query processor,
given the set of operations in the fix, one could
estimate the minimum number of maps, reduces, and jobs it would take to
apply all operations in fix to $v$.
Such an approach requires intimate knowledge of a specific system,
and thus loses the desired generality of a lower bound estimator.
\end{comment}

%Finally, we provide the following lemma describing the $\ocost{}$ property
%for any new candidate view created in $M$ during Algorithm~\ref{alg-viewfinder}.

\begin{comment}
The following theorem describes the $\ocost{}$ property for newly
merged candidates in $M$.
This enables Algorithm~\ref{alg-viewfinder}
to generate candidate views as needed to avoid a pre-explosion
of the space of all candidates.

\begin{theorem}
The $\ocost{}$ of every candidate view in $M$ that is not in $Seen$
is greater than or equal to the $\ocost{}$ of $v$.
\end{theorem}
\begin{proof}
The proof sketch is as follows. The theorem is trivially true for 
$v \in V$ as all candidate views in $M$ cannot be in $Seen$
and have $\ocost$ greater than $v$. 
If $v \notin V$, it is sufficient to point out
that all constituent views of $v$ are already in $Seen$
since they must have had $\ocost{}$ lesser or equal to $v$
Hence all candidate views in $M$ with $\ocost{}$ smaller than $v$ are
 already in $Seen$, and those with $\ocost{}$ greater than $v$ will be added to $PQ$
if they are not already in $PQ$.
 %all the 
%candidate views in $M$ are already present in $Seen$ if smaller, or if greater,
%are still in $\PQ$.
\end{proof}
\end{comment}

\begin{comment}
% RETAIN THE REMAINDER OF THIS PROOF HERE.
\begin{proof}
Suppose that $v'$ is a new candidate  that is created by merging $v$ with $Seen$.
Then we need only consider the case of $v$ being a base view or a composite view.
If $v$ is a base view (i.e., already materialized), then the $\ocost{}$ of $v'$  cannot be
less than $v$ as $\ocost(v)$ only considers its access cost, while $\ocost(v')$
is at least the cost of accessing $v$ as well as accessing the other candidate view that $v$ is joining with.
If $v$ is a composite view (i.e., $v$ is composed of multiple base views),
then the $\ocost{}$ of $v'$ cannot be less than $v$.
To show that by contradiction,
consider the case where $v'$ is not in $Seen$
and $v'$has a lesser $\ocost{}$ than $v$.
As $v$ is a composite view, then all of its constituent views would already
have been joined with all the candidate views in $Seen$.
Thus, $v'$ must already have been created.
If $v'$ has a lesser $\ocost{}$ than $v$,
it would have already been popped out of $\PQ$ and in $Seen$ before we got to $v$.
\end{proof}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}


\begin{itemize}
\item Two queries $Q_1$, $Q_2$
are said to be {\em equivalent} if $Q_1 \subseteq Q_2$ and $Q_2 \subseteq Q_1$.
From a query answering perspective,
the set of tuples in the result set of $Q_1$ are identical
to the set of tuples in the result set of $Q_2$.
To determine if an equivalent rewriting using views exists has been already
shown to be in NP even for the class of conjunctive queries~\cite{Hale01}.

\item A query $Q_1$ is said to be {\em contained } by $Q_2$
if $Q_1 \subseteq Q_2$.
From a query answering perspective,
all the tuples in the result set of $Q_1$ are contained in
the result set of $Q_2$, although the result set of $Q_2$ can contain additional
tuples that is not present in the result set of $Q_1$.
The problem finding contained rewriting is also known to NP-complete
even for conjunctive queries~\cite{Hale01-18}.

\end{itemize}

\item A candidate $c$ is said to be {\em complete} with respect to a $Q$ iff $c$ has
has a superset of the attributes and a subset of the filters and
superset of the groupby keys.
If there are attributes in $Q$ that are not present in $c$, $c$ has
the necessary ingredients (i.e., attributes) to obtain $Q$.
Of course, even if $c$ is complete,  it does not mean that
there exists an equivalent rewrite of $Q$ using $c$.
Thus, this provides a necessary but not sufficient
condition that equivalent rewrite exists.
The sufficient condition is when an equivalent
rewrite of $Q$ using $c$ exists.

\item We provide a set of $k$ transformational rules for
query rewriting using a candidate $c$. We call the
rewrite of complete candidate $c$ to a target $t$ using
our transformational rules a {\em chain}.

\item There are three classes of transformational rules that
we allow in the system.



\begin{itemize}
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item Rules that transform \{A\}, \{F\}, \text{or} \{G\}
\item Rules that transform \{A,F\}, \{F, G\}, \text{or} \{A, G\}
\item Rules that transform \{A, F, G\}
\end{enumerate}
\end{itemize}
\renewcommand{\labelenumi}{\theenumi}


% SJ: Let us add an example here
\item We have 4 transformation rules in our system:
\begin{enumerate}
\item $P$ \textendash Project (class \textsl{i})
\item $F$ \textendash Filter (class \textsl{i})
\item $G$ \textendash Groupby (class \textsl{i} and \textsl{ii})
\item $D$ \textendash Derived (class \textsl{i}, \textsl{ii}, \textsl{iii})
\end{enumerate}

In our $\MinDist$ function presented later, we make the assumption
that each rule can be applied independently.
Furthermore, our algorithm (described later) makes the assumption that the
 Filter rule applies all missing filters, one at a time before completing.
This prevents a large explosion of rule permutations
to apply when searching for a valid rewrite.  However, it presents a limitation on the
ability of our algorithm to find a successful rewrite if one exists.
It may be that no valid rewrite exists using a permutation
of these 4 rules, but one might exist if we consider each missing filter a separate
application of our $F$ transformation rule and thus could produce a successful rewrite such as
$F \rightarrow G \rightarrow F$ whereas due to our restriction of applying all missing filters
with the  $F$ rule before moving to another rule would not be able to produce such a re-write.

The \emph{Derived} rule allows for easy extensions, which is useful for attributes
created by UDFs that can easily be manipulated into other attributes.  For instance, one could add
a derivation that transforms lat-lon into a grid, or positive sentiment with a scoring value of
0.5 to 0.6, or word-count into (approximate) character-count.  Currently we have implemented
several derived attr transformations such as Groupby stats...

\item Determining if a solution $c$ is {\em complete} is  NP-hard
as it involves enumerating all possible chains using the transformation
rules

\item If a candidate is complete we can ``guess''
the minimum number of
transformational rules that go into the chain.
It is minimum ``guess'' as it based on the necessary
condition but not the sufficient condition, so no valid
chain may exist.

\item Why we cannot directly apply the traditional view finding:
  \begin{itemize}
  \item Discarding the non-relevant views using common base relations is not an effective pruning strategy as all queries are posed on a small set of logs, thus many views have the same base relation, a log.
  \end{itemize}
\end{itemize}

\subsection{View Finding Algorithm}

\begin{itemize}

\item Idea of a guess or mindist of a candidate to a target.
\begin{enumerate}
\item Also determine (optimistic guess) complete (winners) vs. partial candidates (losers)
\item Helps prune away the space quickly
\end{enumerate}

\item Describe chain data structure
\begin{enumerate}
\item Series of cmerged or joined candidates, where joined candidates
are restricted to those join predicates that appears in $t$
\item cmerge are keyed equijoins between candidates that shares
common keys
\item joins are equi across different keys or non-keys
\end{enumerate}

\item How to determine mindist?
\item mindist(chain c, t)
\begin{enumerate}
\item Really quick computation
\item Committed cost(c) + guess\_remaining\_cost(c.tail, t)
\item Decouples search from distance computation by assuming independence
\item Magical UDF
\item Claim: Guess is always <= actual cost
\item Finite mindist does not mean existence of chain which
is known to be NP-hard.. (because necessary condition only)
\end{enumerate}

\end{itemize}

Because we explore the solution space incrementally using our MINDIST, we
initialize the viewfinder by registering a target view and a set of candidate
views as follows in Algorithm \ref{viewfinderinit}:

\begin{algorithm}
\caption{ $\VF$-\textsc{initialize}($t$, $C$)}
\label{viewfinder-init}
\begin{algorithmic}[1]
\Require target $t$, candidate pool $C$ % some input
\State {Initialize WinnersPriorityQ, LosersPriorityQ}
\ForAll{$c \in C$}
  \State chain $c' \Leftarrow c$
  \State $d \qlet \MinDist(c', t)$
  \If{$d$ is $\infty$}
    \State LosersPQ.add($c'$, $d$)
  \Else
    \State WinnersPQ.add($c'$, $d$)
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\caption{ $\VF$($t$,\textit{MinCost})}
\label{viewfinder}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ
\State \textsc{mergeables}.\textit{clear()} \\
\Comment {\scriptsize Grow candidate space by merging all (partial view) pairs until the \textsc{committed\_cost} of all Losers is greater than the requested MinCost \normalsize}
\State $m \qlet $ \textit{MinCost}
\While{LosersPQ.peek().committed\_cost $ < m$}
  \State \textsc{mergeables}.\textit{add}( LosersPQ.pop() )
\EndWhile
\State \viewfinderCMerge(\textsc{mergeables})
\While{$ \MinDist$ (Winners.peek()$, t) < m$}
  \State $chain$ $\qlet$ Winners.pop()
  \State   \answer $\qlet$ \viewfinderRefine($chain$, $t$)
  \If {\answer}
    \State $\result$.\textit{add}($\ans$)
  \EndIf
\EndWhile
\State return $\result $

\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{ \viewfinderCMerge(\textsc{mergeables}) }
\label{viewfinder-cmerge}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ \\
\Comment \scriptsize attempt to merge all pairs of views, join order is not considered here \normalsize \\
\Comment \scriptsize This is a keyed equi-join \normalsize
\ForAll{$i \in $ \textsc{mergeables}}
	\ForAll{$j \in $ \textsc{mergeables}}
	  \State $tmp \qlet$\textsl{ColumnMerge}($chain_i$, $chain_j$)
	  \If{$tmp$}
	    \State $newchain \qlet chain_i + chain_j$
	    \State $d \qlet \MinDist(newchain, t)$
	    \State $totalDist \qlet d + newchain$.\textsc{committed\_cost}
        \If{$d$ is $\infty$}
          \State LosersPQ.add($newchain$, $totalDist$)
        \Else
          \State WinnersPQ.add($newchain$,$totalDist$)
        \EndIf
      \EndIf
	\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{ \viewfinderRefine($chain$, $t$)}
\label{viewfinder-refine}
\begin{algorithmic}[1]
\Require transformation rules (P, F, G, D)
\State $P \qlet permutations$(transformation\_rules)
\ForAll{$p \in P$}
  \For {rule $\in p$}
   \State  $newchain \qlet$ \textsc{ApplyRule}(rule, $chain$, $t$)
   \If{$newchain$.\textsl{isEquivalent}($t$)}
     \State return $newchain$
   \EndIf
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\begin{itemize}
\item Mindist allows to look at the existence of shorter chain
first before exploring the longer chains

\item Why best first? Each iteration of the loser pile
keeps merging the chains cost up to $n$ way joins.
We do only two way of joins


\item cmerge is expensive so the cost grows very quickly.
A best first nature means you do not explode your space too much
because the remaining cost fo the minimum people is less than $m$.


\item Don't know there is a rewrite but have to look for  them all
to see which is the cheapest but we take advantage of the fact
that there are multiple opportunities for plumbing at different
targets, which means that if you find a valid rewrite at one target
it immediately bounds the search space of all the targets in the workflow.

\item Mindist allows the incremental exploration of the space in two place
a) Is it winner or loser?
b) Look for short rewrites if they exist
c) Grow the loser partial candidates slowly

\end{itemize}

\subsection{Artifacts}
We call a Materialized View that is created as the output of any query $q \in Q$ an artifact.  We make the assumption that this output is
always written to stable storage in the DFS.

We model an artifact in a minimalistic way as follows.  An artifact is considered to have 3 properties:
\begin{enumerate}
\item Attributes
\item Filters
\item Groupbys
\end{enumerate}


\end{comment}



\begin{comment}
Our system considers every operation as a UDF.
Given that our execution framework is a simple MR system, we identify the types of operations that are possible.
Table \ref{tab:mrops} shows these operations and indicates which phase (Map or Reduce) they can occur.
UDFs may apply any of the operations shown.
Clearly this framework limits the expressivity of UDFs.
Yet many complex UDFs such as ... can still be applied in this framework as shown in example X.
Thus the framework is sufficient for many analytics we consider.
An execution (MapReduce job) may apply filters,
apply projections,
create new attributes via transformations,
or perform aggregations to produce the result.
Given the allowable operations, a result can be modeled as a set of Attributes (\textsf{A}),
a set of filters (\textsf{F}), and group by attributes (\textsf{G}).
We consider \textsf{F} to contain conjunctions of simple selection predicates.
In this model, the result of a equijoin operation appears as an additional filter representing the join predicate.
A result is considered a materialized view in our system (a view extension).

Because UDFs can perform complicated transformations any derived attribute produced must contain
some metadata about itself.
Consequently each attribute has a \textit{signature}, which is a minimal form of provenance that captures the nature of the
view's direct input in terms of \textsf{A}, \textsf{F}, \textsf{G} along with some other small metadata such as the operation applied
(UDF name) to the input to produce the view.

This representation enables us to easily understand UDF as a grey box, rather than a black box.
It is considered to be grey since we don't really understand what the function actually does,
we only understand the label of the function and what the input and output look like.
This means that two identical functions with different labels will not appear identical to our model.
Or UDFs that may subsume each other will not be identified.
Our method is extensible toward a more fine-grained understanding of the function where some UDFs may become a white box.
This requires additional complexity while here we focus on the usefulness of our method
even on the level of understanding a UDF as a grey box.

We now define our grammar that is used by all UDFs.
All UDFs operations are described in this grammar.
A UDF takes at least one view as input and produces a view as output.
To understand a UDF as a grey box, each attribute created by a
UDF records the following metadata describing itself.
\begin{enumerate}
\item {\sf B} - the name of the UDF that produced the attribute
\item {\sf M} - a modifier argument given to the UDF (if any)
\item {\sf A} - the input attributes to the UDF
\item {\sf F} - the filters previously applied to the input
\item {\sf G} - the group-bys previously applied to the input
\end{enumerate}

The output of the UDF is a materialized view which is described
in terms of \textsf{A}, \textsf{F}, \textsf{G}.
The grammar of the UDF must describe the transformations from
{\sf B, M, A, F, G} to {\sf A, F, G}.
\end{comment}



==> old/Viewfinder-rewrite3.tex <==
\section{ViewFinder}\label{sec-viewfinder}

The key feature of $\VF{}$ is its $\ocost{}$ functionality
% that enables it to incrementally explore the the space of rewrites using
% the views in $V$.
%This functionality is used by $\WF{}$ to explore 
which is used by the $\WF{}$ to explore
the space in an incremental manner and prune unnecessary sub-spaces
as shown in Section~\ref{sec-solution-outline}.
% Thus we incorporate $\ocost{}$ with the traditional approach
% which consists of finding {\em complete} candidate views and enumerating
% rewrites for each candidate.
% As noted in Section~\ref{sec-problem-definition} rewriting queries
As noted earlier, rewriting queries
using views is known to be a hard problem.
Traditionally, methods for rewriting queries using views for the
class of SPJG queries use a two stage approach~\cite{Hale2001, Agra2000}.
The prune stage determines which views are \emph{relevant} to the query,
and among the relevant views those that contain
all the required join predicates  are termed as \emph{complete},
otherwise they are called {\em partial} solutions.
This is typically followed by a merge stage that joins the partial
solutions using all possible equijoin methods on all join orders to form
additional relevant views.
The algorithm repeats until only those views that are
useful for answering the query remain.

We take a similar approach in that we identify partial and
complete solutions, then follow with a merge phase.
The $\VF{}$ considers candidate views $C$ when 
searching for rewrite of a target.
$C$ includes views in $V$ as well as views
formed by ``merging'' views in $V$ using a
\textsc{Merge} function, which is an implementation of a 
standard view-merging procedure (e.g.,~\cite{Agra2000,Hale2001}).
Traditional approaches merge all partial solutions to create complete solutions,
and continues until no partial solutions remain.
This ``explodes'' the space of candidate views exponentially.
Our approach allows for a gradual explosion of the space as needed,
which results in far fewer candidates views from being considered.

% Here we will describe the functionality of the \VF{}, and later in
% Section~\ref{sec-best-first-workflow-rewrite} we
% will present the \WF{} which exploits the \VF's{} ability to incrementally examine
% the space of solutions for each target.
% However, the direct applicability of existing approach
% to our problem is limited.
With no early termination condition existing approaches 
would have explore the space exhaustively at all targets.
Thus we desire a rewriting algorithm  that can
enumerate the space and incrementally explore
only as much as required, frequently stopping
and resuming the search as requested by \WF.
% We note that while an equivalent rewrite for a target may exist,
% the \VF may never be asked to find it,
% as illustrated by Example~\ref{example-greedy-plumbing} for
% the case of the candidate view with cost 12 at $n_3$. 

%\subsection{V\fakesc{iew}F\fakesc{inder} Algorithm}
\subsection{Algorithm}

The $\VF{}$ is presented in Algorithm~\ref{alg-viewfinder}.
At a high level, the $\VF{}$ is {\em stateful} which
enables the $\WF$ to start, stop and resume the incremental searches at each target.
The $\VF{}$ maintains state using 
a priority queue of candidate views. % for each target.
The $\VF{}$ implements three functions {\sc Init}, {\sc Peek} and {\sc Refine} which 
we describe next.

The \Init{} function instantiates an instance of the $\VF{}$ 
with a $query$ which a logical representation of a target $W_i \in W$
and a set of materialized views $V$ present in the system.
Next, $query$ is assigned to $q$ and each view in $V$ is added to priority queue
using $\ocost(q,v)$ as the sorting key.
At the end of \Init{}, the candidate views in $\PQ$ includes only those views in $V$.

The $\Peek{}$ function is used by $\WF{}$ to obtain the $\ocost{}$ of the head item
in the $\PQ$.

The $\Refine{}$ function is invoked when $\WF{}$ asks the $\VF{}$
to examine the next candidate view.
At this stage, the $\VF{}$ pops the head item $v$ out of $\PQ$.
The $\VF{}$ then generates a set of new candidate views $M$
by merging $v$ with previously popped  candidate views (i.e., views in $Seen$),
thereby incrementally exploding the space of candidate views.
Note that $Seen$ contains candidate views that have an $\ocost{}$ 
less than or equal to that of $v$.
$M$ only retains those candidate  that are
not already in $Seen$, which are then inserted into $\PQ$.
% TODO: Need a proof for that statement
A property of $\ocost{}$ provided as a theorem later is that
the candidate views in $M$ have an
$\ocost{}$ that is greater than that of $v$ and hence none
of these views should have been examined before $v$.
This property enables a gradual explosion of the space of candidate views.
Then, $v$ is added to $Seen$.

If $v$ is guessed to be complete,  
we try to find rewrites of $q$ using $v$ by invoking the $\RE$ function
      (described in Section~\ref{sec-rewrite-enumeration}).
Among the rewrites found by $\RE{}$,
the cheapest rewrite is returned to $\WF{}$ as the result.
% TODO: Do we need to talk about join ordering?


% The \VF{} finds a rewrite for a target in $W$ given a set of materialized views $V$.
% This problem is referred to as \emph{query} rewriting, hence our 
% input is a query $q$ representing the target, and $V$.
% Given our problem formulation, we require one instance of the \VF{} per target in $W$.
% The space of candidate views $C$ can be very large due to merging
% views in $V$. 
% Our approach allows for a gradual explosion of the space as needed.
% Here we will describe the functionality of the \VF{}, and later in
% Section~\ref{sec-best-first-workflow-rewrite} we
% will present the \WF{} which exploits the \VF's{} ability to incrementally examine
% the space of solutions for each target.
% The lower bound provided by $\ocost{}$ enables the \VF{} to explore the space
% incrementally, at every step examining any potentially lower-cost rewrites before exploding the
% space further to produce candidate views that have higher potential cost.

\begin{comment}
% Good text but got rid of it in the Alkis rewrite
Answering queries using views is a long-studied problem.
It is primarily considered in the context of data integration or data warehouse
design (query optimization)~\cite{Hale2001}.
Data integration is often interested in maximally-contained rewrites while
query optimization is concerned with equivalent rewrites.
Our interest is the latter.
The complexity of the problem is described with respect to the
expressivity of the languages used for both the queries
and the view definitions~\cite{Abit1998}.
Even when both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete
both for determining whether a rewrite exists~\cite{Levy1995} and
checking the correctness of a rewrite.
Checking the correctness of the rewrite is the same problem as
determining containment (i.e. $ Q_1 \subseteq Q_2$), which is
NP-complete~\cite{Chan1977} for conjunctive queries.
A \textit{complete} rewriting of $Q$ using $V$ is said to be one
that only uses $V$, and does not use any of the base relations.
Determining whether there is a complete rewriting of $Q$ using $V$
(again for the class of conjunctive queries) is NP-complete~\cite{Levy1995}.
Furthermore, when $Q$ and $V$ are disjunctions of conjunctive queries,
finding a complete rewriting is NP-complete~\cite{Levy1995}.
Producing a \textit{minimal} rewrite entails using the minimal number
of views in the rewrite such that no view can be removed
without invalidating the rewrite.
This problem is also NP-complete~\cite{Levy1995}.
We only consider complete rewrites, those using
the existing views, without extracting new views from the log.
\end{comment}

\begin{comment}
% CUT due to lack of space.
The reason we do not return to the log (i.e., base relation) is that
more and more views become materialized in the system as analysts
perform their data exploration and furthermore log extraction is expensive.
The rewrites are expressions in $L_R$ which may include
additional transformations on $V$ in order to produce an equivalent rewrite.
\end{comment}

\begin{comment}

\begin{enumerate}
\item {\bf Prune Step}:  Retain only those views that are relevant 
to the query (have the required attributes, have a mapping to the 
same base relations, logically-weaker selection and join predicates).

Find {\em all} relevant views $v$ to the query $q$.
Views that are not relevant to the query are pruned.

Determining a relevant view $v$ involves
(a) $v$ shares common base relations with $q$,
(b) $v$ must not have projected out any attributes required by $q$, and
(c) $v$ must contain a subset of the join predicates in $q$ and (d) must have
identical or logically weaker selection predicates.

The views in $V$ that pass the prune step are called {\em relevant} views.

Among the relevant views those that contain all the join predicates in $q$
are termed as \emph{complete}, otherwise they are called {\em partial} solutions.
%% Note that the {\em complete} solutions are added to the {\em winner} pile,whereas the partial solutions are added to the {\em loser} pile.
Next, a {\em  dominance} pruning is performed by comparing all pairs of relevant views, from each pair
discard the view with lower contribution or higher cost.

%%For all the complete solutions, it tries to find an equivalent rewrite using the views, which we term as {\em chain forming}.
% SJ: Need to figure out what the hardness result of "chain formation"

\item {\bf Merge Step}: Join all partial solutions using all
possible equijoin methods on all join orders to form
additional relevant views. Return to prune step.
\end{enumerate}
\end{comment}




% The lower bound provided by $\ocost{}$ allows the \VF{} to search the space
% incrementally, exploring any potentially
% lower-cost rewrites first before exploding the
% space unnecessarily to find and enumerate them all.
%The $\VF{}$ takes as inputs
%a query $q$, the set of existing materialized views $V$,
%two values $d',d$, s.t., $d' < d$ and outputs an equivalent
%rewrite $r$ of $q$ using a set of views in $V$, such that
%$d' < \ocost(r) \leq d$ if $r$ exists.
%Note that $V$ is only required in the initialization step,
%and in subsequent invocations $d'$ is implicit in the sense that it records
%the value of $d$ from the previous invocation.


\begin{comment}
% SJ: Given that we now use Surajit Chaudhuri's method, this text is not needed 
%
The $\VF{}$ maintains a priority queue $\PQ$ which contains all candidate views.
The candidate views include those in $V$ as well as views
formed by ``merging'' of views in $V$.
To merge a pair of candidate views $v_1$ and $v_2$,
we consider all possible equi-join methods based on common keys,
as well as trying all possible subsets of join predicates that are present in $q$
which is similar to the approaches in~\cite{Agra2000,Hale2001}.
In~\cite{Hale2001} partial views are only considered for merging if they satisfy join
predicates in $q$, while~\cite{Agra2000} merges views to create parent
views that can answer the same or larger subset of queries
in the given workload than their constituent views (i.e, $v_1$ and $v_2$).
We adapt both approaches as a way of making partial views complete with respect to $q$.
As in~\cite{Agra2000}, we generate new views by a series of pair-wise merges.
This process is captured in the procedure $\merge(v_1, v_2)$, 
where $v_1$ and $v_2$ are candidate views
and the output is a new candidate view $v_{12}$.
Because the merging process adds exponentially more
views for consideration, we should avoid growing the space larger than necessary.
Thus we control the candidate generation process by merging a candidate view with those
candidates views that have a lesser $\ocost{}$.
The use of the $\PQ$ enables the merge process to be resumed later when the
$\VF{}$ is invoked in the next iteration, if it is needed.

While~\cite{Agra2000} only retains candidate views that the optimizer considers 
 useful for answering queries and their merge step only considers
merging based on the join condition specified in $p$,
we consider merging views when they share a common key.
The utility of merging views based on a common key can 
be seen from the following example.
Consider a query $q$ that requires the key $\{A,D\}$.
Suppose that $v_1$ contains key $\{A,B\}$, $v_2$ contains key $\{B,C\}$ and $v_3$ contains
key $\{C,D\}$.
A typical pruning step would discard $v_2$ as it does not contain any attributes
syntactically relevant to $q$.
We note that merging $v_1$ with $v_2$, followed by a merge with $v_3$ will obtain a superset
of keys needed by $q$.
This merged view is complete with respect to $q$.
\end{comment}

\begin{algorithm}[h!]
\caption{$\VF$\label{alg-viewfinder}}
{\small
\begin{algorithmic}[1]
\Function{\sc Init}{$query$, $V$}\label{alg-vf-init}
 \State Priority Queue $PQ$ \qlet $\emptyset$; $Seen$ \qlet $\emptyset$; Query $q$ 
  \State $q$ \qlet $query$
  \ForAll{$v \in V$}
     \State $PQ$.\texttt{add}($v$, $\ocost(q,v))$
  \EndFor
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Peek}{}\label{alg-vf-peek}
%\State \Return ($PQ$.\texttt{peek}().$\ocost$: $\infty$) ? 
\State {\bf if} $PQ$ is not empty {\bf return} $PQ$.\texttt{peek}().$\ocost$ {\bf else} $\infty$
%   \If{not $PQ$.\texttt{empty}()}
%   \State \Return $PQ$.\texttt{peek}().$\ocost$ 
%   \Else 
%   \State \Return $\infty$
%   \EndIf  
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Refine}{}\label{alg-vf-refine}
  \If{\texttt{not} $PQ$.\texttt{empty}()}
    \State $v$ \qlet $PQ$.\texttt{pop}()
    \State $M$ \qlet \merge($v$, $Seen$) \Comment{Discard from $M$ those in $Seen \cap M$}
    \ForAll{$v' \in M$}
      \State $PQ$.\texttt{add}($v'$, $\ocost(q,v')$)
    \EndFor
    \State $Seen$.\texttt{add}($v$)
    \If{\complete($q$, $v$)}
      \State \Return $\RE(q, v)$
    \EndIf
  \EndIf \\
  \Return {\sc null}
\EndFunction
\end{algorithmic}}
\end{algorithm}


\subsection{Rewrite Enumeration}\label{sec-rewrite-enumeration}

% Suppose that a candidate view $v$ is guessed to be complete.
% To determine if an equivalent rewrite exists requires finding at
% least one valid rewrite among all possible rewrites,
% is known to be a hard problem~\cite{Levy1995}.
In our system, we implemented the \RE{} procedure (described next) 
to produce a valid rewrite
of a query using a view that is guessed to be complete.
% \RE{} takes as input a query $q$ and a view $v$ that is guessed to be complete
% and outputs a rewrite $r$ if one exists.
Given that \complete{} can result in false positives, a rewrite may not be
found.
If a rewrite is found, it represents the cheapest among
all possible equivalent rewrites of $q$ using $v$.
The cost of a rewrite is evaluated by the \cost{} function,
and corresponds to the cheapest execution \textit{plan} that implements the rewrite.
Equivalence is determined by ensuring that the rewrite and query contain the same attributes,
filters, and group-by as detailed in Section~\ref{sec-equivalence}.
%This type of equivalence testing is simple but effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%Although this type of equivalence testing may seem simple it is effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%We replace an SPJ+G expression with a single view.  as in GL2001

From Section~\ref{sec-problem-definition}, recall that the rewrite language is
less expressive than the query language because we want to limit the number of
UDFs in the rewrite language but not the query language. 
We refer to the rewrite language as $L_R$.
We enumerate equivalent rewrites of $q$ by applying {\em compensations}~\cite{Zaha2000}
to a guessed to be complete view $v$ using $L_R$.
We do this by generating all permutations of required compensations and
testing for equivalence, which
amounts to a brute force enumeration of all possible rewrites given $L_R$.
This makes the case for the system to keep $|L_R|$ small.
When $L_R$ is restricted to a known, fixed 
set of operators it may suffice to examine a polynomial number of 
rewrites attempts, as in~\cite{Grum2003} for the specific case 
of simple aggregations involving group-bys.
Such approaches are not applicable to our case as 
the system should have the flexibility of extending $L_R$ with any UDF in the 
system.  


Given the computational cost of finding valid rewrites,
$\WF{}$ limits the invocation of $\RE{}$ algorithm using two strategies.
% we employ the following two strategies.
First,  we avoid having to apply $\RE{}$ on every candidate view making
a guess for the completeness of a view based
on the three properties described earlier.
Second, we delay the application of $\RE$ to every complete view 
by determining a lower bound on the cost of a rewrite using $v$ should one exist.
For the lower bound we use the $\ocost$, which helps   
% The goal of guessing completeness and estimating a lower bound is
to quickly distinguish between potentially low cost rewrite from those with higher cost.

\begin{comment} %% JL temp
\subsection{Determining O\fakesc{pt}C\fakesc{ost}}\label{sec-ocost}
The utility of  a lower bound we develop in this section enables
the enumeration of the candidate views based their potential 
to provide a low cost rewrite.
% Our expectation of the lower bound is only that it should be able to quickly distinguish between 
% candidate views with potential to produce cheap versus very expensive rewrites.
% Given a candidate view $v$ and a query $q$,
% we wish to determine a lower bound on the cost of \textit{any} plan yielded by
% an equivalent rewrite of $q$ using $v$ if one exists without enumerating all possible rewrites,
% checking for equivalence and examining their plan costs.
% We refer to this lower bound as the optimistic cost, or \ocost.
\ocost relies on the non-subsumable cost property of the $\cost{}$ function
to arrive at a lower-bound.

Given that $v$ is guessed to be complete with respect to $q$, 
a set difference between the attributes, filters and group-bys representation 
of $q$ and $v$ is referred to as the {\em fix}.
Fix denotes a hypothetical local function that can
transform $v$'s representation into $q$'s.
Note that a UDF containing such a local function may not really exist.
We have to invoke $\RE{}$ which produces a rewrite
containing compensations from $L_R$.
The composition of the local functions in the compensation
transforms $v$'s representation to $q$.
%\ocost{} uses the attributes, filters, and group-by representation 
%of $q$ and $v$ to take a set difference between each of these properties.
%This denotes a minimum set of non-subsumable operations
%by Definition~\ref{definition-non-subsumable-property}
%needed to transform $v$'s representation into $q$'s.
Finally, note that the existence of fix guarantee that $v$ will result in a valid rewrite 
for the same reason that  guessed to be complete can result in a false positive.
Both assume that the required
compensation operations can be applied independently of each other to $v$.
% resolve the differences  in the attributes, filters, and group-bys of $q$ and $v$.
%compensate these properties independently.
% is possible to compensate $v$ using operations in $L_r$
%independently of the others.

%We refer to this set as the {\em fix} of $v$ with respect to $q$.
%The non-subsumable property allows \ocost{} 
%to consider operations in the fix as independent of one another,
%although they can still affect each other's cost.
% \ocost{} then returns the sum of the create cost $c'_1$, access cost $c'_2$, and the
% minimum operation cost $c'_3$ in the fix as the
% lower bound on the cost of \textit{any} plan.

%If $v$ is not materialized in the process of rewriting a query and then any
%necessary compensation is applied. 
We now describe a $\ocost{}$ function with the two properties 
that it is a lower bound on the cost of \textit{any} plan returned by $\RE(q,v)$
and inexpensive to compute.
If $v$ is a materialized view then $c_1$ is equal to the cost of accessing $v$. 
Otherwise, if $v$ results from the merging of views, 
then $c_1$ is the total cost to access the constituent views of $v$. 
% We denote $c_1$ as the cost of accessing all the constituent views in $v$ (i.e., access cost).
We denote $c_2$ as the cost of merging the constituent views in $v$ (i.e., creation cost)
if $v$ is already not materialized, else $c_2$ = 0 if it is already materialized.
We denote $c_3$ as the cost of applying the least expensive operation in the fix on $v$,
obtained by invoking the \cost{} to obtain the cost of 
performing each of the operations in the fix on $v$.
$c_3$ is obtained by $\min(\cost(x, v))$ such that $x$ is an operation in {\em fix}.

% If a plan of the rewrite using $v$, materializes $v$ before applying
% all the applicable compensation, then 
The \ocost{} of $v$ with respect to $q$ is given
by: $c = c_1 + c_2 + c_3$, where $c$ is less than the cost of any
plan of the rewrite using $v$.
If $v$ is partial with respect to $q$,
then $c_3 = 0$ since no compensation should be applied.

Suppose that the optimizer can generate plans where some of compensations
can be pushed into the candidate view $v$ before materializing it.
In this case, $\ocost{}$ can provide a weaker lower bound
as it can only consider the cost ($c_1$) of accessing all the constituent views of $v$ 
plus the minimum cost $c'_3$ of applying the least expensive operation 
in the fix on any constituent views of $v$ or on any intermediate view
that can be created in the process of creating $v$.
If $v$ is partial with respect to $q$, then $\ocost{}$ only includes $c_1$.

We provide the following proof sketch to capture the correctness of the 
$\ocost{}$ function.
\end{comment} %% JL


\begin{comment}
%\ocost takes an optimistic approach in determining the minimum possible plan cost.
If a candidate view $v$ is not yet materialized (i.e., to be created by merging),
$\RE{}$ might consider
materializing it first before applying all necessary compensation.
%If $v$ is not materialized in the process of rewriting a query and then any
%neccessary compensation is applied. 
Then, intuitively it can be seen that any plan yielded by an equivalent rewrite would incur at
the least the sum of
the cost $c_1$ for accessing all the constituent views in $v$ (i.e., access cost),
the cost $c_2$ for materializing any new views it requires (i.e., creation cost), and
the cost $c_3$ 
of applying the least expensive compensation operation on the view $v$.
\ocost{} invokes \cost{} to obtain the cost of 
performing each of the operations in the fix on $v$.
It chooses the least expensive operation in the fix
as the third component $c_3$ of the \ocost, where
$c_3$ is given by $\min(\cost(x, v))$ such that
$x$ is an operation in {\em fix}.
We define \ocost{} as $c = c_1 + c_2 + c_3$, which has the property 
that it is a lower bound on the cost of \textit{any} plan returned by $\RE(q,v)$
and inexpensive to compute.
If $v$ is partial (i.e., not guessed to be complete) with respect to $q$,
then $c_3 = 0$ since no compensation should be applied.
\end{comment}

%Note that if using the push-down approach, 
%when the view is partial then \ocost{} is only $c'_1$,
%since push-down predicates may change the join ordering.
%Further details  of this \ocost{} function 
%and our proof of the lower bound property when considering predicate pushdown is 
%omitted here due to lack of space.


\begin{comment}
There are certain benefits to both approaches.
The choice to create $v$ is similar to the approach that a view recommender~\cite{Agra2000} might take,
while pushing down predicates into $v$ to create $v'$ is an approach that a query optimizer may take for
answering a single query $q$.
One way to think about this is that $v$ is a recommended view by the $\VF{}$ and here we
decide to piggyback its creation as a part of execution of query $q$.
Given the use case of the system, we prefer this approach as we
wish for the artifacts created (i.e., $v$) as part of answering $q$ to
be as beneficial as possible to the subsequent queries by future users.

The $\VF{}$ could be modified to support predicate pushdown by
modifying $\ocost$ to order partial views by their access cost for $v$ (i.e., $c'_1$).
The pushdown predicates can potentially change the cost of all the joins and their orderings.
\end{comment}


% RETAIN THE REMAINDER OF THIS PROOF HERE. -- REFERS TO Appendix
% An $\ocost{}$ function that considers predicate pushdown 
% is given in Appendix~\ref{appendix-pushdown}.

%%%\input{scenario-no-plug}

\begin{comment} %% JL temp
\begin{theorem}
$c$ is a lower-bound on on the cost of \textit{any} plan yielded by
an equivalent rewrite $r$ of $q$ using $v$ if one exists.
\end{theorem}

\begin{proof}
Any plan of the rewrite $r$ will have to access all the constituent views in $v$
and materialize it. So, $c_1$ and $c_2$ is common to $\ocost{}$
and the cost of any plan of $r$.

In order to find the lowest cost $r$, $\RE{}$ applies all 
permutations of compensation operations to achieve 
an equivalent rewrite.
% that achieves the same
% effect as the fix, although each operation in the compensations
% can ``cover'' more than one operations in fix.
% The end-to-transformation produced by the compensation 
% is the same as that denoted by fix, regardless of whether
% there is a one-to-one correspondence between the operators in the compensation
% and fix, or a single operation in the compensation covers all of fix.
Regardless of how many operations are used in the compensation,
by Definition~\ref{definition-non-subsumable-property}, the cost
of applying the compensations has to be at least as expensive as 
the cheapest operation $c_3$ in the fix.

Next we consider the $\ocost{}$ function 
for the case involving push-down of compensations.
For this case, both the ordering of the merges of the
constituent views of $v$ as well as the applicable compensations are as yet unknown.
Our lower-bound holds as it does not make any assumptions about
the ordering of the constituent views in $v$ (i.e., by using $c_1$) as well as 
the position of any compensation operator in any plan of $r$ (i.e., $c'_3$) . \qed
\end{proof}
\end{comment} %% JL temp


\begin{comment}
Base Case: Let the fix be denoted by the operators $x$, $y$, $z$,
such that $op^* = z$ is the cheapest operator in fix.
A rewrite $r$  using {\em fix} can
apply operators in the following sequence:
a) apply one operator followed by another or both,
b) apply two operators (e.g., $xz$) followed by a third
operator (e.g., $y$), or
c) apply operators $xyz$ all at once.
For case a) the cost of $r$ is greater than or equal to
either $\cost(x,v)$ or $\cost(y,v)$  or $\cost(z,v)$.
For case b) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(z,v))$ if the first operation
is given by $xz$.
For case c) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$.
As $r^*$ represents the lowest cost rewrite across
all rewrites denoted by the three cases, it is bounded by:
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$, which proves
the base case of {\em fix} with 3 operators.

Induction Step:
Let $y$ be the cheapest operation in the set denoted by $\mbox{\em fix}-x$, such that
$\cost(r^*,v) \geq \cost(y,v)$ where $r^*$ corresponds
to lowest cost rewrite on $\mbox{\em fix}-x$.
In other words, the cost of $r^*$ is at least the cost of applying
the cheapest operator in $\mbox{\em fix} -x$.

Add $x$ back to the {\em fix}.
Now, let $r^*$ be the lowest cost rewrite
using {\em fix}.
Suppose that $r^*$ is composed of sets operators $p_1, p_2 \cdots p_k$, such that
$p_1 \cup p_2 \cdots \cup p_k = \mbox{\em fix}$ and
the output of $p_1$ forms the input to $p_2$ and so on.
Then, $\cost(r^*,v) = \cost(p_1, v) + \cost(p_2, v|p_1) + \cdots + \cost(p_k, v|p_1\cdots{}p_{k-1})$,
where $v|p_1$ means that operators in $p_1$ have been applied to $v$.
This means that $\cost(r^*,v) \geq \cost(p_1, v)$ given that $\cost{}$ is always non-negative.
The lowest value of $\cost(p_1,v)$ occurs when $op^*$ is present in
$p_1$ possibly along with other operators in the {\em fix}.
Thus, $op^*$ must either be $y$ which was the cheapest operator in $\mbox{\em fix} - x$
or $op^*$ must equal to $x$.
Then, $\cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$.
Finally, $\cost(r^*,v) \geq \cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$. \qed
\end{comment}


\begin{comment}
\begin{theorem}
$c'$ is a lower-bound on on the cost of \textit{any} plan yielded by
an equivalent rewrite of $q$ using $v$ if one exists.
\end{theorem}

\begin{proof}
Let $c$ be the minimum cost plan generated by the $\RE(q,v)$ corresponding
to the rewrite $r$.
$c$ is composed of
the cost $c_1$ for accessing all the views, and
the cost $c_2$ for materializing any new views it requires,
the cost $c_3$ for least expensive ordering of transformation 
rules in $L_R$ applied to $v$.
As $v$ is guessed to be complete for the query $q$,
both $\RE$ and $\ocost$ use $\cost$ to obtain the cost to create and access $v$,
then $c_1 = c'_1$ and $c_2 = c'_2$.

In order to find the lowest cost $r$, $\RE{}$ will have
to enumerate all permutations of rules in $L_R$ required
to achieve the fix.
If \RE{} finds a rewrite, $r$ will have covered all operations in fix,
choosing the cheapest rewrite found to be $c_3$.
$\ocost{}$ uses \cost{} once per each operation in fix
choosing the cheapest as $c'_3$.
As $c'_1$ and $c'_2$ are common to both $c$ and $c'$,
it suffices to show that $c_3 \geq c'_3$.

Recall that \emph{fix} is made up of non-subsumable operations.
A property of two non-subsumable operations as mentioned
earlier in Definition~\ref{definition-non-subsumable-property} is that:
$\cost(xy, D) \geq \min(\cost(x, D),
\cost(y, D))$, where $v$ is an instance of a database $D$, and
$x$, $y$ are operators in fix, and $xy$ performs both $x$ and $y$.

By induction we can show that the cost of the cheapest
rewrite that applies  the fix to $v$
is greater than or equal to $\cost(op^*, v)$, 
where $op^* \in \mbox{\em fix}$
and is the cheapest operator present in the {\em fix} but we
omit the remainder of the induction for lack of space.\qed

-- RETAIN THE REMAINDER OF THIS PROOF HERE. -- 
Base Case: Let the fix be denoted by the operators $x$, $y$, $z$,
such that $op^* = z$ is the cheapest operator in fix.
A rewrite $r$  using {\em fix} can
apply operators in the following sequence:
a) apply one operator followed by another or both,
b) apply two operators (e.g., $xz$) followed by a third
operator (e.g., $y$), or
c) apply operators $xyz$ all at once.
For case a) the cost of $r$ is greater than or equal to
either $\cost(x,v)$ or $\cost(y,v)$  or $\cost(z,v)$.
For case b) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(z,v))$ if the first operation
is given by $xz$.
For case c) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$.
As $r^*$ represents the lowest cost rewrite across
all rewrites denoted by the three cases, it is bounded by:
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$, which proves
the base case of {\em fix} with 3 operators.

Induction Step:
Let $y$ be the cheapest operation in the set denoted by $\mbox{\em fix}-x$, such that
$\cost(r^*,v) \geq \cost(y,v)$ where $r^*$ corresponds
to lowest cost rewrite on $\mbox{\em fix}-x$.
In other words, the cost of $r^*$ is at least the cost of applying
the cheapest operator in $\mbox{\em fix} -x$.

Add $x$ back to the {\em fix}.
Now, let $r^*$ be the lowest cost rewrite
using {\em fix}.
Suppose that $r^*$ is composed of sets operators $p_1, p_2 \cdots p_k$, such that
$p_1 \cup p_2 \cdots \cup p_k = \mbox{\em fix}$ and
the output of $p_1$ forms the input to $p_2$ and so on.
Then, $\cost(r^*,v) = \cost(p_1, v) + \cost(p_2, v|p_1) + \cdots + \cost(p_k, v|p_1\cdots{}p_{k-1})$,
where $v|p_1$ means that operators in $p_1$ have been applied to $v$.
This means that $\cost(r^*,v) \geq \cost(p_1, v)$ given that $\cost{}$ is always non-negative.
The lowest value of $\cost(p_1,v)$ occurs when $op^*$ is present in
$p_1$ possibly along with other operators in the {\em fix}.
Thus, $op^*$ must either be $y$ which was the cheapest operator in $\mbox{\em fix} - x$
or $op^*$ must equal to $x$.
Then, $\cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$.
Finally, $\cost(r^*,v) \geq \cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$. \qed
\end{proof}
\end{comment}

%The $\ocost{}$ does not cause the algorithm to lose its optimality property,
%regardless of considering an even larger (or pruned)
%rewrite space  than the one we consider here.


\begin{comment}
The lower bound provided by our $\ocost{}$ function could be tightened if we are
willing to commit to a particular execution environment and a specific query optimizer.
For example in an MR environment with a Hive query processor,
given the set of operations in the fix, one could
estimate the minimum number of maps, reduces, and jobs it would take to
apply all operations in fix to $v$.
Such an approach requires intimate knowledge of a specific system,
and thus loses the desired generality of a lower bound estimator.
\end{comment}

%Finally, we provide the following lemma describing the $\ocost{}$ property
%for any new candidate view created in $M$ during Algorithm~\ref{alg-viewfinder}.

\begin{comment}
The following theorem describes the $\ocost{}$ property for newly
merged candidates in $M$.
This enables Algorithm~\ref{alg-viewfinder}
to generate candidate views as needed to avoid a pre-explosion
of the space of all candidates.

\begin{theorem}
The $\ocost{}$ of every candidate view in $M$ that is not in $Seen$
is greater than or equal to the $\ocost{}$ of $v$.
\end{theorem}
\begin{proof}
The proof sketch is as follows. The theorem is trivially true for 
$v \in V$ as all candidate views in $M$ cannot be in $Seen$
and have $\ocost$ greater than $v$. 
If $v \notin V$, it is sufficient to point out
that all constituent views of $v$ are already in $Seen$
since they must have had $\ocost{}$ lesser or equal to $v$
Hence all candidate views in $M$ with $\ocost{}$ smaller than $v$ are
 already in $Seen$, and those with $\ocost{}$ greater than $v$ will be added to $PQ$
if they are not already in $PQ$.
 %all the 
%candidate views in $M$ are already present in $Seen$ if smaller, or if greater,
%are still in $\PQ$.
\end{proof}
\end{comment}

\begin{comment}
% RETAIN THE REMAINDER OF THIS PROOF HERE.
\begin{proof}
Suppose that $v'$ is a new candidate  that is created by merging $v$ with $Seen$.
Then we need only consider the case of $v$ being a base view or a composite view.
If $v$ is a base view (i.e., already materialized), then the $\ocost{}$ of $v'$  cannot be
less than $v$ as $\ocost(v)$ only considers its access cost, while $\ocost(v')$
is at least the cost of accessing $v$ as well as accessing the other candidate view that $v$ is joining with.
If $v$ is a composite view (i.e., $v$ is composed of multiple base views),
then the $\ocost{}$ of $v'$ cannot be less than $v$.
To show that by contradiction,
consider the case where $v'$ is not in $Seen$
and $v'$has a lesser $\ocost{}$ than $v$.
As $v$ is a composite view, then all of its constituent views would already
have been joined with all the candidate views in $Seen$.
Thus, $v'$ must already have been created.
If $v'$ has a lesser $\ocost{}$ than $v$,
it would have already been popped out of $\PQ$ and in $Seen$ before we got to $v$.
\end{proof}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}


\begin{itemize}
\item Two queries $Q_1$, $Q_2$
are said to be {\em equivalent} if $Q_1 \subseteq Q_2$ and $Q_2 \subseteq Q_1$.
From a query answering perspective,
the set of tuples in the result set of $Q_1$ are identical
to the set of tuples in the result set of $Q_2$.
To determine if an equivalent rewriting using views exists has been already
shown to be in NP even for the class of conjunctive queries~\cite{Hale01}.

\item A query $Q_1$ is said to be {\em contained } by $Q_2$
if $Q_1 \subseteq Q_2$.
From a query answering perspective,
all the tuples in the result set of $Q_1$ are contained in
the result set of $Q_2$, although the result set of $Q_2$ can contain additional
tuples that is not present in the result set of $Q_1$.
The problem finding contained rewriting is also known to NP-complete
even for conjunctive queries~\cite{Hale01-18}.

\end{itemize}

\item A candidate $c$ is said to be {\em complete} with respect to a $Q$ iff $c$ has
has a superset of the attributes and a subset of the filters and
superset of the groupby keys.
If there are attributes in $Q$ that are not present in $c$, $c$ has
the necessary ingredients (i.e., attributes) to obtain $Q$.
Of course, even if $c$ is complete,  it does not mean that
there exists an equivalent rewrite of $Q$ using $c$.
Thus, this provides a necessary but not sufficient
condition that equivalent rewrite exists.
The sufficient condition is when an equivalent
rewrite of $Q$ using $c$ exists.

\item We provide a set of $k$ transformational rules for
query rewriting using a candidate $c$. We call the
rewrite of complete candidate $c$ to a target $t$ using
our transformational rules a {\em chain}.

\item There are three classes of transformational rules that
we allow in the system.




\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item Rules that transform \{A\}, \{F\}, \text{or} \{G\}
\item Rules that transform \{A,F\}, \{F, G\}, \text{or} \{A, G\}
\item Rules that transform \{A, F, G\}
\end{enumerate}

\renewcommand{\labelenumi}{\theenumi}


% SJ: Let us add an example here
\item We have 4 transformation rules in our system:
\begin{enumerate}
\item $P$ \textendash Project (class \textsl{i})
\item $F$ \textendash Filter (class \textsl{i})
\item $G$ \textendash Groupby (class \textsl{i} and \textsl{ii})
\item $D$ \textendash Derived (class \textsl{i}, \textsl{ii}, \textsl{iii})
\end{enumerate}

In our $\MinDist$ function presented later, we make the assumption
that each rule can be applied independently.
Furthermore, our algorithm (described later) makes the assumption that the
 Filter rule applies all missing filters, one at a time before completing.
This prevents a large explosion of rule permutations
to apply when searching for a valid rewrite.  However, it presents a limitation on the
ability of our algorithm to find a successful rewrite if one exists.
It may be that no valid rewrite exists using a permutation
of these 4 rules, but one might exist if we consider each missing filter a separate
application of our $F$ transformation rule and thus could produce a successful rewrite such as
$F \rightarrow G \rightarrow F$ whereas due to our restriction of applying all missing filters
with the  $F$ rule before moving to another rule would not be able to produce such a re-write.

The \emph{Derived} rule allows for easy extensions, which is useful for attributes
created by UDFs that can easily be manipulated into other attributes.  For instance, one could add
a derivation that transforms lat-lon into a grid, or positive sentiment with a scoring value of
0.5 to 0.6, or word-count into (approximate) character-count.  Currently we have implemented
several derived attr transformations such as Groupby stats...

\item Determining if a solution $c$ is {\em complete} is  NP-hard
as it involves enumerating all possible chains using the transformation
rules

\item If a candidate is complete we can ``guess''
the minimum number of
transformational rules that go into the chain.
It is minimum ``guess'' as it based on the necessary
condition but not the sufficient condition, so no valid
chain may exist.

\item Why we cannot directly apply the traditional view finding:
  \begin{itemize}
  \item Discarding the non-relevant views using common base relations is not an effective pruning strategy as all queries are posed on a small set of logs, thus many views have the same base relation, a log.
  \end{itemize}
\end{itemize}

\subsection{View Finding Algorithm}

\begin{itemize}

\item Idea of a guess or mindist of a candidate to a target.
\begin{enumerate}
\item Also determine (optimistic guess) complete (winners) vs. partial candidates (losers)
\item Helps prune away the space quickly
\end{enumerate}

\item Describe chain data structure
\begin{enumerate}
\item Series of cmerged or joined candidates, where joined candidates
are restricted to those join predicates that appears in $t$
\item cmerge are keyed equijoins between candidates that shares
common keys
\item joins are equi across different keys or non-keys
\end{enumerate}

\item How to determine mindist?
\item mindist(chain c, t)
\begin{enumerate}
\item Really quick computation
\item Committed cost(c) + guess\_remaining\_cost(c.tail, t)
\item Decouples search from distance computation by assuming independence
\item Magical UDF
\item Claim: Guess is always <= actual cost
\item Finite mindist does not mean existence of chain which
is known to be NP-hard.. (because necessary condition only)
\end{enumerate}

\end{itemize}

Because we explore the solution space incrementally using our MINDIST, we
initialize the viewfinder by registering a target view and a set of candidate
views as follows in Algorithm \ref{viewfinderinit}:

\begin{algorithm}
\caption{ $\VF$-\textsc{initialize}($t$, $C$)}
\label{viewfinder-init}
\begin{algorithmic}[1]
\Require target $t$, candidate pool $C$ % some input
\State {Initialize WinnersPriorityQ, LosersPriorityQ}
\ForAll{$c \in C$}
  \State chain $c' \Leftarrow c$
  \State $d \qlet \MinDist(c', t)$
  \If{$d$ is $\infty$}
    \State LosersPQ.add($c'$, $d$)
  \Else
    \State WinnersPQ.add($c'$, $d$)
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\caption{ $\VF$($t$,\textit{MinCost})}
\label{viewfinder}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ
\State \textsc{mergeables}.\textit{clear()} \\
\Comment {\scriptsize Grow candidate space by merging all (partial view) pairs until the \textsc{committed\_cost} of all Losers is greater than the requested MinCost \normalsize}
\State $m \qlet $ \textit{MinCost}
\While{LosersPQ.peek().committed\_cost $ < m$}
  \State \textsc{mergeables}.\textit{add}( LosersPQ.pop() )
\EndWhile
\State \viewfinderCMerge(\textsc{mergeables})
\While{$ \MinDist$ (Winners.peek()$, t) < m$}
  \State $chain$ $\qlet$ Winners.pop()
  \State   \answer $\qlet$ \viewfinderRefine($chain$, $t$)
  \If {\answer}
    \State $\result$.\textit{add}($\ans$)
  \EndIf
\EndWhile
\State return $\result $

\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{ \viewfinderCMerge(\textsc{mergeables}) }
\label{viewfinder-cmerge}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ \\
\Comment \scriptsize attempt to merge all pairs of views, join order is not considered here \normalsize \\
\Comment \scriptsize This is a keyed equi-join \normalsize
\ForAll{$i \in $ \textsc{mergeables}}
	\ForAll{$j \in $ \textsc{mergeables}}
	  \State $tmp \qlet$\textsl{ColumnMerge}($chain_i$, $chain_j$)
	  \If{$tmp$}
	    \State $newchain \qlet chain_i + chain_j$
	    \State $d \qlet \MinDist(newchain, t)$
	    \State $totalDist \qlet d + newchain$.\textsc{committed\_cost}
        \If{$d$ is $\infty$}
          \State LosersPQ.add($newchain$, $totalDist$)
        \Else
          \State WinnersPQ.add($newchain$,$totalDist$)
        \EndIf
      \EndIf
	\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{ \viewfinderRefine($chain$, $t$)}
\label{viewfinder-refine}
\begin{algorithmic}[1]
\Require transformation rules (P, F, G, D)
\State $P \qlet permutations$(transformation\_rules)
\ForAll{$p \in P$}
  \For {rule $\in p$}
   \State  $newchain \qlet$ \textsc{ApplyRule}(rule, $chain$, $t$)
   \If{$newchain$.\textsl{isEquivalent}($t$)}
     \State return $newchain$
   \EndIf
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\begin{itemize}
\item Mindist allows to look at the existence of shorter chain
first before exploring the longer chains

\item Why best first? Each iteration of the loser pile
keeps merging the chains cost up to $n$ way joins.
We do only two way of joins


\item cmerge is expensive so the cost grows very quickly.
A best first nature means you do not explode your space too much
because the remaining cost fo the minimum people is less than $m$.


\item Don't know there is a rewrite but have to look for  them all
to see which is the cheapest but we take advantage of the fact
that there are multiple opportunities for plumbing at different
targets, which means that if you find a valid rewrite at one target
it immediately bounds the search space of all the targets in the workflow.

\item Mindist allows the incremental exploration of the space in two place
a) Is it winner or loser?
b) Look for short rewrites if they exist
c) Grow the loser partial candidates slowly

\end{itemize}

\subsection{Artifacts}
We call a Materialized View that is created as the output of any query $q \in Q$ an artifact.  We make the assumption that this output is
always written to stable storage in the DFS.

We model an artifact in a minimalistic way as follows.  An artifact is considered to have 3 properties:
\begin{enumerate}
\item Attributes
\item Filters
\item Groupbys
\end{enumerate}


\end{comment}



\begin{comment}
Our system considers every operation as a UDF.
Given that our execution framework is a simple MR system, we identify the types of operations that are possible.
Table \ref{tab:mrops} shows these operations and indicates which phase (Map or Reduce) they can occur.
UDFs may apply any of the operations shown.
Clearly this framework limits the expressivity of UDFs.
Yet many complex UDFs such as ... can still be applied in this framework as shown in example X.
Thus the framework is sufficient for many analytics we consider.
An execution (MapReduce job) may apply filters,
apply projections,
create new attributes via transformations,
or perform aggregations to produce the result.
Given the allowable operations, a result can be modeled as a set of Attributes (\textsf{A}),
a set of filters (\textsf{F}), and group by attributes (\textsf{G}).
We consider \textsf{F} to contain conjunctions of simple selection predicates.
In this model, the result of a equijoin operation appears as an additional filter representing the join predicate.
A result is considered a materialized view in our system (a view extension).

Because UDFs can perform complicated transformations any derived attribute produced must contain
some metadata about itself.
Consequently each attribute has a \textit{signature}, which is a minimal form of provenance that captures the nature of the
view's direct input in terms of \textsf{A}, \textsf{F}, \textsf{G} along with some other small metadata such as the operation applied
(UDF name) to the input to produce the view.

This representation enables us to easily understand UDF as a grey box, rather than a black box.
It is considered to be grey since we don't really understand what the function actually does,
we only understand the label of the function and what the input and output look like.
This means that two identical functions with different labels will not appear identical to our model.
Or UDFs that may subsume each other will not be identified.
Our method is extensible toward a more fine-grained understanding of the function where some UDFs may become a white box.
This requires additional complexity while here we focus on the usefulness of our method
even on the level of understanding a UDF as a grey box.

We now define our grammar that is used by all UDFs.
All UDFs operations are described in this grammar.
A UDF takes at least one view as input and produces a view as output.
To understand a UDF as a grey box, each attribute created by a
UDF records the following metadata describing itself.
\begin{enumerate}
\item {\sf B} - the name of the UDF that produced the attribute
\item {\sf M} - a modifier argument given to the UDF (if any)
\item {\sf A} - the input attributes to the UDF
\item {\sf F} - the filters previously applied to the input
\item {\sf G} - the group-bys previously applied to the input
\end{enumerate}

The output of the UDF is a materialized view which is described
in terms of \textsf{A}, \textsf{F}, \textsf{G}.
The grammar of the UDF must describe the transformations from
{\sf B, M, A, F, G} to {\sf A, F, G}.
\end{comment}



==> old/Viewfinder.tex <==
\section{ViewFinder}\label{sec-viewfinder}

Answering queries using views is a long-studied problem.
It is primarily considered in the context of data integration or data warehouse
design (query optimization)~\cite{Hale2001}.
Data integration is often interested in maximally-contained rewrites while
query optimization is concerned with equivalent rewrites.
Our interest is the latter.
The complexity of the problem is described with respect to the
expressivity of the languages used for both the queries
and the view definitions~\cite{Abit1998}.
Even when both queries and views are expressed in a language that
only includes conjunctive queries, it is known to be NP-complete
both for determining whether a rewrite exists~\cite{Levy1995} and
checking the correctness of a rewrite.
Checking the correctness of the rewrite is the same problem as
determining containment (i.e. $ Q_1 \subseteq Q_2$), which is
NP-complete~\cite{Chan1977} for conjunctive queries.
A \textit{complete} rewriting of $Q$ using $V$ is said to be one
that only uses $V$, and does not use any of the base relations.
Determining whether there is a complete rewriting of $Q$ using $V$
(again for the class of conjunctive queries) is NP-complete~\cite{Levy1995}.
Furthermore, when $Q$ and $V$ are disjunctions of conjunctive queries,
finding a complete rewriting is NP-complete~\cite{Levy1995}.
Producing a \textit{minimal} rewrite entails using the minimal number
of views in the rewrite such that no view can be removed
without invalidating the rewrite.
This problem is also NP-complete~\cite{Levy1995}.
We only consider complete rewrites, those using
the existing views, without extracting new views from the log.

\begin{comment}
% CUT due to lack of space.
The reason we do not return to the log (i.e., base relation) is that
more and more views become materialized in the system as analysts
perform their data exploration and furthermore log extraction is expensive.
The rewrites are expressions in $L_R$ which may include
additional transformations on $V$ in order to produce an equivalent rewrite.
\end{comment}

Traditionally methods for rewriting queries using views for the
class of SPJG queries use a two stage approach~\cite{Hale2001, Agra2000}.
The prune stage determines which views are \emph{relevant} to the query,
and among the relevant views those that contain
all the join predicates in $q$ are termed as \emph{complete},
otherwise they are called {\em partial} solutions.
This is typically followed by a merge step that joins the partial
solutions using all possible equijoin methods on all join orders to form
additional relevant views.
% TODO-JEFF: Define space here
The algorithm repeats until only those views that are
useful for answering the query remain.
We take a similar approach in that we identify partial and
complete solutions, then follow with a merge phase.

\begin{comment}

\begin{enumerate}
\item {\bf Prune Step}:  Retain only those views that are relevant to the query (have the required attributes, have a mapping to the same base relations, logically-weaker selection and join predicates).

Find {\em all} relevant views $v$ to the query $q$.
Views that are not relevant to the query are pruned.

Determining a relevant view $v$ involves
(a) $v$ shares common base relations with $q$,
(b) $v$ must not have projected out any attributes required by $q$, and
(c) $v$ must contain a subset of the join predicates in $q$ and (d) must have
identical or logically weaker selection predicates.

The views in $V$ that pass the prune step are called {\em relevant} views.

Among the relevant views those that contain all the join predicates in $q$
are termed as \emph{complete}, otherwise they are called {\em partial} solutions.
%% Note that the {\em complete} solutions are added to the {\em winner} pile,whereas the partial solutions are added to the {\em loser} pile.
Next, a {\em  dominance} pruning is performed by comparing all pairs of relevant views, from each pair
discard the view with lower contribution or higher cost.

%%For all the complete solutions, it tries to find an equivalent rewrite using the views, which we term as {\em chain forming}.
% SJ: Need to figure out what the hardness result of "chain formation"

\item {\bf Merge Step}: Join all partial solutions using all
possible equijoin methods on all join orders to form
additional relevant views. Return to prune step.
\end{enumerate}
\end{comment}

However, the direct applicability of existing approaches 
to our problem is limited
in part because with no early termination condition they
explore the space exhaustively, thus degenerating into the 
bottom-up approach.
Thus we desire a rewriting algorithm (\VF) that can
enumerate the space and incrementally explore
only as much as required, frequently stopping
and resuming the search as requested by \WF.
We note that while an equivalent rewrite for a target $W_i$ may exist,
the \VF may never be asked to find it,
as illustrated by Example~\ref{example-greedy-plumbing}.

We take an optimistic approach toward initially
determining if a complete rewrite of query $q$ exists using a view $v$.
This represents a \emph{guess} that a complete rewrite exists.
A guess requires the following necessary conditions
as described in~\cite{Hale2001} (SPJ) and~\cite{Gold2001} (SPJG)
that a view must satisfy to participate in a rewrite of $q$, 
although these conditions are not sufficient to
confirm the existence of an equivalent rewrite using $v$.

\begin{itemize}
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item $v$ contains all the attributes required by $q$; or contains all the 
    necessary attributes to produce those attributes in $q$ that are not in $v$
\item $v$ contains weaker selection predicates than $q$
\item $v$ is less aggregated than $q$
\end{enumerate}
\end{itemize}

The function $\complete(q,v)$ performs these checks and returns true if $v$
satisfies the properties i--iii with respect to $q$.

\subsection{V\fakesc{iew}F\fakesc{inder} Algorithm}

% The lower bound provided by $\ocost{}$ allows the \VF{} to search the space
% incrementally, exploring any potentially
% lower-cost rewrites first before exploding the
% space unnecessarily to find and enumerate them all.
%The $\VF{}$ takes as inputs
%a query $q$, the set of existing materialized views $V$,
%two values $d',d$, s.t., $d' < d$ and outputs an equivalent
%rewrite $r$ of $q$ using a set of views in $V$, such that
%$d' < \ocost(r) \leq d$ if $r$ exists.
%Note that $V$ is only required in the initialization step,
%and in subsequent invocations $d'$ is implicit in the sense that it records
%the value of $d$ from the previous invocation.

The \VF{} finds a rewrite for a sub-workflow given a set of materialized views $V$.
This problem is referred to as \emph{query} rewriting, hence our 
input is a query $q$ representing the sub-workflow, and $V$.
Given our problem formulation, we require one instance of the \VF{} per target
in the workflow $W$.
The $\VF{}$ is {\em stateful} which
enables the $\WF$ to start, stop and resume the incremental searches at each target.
Here we will describe the functionality of the \VF{}, and later in
Section~\ref{sec-best-first-workflow-rewrite} we
will present the \WF{} which exploits the \VF's{} ability to incrementally examine
the space of solutions for each target.
The lower bound provided by $\ocost{}$ allows the \VF{} to explore the space
incrementally, at every step examining any potentially lower-cost rewrites before exploding the
space further.

The $\VF{}$ maintains a priority queue $\PQ$ which contains all candidate views.
The candidate views include those in $V$ as well as views
formed by ``merging'' of views in $V$.
To merge a pair of candidate views $v_1$ and $v_2$,
we consider all possible equi-join methods based on common keys,
as well as trying all possible subsets of join predicates that are present in $q$
which is similar to the approaches in~\cite{Agra2000,Hale2001}.
In~\cite{Hale2001} partial views are only considered for merging if they satisfy join
predicates in $q$, while~\cite{Agra2000} merges views to create parent
views that can answer the same or larger subset of queries
in the given workload than their constituent views (i.e, $v_1$ and $v_2$).
We adapt both approaches as a way of making partial views complete with respect to $q$.
As in~\cite{Agra2000}, we generate new views by a series of pair-wise merges.
This process is captured in the procedure $\merge(v_1, v_2)$, 
where $v_1$ and $v_2$ are candidate views
and the output is a new candidate view $v_{12}$.
Because the merging process adds exponentially more
views for consideration, we should avoid growing the space larger than necessary.
Thus we control the candidate generation process by merging a candidate view with those
candidates views that have a lesser $\ocost{}$.
The use of the $\PQ$ enables the merge process to be resumed later when the
$\VF{}$ is invoked in the next iteration, if it is needed.

While~\cite{Agra2000} only retains candidate views that the optimizer considers 
 useful for answering queries and their merge step only considers
merging based on the join condition specified in $q$,
we consider merging views when they share a common key.
The utility of merging views based on a common key can 
be seen from the following example.
Consider a query $q$ that requires the key $\{A,D\}$.
Suppose that $v_1$ contains key $\{A,B\}$, $v_2$ contains key $\{B,C\}$ and $v_3$ contains
key $\{C,D\}$.
A typical pruning step would discard $v_2$ as it does not contain any attributes
syntactically relevant to $q$.
We note that merging $v_1$ with $v_2$, followed by a merge with $v_3$ will obtain a superset
of keys needed by $q$.
This merged view is complete with respect to $q$.


\begin{algorithm}[h!]
\caption{$\VF$\label{alg-viewfinder}}
{\small
\begin{algorithmic}[1]
\Function{\sc Init}{$query$, $V$}\label{alg-vf-init}
 \State Priority Queue $PQ$ \qlet $\emptyset$; $Seen$ \qlet $\emptyset$; Query $q$ 
  \State $q$ \qlet $query$
  \ForAll{$v \in V$}
     \State $PQ$.\texttt{add}($v$, $\ocost(q,v))$
  \EndFor
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Peek}{}\label{alg-vf-peek}
%\State \Return ($PQ$.\texttt{peek}().$\ocost$: $\infty$) ? 
\State {\bf if} $PQ$ is not empty {\bf return} $PQ$.\texttt{peek}().$\ocost$ {\bf else} $\infty$
%   \If{not $PQ$.\texttt{empty}()}
%   \State \Return $PQ$.\texttt{peek}().$\ocost$ 
%   \Else 
%   \State \Return $\infty$
%   \EndIf  
\EndFunction
\end{algorithmic}
\Line
\begin{algorithmic}[1]
\Function{\sc Refine}{}\label{alg-vf-refine}
  \If{\texttt{not} $PQ$.\texttt{empty}()}
    \State $v$ \qlet $PQ$.\texttt{pop}()
    \State $M$ \qlet \merge($v$, $Seen$) \Comment{Ensure $Seen \cap M = \emptyset$}
    \ForAll{$v' \in M$}
      \State $PQ$.\texttt{add}($v'$, $\ocost(q,v')$)
    \EndFor
    \State $Seen$.\texttt{add}($v$)
    \If{\complete($q$, $v$)}
      \State \Return $\RE(q, v)$
    \EndIf
  \EndIf \\
  \Return {\sc null}
\EndFunction
\end{algorithmic}}
\end{algorithm}

The outline of the $\VF{}$ algorithm shown in Algorithm~\ref{alg-viewfinder} is as follows.
In \Init{} the \VF{} is instantiated with a $query$ which is assigned to $q$
and a set of materialized views $V$ present in the system, which are added to a priority queue $\PQ$.
$\PQ$ contains candidate views that are ordered by their $\ocost{}$.
At the end of \Init{}, $\PQ$ contains only those candidate views that make up $V$.

The $\Peek{}$ function is used by the $\WF{}$ obtains the $\ocost{}$ of the head item
in the $\PQ$ if one exists.

The $\Refine{}$ function is invoked by the $\WF{}$ when $\WF{}$ decides to ask the $\VF{}$
to examine the next candidate view.
At this stage, the $\VF{}$ pops the head item $v$ out of $\PQ$ 
and generates a set of new candidate views $M$
by merging $v$ with previously popped  candidate views  $Seen$.
Note that $Seen$ contains candidate views that have an $\ocost{}$ 
less than or equal to that of $v$.
$M$ only retains those candidate  that are
not already in $Seen$, which are then inserted into $\PQ$.
% TODO: Need a proof for that statement
A property of $\ocost{}$ provided as a lemma later is that
the candidate views  in $M$ have an
$\ocost{}$ that is greater than that of $v$.
Now, $v$ is added to $Seen$.
If $v$ is guessed to be complete,  we try to find all possible rewrites of $q$
using $v$ by invoking the $\RE$ function.
Among the rewrites found by $\RE{}$, the cheapest rewrite $r$ is returned to $\WF{}$ as the result.
% TODO: Do we need to talk about join ordering?


\subsection{Rewrite Enumeration}\label{sec-rewrite-enumeration}

Suppose that a candidate view $v$ is guessed to be complete.
To determine if an equivalent rewrite exists requires finding at
least one valid rewrite among all possible rewrites,
is known to be a hard problem~\cite{Levy1995}.
In our system the \RE{} algorithm finds an equivalent rewrite
of a query using a given view.
\RE{} takes as input a query $q$ and a view $v$ that is guessed to be complete
and outputs a rewrite $r$ if one exists.
The rewrite $r$ represents the cheapest among
all possible equivalent rewrites of $q$ using $v$.
The cost of a rewrite is evaluated by the \cost{} function,
and corresponds to the cheapest execution \textit{plan} that
implements the rewrite.
Equivalence is determined by ensuring
if both $r$ and $q$ contain the same set of attributes,
same set of filters, and the same final groupby.
%This type of equivalence testing is simple but effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%Although this type of equivalence testing may seem simple it is effective because we produce all possible rewrites
%using $v$, and any perceived shortcoming with the test can be overcome by extending  $L_R$.
%We replace an SPJ+G expression with a single view.  as in GL2001


We search for equivalent
rewrites of $q$ by applying all transformational rules
in $L_R$ to those
views guessed to be complete with respect to the query $q$.
%A transformational rule is a UDF in the system that may
%modify any set of the properties in our UDF model
%which are attributes, filters, and groupbys.
Given the complex interactions possible 
for any arbitrary set of $k$ rules in $L_R$,
it may require generating all possible rewrites of $r$ using $L_R$
before identifying an equivalent rewrite if one exists.
We do this by generating all permutations of the transformational rules,
which can also include multiple applications of the same rule.
This amounts to a brute force enumeration
of all possible rewrites using $v$ given $L_R$, which makes
a case for the system to keep $|L_R|$ small.
When $L_R$ is restricted to a known, fixed 
set of operators it may suffice to examine a polynomial number of 
rewrites such as shown in~\cite{Grum2003} for the specific case 
of simple aggregations involving group-bys.
Such approaches are not applicable to our case as 
the system should have the flexibility of extending $L_R$ with 
any operator from $L_W$ if it results in overall system benefit.

Given the computational complexity of finding valid rewrites,
we limit the invocation of $\RE{}$ algorithm using two strategies.
First, we make good guesses for completeness of a view based
on the three properties described earlier, this
avoids having to apply $\RE{}$ on every $v$. % TODO: Label
Second, we delay the application of $\RE$ to every complete view 
by determining a lower bound on the cost of a rewrite using $v$ should one exist.
For the lower bound we use the $\ocost$, which is described in the next section.
The goal of guessing completeness and estimating a lower bound is
to quickly distinguish between potentially low cost rewrite from those with higher cost.
Note these conditions under-specify the requirements for
determining that a rewrite exists, thus a guess may
result in a false positive, but will never result in a false negative.

\subsection{Determining O\fakesc{pt}C\fakesc{ost}}

Given a candidate view $v$ and a query $q$,
we wish to determine a lower bound on the cost of \textit{any} plan yielded by
an equivalent rewrite of $q$ using $v$ if one exists without enumerating all possible rewrites,
checking for equivalence and examining their plan costs.
We refer to this lower bound as the optimistic cost (\ocost).

There are two possible approaches we can take here.
One approach assumes that we want to materialize $v$ in the process of rewriting the query
and then apply any necessary transformational rules.
Another approach is to allow any necessary transformations 
to be pushed down into $v$ when possible, 
thereby creating $v'$ which may be cheaper to materialize than $v$,
yet more specific in its goal to optimize $q$.
Given the use case of the system, we prefer the first approach as we
wish for the artifacts created (i.e., $v$) to
be as beneficial as possible to the subsequent 
queries by future users.

\ocost takes an optimistic approach in determining the minimum possible plan cost.
Intuitively, it can be seen that any plan yielded by an equivalent rewrite would incur at
the least the sum of
the cost $c'_1$ for accessing all the constituent views in $v$ (i.e., access cost),
the cost $c'_2$ for materializing any new views it requires (i.e., creation cost), and
the cost $c'_3$ of applying the least expensive transformation operation on the view on $v$.
If $v$ is partial (i.e., not guessed to be complete) with respect to $q$,
the $\ocost{}$ is the sum of $c'_1$ and $c'_2$ 
since no operation can transform $v$
to be equivalent to $q$.
\ocost relies on the existence of the $\cost{}$ function, which
estimates the cost of performing operations on views.

Note that if using the push-down approach, 
when the view is partial then \ocost{} is only $c'_1$,
since push-down predicates may change the join ordering.
Further details  of this \ocost{} function 
and our proof of the lower bound property when considering predicate pushdown is 
omitted here due to lack of space.


\begin{comment}
There are certain benefits to both approaches.
The choice to create $v$ is similar to the approach that a view recommender~\cite{Agra2000} might take,
while pushing down predicates into $v$ to create $v'$ is an approach that a query optimizer may take for
answering a single query $q$.
One way to think about this is that $v$ is a recommended view by the $\VF{}$ and here we
decide to piggyback its creation as a part of execution of query $q$.
Given the use case of the system, we prefer this approach as we
wish for the artifacts created (i.e., $v$) as part of answering $q$ to
be as beneficial as possible to the subsequent queries by future users.

The $\VF{}$ could be modified to support predicate pushdown by
modifying $\ocost$ to order partial views by their access cost for $v$ (i.e., $c'_1$).
The pushdown predicates can potentially change the cost of all the joins and their orderings.
\end{comment}


% RETAIN THE REMAINDER OF THIS PROOF HERE. -- REFERS TO APPENDIx
% An $\ocost{}$ function that considers predicate pushdown 
% is given in Appendix~\ref{appendix-pushdown}.

\ocost{} uses the attributes, filters and group-bys representation 
of $q$ and $v$ to
take a set difference between each of these properties.
This denotes a minimum set of non-subsumable operations
by Definition~\ref{definition-non-subsumable-property}
needed to transform $v$'s representation into $q$'s.
We refer to this set as the {\em fix} of $v$ with respect to $q$.
The non-subsumable property allows \ocost{} 
to consider operations in the fix as independent of one another,
although they can still affect each other's cost.
\ocost{} invokes  \cost{} to obtain the cost of 
performing each of the operations in the fix on $v$.
It chooses the least expensive operation in the fix, which
forms the third component $c'_3$ of the \ocost, where
$c'_3$ is given by $\min(\cost(x, v))$ such that
$x$ is an operation in {\em fix}.
\ocost{} then returns $c' = c'_1 + c'_2 + c'_3$, such that
$c'$ is inexpensive to compute and is a lower bound on the cost of \textit{any} plan
returned by $\RE(q,v)$.
% \ocost{} then returns the sum of the create cost $c'_1$, access cost $c'_2$, and the
% minimum operation cost $c'_3$ in the fix as the
% lower bound on the cost of \textit{any} plan.

\begin{theorem}
$c'$ is a lower-bound on on the cost of \textit{any} plan yielded by
an equivalent rewrite of $q$ using $v$ if one exists.
\end{theorem}

\begin{proof}
Let $c$ be the minimum cost plan generated by the $\RE(q,v)$ corresponding
to the rewrite $r$.
$c$ is composed of
the cost $c_1$ for accessing all the views, and
the cost $c_2$ for materializing any new views it requires,
the cost $c_3$ for least expensive ordering of transformation 
rules in $L_R$ applied to $v$.
As $v$ is guessed to be complete for the query $q$,
both $\RE$ and $\ocost$ use $\cost$ to obtain the cost to create and access $v$,
then $c_1 = c'_1$ and $c_2 = c'_2$.

In order to find the lowest cost $r$, $\RE{}$ will have
to enumerate all permutations of rules in $L_R$ required
to achieve the fix.
If \RE{} finds a rewrite, $r$ will have covered all operations in fix,
choosing the cheapest rewrite found to be $c_3$.
$\ocost{}$ uses \cost{} once per each operation in fix
choosing the cheapest as $c'_3$.
As $c'_1$ and $c'_2$ are common to both $c$ and $c'$,
it suffices to show that $c_3 \geq c'_3$.

Recall that \emph{fix} is made up of non-subsumable operations.
A property of two non-subsumable operations as mentioned
earlier in Definition~\ref{definition-non-subsumable-property} is that:
$\cost(xy, D) \geq \min(\cost(x, D),
\cost(y, D))$, where $v$ is an instance of a database $D$, and
$x$, $y$ are operators in fix, and $xy$ performs both $x$ and $y$.

By induction we can show that the cost of the cheapest
rewrite that applies  the fix to $v$
is greater than or equal to $\cost(op^*, v)$, 
where $op^* \in \mbox{\em fix}$
and is the cheapest operator present in the {\em fix} but we
omit the remainder of the induction for lack of space.\qed

\begin{comment} 
% RETAIN THE REMAINDER OF THIS PROOF HERE.
Base Case: Let the fix be denoted by the operators $x$, $y$, $z$,
such that $op^* = z$ is the cheapest operator in fix.
A rewrite $r$  using {\em fix} can
apply operators in the following sequence:
a) apply one operator followed by another or both,
b) apply two operators (e.g., $xz$) followed by a third
operator (e.g., $y$), or
c) apply operators $xyz$ all at once.
For case a) the cost of $r$ is greater than or equal to
either $\cost(x,v)$ or $\cost(y,v)$  or $\cost(z,v)$.
For case b) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(z,v))$ if the first operation
is given by $xz$.
For case c) the cost of $r$ is greater than or equal to
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$.
As $r^*$ represents the lowest cost rewrite across
all rewrites denoted by the three cases, it is bounded by:
$\min(\cost(x,v), \cost(y,v), \cost(z,v))$, which proves
the base case of {\em fix} with 3 operators.

Induction Step:
Let $y$ be the cheapest operation in the set denoted by $\mbox{\em fix}-x$, such that
$\cost(r^*,v) \geq \cost(y,v)$ where $r^*$ corresponds
to lowest cost rewrite on $\mbox{\em fix}-x$.
In other words, the cost of $r^*$ is at least the cost of applying
the cheapest operator in $\mbox{\em fix} -x$.

Add $x$ back to the {\em fix}.
Now, let $r^*$ be the lowest cost rewrite
using {\em fix}.
Suppose that $r^*$ is composed of sets operators $p_1, p_2 \cdots p_k$, such that
$p_1 \cup p_2 \cdots \cup p_k = \mbox{\em fix}$ and
the output of $p_1$ forms the input to $p_2$ and so on.
Then, $\cost(r^*,v) = \cost(p_1, v) + \cost(p_2, v|p_1) + \cdots + \cost(p_k, v|p_1\cdots{}p_{k-1})$,
where $v|p_1$ means that operators in $p_1$ have been applied to $v$.
This means that $\cost(r^*,v) \geq \cost(p_1, v)$ given that $\cost{}$ is always non-negative.
The lowest value of $\cost(p_1,v)$ occurs when $op^*$ is present in
$p_1$ possibly along with other operators in the {\em fix}.
Thus, $op^*$ must either be $y$ which was the cheapest operator in $\mbox{\em fix} - x$
or $op^*$ must equal to $x$.
Then, $\cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$.
Finally, $\cost(r^*,v) \geq \cost(p_1, v) \geq \min(\cost(x, v), \cost(y,v))$. \qed
\end{comment}
\end{proof}

The $\ocost{}$ does not cause the algorithm to lose its optimality property,
regardless of considering an even larger (or pruned)
rewrite space  than the one we consider here.
The utility of $\ocost{}$ is that it 
provides a ``spread''  of the possible rewrites based on 
their optimistic cost.
Thus our expectation of any lower bound is only
that it should provide a reasonable spread 
between the very cheap and very expensive rewrites.
Intuitively, $\ocost{}$ represents a  strategy to avoid 
expanding the search space unnecessarily and also 
 calling $\RE$ on the most promising (lower-cost) candidates first.
The following lemma describes the $\ocost{}$ property
for new candidate views in $M$.
% during Algorithm~\ref{alg-viewfinder}.

\begin{comment}
The lower bound provided by our $\ocost{}$ function could be tightened if we are
willing to commit to a particular execution environment and a specific query optimizer.
For example in an MR environment with a Hive query processor,
given the set of operations in the fix, one could
estimate the minimum number of maps, reduces, and jobs it would take to
apply all operations in fix to $v$.
Such an approach requires intimate knowledge of a specific system,
and thus loses the desired generality of a lower bound estimator.
\end{comment}

%Finally, we provide the following lemma describing the $\ocost{}$ property
%for any new candidate view created in $M$ during Algorithm~\ref{alg-viewfinder}.



\begin{lemma}
The $\ocost{}$ of every candidate view in $M$ that is not in $Seen$
is greater than or equal to the $\ocost{}$ of $v$.
\end{lemma}
\begin{proof}
The proof sketch is as follows. The lemma is trivially true for 
$v \in V$ as all candidate views in $M$ cannot be in $Seen$
and have $\ocost$ greater than $v$. 
If $v$ is a merged view, it is sufficient to point out
that all constituent views of $v$ are already in $Seen$, hence
candidate views in $M$ are already in $Seen$ if smaller, or if greater,
are still in $\PQ$.
\end{proof}

\begin{comment}
% RETAIN THE REMAINDER OF THIS PROOF HERE.
\begin{proof}
Suppose that $v'$ is a new candidate  that is created by merging $v$ with $Seen$.
Then we need only consider the case of $v$ being a base view or a composite view.
If $v$ is a base view (i.e., already materialized), then the $\ocost{}$ of $v'$  cannot be
less than $v$ as $\ocost(v)$ only considers its access cost, while $\ocost(v')$
is at least the cost of accessing $v$ as well as accessing the other candidate view that $v$ is joining with.
If $v$ is a composite view (i.e., $v$ is composed of multiple base views),
then the $\ocost{}$ of $v'$ cannot be less than $v$.
To show that by contradiction,
consider the case where $v'$ is not in $Seen$
and $v'$has a lesser $\ocost{}$ than $v$.
As $v$ is a composite view, then all of its constituent views would already
have been joined with all the candidate views in $Seen$.
Thus, $v'$ must already have been created.
If $v'$ has a lesser $\ocost{}$ than $v$,
it would have already been popped out of $\PQ$ and in $Seen$ before we got to $v$.
\end{proof}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{itemize}


\begin{itemize}
\item Two queries $Q_1$, $Q_2$
are said to be {\em equivalent} if $Q_1 \subseteq Q_2$ and $Q_2 \subseteq Q_1$.
From a query answering perspective,
the set of tuples in the result set of $Q_1$ are identical
to the set of tuples in the result set of $Q_2$.
To determine if an equivalent rewriting using views exists has been already
shown to be in NP even for the class of conjunctive queries~\cite{Hale01}.

\item A query $Q_1$ is said to be {\em contained } by $Q_2$
if $Q_1 \subseteq Q_2$.
From a query answering perspective,
all the tuples in the result set of $Q_1$ are contained in
the result set of $Q_2$, although the result set of $Q_2$ can contain additional
tuples that is not present in the result set of $Q_1$.
The problem finding contained rewriting is also known to NP-complete
even for conjunctive queries~\cite{Hale01-18}.

\end{itemize}

\item A candidate $c$ is said to be {\em complete} with respect to a $Q$ iff $c$ has
has a superset of the attributes and a subset of the filters and
superset of the groupby keys.
If there are attributes in $Q$ that are not present in $c$, $c$ has
the necessary ingredients (i.e., attributes) to obtain $Q$.
Of course, even if $c$ is complete,  it does not mean that
there exists an equivalent rewrite of $Q$ using $c$.
Thus, this provides a necessary but not sufficient
condition that equivalent rewrite exists.
The sufficient condition is when an equivalent
rewrite of $Q$ using $c$ exists.

\item We provide a set of $k$ transformational rules for
query rewriting using a candidate $c$. We call the
rewrite of complete candidate $c$ to a target $t$ using
our transformational rules a {\em chain}.

\item There are three classes of transformational rules that
we allow in the system.



\begin{itemize}
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\item Rules that transform \{A\}, \{F\}, \text{or} \{G\}
\item Rules that transform \{A,F\}, \{F, G\}, \text{or} \{A, G\}
\item Rules that transform \{A, F, G\}
\end{enumerate}
\end{itemize}
\renewcommand{\labelenumi}{\theenumi}


% SJ: Let us add an example here
\item We have 4 transformation rules in our system:
\begin{enumerate}
\item $P$ \textendash Project (class \textsl{i})
\item $F$ \textendash Filter (class \textsl{i})
\item $G$ \textendash Groupby (class \textsl{i} and \textsl{ii})
\item $D$ \textendash Derived (class \textsl{i}, \textsl{ii}, \textsl{iii})
\end{enumerate}

In our $\MinDist$ function presented later, we make the assumption
that each rule can be applied independently.
Furthermore, our algorithm (described later) makes the assumption that the
 Filter rule applies all missing filters, one at a time before completing.
This prevents a large explosion of rule permutations
to apply when searching for a valid rewrite.  However, it presents a limitation on the
ability of our algorithm to find a successful rewrite if one exists.
It may be that no valid rewrite exists using a permutation
of these 4 rules, but one might exist if we consider each missing filter a separate
application of our $F$ transformation rule and thus could produce a successful rewrite such as
$F \rightarrow G \rightarrow F$ whereas due to our restriction of applying all missing filters
with the  $F$ rule before moving to another rule would not be able to produce such a re-write.

The \emph{Derived} rule allows for easy extensions, which is useful for attributes
created by UDFs that can easily be manipulated into other attributes.  For instance, one could add
a derivation that transforms lat-lon into a grid, or positive sentiment with a scoring value of
0.5 to 0.6, or word-count into (approximate) character-count.  Currently we have implemented
several derived attr transformations such as Groupby stats...

\item Determining if a solution $c$ is {\em complete} is  NP-hard
as it involves enumerating all possible chains using the transformation
rules

\item If a candidate is complete we can ``guess''
the minimum number of
transformational rules that go into the chain.
It is minimum ``guess'' as it based on the necessary
condition but not the sufficient condition, so no valid
chain may exist.

\item Why we cannot directly apply the traditional view finding:
  \begin{itemize}
  \item Discarding the non-relevant views using common base relations is not an effective pruning strategy as all queries are posed on a small set of logs, thus many views have the same base relation, a log.
  \end{itemize}
\end{itemize}

\subsection{View Finding Algorithm}

\begin{itemize}

\item Idea of a guess or mindist of a candidate to a target.
\begin{enumerate}
\item Also determine (optimistic guess) complete (winners) vs. partial candidates (losers)
\item Helps prune away the space quickly
\end{enumerate}

\item Describe chain data structure
\begin{enumerate}
\item Series of cmerged or joined candidates, where joined candidates
are restricted to those join predicates that appears in $t$
\item cmerge are keyed equijoins between candidates that shares
common keys
\item joins are equi across different keys or non-keys
\end{enumerate}

\item How to determine mindist?
\item mindist(chain c, t)
\begin{enumerate}
\item Really quick computation
\item Committed cost(c) + guess\_remaining\_cost(c.tail, t)
\item Decouples search from distance computation by assuming independence
\item Magical UDF
\item Claim: Guess is always <= actual cost
\item Finite mindist does not mean existence of chain which
is known to be NP-hard.. (because necessary condition only)
\end{enumerate}

\end{itemize}

Because we explore the solution space incrementally using our MINDIST, we
initialize the viewfinder by registering a target view and a set of candidate
views as follows in Algorithm \ref{viewfinderinit}:

\begin{algorithm}
\caption{ $\VF$-\textsc{initialize}($t$, $C$)}
\label{viewfinder-init}
\begin{algorithmic}[1]
\Require target $t$, candidate pool $C$ % some input
\State {Initialize WinnersPriorityQ, LosersPriorityQ}
\ForAll{$c \in C$}
  \State chain $c' \Leftarrow c$
  \State $d \qlet \MinDist(c', t)$
  \If{$d$ is $\infty$}
    \State LosersPQ.add($c'$, $d$)
  \Else
    \State WinnersPQ.add($c'$, $d$)
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}




\begin{algorithm}
\caption{ $\VF$($t$,\textit{MinCost})}
\label{viewfinder}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ
\State \textsc{mergeables}.\textit{clear()} \\
\Comment {\scriptsize Grow candidate space by merging all (partial view) pairs until the \textsc{committed\_cost} of all Losers is greater than the requested MinCost \normalsize}
\State $m \qlet $ \textit{MinCost}
\While{LosersPQ.peek().committed\_cost $ < m$}
  \State \textsc{mergeables}.\textit{add}( LosersPQ.pop() )
\EndWhile
\State \viewfinderCMerge(\textsc{mergeables})
\While{$ \MinDist$ (Winners.peek()$, t) < m$}
  \State $chain$ $\qlet$ Winners.pop()
  \State   \answer $\qlet$ \viewfinderRefine($chain$, $t$)
  \If {\answer}
    \State $\result$.\textit{add}($\ans$)
  \EndIf
\EndWhile
\State return $\result $

\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{ \viewfinderCMerge(\textsc{mergeables}) }
\label{viewfinder-cmerge}
\begin{algorithmic}[1]
\Require WinnersPriorityQ, LosersPriorityQ \\
\Comment \scriptsize attempt to merge all pairs of views, join order is not considered here \normalsize \\
\Comment \scriptsize This is a keyed equi-join \normalsize
\ForAll{$i \in $ \textsc{mergeables}}
	\ForAll{$j \in $ \textsc{mergeables}}
	  \State $tmp \qlet$\textsl{ColumnMerge}($chain_i$, $chain_j$)
	  \If{$tmp$}
	    \State $newchain \qlet chain_i + chain_j$
	    \State $d \qlet \MinDist(newchain, t)$
	    \State $totalDist \qlet d + newchain$.\textsc{committed\_cost}
        \If{$d$ is $\infty$}
          \State LosersPQ.add($newchain$, $totalDist$)
        \Else
          \State WinnersPQ.add($newchain$,$totalDist$)
        \EndIf
      \EndIf
	\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{ \viewfinderRefine($chain$, $t$)}
\label{viewfinder-refine}
\begin{algorithmic}[1]
\Require transformation rules (P, F, G, D)
\State $P \qlet permutations$(transformation\_rules)
\ForAll{$p \in P$}
  \For {rule $\in p$}
   \State  $newchain \qlet$ \textsc{ApplyRule}(rule, $chain$, $t$)
   \If{$newchain$.\textsl{isEquivalent}($t$)}
     \State return $newchain$
   \EndIf
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\begin{itemize}
\item Mindist allows to look at the existence of shorter chain
first before exploring the longer chains

\item Why best first? Each iteration of the loser pile
keeps merging the chains cost up to $n$ way joins.
We do only two way of joins


\item cmerge is expensive so the cost grows very quickly.
A best first nature means you do not explode your space too much
because the remaining cost fo the minimum people is less than $m$.


\item Don't know there is a rewrite but have to look for  them all
to see which is the cheapest but we take advantage of the fact
that there are multiple opportunities for plumbing at different
targets, which means that if you find a valid rewrite at one target
it immediately bounds the search space of all the targets in the workflow.

\item Mindist allows the incremental exploration of the space in two place
a) Is it winner or loser?
b) Look for short rewrites if they exist
c) Grow the loser partial candidates slowly

\end{itemize}

\subsection{Artifacts}
We call a Materialized View that is created as the output of any query $q \in Q$ an artifact.  We make the assumption that this output is
always written to stable storage in the DFS.

We model an artifact in a minimalistic way as follows.  An artifact is considered to have 3 properties:
\begin{enumerate}
\item Attributes
\item Filters
\item Groupbys
\end{enumerate}


\end{comment}



\begin{comment}
Our system considers every operation as a UDF.
Given that our execution framework is a simple MR system, we identify the types of operations that are possible.
Table \ref{tab:mrops} shows these operations and indicates which phase (Map or Reduce) they can occur.
UDFs may apply any of the operations shown.
Clearly this framework limits the expressivity of UDFs.
Yet many complex UDFs such as ... can still be applied in this framework as shown in example X.
Thus the framework is sufficient for many analytics we consider.
An execution (MapReduce job) may apply filters,
apply projections,
create new attributes via transformations,
or perform aggregations to produce the result.
Given the allowable operations, a result can be modeled as a set of Attributes (\textsf{A}),
a set of filters (\textsf{F}), and group by attributes (\textsf{G}).
We consider \textsf{F} to contain conjunctions of simple selection predicates.
In this model, the result of a equijoin operation appears as an additional filter representing the join predicate.
A result is considered a materialized view in our system (a view extension).

Because UDFs can perform complicated transformations any derived attribute produced must contain
some metadata about itself.
Consequently each attribute has a \textit{signature}, which is a minimal form of provenance that captures the nature of the
view's direct input in terms of \textsf{A}, \textsf{F}, \textsf{G} along with some other small metadata such as the operation applied
(UDF name) to the input to produce the view.

This representation enables us to easily understand UDF as a grey box, rather than a black box.
It is considered to be grey since we don't really understand what the function actually does,
we only understand the label of the function and what the input and output look like.
This means that two identical functions with different labels will not appear identical to our model.
Or UDFs that may subsume each other will not be identified.
Our method is extensible toward a more fine-grained understanding of the function where some UDFs may become a white box.
This requires additional complexity while here we focus on the usefulness of our method
even on the level of understanding a UDF as a grey box.

We now define our grammar that is used by all UDFs.
All UDFs operations are described in this grammar.
A UDF takes at least one view as input and produces a view as output.
To understand a UDF as a grey box, each attribute created by a
UDF records the following metadata describing itself.
\begin{enumerate}
\item {\sf B} - the name of the UDF that produced the attribute
\item {\sf M} - a modifier argument given to the UDF (if any)
\item {\sf A} - the input attributes to the UDF
\item {\sf F} - the filters previously applied to the input
\item {\sf G} - the group-bys previously applied to the input
\end{enumerate}

The output of the UDF is a materialized view which is described
in terms of \textsf{A}, \textsf{F}, \textsf{G}.
The grammar of the UDF must describe the transformations from
{\sf B, M, A, F, G} to {\sf A, F, G}.
\end{comment}



==> old/macros.old.tex <==

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{lemma}{lemma}
\newtheorem{assumption}{Assumption}

% Onefig macro
\newcommand{\onefig}[3]{
 \begin{figure}[h!]
 \vspace{-0.1in}
  \centering % SJ: Apparently, \centering is more space efficient that \begin{center}
% \begin{center}
    \includegraphics[width=#3]{#1}
    \vspace{-0.1in}
    \caption{\label{#1}#2}
    \vspace{-0.13in}
% \end{center}
 \end{figure}
}

\newcommand{\twofig}[4]{
 \begin{figure}[h!]
 \vspace{-0.1in}
 \centering
    \includegraphics[width=#4]{#1}%
    \includegraphics[width=#4]{#2}\\
    \vspace{-0.06in}
    {\tiny{\hspace{0.3in}{\sf (a)}\hspace{#4}\hspace{-0.1in}{\sf (b)}}}
    \vspace{-0.13in}
    \caption{\label{#1}{#3}}
 \vspace{-0.13in}
 \end{figure}
}

\newcommand{\threefig}[5]{
 \begin{figure}[h!]
 \vspace{-0.1in}
\begin{minipage}{1.05\columnwidth}
\centering
    \includegraphics[width=#5]{#1}%
    \includegraphics[width=#5]{#2}%
    \includegraphics[width=#5]{#3}\\
    \vspace{-0.06in}
    {\tiny{\hspace{0.3in}{\sf (a)}\hspace{#5}\hspace{-0.1in}{\sf (b)}\hspace{#5}\hspace{-0.1in}{\sf (c)}}}
\end{minipage}
 \vspace{-0.2in}
    \caption{\label{#1}#4}
 \vspace{-0.1in}
 \end{figure}
}

\newcommand{\fourfig}[6]{
 \begin{figure}
\centering%
    \includegraphics[width=#6]{#1}%
    \includegraphics[width=#6]{#2}\\
    \vspace{-0.05in}%
    {\tiny{{\sf (a)}\hspace{#6}{\sf (b)}}}\\
    \vspace{-0.05in}%
    \includegraphics[width=#6]{#3}%
    \includegraphics[width=#6]{#4}\\
    \vspace{-0.1in}%
    {\tiny{{\sf (c)}\hspace{#6}{\sf (d)}}}\\
    \vspace{-0.1in}
    \caption{\label{#1}#5}
 \vspace{-0.15in}
 \end{figure}
}

\newcommand{\fourfigonerow}[6]{
 \begin{figure}
\centering%
    \hspace{-0.25in}\includegraphics[width=#6]{#1}\hspace{-0.17in}%
    \includegraphics[width=#6]{#2}\hspace{-0.17in}%
    \includegraphics[width=#6]{#3}\hspace{-0.17in}%
    \includegraphics[width=#6]{#4}\hspace{-0.5in}\\
    \vspace{-0.1in}%
    \centering{\tiny{{\sf (a)}\hspace{#6}\hspace{-0.17in}{\sf (b)}\hspace{#6}\hspace{-0.17in}{\sf (c)}\hspace{#6}\hspace{-0.17in}{\sf (d)}}}\\
    \vspace{-0.1in}
    \caption{\label{#1}#5}
 \vspace{-0.15in}
 \end{figure}
}

\newcommand{\onetabletwocol}[3]{
  \begin{table*}
  \centering
 \caption{#2\label{#1}}
  \scriptsize #3
    \end{table*}
}

% Macro to fix the intendation of the comments
\renewcommand{\algorithmicforall}{\textbf{for each}}
\renewcommand{\algorithmicindent}{8pt}
\newcommand{\Line}{\vspace{-0.08in}\hrulefill\vspace{-0.04in}}
\algblock[Init]{Init}{EndInit}

\newcommand{\up}{\ensuremath{\mbox{\sc up}}}
\newcommand{\down}{\ensuremath{\mbox{\sc down}}}
\newcommand{\updown}{\ensuremath{\mbox{\sc updown}}}
\newcommand{\dir}{\ensuremath{\mbox{\sc dir}}}

\newcommand{\true}{\ensuremath{\mbox{\sc true}}}
\newcommand{\false}{\ensuremath{\mbox{\sc false}}}
\newcommand{\MaxDist}{\ensuremath{\mbox{\sc Max\-Dist}}}

\newcommand{\MinDist}{\ensuremath{\mbox{\sc Min\-Dist}}}
\newcommand{\seenSoFar}{\ensuremath{\mbox{\sc expl\-Cst}}}
\newcommand{\plans}{\ensuremath{\mbox{\sc plans}}}

% Remove me
\newcommand{\result}{\ensuremath{\mbox{\sc plans}}}

\newcommand{\BestFirstWorkflowRewrite}{\ensuremath{\mbox{\sc Best\-First\-Rewrite}}}
\newcommand{\WorkflowRewrite}{\ensuremath{\mbox{\sc Work\-Flow\-Rewrite}}}
\newcommand{\WFR}{\ensuremath{\mbox{\sc Work\-Flow\-Rewrite}}}
\newcommand{\WF}{\ensuremath{\mbox{\sc Work\-Flow\-Rewrite\xspace}}}
\newcommand{\ApplyBottomUpPlanRewrite}{\ensuremath{\mbox{\sc Apply\-Bottom\-Up\-Plan\-Rewrite}}}

\newcommand{\minCost}{\ensuremath{\mbox{\sc bst\-Pln\-Cst}}}
\newcommand{\complete}{\ensuremath{\mbox{\sc GuessComplete}}}
\newcommand{\merge}{\ensuremath{\mbox{\sc Merge}}}
\newcommand{\minPlumb}{\ensuremath{\mbox{\sc bst\-Pln}}}

\newcommand{\PropagateBestRewrites}{\ensuremath{\mbox{\sc Propagate\-Best\-Rewrites}}}
\newcommand{\PropagateStats}{\ensuremath{\mbox{\sc Propagate\-Stats}}}
\newcommand{\ComputeMinCostEstimate}{\ensuremath{\mbox{\sc Compute\-Opt\-Plan\-Cost\-Estimate}}}
\newcommand{\RefineTarget}{\ensuremath{\mbox{\sc Refine\-Target}}}
\newcommand{\ViewFinder}{\ensuremath{\mbox{\sc View\-Finder}}}
\newcommand{\VF}{\ensuremath{\mbox{\sc View\-Finder\xspace}}}
\newcommand{\ViewFinderRegister}{\ensuremath{\mbox{\sc View\-Finder\-Register}}}
\newcommand{\CheapPlumbing}{\ensuremath{\mbox{\sc Cheap\-Plumbing}}}
\newcommand{\EstimateCost}{\ensuremath{\mbox{\sc Estimate\-Cost}}}
\newcommand{\plumbHere}{\ensuremath{\mbox{\sc plumb\-Here}}}

\newcommand{\cost}{\ensuremath{\mbox{\sc Cost}}}
\newcommand{\ocost}{\ensuremath{\mbox{\sc OptCost }}}
\newcommand{\qlet}{\ensuremath{\leftarrow}}
\newcommand{\ans}{\ensuremath{\mbox{\sc Ansc}}}
\newcommand{\answer}{\ensuremath{\mbox{\sc answer}}}
\newcommand{\viewfinderRefine}{\ensuremath{\mbox{\sc ViewFinder-Refine}}}
\newcommand{\viewfinderCMerge}{\ensuremath{\mbox{\sc ViewFinder-CMerge}}}

\newcommand{\RE}{\ensuremath{\mbox{\sc Rewrite\-Enumerator}\xspace}}
\newcommand{\PQ}{\ensuremath{\mbox{PQ}}}
\newcommand{\PQW}{\ensuremath{\mbox{PQ}_{\mbox{\sc\tiny c}}}}
\newcommand{\PQL}{\ensuremath{\mbox{PQ}_{\mbox{\sc\tiny p}}}}
\newcommand{\FindNextMinTarget}{\ensuremath{\mbox{\sc Find\-Next\-Min\-Target}}}

\renewcommand{\Init}{\ensuremath{\mbox{\sc Init}}}
\newcommand{\Peek}{\ensuremath{\mbox{\sc Peek}}}
\newcommand{\Refine}{\ensuremath{\mbox{\sc Refine}}}

\newcommand{\A}{\ensuremath{\mbox{\sc A}}}
\newcommand{\F}{\ensuremath{\mbox{\sc F}}}
\newcommand{\G}{\ensuremath{\mbox{\sc G}}}

\newcommand{\node}[1]{\ensuremath{\mbox{\sc node}_{#1}}}


%\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}


==> old/mindist.tex <==

Given a workflow $W$ 


For any UDF in our system, the author of the UDF expresses the 
UDF in terms of how many jobs, maps, reduce, shuffle processes
are performed by the UDF. 

Optimistic cost 




==> old/notes.tex <==
1.  Provable ?   (discussion follows below for A and B)
A.  Allowing no filter pushdown
B.  Allowing filter pushdown

2.  Is lower bound useful?

% SJ: A good argument here should focus on what 
% can we show here given a minimal assumption of the nature
% of a cost model

% What is CM is a cost model, vs. Query Optimizer vs. a more
% intricate knowledge of the plan it produces.

Consider the projection of all views onto a 1-D axis 
based on their expected cost. 
Assume a lower bound of zero on the cost of a rewrite using v. 
For every view in V, project it onto the axis based on their expected cost.
All views will project onto the same point on axis.
Thus if we are only looking a rewrite with cost less than d, we must start will all the views whose cost is zero, and check every one to determine if it is less than d.
Computational complexity to explore this is in size of V plus the exponential size of merging all views in V, and enumerating their rewrites.  This is very expensive, and there is no pruning of V.  Which means you must produce everything possible from everything existing and attempt to find a rewrite with everything you found.
Assume a non-zero lower bound on the cost of a rewrite using v.
For all v in V, project each onto the axis based on its lower bound cost.
Given their lower bounds are not all identical, they should fall into different places along the axis. 
This is the “spread” of the views in based on their expected costs.
If we are looking for a rewrite with cost < d, we only need to consider those views that lie on the axis at a value < d, call this set V’.
Then we must find a rewrite with only those views in V’.  
Depending on the spread, V’ < V, or V’ <<V.
Thus we have pruned V.
Furthermore, by judiciously growing the loser pile only until all merges have a cost > d, we avoid enumerating more merged views than necessary.
Note that we still may need to do them all, but the lower bound allows us to grow the space slowly, and also allows us to have an early termination condition if we desire.

3.  Is lower bound tight?

A. Needs to be correct.   i.e. c’ <= c.
c’ is lower bound cost.
c is actual cost.
B.  Must only help us to quickly distinguish between very bad rewrites and very good rewrites.
This is because we have n rewrite search problems.  And if the search at any n can be correctly restricted, this reduces the sum of the global search space explored.  This is important as it depends on size n (a small integer), and depends on size of V, which could be a much larger integer.
C.  Its tightness can be refined as much as possible while not violating correctness, but even a loose one enables B, which is beneficial.  Tightening it to be very tight involves a lot of added complexity, which is possible, but we choose to avoid this as long as it serves the purpose of B well.  

OPTCOST 

Allow no filter/project pushdowns.

$D' \subseteq D$, $\cost(q, D') \leq \cost(q, D)$, where
$D$ is a database instance. (property 1.0c)

Suppose the queries are made up of operators that cannot be 
not subsumed by one another.  (property1.0b)

$\cost(\mbox{op}_{12}, D) \geq \min(\cost(\mbox{op}_1, D),
\cost(\mbox{op}_2, D))$, where 
$\mbox{op}_1$ and $\mbox{op}_2$ are operators
and $\mbox{op}_{12}$ performs both $\mbox{op}_1$ and $\mbox{op}_2$.

% SJ: We could potentially improve this further by assuming more
% about the property of the CM.

NOTE: when considering the fix for A,F,G: we mean the symmetric difference, the items in one or the other but not both.  http://mathworld.wolfram.com/SymmetricDifference.html
A-B is just the complement, or set difference.
symm_diff (v,q) contains {x}, {y}, {z}, corresponding to all operators in A, F, G.

$S$ = $x U y U z$
S is said to the fix.
The fix is the compensation operations to transform v into q.

$\cost(S, v) \geq \cost (min-op in S, v)$
s.t. min-op in S, and min-op = MIN[cost(op_i,v)] 
for all op_i=1 to |S| in S

Suppose S contains x, y.
Then assuming x and y do not subsume each other (property1.0b), we have 3 options for completing the fix.
1. v->x->y
2. v->y->x
3. v->(xy)

Let D’ = x(D)
Let D” = y(D)
Then given property 1.0a, 
D’ \subseteq D 
D” \subesteq D
and cost(x,D’) <= cost(x,D)
and cost(y,D”) <= cost(y,D”)

The we can say:
cost(1) = cost(x,D) + cost(y,D’).
cost(2) = cost(y,D) + cost(x, D’’).  
cost(3) = cost(xy,D)

Then, 
a. cost(1) >= cost(x,D) by property 1.0b
b. cost(2) >= cost(y,D) by property 1.0b
c. cost(3) >= cost(1) by property 1.1
   cost(3) >= cost(2)) by property 1.1

Given 1,2,3 are our only choices to complete the fix, 
then MIN(cost(1), cost(2), cost(3))  (the lower bound we desire)
is exactly MIN(cost(1), cost(2)) by (c) above. 
This represents the minimum cost of any op in the fix (S) on v.  
Tie the S back in here with min-op.


5.  Further arguments for no allowing pushdowns (this case):
a.  we don't want to push down a filter into v, since v could be useful in answering future queries.
if we choose to store the complete view v, and we also store the rewrite(q,v) which  finally produces v_q, then v may be a useful view for queries other than q.  But if v contains a filter, call this v_f, this makes v_f rather than v, and since filters cannot be removed, v_f is less-sharable than v.
Argue that our goal is maximum sharability, since we are going to create some version of v anyway in the process of answering q, we should prefer to create the more sharable version of v, which is not v_f.
v could be retain and all constituent views of v can be dropped by a garbage collector, using some metric like v ~= views and completely covers q.

I think here we might like to argue that v can potentially contain more possible queries than v_f, maybe based on the fact the v_f \subseteq v.  Some theoretical reference may show that the universe of queries answerable by some instance I’ is contained by the universe of queries answerable by another instance I when I’ \subseteq I.
Maybe (|Q|,I’) <= (|Q|,I)  for any Q.  ?





OPTCOST 
1B.  Allow filter pushdowns.

1.  order PQ_L by AccessCost(v) only.  Do not consider join cost.
This means that any join order of  v1,v2,v3 has the same cost as any other join order, which is simply the sum of their individual access costs.

2.  Keep views as sets in PQ_P as sets (v1 join v2 join v3) is simply represented as a set of views
{v1,v2,v3}
Call this set v123.

3.  Filter and project are the only operators considered for push down. 
---SIDE NOTE: we could also restrict the RE pushdown operators to only consider the subset of FA that a greedy optimizer actually did push down.  note that we decided this is probably not required since we say that RE exhaustively enumerates all join orderings for v123 considering the same FA. ---

4.  RE is expanded (RE-expanded) to consider join ordering given its set of constituent views and the FA in the fix.  Note this means the input to RE is no longer a complete view v, but is a set of views, i.e. v123.  After RE attempts all possible pushdowns of FA with all possible join orderings, it can then attempt apply the remaining transformations required in the fix.  This generates all successful rewrites r+, and from those the lowest cost rewrite, r* is returned by RE.


5.  
let f be equal to the original fix.
let f’ \subseteq f where f’ = f - {G,D}
let f” \subseteq f where f"= f - {G}
let f1 \subseteq f, where f1 are the remaining ops in fix after creating v2
let f2 \subseteq f, where f1 are the remaining ops in fix after creating v3

We want to prove the following inequality:
cost-to-create(v2, GREEDY) + optcost(v2, f1)  
<= cost-to-create(v3, RE-Expanded) + opcost(v3, f2) 
<= cost(r*, V, RE)

Let:
S1 = cost-to-create(v2)
S2 =  opcost(v2, f1)
S12 = S1+S2
S3 = cost-to-create(v3) 
S4 = opcost(v3, f2)
S34 = S3 +S4
S5 = cost(r*, V, RE)


Note we may need to state that v123 is the guessed to be complete view v, which itself is in V or is composed of views in V.  -- in order to relate this to r* on something, which is what the VIEWFINDER solves  i.e. VF(q,V) ==> r*, cost(r*).

6.  We should state that given a guessed to be complete set of views is v123 = {v1,v2,v3}.

Assumption A0:  GREEDY and RE-Expanded to be able to compute the dependencies of items in the fixes given to them  (f’ and f” respectively).

Property A. GREEDY and RE-Expanded must join all views in v123.

Property B. GREEDY and RE-Expanded must push down all filters or projects they can based on their dependencies, given assumption A0.


Create v2: 
v123, {f’} ==> GREEDY ==> v2, f1

Create V3:
v123, {f”} ==> RE-Expanded => v3 , f2  note that f” contains D where f’ does not.

f1 = remaining filters GREEDY could not push down, and f1 <= f’ <= f
f2 = remaining filters RE-Expanded could not push down, and f2 <=f”<= f.

GREEDY (exhaustively) enumerates all join orders on all pushdowns given its known dependency constraints in f’.
RE-Expanded exhaustively enumerates all join orders on all pushdowns given it’s known dependency constraints in f".


Due to additional dependency constraints:
P0:  f1 <= f2;  by property B

Note that the result v3 contains all of the joins that v2 does, but v3 may have fewer filters due to a constraint on D that RE-Expanded was aware of that disallowed a push.

Assumption A1:  pushing operators has a cost benefit to a subsequent join operation.
Assumption A2:  pushdown-op(v) ==> v’ where v’ <= v in size, where a pushdown-op is an op that can result in a data size reduction.  i.e. F(D) = D’, and D’ \subseteq D.  Maybe we should simply state that a pushdown-op applied to some D always results in a D’ \subseteq D.

Note Property A says we must perform all joins.
Note Property B says we must push down all ops possible that reduce a join cost.

Then:
C1: cost-to-create(v2) <= cost-to-create(v3) by properties {A, B}, assumption A1, and PremiseP0.

C2: |v2| <= |v3| by properties{A, B}, assumptions {A1,A2} and Premise P0. 
Note that if there are no UDFs (i.e. no D) then v2==v3 since f” and f’ have the same fix (f"==f’) and since GREEDY and RE-Expanded are given the same set of views v123 and the same fix, the pushdown ops will be exactly the same so that is why v2==v3 would be true.

7.  
P3: optcost(v2, f1) <= optcost(v2,f2) ; by P0 and the OPTCOST definition of choosing the 
min-op in the fix provided to it.  See previous section on OPTCOST property of lower bound.

P4: optcost(v2, f2) <= optcost(v3,f2); by L2.  

Then:
C5: optcost(v2, f1) <= optcost(v2, f2) <= optcost(v3,f2); by P3 and P4.

Now we should be able to do the substitution  for S1,S2,S3,S4,S5 in the original statement we wanted to prove in #5.  Hopefully these conclusions C1,C2,C3 are complete for that purpose, else we can add whatever is missing.














==> old/viewfinder.bbl.tex <==

\begin{thebibliography}{10}\setlength{\parsep}{0pt}\setlength{\itemsep}{0pt}

\bibitem{Abit1998}
S.~Abiteboul and O.~M. Duschka.
\newblock Complexity of answering queries using materialized views.
\newblock In {\em PODS}, 1998.

\bibitem{Agra2000}
S.~Agrawal, S.~Chaudhuri, and V.~Narasayya.
\newblock Automated selection of materialized views and indexes in sql
  databases.
\newblock In {\em VLDB}, 2000.

\bibitem{Bryn2011}
E.~Brynjolfsson, L.~M. Hitt, and H.~H. Kim.
\newblock Strength in numbers: How does data-driven decision making affect firm
  performance?
\newblock {\em SSRN eLibrary}, 2011.

\bibitem{Chan1977}
A.~Chandra and P.~M. Merlin.
\newblock Optimal implementation of conjunctive queries in relational data
  bases.
\newblock In {\em STOC}, 1977.

\bibitem{Elgh2012}
I.~Elghandour and A.~Aboulnaga.
\newblock Restore: reusing results of mapreduce jobs.
\newblock {\em VLDB}, 5(6), 2012.

\bibitem{Gold2001}
J.~Goldstein and P.-A. Larson.
\newblock Optimizing queries using materialized views: {A} practical, scalable
  solution.
\newblock In {\em SIGMOD}, 2001.

\bibitem{Grum2003}
S.~Grumbach and L.~Tininini.
\newblock On the content of materialized aggregate views.
\newblock In {\em PODS}, 2000.

\bibitem{Hale2001}
A.~Halevy.
\newblock Answering queries using views: A survey.
\newblock {\em VLDBJ}, 10(4), 2001.

\bibitem{Khou2009}
N.~Khoussainova, M.~Balazinska, W.~Gatterbauer, Y.~Kwon, and D.~Suciu.
\newblock A case for a collaborative query management system.
\newblock CIDR, 2009.

\bibitem{Konst2012}
G.~Konstantinidis and J.~Ambite.
\newblock Optimizing query rewriting for multiple queries.
\newblock In {\em IIWeb}, 2012.

\bibitem{Konst2011}
G.~Konstantinidis and J.~L. Ambite.
\newblock Scalable query rewriting: a graph-based approach.
\newblock In {\em SIGMOD}, 2011.

\bibitem{Schn2007}
K.Schnaitter, S.~Abiteboul, T.~Milo, and N.~Polyzotis.
\newblock On-line index selection for shifting workloads.
\newblock In {\em SMDB}, 2007.

\bibitem{Levy1995}
A.~Y. Levy, A.~O. Mendelzon, and Y.~Sagiv.
\newblock Answering queries using views (extended abstract).
\newblock In {\em PODS}, 1995.

\bibitem{Li2011}
B.~Li, E.~Mazur, Y.~Diao, A.~Mc{G}regor, and P.~Shenoy.
\newblock A platform for scalable one-pass analytics using mapreduce.
\newblock In {\em SIGMOD}, 2011.

\bibitem{Mami2012}
I.~Mami and Z.~Bellahsene.
\newblock A survey of view selection methods.
\newblock {\em SIGMOD Rec.}, 41(1), 2012.

\bibitem{Nyki2010}
T.~Nykiel, M.~Potamias, C.~Mishra, G.~Kollios, and N.~Koudas.
\newblock {MRS}hare: sharing across multiple queries in mapreduce.
\newblock {\em VLDB}, 3(1-2), 2010.

\bibitem{Pati2011}
D.~Patil.
\newblock {\em {Building Data Science Teams}}.
\newblock O'Reilly Media, 2011.

\bibitem{Pott2001}
R.~Pottinger and A.~Halevy.
\newblock Minicon: A scalable algorithm for answering queries using views.
\newblock {\em VLDB}, 10(2), 2001.

\bibitem{Simi2009}
A.~Simitsis, K.~Wilkinson, M.~Castellanos, and U.~Dayal.
\newblock {QoX}-driven {ETL} design: Reducing the cost of {ETL} consulting
  engagements.
\newblock In {\em SIGMOD}, 2009.

\bibitem{Thus2009}
A.~Thusoo, J.~S. Sarma, N.~Jain, Z.~Shao, P.~Chakka, S.~Anthony, H.~Liu,
  P.~Wyckoff, and R.~Murthy.
\newblock Hive: {A} warehousing solution over a map-reduce framework.
\newblock {\em VLDB}, 2(2), 2009.

\bibitem{tpcds}
{Transaction Performance Council}.
\newblock {TPC-H and TPC-DS Benchmarks}.

\bibitem{Sell1988}
T.~Sellis.
\newblock Multiple-Query Optimization.
\newblock {\em ACM Trans. on Database Systems}, 13(1), 1988.


\bibitem{Hues2012}
F. Hueske, M. Peters, M. Sax, A. Rheinl\"{a}nder, R. Bergmann, A. Krettek, and K. Tzoumas.
\newblock Opening the black boxes in data flow optimization.
\newblock {\em VLDB}, 5(11), 2012.
 
\end{thebibliography}


==> pushdowns-proof.tex <==
To keep the $\cost{}$ function inexpensive, our model does not consider re-ordering
of joins, predicate push down, or other types of optimizations involved in
group bys and udfs, but does merge sequential operations (e.g. a sequence of filters)
into the same job whenever possible.


This is a reasonable approach given that we have already committed to creating $v$,
and the $\RE{}$ explores all possible rewrites, such a cost function serves
our purposes here.

An extension to this basic cost model could consider push downs when computing the cost
to create $v$.  The requirements to including push-downs into the optimization
process would be to employ a cost model $\cost{}$ that is able to
apply all possible join orderings to creating $v$ along with applying filters
to all orders.

Appendix~\ref{appendix-pushdown} provides a proof for using $\RE{}$ and $\ocost$ with an extended
$\cost{}$ function that considers join ordering and predicate pushdowns,
while still producing a correct lower bound for $\RE{(v,q)}$.

There are 2 reasons we do not consider predicate push downs here.
First $\cost{}$ becomes much more expensive to invoke due to considering all
of the ordering options.
Second, we may not wish to push down a filter into $v$ since this could render $v$
less useful for answering future queries.
A more sophisticated algorithm could weigh the cost and benefits of different
versions of $v$ (with and without filters) given their benefit to other queries
and their added cost due to avoiding filter push downs.


==> sec-scenario-no-plug.tex <==
\begin{table*}[!t]
\caption{\label{tab-experiment-scenarios}Eight analyst marketing scenarios used in evaluation}
%\small{
\centering
%\begin{tabular}{| p{0.70\linewidth} | p{0.30\linewidth}|}
\begin{tabular}{| p{1.02\linewidth}|}
\hline                        
 Analyst 1 wants to find influential users who are
interested in food for an advertisement campaign.
The evolution of this scenario includes increasingly
sophisticated interpretations of what it means to be ``influential''. 
\\\hline
 Analyst2 wants to identity 100 ``wine lovers'' to
send them a coupon for a new wine being introduced. 
This evolution investigates ways of finding suitable users to whom
sending a coupon would have the most impact.
\\ \hline
 Analyst3 wants to start a gift recommendation service where friends
can send a gift certificate to a user $u$.
We want to generate a few restaurant choices based on $u$'s preferences.
The evolution in this scenario will investigate how to 
generate a diverse set of recommendations that would cater to $u$ and 
his close set of friends.
\\ \hline
Analyst4 wants to identify a good area to locate a sports bar.
The area must have a lot of people who like sports and check-in to bars, 
but the area does not already have too many sports bars
in relation to other areas.
The evolution focuses on identifying a suitable area where
there is good interest but low density of sports
bars.\looseness=-1
% Analyst4 wants to provide restaurants with a breakdown of their
%customer population. 
%In particular, the analyst wants to provide breakdowns in terms of who goes to a
%particular restaurant.
%The analyst may also want to perform analysis in terms for geographical area.
%For instance, for any area which are the popular restaurants by categories etc.
%The goal of this scenario is to perform increasingly complicated analytical 
%operations on the log.
\\ \hline
 Analyst5 wants to give restaurant owners a customer poaching tool.
For each restaurant $r$, we identify customers who go to a ``similar'' 
restaurant in the area but do not visit $r$.
The owner of $r$ may use this to target advertisements.
The evolutionary nature focuses on determining ``similar'' restaurants and their users. 
\\ \hline
 Analyst6 tries to find out if restaurants are losing loyal customers.
He wants to identify those customers 
who used to visit more frequently but are now visiting other restaurants in the area
so that he can send them a coupon to win them back.
The evolutionary nature of this scenario will focus on 
how to identify prior active users.\looseness=-1
\\ \hline
 Analyst7 wants to identify the direct competition for each restaurant.
He first tries to determine if there is a more successful restaurant 
of similar type in the same area.
The evolutionary nature focuses on identifying what customers 
like about the menu, food, service, etc. that makes 
these restaurants successful.
\\ \hline
%Analyst8 wants to identity what category (i.e., american, indian,
%chinese, steak) of restaurants is missing from a
%certain region. For example, one of the outcome can be that 
%Cupertino could really use a Moroccan restaurant. 
%The evolutionary nature of this scenario will focus on how to 
%find out if there is a need for a good restaurant in a certain
%category and if so what is the nature of their clientele etc.
%&
%$Q \rightarrow \{x,x,x\} \rightarrow \{x,x,x\} \rightarrow \{x,x,x\}$
%\\ \hline
Analyst8 wants to recommend a high-end hotel vacation in an area users will
like based on their known preferences for restaurants, theaters, and luxury items.
The evolutionary nature focuses on matching user's
preferences with the types of businesses in an area.
%Analyst8 wants to recommend a high-end hotel vacation to affluent people.
%This involves finding users who like luxury items 
%and like to travel, and identifying the types of locations such as
%restaurants or theater these clientele frequent in their local areas.  
%Then the analyst determines the density of these same types 
%of locations per global cell grid.
%The analyst can then send a coupon to those users for a high-end
%hotel with a high density of nearby activities that user would like.
%The evolutionary nature of this scenario is how to identify
%users who like luxury items and events and find a grid cell location 
%with a luxury hotel that has these same activities for a given user.
\\ \hline
\end{tabular}
%}
\vspace{-0.2in}
\end{table*}


==> sec-scenario.tex <==
\begin{table*}[!t]
\caption{\label{tab-experiment-scenarios}Eight scenarios used in evaluation, 
along with the dimensions modified during each of the 4 evolutions}
%\small{
\centering
\begin{tabular}{| p{0.70\linewidth} | p{0.30\linewidth}|}
\hline                        
 Analyst 1 wants to find influential users who are
interested in food for an advertisement campaign.
The evolution of this scenario includes increasingly
sophisticated interpretations of what it means to be ``influential''. 
& 
$Q \rightarrow \{P,G\} \rightarrow \{P,L,G\} \rightarrow \{P,G\}$
\\\hline

 Analyst2 wants to identity 100 ``wine lovers'' to
send them a coupon for a new wine being introduced. 
This evolution investigates ways of finding suitable users to whom
sending a coupon would have the most impact.
&
$Q \rightarrow \{P,L,G\} \rightarrow \{P,G\} \rightarrow \{P,U,G\}$
\\ \hline

 Analyst3 wants to start a gift recommendation service where friends
can send a gift certificate to a user $u$.
We want to generate a few restaurant choices based on $u$'s preferences.
The evolution in this scenario will investigate how to 
generate a diverse set of recommendations that would cater to $u$ and 
his close set of friends.
&
$Q \rightarrow \{P,G\} \rightarrow \{P,U,G\} \rightarrow \{P,G\}$
\\ \hline

Analyst4 wants to identify a good area to locate a sports bar.
The area must have a lot of people who like sports and check-in to bars, 
but the area does not already have too many sports bars
in relation to other areas.
The evolution focuses on identifying a suitable area where
there is high interest but a low density of sports
bars.
% Analyst4 wants to provide restaurants with a breakdown of their
%customer population. 
%In particular, the analyst wants to provide breakdowns in terms of who goes to a
%particular restaurant.
%The analyst may also want to perform analysis in terms for geographical area.
%For instance, for any area which are the popular restaurants by categories etc.
%The goal of this scenario is to perform increasingly complicated analytical 
%operations on the log.
&
$Q \rightarrow \{U,G\} \rightarrow \{L,G\} \rightarrow \{P\}$
\\ \hline

 Analyst5 wants to give restaurant owners a customer poaching tool.
For each restaurant $r$, we identify customers who go to a ``similar'' 
restaurant in the area but do not visit $r$.
The owner of $r$ may use this to target advertisements.
The evolutionary nature focuses on determining ``similar'' restaurants and their users. 
&
$Q \rightarrow \{P,L,U,G\} \rightarrow \{P,L,G\} \rightarrow \{P,G\}$
\\ \hline

 Analyst6 tries to find out if restaurants are losing loyal customers.
He wants to identify those customers 
who used to visit more frequently but are now visiting other restaurants in the area
so that he can send them a coupon to win them back.
The evolutionary nature of this scenario will focus on 
how to identify prior active users. 
&
$Q \rightarrow \{P,L,G\} \rightarrow \{P\} \rightarrow \{P,G\}$
\\ \hline

 Analyst7 wants to identify the direct competition for each restaurant.
He first tries to determine if there is a more successful restaurant 
of similar type in the same area.
The evolutionary nature focuses on identifying what customers 
like about the menu, food, service, etc. that makes 
these restaurants successful.
&
$Q \rightarrow \{U,G\} \rightarrow \{P,G\} \rightarrow \{P,U,G\}$
\\ \hline

%Analyst8 wants to identity what category (i.e., american, indian,
%chinese, steak) of restaurants is missing from a
%certain region. For example, one of the outcome can be that 
%Cupertino could really use a Moroccan restaurant. 
%The evolutionary nature of this scenario will focus on how to 
%find out if there is a need for a good restaurant in a certain
%category and if so what is the nature of their clientele etc.
%&
%$Q \rightarrow \{x,x,x\} \rightarrow \{x,x,x\} \rightarrow \{x,x,x\}$
%\\ \hline

Analyst8 wants to recommend a high-end hotel vacation in an area users will
like based on their known preferences for restaurants, theaters, and luxury items.
The evolutionary nature focuses on matching user's
preferences with the types of businesses in an area.
%Analyst8 wants to recommend a high-end hotel vacation to affluent people.
%This involves finding users who like luxury items 
%and like to travel, and identifying the types of locations such as
%restaurants or theater these clientele frequent in their local areas.  
%Then the analyst determines the density of these same types 
%of locations per global cell grid.
%The analyst can then send a coupon to those users for a high-end
%hotel with a high density of nearby activities that user would like.
%The evolutionary nature of this scenario is how to identify
%users who like luxury items and events and find a grid cell location 
%with a luxury hotel that has these same activities for a given user.
&
$Q \rightarrow \{L,G\} \rightarrow \{P,G\} \rightarrow \{P,U,G\}$
\\ \hline
\end{tabular}
%}
\vspace{-0.2in}
\end{table*}

